Local Area Transform for Cross-Modality Correspondence Matching and Deep Scene Recognition

Establishing correspondences is a fundamental task in variety of image processing and computer vision applications. In particular, finding the correspondences between a non-linearly deformed image pair induced by different modality conditions is a challenging problem. This paper describes a efficient but powerful image transform called local area transform (LAT) for modality-robust correspondence estimation. Specifically, LAT transforms an image from the intensity domain to the local area domain, which is invariant under nonlinear intensity deformations, especially radiometric, photometric, and spectral deformations. In addition, robust feature descriptors are reformulated with LAT for several practical applications. Furthermore, LAT-convolution layer and Aception block are proposed and, with these novel components, deep neural network called LAT-Net is proposed especially for scene recognition task. Experimental results show that LATransformed images provide a consistency for nonlinearly deformed images, even under random intensity deformations. LAT reduces the mean absolute difference as compared to conventional methods. Furthermore, the reformulation of descriptors with LAT shows superiority to conventional methods, which is a promising result for the tasks of cross-spectral and modality correspondence matching. the local area can be considered as an alternative domain to the intensity domain to achieve robust correspondence matching, image recognition, and a lot of applications: such as feature matching, stereo matching, dense correspondence matching, image recognition, and image retrieval.

==> Classes/glyphtounicode.tex <==
% this file was converted from the following files:
%   - glyphlist.txt       (Adobe Glyph List v2.0)
%   - zapfdingbats.txt    (ITC Zapf Dingbats Glyph List)
%   - texglyphlist.txt    (lcdf-typetools texglyphlist.txt, v2.33)
%   - additional.tex      (additional entries)
%
% Notes:
% - entries containing duplicates in glyphlist.txt like
%   'dalethatafpatah;05D3 05B2' are ignored (commented out)
%
% - entries containing duplicates in texglyphlist.txt like
%   'angbracketleft;27E8,2329' are changed so that only the first
%   choice remains, ie 'angbracketleft;27E8'
%
% - a few entries in texglyphlist.txt like Delta, Omega, etc. are
%   commented out (they are already in glyphlist.txt)

% entries from glyphlist.txt:
\pdfglyphtounicode{A}{0041}
\pdfglyphtounicode{AE}{00C6}
\pdfglyphtounicode{AEacute}{01FC}
\pdfglyphtounicode{AEmacron}{01E2}
\pdfglyphtounicode{AEsmall}{F7E6}
\pdfglyphtounicode{Aacute}{00C1}
\pdfglyphtounicode{Aacutesmall}{F7E1}
\pdfglyphtounicode{Abreve}{0102}
\pdfglyphtounicode{Abreveacute}{1EAE}
\pdfglyphtounicode{Abrevecyrillic}{04D0}
\pdfglyphtounicode{Abrevedotbelow}{1EB6}
\pdfglyphtounicode{Abrevegrave}{1EB0}
\pdfglyphtounicode{Abrevehookabove}{1EB2}
\pdfglyphtounicode{Abrevetilde}{1EB4}
\pdfglyphtounicode{Acaron}{01CD}
\pdfglyphtounicode{Acircle}{24B6}
\pdfglyphtounicode{Acircumflex}{00C2}
\pdfglyphtounicode{Acircumflexacute}{1EA4}
\pdfglyphtounicode{Acircumflexdotbelow}{1EAC}
\pdfglyphtounicode{Acircumflexgrave}{1EA6}
\pdfglyphtounicode{Acircumflexhookabove}{1EA8}
\pdfglyphtounicode{Acircumflexsmall}{F7E2}
\pdfglyphtounicode{Acircumflextilde}{1EAA}
\pdfglyphtounicode{Acute}{F6C9}
\pdfglyphtounicode{Acutesmall}{F7B4}
\pdfglyphtounicode{Acyrillic}{0410}
\pdfglyphtounicode{Adblgrave}{0200}
\pdfglyphtounicode{Adieresis}{00C4}
\pdfglyphtounicode{Adieresiscyrillic}{04D2}
\pdfglyphtounicode{Adieresismacron}{01DE}
\pdfglyphtounicode{Adieresissmall}{F7E4}
\pdfglyphtounicode{Adotbelow}{1EA0}
\pdfglyphtounicode{Adotmacron}{01E0}
\pdfglyphtounicode{Agrave}{00C0}
\pdfglyphtounicode{Agravesmall}{F7E0}
\pdfglyphtounicode{Ahookabove}{1EA2}
\pdfglyphtounicode{Aiecyrillic}{04D4}
\pdfglyphtounicode{Ainvertedbreve}{0202}
\pdfglyphtounicode{Alpha}{0391}
\pdfglyphtounicode{Alphatonos}{0386}
\pdfglyphtounicode{Amacron}{0100}
\pdfglyphtounicode{Amonospace}{FF21}
\pdfglyphtounicode{Aogonek}{0104}
\pdfglyphtounicode{Aring}{00C5}
\pdfglyphtounicode{Aringacute}{01FA}
\pdfglyphtounicode{Aringbelow}{1E00}
\pdfglyphtounicode{Aringsmall}{F7E5}
\pdfglyphtounicode{Asmall}{F761}
\pdfglyphtounicode{Atilde}{00C3}
\pdfglyphtounicode{Atildesmall}{F7E3}
\pdfglyphtounicode{Aybarmenian}{0531}
\pdfglyphtounicode{B}{0042}
\pdfglyphtounicode{Bcircle}{24B7}
\pdfglyphtounicode{Bdotaccent}{1E02}
\pdfglyphtounicode{Bdotbelow}{1E04}
\pdfglyphtounicode{Becyrillic}{0411}
\pdfglyphtounicode{Benarmenian}{0532}
\pdfglyphtounicode{Beta}{0392}
\pdfglyphtounicode{Bhook}{0181}
\pdfglyphtounicode{Blinebelow}{1E06}
\pdfglyphtounicode{Bmonospace}{FF22}
\pdfglyphtounicode{Brevesmall}{F6F4}
\pdfglyphtounicode{Bsmall}{F762}
\pdfglyphtounicode{Btopbar}{0182}
\pdfglyphtounicode{C}{0043}
\pdfglyphtounicode{Caarmenian}{053E}
\pdfglyphtounicode{Cacute}{0106}
\pdfglyphtounicode{Caron}{F6CA}
\pdfglyphtounicode{Caronsmall}{F6F5}
\pdfglyphtounicode{Ccaron}{010C}
\pdfglyphtounicode{Ccedilla}{00C7}
\pdfglyphtounicode{Ccedillaacute}{1E08}
\pdfglyphtounicode{Ccedillasmall}{F7E7}
\pdfglyphtounicode{Ccircle}{24B8}
\pdfglyphtounicode{Ccircumflex}{0108}
\pdfglyphtounicode{Cdot}{010A}
\pdfglyphtounicode{Cdotaccent}{010A}
\pdfglyphtounicode{Cedillasmall}{F7B8}
\pdfglyphtounicode{Chaarmenian}{0549}
\pdfglyphtounicode{Cheabkhasiancyrillic}{04BC}
\pdfglyphtounicode{Checyrillic}{0427}
\pdfglyphtounicode{Chedescenderabkhasiancyrillic}{04BE}
\pdfglyphtounicode{Chedescendercyrillic}{04B6}
\pdfglyphtounicode{Chedieresiscyrillic}{04F4}
\pdfglyphtounicode{Cheharmenian}{0543}
\pdfglyphtounicode{Chekhakassiancyrillic}{04CB}
\pdfglyphtounicode{Cheverticalstrokecyrillic}{04B8}
\pdfglyphtounicode{Chi}{03A7}
\pdfglyphtounicode{Chook}{0187}
\pdfglyphtounicode{Circumflexsmall}{F6F6}
\pdfglyphtounicode{Cmonospace}{FF23}
\pdfglyphtounicode{Coarmenian}{0551}
\pdfglyphtounicode{Csmall}{F763}
\pdfglyphtounicode{D}{0044}
\pdfglyphtounicode{DZ}{01F1}
\pdfglyphtounicode{DZcaron}{01C4}
\pdfglyphtounicode{Daarmenian}{0534}
\pdfglyphtounicode{Dafrican}{0189}
\pdfglyphtounicode{Dcaron}{010E}
\pdfglyphtounicode{Dcedilla}{1E10}
\pdfglyphtounicode{Dcircle}{24B9}
\pdfglyphtounicode{Dcircumflexbelow}{1E12}
\pdfglyphtounicode{Dcroat}{0110}
\pdfglyphtounicode{Ddotaccent}{1E0A}
\pdfglyphtounicode{Ddotbelow}{1E0C}
\pdfglyphtounicode{Decyrillic}{0414}
\pdfglyphtounicode{Deicoptic}{03EE}
\pdfglyphtounicode{Delta}{2206}
\pdfglyphtounicode{Deltagreek}{0394}
\pdfglyphtounicode{Dhook}{018A}
\pdfglyphtounicode{Dieresis}{F6CB}
\pdfglyphtounicode{DieresisAcute}{F6CC}
\pdfglyphtounicode{DieresisGrave}{F6CD}
\pdfglyphtounicode{Dieresissmall}{F7A8}
\pdfglyphtounicode{Digammagreek}{03DC}
\pdfglyphtounicode{Djecyrillic}{0402}
\pdfglyphtounicode{Dlinebelow}{1E0E}
\pdfglyphtounicode{Dmonospace}{FF24}
\pdfglyphtounicode{Dotaccentsmall}{F6F7}
\pdfglyphtounicode{Dslash}{0110}
\pdfglyphtounicode{Dsmall}{F764}
\pdfglyphtounicode{Dtopbar}{018B}
\pdfglyphtounicode{Dz}{01F2}
\pdfglyphtounicode{Dzcaron}{01C5}
\pdfglyphtounicode{Dzeabkhasiancyrillic}{04E0}
\pdfglyphtounicode{Dzecyrillic}{0405}
\pdfglyphtounicode{Dzhecyrillic}{040F}
\pdfglyphtounicode{E}{0045}
\pdfglyphtounicode{Eacute}{00C9}
\pdfglyphtounicode{Eacutesmall}{F7E9}
\pdfglyphtounicode{Ebreve}{0114}
\pdfglyphtounicode{Ecaron}{011A}
\pdfglyphtounicode{Ecedillabreve}{1E1C}
\pdfglyphtounicode{Echarmenian}{0535}
\pdfglyphtounicode{Ecircle}{24BA}
\pdfglyphtounicode{Ecircumflex}{00CA}
\pdfglyphtounicode{Ecircumflexacute}{1EBE}
\pdfglyphtounicode{Ecircumflexbelow}{1E18}
\pdfglyphtounicode{Ecircumflexdotbelow}{1EC6}
\pdfglyphtounicode{Ecircumflexgrave}{1EC0}
\pdfglyphtounicode{Ecircumflexhookabove}{1EC2}
\pdfglyphtounicode{Ecircumflexsmall}{F7EA}
\pdfglyphtounicode{Ecircumflextilde}{1EC4}
\pdfglyphtounicode{Ecyrillic}{0404}
\pdfglyphtounicode{Edblgrave}{0204}
\pdfglyphtounicode{Edieresis}{00CB}
\pdfglyphtounicode{Edieresissmall}{F7EB}
\pdfglyphtounicode{Edot}{0116}
\pdfglyphtounicode{Edotaccent}{0116}
\pdfglyphtounicode{Edotbelow}{1EB8}
\pdfglyphtounicode{Efcyrillic}{0424}
\pdfglyphtounicode{Egrave}{00C8}
\pdfglyphtounicode{Egravesmall}{F7E8}
\pdfglyphtounicode{Eharmenian}{0537}
\pdfglyphtounicode{Ehookabove}{1EBA}
\pdfglyphtounicode{Eightroman}{2167}
\pdfglyphtounicode{Einvertedbreve}{0206}
\pdfglyphtounicode{Eiotifiedcyrillic}{0464}
\pdfglyphtounicode{Elcyrillic}{041B}
\pdfglyphtounicode{Elevenroman}{216A}
\pdfglyphtounicode{Emacron}{0112}
\pdfglyphtounicode{Emacronacute}{1E16}
\pdfglyphtounicode{Emacrongrave}{1E14}
\pdfglyphtounicode{Emcyrillic}{041C}
\pdfglyphtounicode{Emonospace}{FF25}
\pdfglyphtounicode{Encyrillic}{041D}
\pdfglyphtounicode{Endescendercyrillic}{04A2}
\pdfglyphtounicode{Eng}{014A}
\pdfglyphtounicode{Enghecyrillic}{04A4}
\pdfglyphtounicode{Enhookcyrillic}{04C7}
\pdfglyphtounicode{Eogonek}{0118}
\pdfglyphtounicode{Eopen}{0190}
\pdfglyphtounicode{Epsilon}{0395}
\pdfglyphtounicode{Epsilontonos}{0388}
\pdfglyphtounicode{Ercyrillic}{0420}
\pdfglyphtounicode{Ereversed}{018E}
\pdfglyphtounicode{Ereversedcyrillic}{042D}
\pdfglyphtounicode{Escyrillic}{0421}
\pdfglyphtounicode{Esdescendercyrillic}{04AA}
\pdfglyphtounicode{Esh}{01A9}
\pdfglyphtounicode{Esmall}{F765}
\pdfglyphtounicode{Eta}{0397}
\pdfglyphtounicode{Etarmenian}{0538}
\pdfglyphtounicode{Etatonos}{0389}
\pdfglyphtounicode{Eth}{00D0}
\pdfglyphtounicode{Ethsmall}{F7F0}
\pdfglyphtounicode{Etilde}{1EBC}
\pdfglyphtounicode{Etildebelow}{1E1A}
\pdfglyphtounicode{Euro}{20AC}
\pdfglyphtounicode{Ezh}{01B7}
\pdfglyphtounicode{Ezhcaron}{01EE}
\pdfglyphtounicode{Ezhreversed}{01B8}
\pdfglyphtounicode{F}{0046}
\pdfglyphtounicode{Fcircle}{24BB}
\pdfglyphtounicode{Fdotaccent}{1E1E}
\pdfglyphtounicode{Feharmenian}{0556}
\pdfglyphtounicode{Feicoptic}{03E4}
\pdfglyphtounicode{Fhook}{0191}
\pdfglyphtounicode{Fitacyrillic}{0472}
\pdfglyphtounicode{Fiveroman}{2164}
\pdfglyphtounicode{Fmonospace}{FF26}
\pdfglyphtounicode{Fourroman}{2163}
\pdfglyphtounicode{Fsmall}{F766}
\pdfglyphtounicode{G}{0047}
\pdfglyphtounicode{GBsquare}{3387}
\pdfglyphtounicode{Gacute}{01F4}
\pdfglyphtounicode{Gamma}{0393}
\pdfglyphtounicode{Gammaafrican}{0194}
\pdfglyphtounicode{Gangiacoptic}{03EA}
\pdfglyphtounicode{Gbreve}{011E}
\pdfglyphtounicode{Gcaron}{01E6}
\pdfglyphtounicode{Gcedilla}{0122}
\pdfglyphtounicode{Gcircle}{24BC}
\pdfglyphtounicode{Gcircumflex}{011C}
\pdfglyphtounicode{Gcommaaccent}{0122}
\pdfglyphtounicode{Gdot}{0120}
\pdfglyphtounicode{Gdotaccent}{0120}
\pdfglyphtounicode{Gecyrillic}{0413}
\pdfglyphtounicode{Ghadarmenian}{0542}
\pdfglyphtounicode{Ghemiddlehookcyrillic}{0494}
\pdfglyphtounicode{Ghestrokecyrillic}{0492}
\pdfglyphtounicode{Gheupturncyrillic}{0490}
\pdfglyphtounicode{Ghook}{0193}
\pdfglyphtounicode{Gimarmenian}{0533}
\pdfglyphtounicode{Gjecyrillic}{0403}
\pdfglyphtounicode{Gmacron}{1E20}
\pdfglyphtounicode{Gmonospace}{FF27}
\pdfglyphtounicode{Grave}{F6CE}
\pdfglyphtounicode{Gravesmall}{F760}
\pdfglyphtounicode{Gsmall}{F767}
\pdfglyphtounicode{Gsmallhook}{029B}
\pdfglyphtounicode{Gstroke}{01E4}
\pdfglyphtounicode{H}{0048}
\pdfglyphtounicode{H18533}{25CF}
\pdfglyphtounicode{H18543}{25AA}
\pdfglyphtounicode{H18551}{25AB}
\pdfglyphtounicode{H22073}{25A1}
\pdfglyphtounicode{HPsquare}{33CB}
\pdfglyphtounicode{Haabkhasiancyrillic}{04A8}
\pdfglyphtounicode{Hadescendercyrillic}{04B2}
\pdfglyphtounicode{Hardsigncyrillic}{042A}
\pdfglyphtounicode{Hbar}{0126}
\pdfglyphtounicode{Hbrevebelow}{1E2A}
\pdfglyphtounicode{Hcedilla}{1E28}
\pdfglyphtounicode{Hcircle}{24BD}
\pdfglyphtounicode{Hcircumflex}{0124}
\pdfglyphtounicode{Hdieresis}{1E26}
\pdfglyphtounicode{Hdotaccent}{1E22}
\pdfglyphtounicode{Hdotbelow}{1E24}
\pdfglyphtounicode{Hmonospace}{FF28}
\pdfglyphtounicode{Hoarmenian}{0540}
\pdfglyphtounicode{Horicoptic}{03E8}
\pdfglyphtounicode{Hsmall}{F768}
\pdfglyphtounicode{Hungarumlaut}{F6CF}
\pdfglyphtounicode{Hungarumlautsmall}{F6F8}
\pdfglyphtounicode{Hzsquare}{3390}
\pdfglyphtounicode{I}{0049}
\pdfglyphtounicode{IAcyrillic}{042F}
\pdfglyphtounicode{IJ}{0132}
\pdfglyphtounicode{IUcyrillic}{042E}
\pdfglyphtounicode{Iacute}{00CD}
\pdfglyphtounicode{Iacutesmall}{F7ED}
\pdfglyphtounicode{Ibreve}{012C}
\pdfglyphtounicode{Icaron}{01CF}
\pdfglyphtounicode{Icircle}{24BE}
\pdfglyphtounicode{Icircumflex}{00CE}
\pdfglyphtounicode{Icircumflexsmall}{F7EE}
\pdfglyphtounicode{Icyrillic}{0406}
\pdfglyphtounicode{Idblgrave}{0208}
\pdfglyphtounicode{Idieresis}{00CF}
\pdfglyphtounicode{Idieresisacute}{1E2E}
\pdfglyphtounicode{Idieresiscyrillic}{04E4}
\pdfglyphtounicode{Idieresissmall}{F7EF}
\pdfglyphtounicode{Idot}{0130}
\pdfglyphtounicode{Idotaccent}{0130}
\pdfglyphtounicode{Idotbelow}{1ECA}
\pdfglyphtounicode{Iebrevecyrillic}{04D6}
\pdfglyphtounicode{Iecyrillic}{0415}
\pdfglyphtounicode{Ifraktur}{2111}
\pdfglyphtounicode{Igrave}{00CC}
\pdfglyphtounicode{Igravesmall}{F7EC}
\pdfglyphtounicode{Ihookabove}{1EC8}
\pdfglyphtounicode{Iicyrillic}{0418}
\pdfglyphtounicode{Iinvertedbreve}{020A}
\pdfglyphtounicode{Iishortcyrillic}{0419}
\pdfglyphtounicode{Imacron}{012A}
\pdfglyphtounicode{Imacroncyrillic}{04E2}
\pdfglyphtounicode{Imonospace}{FF29}
\pdfglyphtounicode{Iniarmenian}{053B}
\pdfglyphtounicode{Iocyrillic}{0401}
\pdfglyphtounicode{Iogonek}{012E}
\pdfglyphtounicode{Iota}{0399}
\pdfglyphtounicode{Iotaafrican}{0196}
\pdfglyphtounicode{Iotadieresis}{03AA}
\pdfglyphtounicode{Iotatonos}{038A}
\pdfglyphtounicode{Ismall}{F769}
\pdfglyphtounicode{Istroke}{0197}
\pdfglyphtounicode{Itilde}{0128}
\pdfglyphtounicode{Itildebelow}{1E2C}
\pdfglyphtounicode{Izhitsacyrillic}{0474}
\pdfglyphtounicode{Izhitsadblgravecyrillic}{0476}
\pdfglyphtounicode{J}{004A}
\pdfglyphtounicode{Jaarmenian}{0541}
\pdfglyphtounicode{Jcircle}{24BF}
\pdfglyphtounicode{Jcircumflex}{0134}
\pdfglyphtounicode{Jecyrillic}{0408}
\pdfglyphtounicode{Jheharmenian}{054B}
\pdfglyphtounicode{Jmonospace}{FF2A}
\pdfglyphtounicode{Jsmall}{F76A}
\pdfglyphtounicode{K}{004B}
\pdfglyphtounicode{KBsquare}{3385}
\pdfglyphtounicode{KKsquare}{33CD}
\pdfglyphtounicode{Kabashkircyrillic}{04A0}
\pdfglyphtounicode{Kacute}{1E30}
\pdfglyphtounicode{Kacyrillic}{041A}
\pdfglyphtounicode{Kadescendercyrillic}{049A}
\pdfglyphtounicode{Kahookcyrillic}{04C3}
\pdfglyphtounicode{Kappa}{039A}
\pdfglyphtounicode{Kastrokecyrillic}{049E}
\pdfglyphtounicode{Kaverticalstrokecyrillic}{049C}
\pdfglyphtounicode{Kcaron}{01E8}
\pdfglyphtounicode{Kcedilla}{0136}
\pdfglyphtounicode{Kcircle}{24C0}
\pdfglyphtounicode{Kcommaaccent}{0136}
\pdfglyphtounicode{Kdotbelow}{1E32}
\pdfglyphtounicode{Keharmenian}{0554}
\pdfglyphtounicode{Kenarmenian}{053F}
\pdfglyphtounicode{Khacyrillic}{0425}
\pdfglyphtounicode{Kheicoptic}{03E6}
\pdfglyphtounicode{Khook}{0198}
\pdfglyphtounicode{Kjecyrillic}{040C}
\pdfglyphtounicode{Klinebelow}{1E34}
\pdfglyphtounicode{Kmonospace}{FF2B}
\pdfglyphtounicode{Koppacyrillic}{0480}
\pdfglyphtounicode{Koppagreek}{03DE}
\pdfglyphtounicode{Ksicyrillic}{046E}
\pdfglyphtounicode{Ksmall}{F76B}
\pdfglyphtounicode{L}{004C}
\pdfglyphtounicode{LJ}{01C7}
\pdfglyphtounicode{LL}{F6BF}
\pdfglyphtounicode{Lacute}{0139}
\pdfglyphtounicode{Lambda}{039B}
\pdfglyphtounicode{Lcaron}{013D}
\pdfglyphtounicode{Lcedilla}{013B}
\pdfglyphtounicode{Lcircle}{24C1}
\pdfglyphtounicode{Lcircumflexbelow}{1E3C}
\pdfglyphtounicode{Lcommaaccent}{013B}
\pdfglyphtounicode{Ldot}{013F}
\pdfglyphtounicode{Ldotaccent}{013F}
\pdfglyphtounicode{Ldotbelow}{1E36}
\pdfglyphtounicode{Ldotbelowmacron}{1E38}
\pdfglyphtounicode{Liwnarmenian}{053C}
\pdfglyphtounicode{Lj}{01C8}
\pdfglyphtounicode{Ljecyrillic}{0409}
\pdfglyphtounicode{Llinebelow}{1E3A}
\pdfglyphtounicode{Lmonospace}{FF2C}
\pdfglyphtounicode{Lslash}{0141}
\pdfglyphtounicode{Lslashsmall}{F6F9}
\pdfglyphtounicode{Lsmall}{F76C}
\pdfglyphtounicode{M}{004D}
\pdfglyphtounicode{MBsquare}{3386}
\pdfglyphtounicode{Macron}{F6D0}
\pdfglyphtounicode{Macronsmall}{F7AF}
\pdfglyphtounicode{Macute}{1E3E}
\pdfglyphtounicode{Mcircle}{24C2}
\pdfglyphtounicode{Mdotaccent}{1E40}
\pdfglyphtounicode{Mdotbelow}{1E42}
\pdfglyphtounicode{Menarmenian}{0544}
\pdfglyphtounicode{Mmonospace}{FF2D}
\pdfglyphtounicode{Msmall}{F76D}
\pdfglyphtounicode{Mturned}{019C}
\pdfglyphtounicode{Mu}{039C}
\pdfglyphtounicode{N}{004E}
\pdfglyphtounicode{NJ}{01CA}
\pdfglyphtounicode{Nacute}{0143}
\pdfglyphtounicode{Ncaron}{0147}
\pdfglyphtounicode{Ncedilla}{0145}
\pdfglyphtounicode{Ncircle}{24C3}
\pdfglyphtounicode{Ncircumflexbelow}{1E4A}
\pdfglyphtounicode{Ncommaaccent}{0145}
\pdfglyphtounicode{Ndotaccent}{1E44}
\pdfglyphtounicode{Ndotbelow}{1E46}
\pdfglyphtounicode{Nhookleft}{019D}
\pdfglyphtounicode{Nineroman}{2168}
\pdfglyphtounicode{Nj}{01CB}
\pdfglyphtounicode{Njecyrillic}{040A}
\pdfglyphtounicode{Nlinebelow}{1E48}
\pdfglyphtounicode{Nmonospace}{FF2E}
\pdfglyphtounicode{Nowarmenian}{0546}
\pdfglyphtounicode{Nsmall}{F76E}
\pdfglyphtounicode{Ntilde}{00D1}
\pdfglyphtounicode{Ntildesmall}{F7F1}
\pdfglyphtounicode{Nu}{039D}
\pdfglyphtounicode{O}{004F}
\pdfglyphtounicode{OE}{0152}
\pdfglyphtounicode{OEsmall}{F6FA}
\pdfglyphtounicode{Oacute}{00D3}
\pdfglyphtounicode{Oacutesmall}{F7F3}
\pdfglyphtounicode{Obarredcyrillic}{04E8}
\pdfglyphtounicode{Obarreddieresiscyrillic}{04EA}
\pdfglyphtounicode{Obreve}{014E}
\pdfglyphtounicode{Ocaron}{01D1}
\pdfglyphtounicode{Ocenteredtilde}{019F}
\pdfglyphtounicode{Ocircle}{24C4}
\pdfglyphtounicode{Ocircumflex}{00D4}
\pdfglyphtounicode{Ocircumflexacute}{1ED0}
\pdfglyphtounicode{Ocircumflexdotbelow}{1ED8}
\pdfglyphtounicode{Ocircumflexgrave}{1ED2}
\pdfglyphtounicode{Ocircumflexhookabove}{1ED4}
\pdfglyphtounicode{Ocircumflexsmall}{F7F4}
\pdfglyphtounicode{Ocircumflextilde}{1ED6}
\pdfglyphtounicode{Ocyrillic}{041E}
\pdfglyphtounicode{Odblacute}{0150}
\pdfglyphtounicode{Odblgrave}{020C}
\pdfglyphtounicode{Odieresis}{00D6}
\pdfglyphtounicode{Odieresiscyrillic}{04E6}
\pdfglyphtounicode{Odieresissmall}{F7F6}
\pdfglyphtounicode{Odotbelow}{1ECC}
\pdfglyphtounicode{Ogoneksmall}{F6FB}
\pdfglyphtounicode{Ograve}{00D2}
\pdfglyphtounicode{Ogravesmall}{F7F2}
\pdfglyphtounicode{Oharmenian}{0555}
\pdfglyphtounicode{Ohm}{2126}
\pdfglyphtounicode{Ohookabove}{1ECE}
\pdfglyphtounicode{Ohorn}{01A0}
\pdfglyphtounicode{Ohornacute}{1EDA}
\pdfglyphtounicode{Ohorndotbelow}{1EE2}
\pdfglyphtounicode{Ohorngrave}{1EDC}
\pdfglyphtounicode{Ohornhookabove}{1EDE}
\pdfglyphtounicode{Ohorntilde}{1EE0}
\pdfglyphtounicode{Ohungarumlaut}{0150}
\pdfglyphtounicode{Oi}{01A2}
\pdfglyphtounicode{Oinvertedbreve}{020E}
\pdfglyphtounicode{Omacron}{014C}
\pdfglyphtounicode{Omacronacute}{1E52}
\pdfglyphtounicode{Omacrongrave}{1E50}
\pdfglyphtounicode{Omega}{2126}
\pdfglyphtounicode{Omegacyrillic}{0460}
\pdfglyphtounicode{Omegagreek}{03A9}
\pdfglyphtounicode{Omegaroundcyrillic}{047A}
\pdfglyphtounicode{Omegatitlocyrillic}{047C}
\pdfglyphtounicode{Omegatonos}{038F}
\pdfglyphtounicode{Omicron}{039F}
\pdfglyphtounicode{Omicrontonos}{038C}
\pdfglyphtounicode{Omonospace}{FF2F}
\pdfglyphtounicode{Oneroman}{2160}
\pdfglyphtounicode{Oogonek}{01EA}
\pdfglyphtounicode{Oogonekmacron}{01EC}
\pdfglyphtounicode{Oopen}{0186}
\pdfglyphtounicode{Oslash}{00D8}
\pdfglyphtounicode{Oslashacute}{01FE}
\pdfglyphtounicode{Oslashsmall}{F7F8}
\pdfglyphtounicode{Osmall}{F76F}
\pdfglyphtounicode{Ostrokeacute}{01FE}
\pdfglyphtounicode{Otcyrillic}{047E}
\pdfglyphtounicode{Otilde}{00D5}
\pdfglyphtounicode{Otildeacute}{1E4C}
\pdfglyphtounicode{Otildedieresis}{1E4E}
\pdfglyphtounicode{Otildesmall}{F7F5}
\pdfglyphtounicode{P}{0050}
\pdfglyphtounicode{Pacute}{1E54}
\pdfglyphtounicode{Pcircle}{24C5}
\pdfglyphtounicode{Pdotaccent}{1E56}
\pdfglyphtounicode{Pecyrillic}{041F}
\pdfglyphtounicode{Peharmenian}{054A}
\pdfglyphtounicode{Pemiddlehookcyrillic}{04A6}
\pdfglyphtounicode{Phi}{03A6}
\pdfglyphtounicode{Phook}{01A4}
\pdfglyphtounicode{Pi}{03A0}
\pdfglyphtounicode{Piwrarmenian}{0553}
\pdfglyphtounicode{Pmonospace}{FF30}
\pdfglyphtounicode{Psi}{03A8}
\pdfglyphtounicode{Psicyrillic}{0470}
\pdfglyphtounicode{Psmall}{F770}
\pdfglyphtounicode{Q}{0051}
\pdfglyphtounicode{Qcircle}{24C6}
\pdfglyphtounicode{Qmonospace}{FF31}
\pdfglyphtounicode{Qsmall}{F771}
\pdfglyphtounicode{R}{0052}
\pdfglyphtounicode{Raarmenian}{054C}
\pdfglyphtounicode{Racute}{0154}
\pdfglyphtounicode{Rcaron}{0158}
\pdfglyphtounicode{Rcedilla}{0156}
\pdfglyphtounicode{Rcircle}{24C7}
\pdfglyphtounicode{Rcommaaccent}{0156}
\pdfglyphtounicode{Rdblgrave}{0210}
\pdfglyphtounicode{Rdotaccent}{1E58}
\pdfglyphtounicode{Rdotbelow}{1E5A}
\pdfglyphtounicode{Rdotbelowmacron}{1E5C}
\pdfglyphtounicode{Reharmenian}{0550}
\pdfglyphtounicode{Rfraktur}{211C}
\pdfglyphtounicode{Rho}{03A1}
\pdfglyphtounicode{Ringsmall}{F6FC}
\pdfglyphtounicode{Rinvertedbreve}{0212}
\pdfglyphtounicode{Rlinebelow}{1E5E}
\pdfglyphtounicode{Rmonospace}{FF32}
\pdfglyphtounicode{Rsmall}{F772}
\pdfglyphtounicode{Rsmallinverted}{0281}
\pdfglyphtounicode{Rsmallinvertedsuperior}{02B6}
\pdfglyphtounicode{S}{0053}
\pdfglyphtounicode{SF010000}{250C}
\pdfglyphtounicode{SF020000}{2514}
\pdfglyphtounicode{SF030000}{2510}
\pdfglyphtounicode{SF040000}{2518}
\pdfglyphtounicode{SF050000}{253C}
\pdfglyphtounicode{SF060000}{252C}
\pdfglyphtounicode{SF070000}{2534}
\pdfglyphtounicode{SF080000}{251C}
\pdfglyphtounicode{SF090000}{2524}
\pdfglyphtounicode{SF100000}{2500}
\pdfglyphtounicode{SF110000}{2502}
\pdfglyphtounicode{SF190000}{2561}
\pdfglyphtounicode{SF200000}{2562}
\pdfglyphtounicode{SF210000}{2556}
\pdfglyphtounicode{SF220000}{2555}
\pdfglyphtounicode{SF230000}{2563}
\pdfglyphtounicode{SF240000}{2551}
\pdfglyphtounicode{SF250000}{2557}
\pdfglyphtounicode{SF260000}{255D}
\pdfglyphtounicode{SF270000}{255C}
\pdfglyphtounicode{SF280000}{255B}
\pdfglyphtounicode{SF360000}{255E}
\pdfglyphtounicode{SF370000}{255F}
\pdfglyphtounicode{SF380000}{255A}
\pdfglyphtounicode{SF390000}{2554}
\pdfglyphtounicode{SF400000}{2569}
\pdfglyphtounicode{SF410000}{2566}
\pdfglyphtounicode{SF420000}{2560}
\pdfglyphtounicode{SF430000}{2550}
\pdfglyphtounicode{SF440000}{256C}
\pdfglyphtounicode{SF450000}{2567}
\pdfglyphtounicode{SF460000}{2568}
\pdfglyphtounicode{SF470000}{2564}
\pdfglyphtounicode{SF480000}{2565}
\pdfglyphtounicode{SF490000}{2559}
\pdfglyphtounicode{SF500000}{2558}
\pdfglyphtounicode{SF510000}{2552}
\pdfglyphtounicode{SF520000}{2553}
\pdfglyphtounicode{SF530000}{256B}
\pdfglyphtounicode{SF540000}{256A}
\pdfglyphtounicode{Sacute}{015A}
\pdfglyphtounicode{Sacutedotaccent}{1E64}
\pdfglyphtounicode{Sampigreek}{03E0}
\pdfglyphtounicode{Scaron}{0160}
\pdfglyphtounicode{Scarondotaccent}{1E66}
\pdfglyphtounicode{Scaronsmall}{F6FD}
\pdfglyphtounicode{Scedilla}{015E}
\pdfglyphtounicode{Schwa}{018F}
\pdfglyphtounicode{Schwacyrillic}{04D8}
\pdfglyphtounicode{Schwadieresiscyrillic}{04DA}
\pdfglyphtounicode{Scircle}{24C8}
\pdfglyphtounicode{Scircumflex}{015C}
\pdfglyphtounicode{Scommaaccent}{0218}
\pdfglyphtounicode{Sdotaccent}{1E60}
\pdfglyphtounicode{Sdotbelow}{1E62}
\pdfglyphtounicode{Sdotbelowdotaccent}{1E68}
\pdfglyphtounicode{Seharmenian}{054D}
\pdfglyphtounicode{Sevenroman}{2166}
\pdfglyphtounicode{Shaarmenian}{0547}
\pdfglyphtounicode{Shacyrillic}{0428}
\pdfglyphtounicode{Shchacyrillic}{0429}
\pdfglyphtounicode{Sheicoptic}{03E2}
\pdfglyphtounicode{Shhacyrillic}{04BA}
\pdfglyphtounicode{Shimacoptic}{03EC}
\pdfglyphtounicode{Sigma}{03A3}
\pdfglyphtounicode{Sixroman}{2165}
\pdfglyphtounicode{Smonospace}{FF33}
\pdfglyphtounicode{Softsigncyrillic}{042C}
\pdfglyphtounicode{Ssmall}{F773}
\pdfglyphtounicode{Stigmagreek}{03DA}
\pdfglyphtounicode{T}{0054}
\pdfglyphtounicode{Tau}{03A4}
\pdfglyphtounicode{Tbar}{0166}
\pdfglyphtounicode{Tcaron}{0164}
\pdfglyphtounicode{Tcedilla}{0162}
\pdfglyphtounicode{Tcircle}{24C9}
\pdfglyphtounicode{Tcircumflexbelow}{1E70}
\pdfglyphtounicode{Tcommaaccent}{0162}
\pdfglyphtounicode{Tdotaccent}{1E6A}
\pdfglyphtounicode{Tdotbelow}{1E6C}
\pdfglyphtounicode{Tecyrillic}{0422}
\pdfglyphtounicode{Tedescendercyrillic}{04AC}
\pdfglyphtounicode{Tenroman}{2169}
\pdfglyphtounicode{Tetsecyrillic}{04B4}
\pdfglyphtounicode{Theta}{0398}
\pdfglyphtounicode{Thook}{01AC}
\pdfglyphtounicode{Thorn}{00DE}
\pdfglyphtounicode{Thornsmall}{F7FE}
\pdfglyphtounicode{Threeroman}{2162}
\pdfglyphtounicode{Tildesmall}{F6FE}
\pdfglyphtounicode{Tiwnarmenian}{054F}
\pdfglyphtounicode{Tlinebelow}{1E6E}
\pdfglyphtounicode{Tmonospace}{FF34}
\pdfglyphtounicode{Toarmenian}{0539}
\pdfglyphtounicode{Tonefive}{01BC}
\pdfglyphtounicode{Tonesix}{0184}
\pdfglyphtounicode{Tonetwo}{01A7}
\pdfglyphtounicode{Tretroflexhook}{01AE}
\pdfglyphtounicode{Tsecyrillic}{0426}
\pdfglyphtounicode{Tshecyrillic}{040B}
\pdfglyphtounicode{Tsmall}{F774}
\pdfglyphtounicode{Twelveroman}{216B}
\pdfglyphtounicode{Tworoman}{2161}
\pdfglyphtounicode{U}{0055}
\pdfglyphtounicode{Uacute}{00DA}
\pdfglyphtounicode{Uacutesmall}{F7FA}
\pdfglyphtounicode{Ubreve}{016C}
\pdfglyphtounicode{Ucaron}{01D3}
\pdfglyphtounicode{Ucircle}{24CA}
\pdfglyphtounicode{Ucircumflex}{00DB}
\pdfglyphtounicode{Ucircumflexbelow}{1E76}
\pdfglyphtounicode{Ucircumflexsmall}{F7FB}
\pdfglyphtounicode{Ucyrillic}{0423}
\pdfglyphtounicode{Udblacute}{0170}
\pdfglyphtounicode{Udblgrave}{0214}
\pdfglyphtounicode{Udieresis}{00DC}
\pdfglyphtounicode{Udieresisacute}{01D7}
\pdfglyphtounicode{Udieresisbelow}{1E72}
\pdfglyphtounicode{Udieresiscaron}{01D9}
\pdfglyphtounicode{Udieresiscyrillic}{04F0}
\pdfglyphtounicode{Udieresisgrave}{01DB}
\pdfglyphtounicode{Udieresismacron}{01D5}
\pdfglyphtounicode{Udieresissmall}{F7FC}
\pdfglyphtounicode{Udotbelow}{1EE4}
\pdfglyphtounicode{Ugrave}{00D9}
\pdfglyphtounicode{Ugravesmall}{F7F9}
\pdfglyphtounicode{Uhookabove}{1EE6}
\pdfglyphtounicode{Uhorn}{01AF}
\pdfglyphtounicode{Uhornacute}{1EE8}
\pdfglyphtounicode{Uhorndotbelow}{1EF0}
\pdfglyphtounicode{Uhorngrave}{1EEA}
\pdfglyphtounicode{Uhornhookabove}{1EEC}
\pdfglyphtounicode{Uhorntilde}{1EEE}
\pdfglyphtounicode{Uhungarumlaut}{0170}
\pdfglyphtounicode{Uhungarumlautcyrillic}{04F2}
\pdfglyphtounicode{Uinvertedbreve}{0216}
\pdfglyphtounicode{Ukcyrillic}{0478}
\pdfglyphtounicode{Umacron}{016A}
\pdfglyphtounicode{Umacroncyrillic}{04EE}
\pdfglyphtounicode{Umacrondieresis}{1E7A}
\pdfglyphtounicode{Umonospace}{FF35}
\pdfglyphtounicode{Uogonek}{0172}
\pdfglyphtounicode{Upsilon}{03A5}
\pdfglyphtounicode{Upsilon1}{03D2}
\pdfglyphtounicode{Upsilonacutehooksymbolgreek}{03D3}
\pdfglyphtounicode{Upsilonafrican}{01B1}
\pdfglyphtounicode{Upsilondieresis}{03AB}
\pdfglyphtounicode{Upsilondieresishooksymbolgreek}{03D4}
\pdfglyphtounicode{Upsilonhooksymbol}{03D2}
\pdfglyphtounicode{Upsilontonos}{038E}
\pdfglyphtounicode{Uring}{016E}
\pdfglyphtounicode{Ushortcyrillic}{040E}
\pdfglyphtounicode{Usmall}{F775}
\pdfglyphtounicode{Ustraightcyrillic}{04AE}
\pdfglyphtounicode{Ustraightstrokecyrillic}{04B0}
\pdfglyphtounicode{Utilde}{0168}
\pdfglyphtounicode{Utildeacute}{1E78}
\pdfglyphtounicode{Utildebelow}{1E74}
\pdfglyphtounicode{V}{0056}
\pdfglyphtounicode{Vcircle}{24CB}
\pdfglyphtounicode{Vdotbelow}{1E7E}
\pdfglyphtounicode{Vecyrillic}{0412}
\pdfglyphtounicode{Vewarmenian}{054E}
\pdfglyphtounicode{Vhook}{01B2}
\pdfglyphtounicode{Vmonospace}{FF36}
\pdfglyphtounicode{Voarmenian}{0548}
\pdfglyphtounicode{Vsmall}{F776}
\pdfglyphtounicode{Vtilde}{1E7C}
\pdfglyphtounicode{W}{0057}
\pdfglyphtounicode{Wacute}{1E82}
\pdfglyphtounicode{Wcircle}{24CC}
\pdfglyphtounicode{Wcircumflex}{0174}
\pdfglyphtounicode{Wdieresis}{1E84}
\pdfglyphtounicode{Wdotaccent}{1E86}
\pdfglyphtounicode{Wdotbelow}{1E88}
\pdfglyphtounicode{Wgrave}{1E80}
\pdfglyphtounicode{Wmonospace}{FF37}
\pdfglyphtounicode{Wsmall}{F777}
\pdfglyphtounicode{X}{0058}
\pdfglyphtounicode{Xcircle}{24CD}
\pdfglyphtounicode{Xdieresis}{1E8C}
\pdfglyphtounicode{Xdotaccent}{1E8A}
\pdfglyphtounicode{Xeharmenian}{053D}
\pdfglyphtounicode{Xi}{039E}
\pdfglyphtounicode{Xmonospace}{FF38}
\pdfglyphtounicode{Xsmall}{F778}
\pdfglyphtounicode{Y}{0059}
\pdfglyphtounicode{Yacute}{00DD}
\pdfglyphtounicode{Yacutesmall}{F7FD}
\pdfglyphtounicode{Yatcyrillic}{0462}
\pdfglyphtounicode{Ycircle}{24CE}
\pdfglyphtounicode{Ycircumflex}{0176}
\pdfglyphtounicode{Ydieresis}{0178}
\pdfglyphtounicode{Ydieresissmall}{F7FF}
\pdfglyphtounicode{Ydotaccent}{1E8E}
\pdfglyphtounicode{Ydotbelow}{1EF4}
\pdfglyphtounicode{Yericyrillic}{042B}
\pdfglyphtounicode{Yerudieresiscyrillic}{04F8}
\pdfglyphtounicode{Ygrave}{1EF2}
\pdfglyphtounicode{Yhook}{01B3}
\pdfglyphtounicode{Yhookabove}{1EF6}
\pdfglyphtounicode{Yiarmenian}{0545}
\pdfglyphtounicode{Yicyrillic}{0407}
\pdfglyphtounicode{Yiwnarmenian}{0552}
\pdfglyphtounicode{Ymonospace}{FF39}
\pdfglyphtounicode{Ysmall}{F779}
\pdfglyphtounicode{Ytilde}{1EF8}
\pdfglyphtounicode{Yusbigcyrillic}{046A}
\pdfglyphtounicode{Yusbigiotifiedcyrillic}{046C}
\pdfglyphtounicode{Yuslittlecyrillic}{0466}
\pdfglyphtounicode{Yuslittleiotifiedcyrillic}{0468}
\pdfglyphtounicode{Z}{005A}
\pdfglyphtounicode{Zaarmenian}{0536}
\pdfglyphtounicode{Zacute}{0179}
\pdfglyphtounicode{Zcaron}{017D}
\pdfglyphtounicode{Zcaronsmall}{F6FF}
\pdfglyphtounicode{Zcircle}{24CF}
\pdfglyphtounicode{Zcircumflex}{1E90}
\pdfglyphtounicode{Zdot}{017B}
\pdfglyphtounicode{Zdotaccent}{017B}
\pdfglyphtounicode{Zdotbelow}{1E92}
\pdfglyphtounicode{Zecyrillic}{0417}
\pdfglyphtounicode{Zedescendercyrillic}{0498}
\pdfglyphtounicode{Zedieresiscyrillic}{04DE}
\pdfglyphtounicode{Zeta}{0396}
\pdfglyphtounicode{Zhearmenian}{053A}
\pdfglyphtounicode{Zhebrevecyrillic}{04C1}
\pdfglyphtounicode{Zhecyrillic}{0416}
\pdfglyphtounicode{Zhedescendercyrillic}{0496}
\pdfglyphtounicode{Zhedieresiscyrillic}{04DC}
\pdfglyphtounicode{Zlinebelow}{1E94}
\pdfglyphtounicode{Zmonospace}{FF3A}
\pdfglyphtounicode{Zsmall}{F77A}
\pdfglyphtounicode{Zstroke}{01B5}
\pdfglyphtounicode{a}{0061}
\pdfglyphtounicode{aabengali}{0986}
\pdfglyphtounicode{aacute}{00E1}
\pdfglyphtounicode{aadeva}{0906}
\pdfglyphtounicode{aagujarati}{0A86}
\pdfglyphtounicode{aagurmukhi}{0A06}
\pdfglyphtounicode{aamatragurmukhi}{0A3E}
\pdfglyphtounicode{aarusquare}{3303}
\pdfglyphtounicode{aavowelsignbengali}{09BE}
\pdfglyphtounicode{aavowelsigndeva}{093E}
\pdfglyphtounicode{aavowelsigngujarati}{0ABE}
\pdfglyphtounicode{abbreviationmarkarmenian}{055F}
\pdfglyphtounicode{abbreviationsigndeva}{0970}
\pdfglyphtounicode{abengali}{0985}
\pdfglyphtounicode{abopomofo}{311A}
\pdfglyphtounicode{abreve}{0103}
\pdfglyphtounicode{abreveacute}{1EAF}
\pdfglyphtounicode{abrevecyrillic}{04D1}
\pdfglyphtounicode{abrevedotbelow}{1EB7}
\pdfglyphtounicode{abrevegrave}{1EB1}
\pdfglyphtounicode{abrevehookabove}{1EB3}
\pdfglyphtounicode{abrevetilde}{1EB5}
\pdfglyphtounicode{acaron}{01CE}
\pdfglyphtounicode{acircle}{24D0}
\pdfglyphtounicode{acircumflex}{00E2}
\pdfglyphtounicode{acircumflexacute}{1EA5}
\pdfglyphtounicode{acircumflexdotbelow}{1EAD}
\pdfglyphtounicode{acircumflexgrave}{1EA7}
\pdfglyphtounicode{acircumflexhookabove}{1EA9}
\pdfglyphtounicode{acircumflextilde}{1EAB}
\pdfglyphtounicode{acute}{00B4}
\pdfglyphtounicode{acutebelowcmb}{0317}
\pdfglyphtounicode{acutecmb}{0301}
\pdfglyphtounicode{acutecomb}{0301}
\pdfglyphtounicode{acutedeva}{0954}
\pdfglyphtounicode{acutelowmod}{02CF}
\pdfglyphtounicode{acutetonecmb}{0341}
\pdfglyphtounicode{acyrillic}{0430}
\pdfglyphtounicode{adblgrave}{0201}
\pdfglyphtounicode{addakgurmukhi}{0A71}
\pdfglyphtounicode{adeva}{0905}
\pdfglyphtounicode{adieresis}{00E4}
\pdfglyphtounicode{adieresiscyrillic}{04D3}
\pdfglyphtounicode{adieresismacron}{01DF}
\pdfglyphtounicode{adotbelow}{1EA1}
\pdfglyphtounicode{adotmacron}{01E1}
\pdfglyphtounicode{ae}{00E6}
\pdfglyphtounicode{aeacute}{01FD}
\pdfglyphtounicode{aekorean}{3150}
\pdfglyphtounicode{aemacron}{01E3}
\pdfglyphtounicode{afii00208}{2015}
\pdfglyphtounicode{afii08941}{20A4}
\pdfglyphtounicode{afii10017}{0410}
\pdfglyphtounicode{afii10018}{0411}
\pdfglyphtounicode{afii10019}{0412}
\pdfglyphtounicode{afii10020}{0413}
\pdfglyphtounicode{afii10021}{0414}
\pdfglyphtounicode{afii10022}{0415}
\pdfglyphtounicode{afii10023}{0401}
\pdfglyphtounicode{afii10024}{0416}
\pdfglyphtounicode{afii10025}{0417}
\pdfglyphtounicode{afii10026}{0418}
\pdfglyphtounicode{afii10027}{0419}
\pdfglyphtounicode{afii10028}{041A}
\pdfglyphtounicode{afii10029}{041B}
\pdfglyphtounicode{afii10030}{041C}
\pdfglyphtounicode{afii10031}{041D}
\pdfglyphtounicode{afii10032}{041E}
\pdfglyphtounicode{afii10033}{041F}
\pdfglyphtounicode{afii10034}{0420}
\pdfglyphtounicode{afii10035}{0421}
\pdfglyphtounicode{afii10036}{0422}
\pdfglyphtounicode{afii10037}{0423}
\pdfglyphtounicode{afii10038}{0424}
\pdfglyphtounicode{afii10039}{0425}
\pdfglyphtounicode{afii10040}{0426}
\pdfglyphtounicode{afii10041}{0427}
\pdfglyphtounicode{afii10042}{0428}
\pdfglyphtounicode{afii10043}{0429}
\pdfglyphtounicode{afii10044}{042A}
\pdfglyphtounicode{afii10045}{042B}
\pdfglyphtounicode{afii10046}{042C}
\pdfglyphtounicode{afii10047}{042D}
\pdfglyphtounicode{afii10048}{042E}
\pdfglyphtounicode{afii10049}{042F}
\pdfglyphtounicode{afii10050}{0490}
\pdfglyphtounicode{afii10051}{0402}
\pdfglyphtounicode{afii10052}{0403}
\pdfglyphtounicode{afii10053}{0404}
\pdfglyphtounicode{afii10054}{0405}
\pdfglyphtounicode{afii10055}{0406}
\pdfglyphtounicode{afii10056}{0407}
\pdfglyphtounicode{afii10057}{0408}
\pdfglyphtounicode{afii10058}{0409}
\pdfglyphtounicode{afii10059}{040A}
\pdfglyphtounicode{afii10060}{040B}
\pdfglyphtounicode{afii10061}{040C}
\pdfglyphtounicode{afii10062}{040E}
\pdfglyphtounicode{afii10063}{F6C4}
\pdfglyphtounicode{afii10064}{F6C5}
\pdfglyphtounicode{afii10065}{0430}
\pdfglyphtounicode{afii10066}{0431}
\pdfglyphtounicode{afii10067}{0432}
\pdfglyphtounicode{afii10068}{0433}
\pdfglyphtounicode{afii10069}{0434}
\pdfglyphtounicode{afii10070}{0435}
\pdfglyphtounicode{afii10071}{0451}
\pdfglyphtounicode{afii10072}{0436}
\pdfglyphtounicode{afii10073}{0437}
\pdfglyphtounicode{afii10074}{0438}
\pdfglyphtounicode{afii10075}{0439}
\pdfglyphtounicode{afii10076}{043A}
\pdfglyphtounicode{afii10077}{043B}
\pdfglyphtounicode{afii10078}{043C}
\pdfglyphtounicode{afii10079}{043D}
\pdfglyphtounicode{afii10080}{043E}
\pdfglyphtounicode{afii10081}{043F}
\pdfglyphtounicode{afii10082}{0440}
\pdfglyphtounicode{afii10083}{0441}
\pdfglyphtounicode{afii10084}{0442}
\pdfglyphtounicode{afii10085}{0443}
\pdfglyphtounicode{afii10086}{0444}
\pdfglyphtounicode{afii10087}{0445}
\pdfglyphtounicode{afii10088}{0446}
\pdfglyphtounicode{afii10089}{0447}
\pdfglyphtounicode{afii10090}{0448}
\pdfglyphtounicode{afii10091}{0449}
\pdfglyphtounicode{afii10092}{044A}
\pdfglyphtounicode{afii10093}{044B}
\pdfglyphtounicode{afii10094}{044C}
\pdfglyphtounicode{afii10095}{044D}
\pdfglyphtounicode{afii10096}{044E}
\pdfglyphtounicode{afii10097}{044F}
\pdfglyphtounicode{afii10098}{0491}
\pdfglyphtounicode{afii10099}{0452}
\pdfglyphtounicode{afii10100}{0453}
\pdfglyphtounicode{afii10101}{0454}
\pdfglyphtounicode{afii10102}{0455}
\pdfglyphtounicode{afii10103}{0456}
\pdfglyphtounicode{afii10104}{0457}
\pdfglyphtounicode{afii10105}{0458}
\pdfglyphtounicode{afii10106}{0459}
\pdfglyphtounicode{afii10107}{045A}
\pdfglyphtounicode{afii10108}{045B}
\pdfglyphtounicode{afii10109}{045C}
\pdfglyphtounicode{afii10110}{045E}
\pdfglyphtounicode{afii10145}{040F}
\pdfglyphtounicode{afii10146}{0462}
\pdfglyphtounicode{afii10147}{0472}
\pdfglyphtounicode{afii10148}{0474}
\pdfglyphtounicode{afii10192}{F6C6}
\pdfglyphtounicode{afii10193}{045F}
\pdfglyphtounicode{afii10194}{0463}
\pdfglyphtounicode{afii10195}{0473}
\pdfglyphtounicode{afii10196}{0475}
\pdfglyphtounicode{afii10831}{F6C7}
\pdfglyphtounicode{afii10832}{F6C8}
\pdfglyphtounicode{afii10846}{04D9}
\pdfglyphtounicode{afii299}{200E}
\pdfglyphtounicode{afii300}{200F}
\pdfglyphtounicode{afii301}{200D}
\pdfglyphtounicode{afii57381}{066A}
\pdfglyphtounicode{afii57388}{060C}
\pdfglyphtounicode{afii57392}{0660}
\pdfglyphtounicode{afii57393}{0661}
\pdfglyphtounicode{afii57394}{0662}
\pdfglyphtounicode{afii57395}{0663}
\pdfglyphtounicode{afii57396}{0664}
\pdfglyphtounicode{afii57397}{0665}
\pdfglyphtounicode{afii57398}{0666}
\pdfglyphtounicode{afii57399}{0667}
\pdfglyphtounicode{afii57400}{0668}
\pdfglyphtounicode{afii57401}{0669}
\pdfglyphtounicode{afii57403}{061B}
\pdfglyphtounicode{afii57407}{061F}
\pdfglyphtounicode{afii57409}{0621}
\pdfglyphtounicode{afii57410}{0622}
\pdfglyphtounicode{afii57411}{0623}
\pdfglyphtounicode{afii57412}{0624}
\pdfglyphtounicode{afii57413}{0625}
\pdfglyphtounicode{afii57414}{0626}
\pdfglyphtounicode{afii57415}{0627}
\pdfglyphtounicode{afii57416}{0628}
\pdfglyphtounicode{afii57417}{0629}
\pdfglyphtounicode{afii57418}{062A}
\pdfglyphtounicode{afii57419}{062B}
\pdfglyphtounicode{afii57420}{062C}
\pdfglyphtounicode{afii57421}{062D}
\pdfglyphtounicode{afii57422}{062E}
\pdfglyphtounicode{afii57423}{062F}
\pdfglyphtounicode{afii57424}{0630}
\pdfglyphtounicode{afii57425}{0631}
\pdfglyphtounicode{afii57426}{0632}
\pdfglyphtounicode{afii57427}{0633}
\pdfglyphtounicode{afii57428}{0634}
\pdfglyphtounicode{afii57429}{0635}
\pdfglyphtounicode{afii57430}{0636}
\pdfglyphtounicode{afii57431}{0637}
\pdfglyphtounicode{afii57432}{0638}
\pdfglyphtounicode{afii57433}{0639}
\pdfglyphtounicode{afii57434}{063A}
\pdfglyphtounicode{afii57440}{0640}
\pdfglyphtounicode{afii57441}{0641}
\pdfglyphtounicode{afii57442}{0642}
\pdfglyphtounicode{afii57443}{0643}
\pdfglyphtounicode{afii57444}{0644}
\pdfglyphtounicode{afii57445}{0645}
\pdfglyphtounicode{afii57446}{0646}
\pdfglyphtounicode{afii57448}{0648}
\pdfglyphtounicode{afii57449}{0649}
\pdfglyphtounicode{afii57450}{064A}
\pdfglyphtounicode{afii57451}{064B}
\pdfglyphtounicode{afii57452}{064C}
\pdfglyphtounicode{afii57453}{064D}
\pdfglyphtounicode{afii57454}{064E}
\pdfglyphtounicode{afii57455}{064F}
\pdfglyphtounicode{afii57456}{0650}
\pdfglyphtounicode{afii57457}{0651}
\pdfglyphtounicode{afii57458}{0652}
\pdfglyphtounicode{afii57470}{0647}
\pdfglyphtounicode{afii57505}{06A4}
\pdfglyphtounicode{afii57506}{067E}
\pdfglyphtounicode{afii57507}{0686}
\pdfglyphtounicode{afii57508}{0698}
\pdfglyphtounicode{afii57509}{06AF}
\pdfglyphtounicode{afii57511}{0679}
\pdfglyphtounicode{afii57512}{0688}
\pdfglyphtounicode{afii57513}{0691}
\pdfglyphtounicode{afii57514}{06BA}
\pdfglyphtounicode{afii57519}{06D2}
\pdfglyphtounicode{afii57534}{06D5}
\pdfglyphtounicode{afii57636}{20AA}
\pdfglyphtounicode{afii57645}{05BE}
\pdfglyphtounicode{afii57658}{05C3}
\pdfglyphtounicode{afii57664}{05D0}
\pdfglyphtounicode{afii57665}{05D1}
\pdfglyphtounicode{afii57666}{05D2}
\pdfglyphtounicode{afii57667}{05D3}
\pdfglyphtounicode{afii57668}{05D4}
\pdfglyphtounicode{afii57669}{05D5}
\pdfglyphtounicode{afii57670}{05D6}
\pdfglyphtounicode{afii57671}{05D7}
\pdfglyphtounicode{afii57672}{05D8}
\pdfglyphtounicode{afii57673}{05D9}
\pdfglyphtounicode{afii57674}{05DA}
\pdfglyphtounicode{afii57675}{05DB}
\pdfglyphtounicode{afii57676}{05DC}
\pdfglyphtounicode{afii57677}{05DD}
\pdfglyphtounicode{afii57678}{05DE}
\pdfglyphtounicode{afii57679}{05DF}
\pdfglyphtounicode{afii57680}{05E0}
\pdfglyphtounicode{afii57681}{05E1}
\pdfglyphtounicode{afii57682}{05E2}
\pdfglyphtounicode{afii57683}{05E3}
\pdfglyphtounicode{afii57684}{05E4}
\pdfglyphtounicode{afii57685}{05E5}
\pdfglyphtounicode{afii57686}{05E6}
\pdfglyphtounicode{afii57687}{05E7}
\pdfglyphtounicode{afii57688}{05E8}
\pdfglyphtounicode{afii57689}{05E9}
\pdfglyphtounicode{afii57690}{05EA}
\pdfglyphtounicode{afii57694}{FB2A}
\pdfglyphtounicode{afii57695}{FB2B}
\pdfglyphtounicode{afii57700}{FB4B}
\pdfglyphtounicode{afii57705}{FB1F}
\pdfglyphtounicode{afii57716}{05F0}
\pdfglyphtounicode{afii57717}{05F1}
\pdfglyphtounicode{afii57718}{05F2}
\pdfglyphtounicode{afii57723}{FB35}
\pdfglyphtounicode{afii57793}{05B4}
\pdfglyphtounicode{afii57794}{05B5}
\pdfglyphtounicode{afii57795}{05B6}
\pdfglyphtounicode{afii57796}{05BB}
\pdfglyphtounicode{afii57797}{05B8}
\pdfglyphtounicode{afii57798}{05B7}
\pdfglyphtounicode{afii57799}{05B0}
\pdfglyphtounicode{afii57800}{05B2}
\pdfglyphtounicode{afii57801}{05B1}
\pdfglyphtounicode{afii57802}{05B3}
\pdfglyphtounicode{afii57803}{05C2}
\pdfglyphtounicode{afii57804}{05C1}
\pdfglyphtounicode{afii57806}{05B9}
\pdfglyphtounicode{afii57807}{05BC}
\pdfglyphtounicode{afii57839}{05BD}
\pdfglyphtounicode{afii57841}{05BF}
\pdfglyphtounicode{afii57842}{05C0}
\pdfglyphtounicode{afii57929}{02BC}
\pdfglyphtounicode{afii61248}{2105}
\pdfglyphtounicode{afii61289}{2113}
\pdfglyphtounicode{afii61352}{2116}
\pdfglyphtounicode{afii61573}{202C}
\pdfglyphtounicode{afii61574}{202D}
\pdfglyphtounicode{afii61575}{202E}
\pdfglyphtounicode{afii61664}{200C}
\pdfglyphtounicode{afii63167}{066D}
\pdfglyphtounicode{afii64937}{02BD}
\pdfglyphtounicode{agrave}{00E0}
\pdfglyphtounicode{agujarati}{0A85}
\pdfglyphtounicode{agurmukhi}{0A05}
\pdfglyphtounicode{ahiragana}{3042}
\pdfglyphtounicode{ahookabove}{1EA3}
\pdfglyphtounicode{aibengali}{0990}
\pdfglyphtounicode{aibopomofo}{311E}
\pdfglyphtounicode{aideva}{0910}
\pdfglyphtounicode{aiecyrillic}{04D5}
\pdfglyphtounicode{aigujarati}{0A90}
\pdfglyphtounicode{aigurmukhi}{0A10}
\pdfglyphtounicode{aimatragurmukhi}{0A48}
\pdfglyphtounicode{ainarabic}{0639}
\pdfglyphtounicode{ainfinalarabic}{FECA}
\pdfglyphtounicode{aininitialarabic}{FECB}
\pdfglyphtounicode{ainmedialarabic}{FECC}
\pdfglyphtounicode{ainvertedbreve}{0203}
\pdfglyphtounicode{aivowelsignbengali}{09C8}
\pdfglyphtounicode{aivowelsigndeva}{0948}
\pdfglyphtounicode{aivowelsigngujarati}{0AC8}
\pdfglyphtounicode{akatakana}{30A2}
\pdfglyphtounicode{akatakanahalfwidth}{FF71}
\pdfglyphtounicode{akorean}{314F}
\pdfglyphtounicode{alef}{05D0}
\pdfglyphtounicode{alefarabic}{0627}
\pdfglyphtounicode{alefdageshhebrew}{FB30}
\pdfglyphtounicode{aleffinalarabic}{FE8E}
\pdfglyphtounicode{alefhamzaabovearabic}{0623}
\pdfglyphtounicode{alefhamzaabovefinalarabic}{FE84}
\pdfglyphtounicode{alefhamzabelowarabic}{0625}
\pdfglyphtounicode{alefhamzabelowfinalarabic}{FE88}
\pdfglyphtounicode{alefhebrew}{05D0}
\pdfglyphtounicode{aleflamedhebrew}{FB4F}
\pdfglyphtounicode{alefmaddaabovearabic}{0622}
\pdfglyphtounicode{alefmaddaabovefinalarabic}{FE82}
\pdfglyphtounicode{alefmaksuraarabic}{0649}
\pdfglyphtounicode{alefmaksurafinalarabic}{FEF0}
\pdfglyphtounicode{alefmaksurainitialarabic}{FEF3}
\pdfglyphtounicode{alefmaksuramedialarabic}{FEF4}
\pdfglyphtounicode{alefpatahhebrew}{FB2E}
\pdfglyphtounicode{alefqamatshebrew}{FB2F}
\pdfglyphtounicode{aleph}{2135}
\pdfglyphtounicode{allequal}{224C}
\pdfglyphtounicode{alpha}{03B1}
\pdfglyphtounicode{alphatonos}{03AC}
\pdfglyphtounicode{amacron}{0101}
\pdfglyphtounicode{amonospace}{FF41}
\pdfglyphtounicode{ampersand}{0026}
\pdfglyphtounicode{ampersandmonospace}{FF06}
\pdfglyphtounicode{ampersandsmall}{F726}
\pdfglyphtounicode{amsquare}{33C2}
\pdfglyphtounicode{anbopomofo}{3122}
\pdfglyphtounicode{angbopomofo}{3124}
\pdfglyphtounicode{angkhankhuthai}{0E5A}
\pdfglyphtounicode{angle}{2220}
\pdfglyphtounicode{anglebracketleft}{3008}
\pdfglyphtounicode{anglebracketleftvertical}{FE3F}
\pdfglyphtounicode{anglebracketright}{3009}
\pdfglyphtounicode{anglebracketrightvertical}{FE40}
\pdfglyphtounicode{angleleft}{2329}
\pdfglyphtounicode{angleright}{232A}
\pdfglyphtounicode{angstrom}{212B}
\pdfglyphtounicode{anoteleia}{0387}
\pdfglyphtounicode{anudattadeva}{0952}
\pdfglyphtounicode{anusvarabengali}{0982}
\pdfglyphtounicode{anusvaradeva}{0902}
\pdfglyphtounicode{anusvaragujarati}{0A82}
\pdfglyphtounicode{aogonek}{0105}
\pdfglyphtounicode{apaatosquare}{3300}
\pdfglyphtounicode{aparen}{249C}
\pdfglyphtounicode{apostrophearmenian}{055A}
\pdfglyphtounicode{apostrophemod}{02BC}
\pdfglyphtounicode{apple}{F8FF}
\pdfglyphtounicode{approaches}{2250}
\pdfglyphtounicode{approxequal}{2248}
\pdfglyphtounicode{approxequalorimage}{2252}
\pdfglyphtounicode{approximatelyequal}{2245}
\pdfglyphtounicode{araeaekorean}{318E}
\pdfglyphtounicode{araeakorean}{318D}
\pdfglyphtounicode{arc}{2312}
\pdfglyphtounicode{arighthalfring}{1E9A}
\pdfglyphtounicode{aring}{00E5}
\pdfglyphtounicode{aringacute}{01FB}
\pdfglyphtounicode{aringbelow}{1E01}
\pdfglyphtounicode{arrowboth}{2194}
\pdfglyphtounicode{arrowdashdown}{21E3}
\pdfglyphtounicode{arrowdashleft}{21E0}
\pdfglyphtounicode{arrowdashright}{21E2}
\pdfglyphtounicode{arrowdashup}{21E1}
\pdfglyphtounicode{arrowdblboth}{21D4}
\pdfglyphtounicode{arrowdbldown}{21D3}
\pdfglyphtounicode{arrowdblleft}{21D0}
\pdfglyphtounicode{arrowdblright}{21D2}
\pdfglyphtounicode{arrowdblup}{21D1}
\pdfglyphtounicode{arrowdown}{2193}
\pdfglyphtounicode{arrowdownleft}{2199}
\pdfglyphtounicode{arrowdownright}{2198}
\pdfglyphtounicode{arrowdownwhite}{21E9}
\pdfglyphtounicode{arrowheaddownmod}{02C5}
\pdfglyphtounicode{arrowheadleftmod}{02C2}
\pdfglyphtounicode{arrowheadrightmod}{02C3}
\pdfglyphtounicode{arrowheadupmod}{02C4}
\pdfglyphtounicode{arrowhorizex}{F8E7}
\pdfglyphtounicode{arrowleft}{2190}
\pdfglyphtounicode{arrowleftdbl}{21D0}
\pdfglyphtounicode{arrowleftdblstroke}{21CD}
\pdfglyphtounicode{arrowleftoverright}{21C6}
\pdfglyphtounicode{arrowleftwhite}{21E6}
\pdfglyphtounicode{arrowright}{2192}
\pdfglyphtounicode{arrowrightdblstroke}{21CF}
\pdfglyphtounicode{arrowrightheavy}{279E}
\pdfglyphtounicode{arrowrightoverleft}{21C4}
\pdfglyphtounicode{arrowrightwhite}{21E8}
\pdfglyphtounicode{arrowtableft}{21E4}
\pdfglyphtounicode{arrowtabright}{21E5}
\pdfglyphtounicode{arrowup}{2191}
\pdfglyphtounicode{arrowupdn}{2195}
\pdfglyphtounicode{arrowupdnbse}{21A8}
\pdfglyphtounicode{arrowupdownbase}{21A8}
\pdfglyphtounicode{arrowupleft}{2196}
\pdfglyphtounicode{arrowupleftofdown}{21C5}
\pdfglyphtounicode{arrowupright}{2197}
\pdfglyphtounicode{arrowupwhite}{21E7}
\pdfglyphtounicode{arrowvertex}{F8E6}
\pdfglyphtounicode{asciicircum}{005E}
\pdfglyphtounicode{asciicircummonospace}{FF3E}
\pdfglyphtounicode{asciitilde}{007E}
\pdfglyphtounicode{asciitildemonospace}{FF5E}
\pdfglyphtounicode{ascript}{0251}
\pdfglyphtounicode{ascriptturned}{0252}
\pdfglyphtounicode{asmallhiragana}{3041}
\pdfglyphtounicode{asmallkatakana}{30A1}
\pdfglyphtounicode{asmallkatakanahalfwidth}{FF67}
\pdfglyphtounicode{asterisk}{002A}
\pdfglyphtounicode{asteriskaltonearabic}{066D}
\pdfglyphtounicode{asteriskarabic}{066D}
\pdfglyphtounicode{asteriskmath}{2217}
\pdfglyphtounicode{asteriskmonospace}{FF0A}
\pdfglyphtounicode{asterisksmall}{FE61}
\pdfglyphtounicode{asterism}{2042}
\pdfglyphtounicode{asuperior}{F6E9}
\pdfglyphtounicode{asymptoticallyequal}{2243}
\pdfglyphtounicode{at}{0040}
\pdfglyphtounicode{atilde}{00E3}
\pdfglyphtounicode{atmonospace}{FF20}
\pdfglyphtounicode{atsmall}{FE6B}
\pdfglyphtounicode{aturned}{0250}
\pdfglyphtounicode{aubengali}{0994}
\pdfglyphtounicode{aubopomofo}{3120}
\pdfglyphtounicode{audeva}{0914}
\pdfglyphtounicode{augujarati}{0A94}
\pdfglyphtounicode{augurmukhi}{0A14}
\pdfglyphtounicode{aulengthmarkbengali}{09D7}
\pdfglyphtounicode{aumatragurmukhi}{0A4C}
\pdfglyphtounicode{auvowelsignbengali}{09CC}
\pdfglyphtounicode{auvowelsigndeva}{094C}
\pdfglyphtounicode{auvowelsigngujarati}{0ACC}
\pdfglyphtounicode{avagrahadeva}{093D}
\pdfglyphtounicode{aybarmenian}{0561}
\pdfglyphtounicode{ayin}{05E2}
\pdfglyphtounicode{ayinaltonehebrew}{FB20}
\pdfglyphtounicode{ayinhebrew}{05E2}
\pdfglyphtounicode{b}{0062}
\pdfglyphtounicode{babengali}{09AC}
\pdfglyphtounicode{backslash}{005C}
\pdfglyphtounicode{backslashmonospace}{FF3C}
\pdfglyphtounicode{badeva}{092C}
\pdfglyphtounicode{bagujarati}{0AAC}
\pdfglyphtounicode{bagurmukhi}{0A2C}
\pdfglyphtounicode{bahiragana}{3070}
\pdfglyphtounicode{bahtthai}{0E3F}
\pdfglyphtounicode{bakatakana}{30D0}
\pdfglyphtounicode{bar}{007C}
\pdfglyphtounicode{barmonospace}{FF5C}
\pdfglyphtounicode{bbopomofo}{3105}
\pdfglyphtounicode{bcircle}{24D1}
\pdfglyphtounicode{bdotaccent}{1E03}
\pdfglyphtounicode{bdotbelow}{1E05}
\pdfglyphtounicode{beamedsixteenthnotes}{266C}
\pdfglyphtounicode{because}{2235}
\pdfglyphtounicode{becyrillic}{0431}
\pdfglyphtounicode{beharabic}{0628}
\pdfglyphtounicode{behfinalarabic}{FE90}
\pdfglyphtounicode{behinitialarabic}{FE91}
\pdfglyphtounicode{behiragana}{3079}
\pdfglyphtounicode{behmedialarabic}{FE92}
\pdfglyphtounicode{behmeeminitialarabic}{FC9F}
\pdfglyphtounicode{behmeemisolatedarabic}{FC08}
\pdfglyphtounicode{behnoonfinalarabic}{FC6D}
\pdfglyphtounicode{bekatakana}{30D9}
\pdfglyphtounicode{benarmenian}{0562}
\pdfglyphtounicode{bet}{05D1}
\pdfglyphtounicode{beta}{03B2}
\pdfglyphtounicode{betasymbolgreek}{03D0}
\pdfglyphtounicode{betdagesh}{FB31}
\pdfglyphtounicode{betdageshhebrew}{FB31}
\pdfglyphtounicode{bethebrew}{05D1}
\pdfglyphtounicode{betrafehebrew}{FB4C}
\pdfglyphtounicode{bhabengali}{09AD}
\pdfglyphtounicode{bhadeva}{092D}
\pdfglyphtounicode{bhagujarati}{0AAD}
\pdfglyphtounicode{bhagurmukhi}{0A2D}
\pdfglyphtounicode{bhook}{0253}
\pdfglyphtounicode{bihiragana}{3073}
\pdfglyphtounicode{bikatakana}{30D3}
\pdfglyphtounicode{bilabialclick}{0298}
\pdfglyphtounicode{bindigurmukhi}{0A02}
\pdfglyphtounicode{birusquare}{3331}
\pdfglyphtounicode{blackcircle}{25CF}
\pdfglyphtounicode{blackdiamond}{25C6}
\pdfglyphtounicode{blackdownpointingtriangle}{25BC}
\pdfglyphtounicode{blackleftpointingpointer}{25C4}
\pdfglyphtounicode{blackleftpointingtriangle}{25C0}
\pdfglyphtounicode{blacklenticularbracketleft}{3010}
\pdfglyphtounicode{blacklenticularbracketleftvertical}{FE3B}
\pdfglyphtounicode{blacklenticularbracketright}{3011}
\pdfglyphtounicode{blacklenticularbracketrightvertical}{FE3C}
\pdfglyphtounicode{blacklowerlefttriangle}{25E3}
\pdfglyphtounicode{blacklowerrighttriangle}{25E2}
\pdfglyphtounicode{blackrectangle}{25AC}
\pdfglyphtounicode{blackrightpointingpointer}{25BA}
\pdfglyphtounicode{blackrightpointingtriangle}{25B6}
\pdfglyphtounicode{blacksmallsquare}{25AA}
\pdfglyphtounicode{blacksmilingface}{263B}
\pdfglyphtounicode{blacksquare}{25A0}
\pdfglyphtounicode{blackstar}{2605}
\pdfglyphtounicode{blackupperlefttriangle}{25E4}
\pdfglyphtounicode{blackupperrighttriangle}{25E5}
\pdfglyphtounicode{blackuppointingsmalltriangle}{25B4}
\pdfglyphtounicode{blackuppointingtriangle}{25B2}
\pdfglyphtounicode{blank}{2423}
\pdfglyphtounicode{blinebelow}{1E07}
\pdfglyphtounicode{block}{2588}
\pdfglyphtounicode{bmonospace}{FF42}
\pdfglyphtounicode{bobaimaithai}{0E1A}
\pdfglyphtounicode{bohiragana}{307C}
\pdfglyphtounicode{bokatakana}{30DC}
\pdfglyphtounicode{bparen}{249D}
\pdfglyphtounicode{bqsquare}{33C3}
\pdfglyphtounicode{braceex}{F8F4}
\pdfglyphtounicode{braceleft}{007B}
\pdfglyphtounicode{braceleftbt}{F8F3}
\pdfglyphtounicode{braceleftmid}{F8F2}
\pdfglyphtounicode{braceleftmonospace}{FF5B}
\pdfglyphtounicode{braceleftsmall}{FE5B}
\pdfglyphtounicode{bracelefttp}{F8F1}
\pdfglyphtounicode{braceleftvertical}{FE37}
\pdfglyphtounicode{braceright}{007D}
\pdfglyphtounicode{bracerightbt}{F8FE}
\pdfglyphtounicode{bracerightmid}{F8FD}
\pdfglyphtounicode{bracerightmonospace}{FF5D}
\pdfglyphtounicode{bracerightsmall}{FE5C}
\pdfglyphtounicode{bracerighttp}{F8FC}
\pdfglyphtounicode{bracerightvertical}{FE38}
\pdfglyphtounicode{bracketleft}{005B}
\pdfglyphtounicode{bracketleftbt}{F8F0}
\pdfglyphtounicode{bracketleftex}{F8EF}
\pdfglyphtounicode{bracketleftmonospace}{FF3B}
\pdfglyphtounicode{bracketlefttp}{F8EE}
\pdfglyphtounicode{bracketright}{005D}
\pdfglyphtounicode{bracketrightbt}{F8FB}
\pdfglyphtounicode{bracketrightex}{F8FA}
\pdfglyphtounicode{bracketrightmonospace}{FF3D}
\pdfglyphtounicode{bracketrighttp}{F8F9}
\pdfglyphtounicode{breve}{02D8}
\pdfglyphtounicode{brevebelowcmb}{032E}
\pdfglyphtounicode{brevecmb}{0306}
\pdfglyphtounicode{breveinvertedbelowcmb}{032F}
\pdfglyphtounicode{breveinvertedcmb}{0311}
\pdfglyphtounicode{breveinverteddoublecmb}{0361}
\pdfglyphtounicode{bridgebelowcmb}{032A}
\pdfglyphtounicode{bridgeinvertedbelowcmb}{033A}
\pdfglyphtounicode{brokenbar}{00A6}
\pdfglyphtounicode{bstroke}{0180}
\pdfglyphtounicode{bsuperior}{F6EA}
\pdfglyphtounicode{btopbar}{0183}
\pdfglyphtounicode{buhiragana}{3076}
\pdfglyphtounicode{bukatakana}{30D6}
\pdfglyphtounicode{bullet}{2022}
\pdfglyphtounicode{bulletinverse}{25D8}
\pdfglyphtounicode{bulletoperator}{2219}
\pdfglyphtounicode{bullseye}{25CE}
\pdfglyphtounicode{c}{0063}
\pdfglyphtounicode{caarmenian}{056E}
\pdfglyphtounicode{cabengali}{099A}
\pdfglyphtounicode{cacute}{0107}
\pdfglyphtounicode{cadeva}{091A}
\pdfglyphtounicode{cagujarati}{0A9A}
\pdfglyphtounicode{cagurmukhi}{0A1A}
\pdfglyphtounicode{calsquare}{3388}
\pdfglyphtounicode{candrabindubengali}{0981}
\pdfglyphtounicode{candrabinducmb}{0310}
\pdfglyphtounicode{candrabindudeva}{0901}
\pdfglyphtounicode{candrabindugujarati}{0A81}
\pdfglyphtounicode{capslock}{21EA}
\pdfglyphtounicode{careof}{2105}
\pdfglyphtounicode{caron}{02C7}
\pdfglyphtounicode{caronbelowcmb}{032C}
\pdfglyphtounicode{caroncmb}{030C}
\pdfglyphtounicode{carriagereturn}{21B5}
\pdfglyphtounicode{cbopomofo}{3118}
\pdfglyphtounicode{ccaron}{010D}
\pdfglyphtounicode{ccedilla}{00E7}
\pdfglyphtounicode{ccedillaacute}{1E09}
\pdfglyphtounicode{ccircle}{24D2}
\pdfglyphtounicode{ccircumflex}{0109}
\pdfglyphtounicode{ccurl}{0255}
\pdfglyphtounicode{cdot}{010B}
\pdfglyphtounicode{cdotaccent}{010B}
\pdfglyphtounicode{cdsquare}{33C5}
\pdfglyphtounicode{cedilla}{00B8}
\pdfglyphtounicode{cedillacmb}{0327}
\pdfglyphtounicode{cent}{00A2}
\pdfglyphtounicode{centigrade}{2103}
\pdfglyphtounicode{centinferior}{F6DF}
\pdfglyphtounicode{centmonospace}{FFE0}
\pdfglyphtounicode{centoldstyle}{F7A2}
\pdfglyphtounicode{centsuperior}{F6E0}
\pdfglyphtounicode{chaarmenian}{0579}
\pdfglyphtounicode{chabengali}{099B}
\pdfglyphtounicode{chadeva}{091B}
\pdfglyphtounicode{chagujarati}{0A9B}
\pdfglyphtounicode{chagurmukhi}{0A1B}
\pdfglyphtounicode{chbopomofo}{3114}
\pdfglyphtounicode{cheabkhasiancyrillic}{04BD}
\pdfglyphtounicode{checkmark}{2713}
\pdfglyphtounicode{checyrillic}{0447}
\pdfglyphtounicode{chedescenderabkhasiancyrillic}{04BF}
\pdfglyphtounicode{chedescendercyrillic}{04B7}
\pdfglyphtounicode{chedieresiscyrillic}{04F5}
\pdfglyphtounicode{cheharmenian}{0573}
\pdfglyphtounicode{chekhakassiancyrillic}{04CC}
\pdfglyphtounicode{cheverticalstrokecyrillic}{04B9}
\pdfglyphtounicode{chi}{03C7}
\pdfglyphtounicode{chieuchacirclekorean}{3277}
\pdfglyphtounicode{chieuchaparenkorean}{3217}
\pdfglyphtounicode{chieuchcirclekorean}{3269}
\pdfglyphtounicode{chieuchkorean}{314A}
\pdfglyphtounicode{chieuchparenkorean}{3209}
\pdfglyphtounicode{chochangthai}{0E0A}
\pdfglyphtounicode{chochanthai}{0E08}
\pdfglyphtounicode{chochingthai}{0E09}
\pdfglyphtounicode{chochoethai}{0E0C}
\pdfglyphtounicode{chook}{0188}
\pdfglyphtounicode{cieucacirclekorean}{3276}
\pdfglyphtounicode{cieucaparenkorean}{3216}
\pdfglyphtounicode{cieuccirclekorean}{3268}
\pdfglyphtounicode{cieuckorean}{3148}
\pdfglyphtounicode{cieucparenkorean}{3208}
\pdfglyphtounicode{cieucuparenkorean}{321C}
\pdfglyphtounicode{circle}{25CB}
\pdfglyphtounicode{circlemultiply}{2297}
\pdfglyphtounicode{circleot}{2299}
\pdfglyphtounicode{circleplus}{2295}
\pdfglyphtounicode{circlepostalmark}{3036}
\pdfglyphtounicode{circlewithlefthalfblack}{25D0}
\pdfglyphtounicode{circlewithrighthalfblack}{25D1}
\pdfglyphtounicode{circumflex}{02C6}
\pdfglyphtounicode{circumflexbelowcmb}{032D}
\pdfglyphtounicode{circumflexcmb}{0302}
\pdfglyphtounicode{clear}{2327}
\pdfglyphtounicode{clickalveolar}{01C2}
\pdfglyphtounicode{clickdental}{01C0}
\pdfglyphtounicode{clicklateral}{01C1}
\pdfglyphtounicode{clickretroflex}{01C3}
\pdfglyphtounicode{club}{2663}
\pdfglyphtounicode{clubsuitblack}{2663}
\pdfglyphtounicode{clubsuitwhite}{2667}
\pdfglyphtounicode{cmcubedsquare}{33A4}
\pdfglyphtounicode{cmonospace}{FF43}
\pdfglyphtounicode{cmsquaredsquare}{33A0}
\pdfglyphtounicode{coarmenian}{0581}
\pdfglyphtounicode{colon}{003A}
\pdfglyphtounicode{colonmonetary}{20A1}
\pdfglyphtounicode{colonmonospace}{FF1A}
\pdfglyphtounicode{colonsign}{20A1}
\pdfglyphtounicode{colonsmall}{FE55}
\pdfglyphtounicode{colontriangularhalfmod}{02D1}
\pdfglyphtounicode{colontriangularmod}{02D0}
\pdfglyphtounicode{comma}{002C}
\pdfglyphtounicode{commaabovecmb}{0313}
\pdfglyphtounicode{commaaboverightcmb}{0315}
\pdfglyphtounicode{commaaccent}{F6C3}
\pdfglyphtounicode{commaarabic}{060C}
\pdfglyphtounicode{commaarmenian}{055D}
\pdfglyphtounicode{commainferior}{F6E1}
\pdfglyphtounicode{commamonospace}{FF0C}
\pdfglyphtounicode{commareversedabovecmb}{0314}
\pdfglyphtounicode{commareversedmod}{02BD}
\pdfglyphtounicode{commasmall}{FE50}
\pdfglyphtounicode{commasuperior}{F6E2}
\pdfglyphtounicode{commaturnedabovecmb}{0312}
\pdfglyphtounicode{commaturnedmod}{02BB}
\pdfglyphtounicode{compass}{263C}
\pdfglyphtounicode{congruent}{2245}
\pdfglyphtounicode{contourintegral}{222E}
\pdfglyphtounicode{control}{2303}
\pdfglyphtounicode{controlACK}{0006}
\pdfglyphtounicode{controlBEL}{0007}
\pdfglyphtounicode{controlBS}{0008}
\pdfglyphtounicode{controlCAN}{0018}
\pdfglyphtounicode{controlCR}{000D}
\pdfglyphtounicode{controlDC1}{0011}
\pdfglyphtounicode{controlDC2}{0012}
\pdfglyphtounicode{controlDC3}{0013}
\pdfglyphtounicode{controlDC4}{0014}
\pdfglyphtounicode{controlDEL}{007F}
\pdfglyphtounicode{controlDLE}{0010}
\pdfglyphtounicode{controlEM}{0019}
\pdfglyphtounicode{controlENQ}{0005}
\pdfglyphtounicode{controlEOT}{0004}
\pdfglyphtounicode{controlESC}{001B}
\pdfglyphtounicode{controlETB}{0017}
\pdfglyphtounicode{controlETX}{0003}
\pdfglyphtounicode{controlFF}{000C}
\pdfglyphtounicode{controlFS}{001C}
\pdfglyphtounicode{controlGS}{001D}
\pdfglyphtounicode{controlHT}{0009}
\pdfglyphtounicode{controlLF}{000A}
\pdfglyphtounicode{controlNAK}{0015}
\pdfglyphtounicode{controlRS}{001E}
\pdfglyphtounicode{controlSI}{000F}
\pdfglyphtounicode{controlSO}{000E}
\pdfglyphtounicode{controlSOT}{0002}
\pdfglyphtounicode{controlSTX}{0001}
\pdfglyphtounicode{controlSUB}{001A}
\pdfglyphtounicode{controlSYN}{0016}
\pdfglyphtounicode{controlUS}{001F}
\pdfglyphtounicode{controlVT}{000B}
\pdfglyphtounicode{copyright}{00A9}
\pdfglyphtounicode{copyrightsans}{F8E9}
\pdfglyphtounicode{copyrightserif}{F6D9}
\pdfglyphtounicode{cornerbracketleft}{300C}
\pdfglyphtounicode{cornerbracketlefthalfwidth}{FF62}
\pdfglyphtounicode{cornerbracketleftvertical}{FE41}
\pdfglyphtounicode{cornerbracketright}{300D}
\pdfglyphtounicode{cornerbracketrighthalfwidth}{FF63}
\pdfglyphtounicode{cornerbracketrightvertical}{FE42}
\pdfglyphtounicode{corporationsquare}{337F}
\pdfglyphtounicode{cosquare}{33C7}
\pdfglyphtounicode{coverkgsquare}{33C6}
\pdfglyphtounicode{cparen}{249E}
\pdfglyphtounicode{cruzeiro}{20A2}
\pdfglyphtounicode{cstretched}{0297}
\pdfglyphtounicode{curlyand}{22CF}
\pdfglyphtounicode{curlyor}{22CE}
\pdfglyphtounicode{currency}{00A4}
\pdfglyphtounicode{cyrBreve}{F6D1}
\pdfglyphtounicode{cyrFlex}{F6D2}
\pdfglyphtounicode{cyrbreve}{F6D4}
\pdfglyphtounicode{cyrflex}{F6D5}
\pdfglyphtounicode{d}{0064}
\pdfglyphtounicode{daarmenian}{0564}
\pdfglyphtounicode{dabengali}{09A6}
\pdfglyphtounicode{dadarabic}{0636}
\pdfglyphtounicode{dadeva}{0926}
\pdfglyphtounicode{dadfinalarabic}{FEBE}
\pdfglyphtounicode{dadinitialarabic}{FEBF}
\pdfglyphtounicode{dadmedialarabic}{FEC0}
\pdfglyphtounicode{dagesh}{05BC}
\pdfglyphtounicode{dageshhebrew}{05BC}
\pdfglyphtounicode{dagger}{2020}
\pdfglyphtounicode{daggerdbl}{2021}
\pdfglyphtounicode{dagujarati}{0AA6}
\pdfglyphtounicode{dagurmukhi}{0A26}
\pdfglyphtounicode{dahiragana}{3060}
\pdfglyphtounicode{dakatakana}{30C0}
\pdfglyphtounicode{dalarabic}{062F}
\pdfglyphtounicode{dalet}{05D3}
\pdfglyphtounicode{daletdagesh}{FB33}
\pdfglyphtounicode{daletdageshhebrew}{FB33}
% dalethatafpatah;05D3 05B2
% dalethatafpatahhebrew;05D3 05B2
% dalethatafsegol;05D3 05B1
% dalethatafsegolhebrew;05D3 05B1
\pdfglyphtounicode{dalethebrew}{05D3}
% dalethiriq;05D3 05B4
% dalethiriqhebrew;05D3 05B4
% daletholam;05D3 05B9
% daletholamhebrew;05D3 05B9
% daletpatah;05D3 05B7
% daletpatahhebrew;05D3 05B7
% daletqamats;05D3 05B8
% daletqamatshebrew;05D3 05B8
% daletqubuts;05D3 05BB
% daletqubutshebrew;05D3 05BB
% daletsegol;05D3 05B6
% daletsegolhebrew;05D3 05B6
% daletsheva;05D3 05B0
% daletshevahebrew;05D3 05B0
% dalettsere;05D3 05B5
% dalettserehebrew;05D3 05B5
\pdfglyphtounicode{dalfinalarabic}{FEAA}
\pdfglyphtounicode{dammaarabic}{064F}
\pdfglyphtounicode{dammalowarabic}{064F}
\pdfglyphtounicode{dammatanaltonearabic}{064C}
\pdfglyphtounicode{dammatanarabic}{064C}
\pdfglyphtounicode{danda}{0964}
\pdfglyphtounicode{dargahebrew}{05A7}
\pdfglyphtounicode{dargalefthebrew}{05A7}
\pdfglyphtounicode{dasiapneumatacyrilliccmb}{0485}
\pdfglyphtounicode{dblGrave}{F6D3}
\pdfglyphtounicode{dblanglebracketleft}{300A}
\pdfglyphtounicode{dblanglebracketleftvertical}{FE3D}
\pdfglyphtounicode{dblanglebracketright}{300B}
\pdfglyphtounicode{dblanglebracketrightvertical}{FE3E}
\pdfglyphtounicode{dblarchinvertedbelowcmb}{032B}
\pdfglyphtounicode{dblarrowleft}{21D4}
\pdfglyphtounicode{dblarrowright}{21D2}
\pdfglyphtounicode{dbldanda}{0965}
\pdfglyphtounicode{dblgrave}{F6D6}
\pdfglyphtounicode{dblgravecmb}{030F}
\pdfglyphtounicode{dblintegral}{222C}
\pdfglyphtounicode{dbllowline}{2017}
\pdfglyphtounicode{dbllowlinecmb}{0333}
\pdfglyphtounicode{dbloverlinecmb}{033F}
\pdfglyphtounicode{dblprimemod}{02BA}
\pdfglyphtounicode{dblverticalbar}{2016}
\pdfglyphtounicode{dblverticallineabovecmb}{030E}
\pdfglyphtounicode{dbopomofo}{3109}
\pdfglyphtounicode{dbsquare}{33C8}
\pdfglyphtounicode{dcaron}{010F}
\pdfglyphtounicode{dcedilla}{1E11}
\pdfglyphtounicode{dcircle}{24D3}
\pdfglyphtounicode{dcircumflexbelow}{1E13}
\pdfglyphtounicode{dcroat}{0111}
\pdfglyphtounicode{ddabengali}{09A1}
\pdfglyphtounicode{ddadeva}{0921}
\pdfglyphtounicode{ddagujarati}{0AA1}
\pdfglyphtounicode{ddagurmukhi}{0A21}
\pdfglyphtounicode{ddalarabic}{0688}
\pdfglyphtounicode{ddalfinalarabic}{FB89}
\pdfglyphtounicode{dddhadeva}{095C}
\pdfglyphtounicode{ddhabengali}{09A2}
\pdfglyphtounicode{ddhadeva}{0922}
\pdfglyphtounicode{ddhagujarati}{0AA2}
\pdfglyphtounicode{ddhagurmukhi}{0A22}
\pdfglyphtounicode{ddotaccent}{1E0B}
\pdfglyphtounicode{ddotbelow}{1E0D}
\pdfglyphtounicode{decimalseparatorarabic}{066B}
\pdfglyphtounicode{decimalseparatorpersian}{066B}
\pdfglyphtounicode{decyrillic}{0434}
\pdfglyphtounicode{degree}{00B0}
\pdfglyphtounicode{dehihebrew}{05AD}
\pdfglyphtounicode{dehiragana}{3067}
\pdfglyphtounicode{deicoptic}{03EF}
\pdfglyphtounicode{dekatakana}{30C7}
\pdfglyphtounicode{deleteleft}{232B}
\pdfglyphtounicode{deleteright}{2326}
\pdfglyphtounicode{delta}{03B4}
\pdfglyphtounicode{deltaturned}{018D}
\pdfglyphtounicode{denominatorminusonenumeratorbengali}{09F8}
\pdfglyphtounicode{dezh}{02A4}
\pdfglyphtounicode{dhabengali}{09A7}
\pdfglyphtounicode{dhadeva}{0927}
\pdfglyphtounicode{dhagujarati}{0AA7}
\pdfglyphtounicode{dhagurmukhi}{0A27}
\pdfglyphtounicode{dhook}{0257}
\pdfglyphtounicode{dialytikatonos}{0385}
\pdfglyphtounicode{dialytikatonoscmb}{0344}
\pdfglyphtounicode{diamond}{2666}
\pdfglyphtounicode{diamondsuitwhite}{2662}
\pdfglyphtounicode{dieresis}{00A8}
\pdfglyphtounicode{dieresisacute}{F6D7}
\pdfglyphtounicode{dieresisbelowcmb}{0324}
\pdfglyphtounicode{dieresiscmb}{0308}
\pdfglyphtounicode{dieresisgrave}{F6D8}
\pdfglyphtounicode{dieresistonos}{0385}
\pdfglyphtounicode{dihiragana}{3062}
\pdfglyphtounicode{dikatakana}{30C2}
\pdfglyphtounicode{dittomark}{3003}
\pdfglyphtounicode{divide}{00F7}
\pdfglyphtounicode{divides}{2223}
\pdfglyphtounicode{divisionslash}{2215}
\pdfglyphtounicode{djecyrillic}{0452}
\pdfglyphtounicode{dkshade}{2593}
\pdfglyphtounicode{dlinebelow}{1E0F}
\pdfglyphtounicode{dlsquare}{3397}
\pdfglyphtounicode{dmacron}{0111}
\pdfglyphtounicode{dmonospace}{FF44}
\pdfglyphtounicode{dnblock}{2584}
\pdfglyphtounicode{dochadathai}{0E0E}
\pdfglyphtounicode{dodekthai}{0E14}
\pdfglyphtounicode{dohiragana}{3069}
\pdfglyphtounicode{dokatakana}{30C9}
\pdfglyphtounicode{dollar}{0024}
\pdfglyphtounicode{dollarinferior}{F6E3}
\pdfglyphtounicode{dollarmonospace}{FF04}
\pdfglyphtounicode{dollaroldstyle}{F724}
\pdfglyphtounicode{dollarsmall}{FE69}
\pdfglyphtounicode{dollarsuperior}{F6E4}
\pdfglyphtounicode{dong}{20AB}
\pdfglyphtounicode{dorusquare}{3326}
\pdfglyphtounicode{dotaccent}{02D9}
\pdfglyphtounicode{dotaccentcmb}{0307}
\pdfglyphtounicode{dotbelowcmb}{0323}
\pdfglyphtounicode{dotbelowcomb}{0323}
\pdfglyphtounicode{dotkatakana}{30FB}
\pdfglyphtounicode{dotlessi}{0131}
\pdfglyphtounicode{dotlessj}{F6BE}
\pdfglyphtounicode{dotlessjstrokehook}{0284}
\pdfglyphtounicode{dotmath}{22C5}
\pdfglyphtounicode{dottedcircle}{25CC}
\pdfglyphtounicode{doubleyodpatah}{FB1F}
\pdfglyphtounicode{doubleyodpatahhebrew}{FB1F}
\pdfglyphtounicode{downtackbelowcmb}{031E}
\pdfglyphtounicode{downtackmod}{02D5}
\pdfglyphtounicode{dparen}{249F}
\pdfglyphtounicode{dsuperior}{F6EB}
\pdfglyphtounicode{dtail}{0256}
\pdfglyphtounicode{dtopbar}{018C}
\pdfglyphtounicode{duhiragana}{3065}
\pdfglyphtounicode{dukatakana}{30C5}
\pdfglyphtounicode{dz}{01F3}
\pdfglyphtounicode{dzaltone}{02A3}
\pdfglyphtounicode{dzcaron}{01C6}
\pdfglyphtounicode{dzcurl}{02A5}
\pdfglyphtounicode{dzeabkhasiancyrillic}{04E1}
\pdfglyphtounicode{dzecyrillic}{0455}
\pdfglyphtounicode{dzhecyrillic}{045F}
\pdfglyphtounicode{e}{0065}
\pdfglyphtounicode{eacute}{00E9}
\pdfglyphtounicode{earth}{2641}
\pdfglyphtounicode{ebengali}{098F}
\pdfglyphtounicode{ebopomofo}{311C}
\pdfglyphtounicode{ebreve}{0115}
\pdfglyphtounicode{ecandradeva}{090D}
\pdfglyphtounicode{ecandragujarati}{0A8D}
\pdfglyphtounicode{ecandravowelsigndeva}{0945}
\pdfglyphtounicode{ecandravowelsigngujarati}{0AC5}
\pdfglyphtounicode{ecaron}{011B}
\pdfglyphtounicode{ecedillabreve}{1E1D}
\pdfglyphtounicode{echarmenian}{0565}
\pdfglyphtounicode{echyiwnarmenian}{0587}
\pdfglyphtounicode{ecircle}{24D4}
\pdfglyphtounicode{ecircumflex}{00EA}
\pdfglyphtounicode{ecircumflexacute}{1EBF}
\pdfglyphtounicode{ecircumflexbelow}{1E19}
\pdfglyphtounicode{ecircumflexdotbelow}{1EC7}
\pdfglyphtounicode{ecircumflexgrave}{1EC1}
\pdfglyphtounicode{ecircumflexhookabove}{1EC3}
\pdfglyphtounicode{ecircumflextilde}{1EC5}
\pdfglyphtounicode{ecyrillic}{0454}
\pdfglyphtounicode{edblgrave}{0205}
\pdfglyphtounicode{edeva}{090F}
\pdfglyphtounicode{edieresis}{00EB}
\pdfglyphtounicode{edot}{0117}
\pdfglyphtounicode{edotaccent}{0117}
\pdfglyphtounicode{edotbelow}{1EB9}
\pdfglyphtounicode{eegurmukhi}{0A0F}
\pdfglyphtounicode{eematragurmukhi}{0A47}
\pdfglyphtounicode{efcyrillic}{0444}
\pdfglyphtounicode{egrave}{00E8}
\pdfglyphtounicode{egujarati}{0A8F}
\pdfglyphtounicode{eharmenian}{0567}
\pdfglyphtounicode{ehbopomofo}{311D}
\pdfglyphtounicode{ehiragana}{3048}
\pdfglyphtounicode{ehookabove}{1EBB}
\pdfglyphtounicode{eibopomofo}{311F}
\pdfglyphtounicode{eight}{0038}
\pdfglyphtounicode{eightarabic}{0668}
\pdfglyphtounicode{eightbengali}{09EE}
\pdfglyphtounicode{eightcircle}{2467}
\pdfglyphtounicode{eightcircleinversesansserif}{2791}
\pdfglyphtounicode{eightdeva}{096E}
\pdfglyphtounicode{eighteencircle}{2471}
\pdfglyphtounicode{eighteenparen}{2485}
\pdfglyphtounicode{eighteenperiod}{2499}
\pdfglyphtounicode{eightgujarati}{0AEE}
\pdfglyphtounicode{eightgurmukhi}{0A6E}
\pdfglyphtounicode{eighthackarabic}{0668}
\pdfglyphtounicode{eighthangzhou}{3028}
\pdfglyphtounicode{eighthnotebeamed}{266B}
\pdfglyphtounicode{eightideographicparen}{3227}
\pdfglyphtounicode{eightinferior}{2088}
\pdfglyphtounicode{eightmonospace}{FF18}
\pdfglyphtounicode{eightoldstyle}{F738}
\pdfglyphtounicode{eightparen}{247B}
\pdfglyphtounicode{eightperiod}{248F}
\pdfglyphtounicode{eightpersian}{06F8}
\pdfglyphtounicode{eightroman}{2177}
\pdfglyphtounicode{eightsuperior}{2078}
\pdfglyphtounicode{eightthai}{0E58}
\pdfglyphtounicode{einvertedbreve}{0207}
\pdfglyphtounicode{eiotifiedcyrillic}{0465}
\pdfglyphtounicode{ekatakana}{30A8}
\pdfglyphtounicode{ekatakanahalfwidth}{FF74}
\pdfglyphtounicode{ekonkargurmukhi}{0A74}
\pdfglyphtounicode{ekorean}{3154}
\pdfglyphtounicode{elcyrillic}{043B}
\pdfglyphtounicode{element}{2208}
\pdfglyphtounicode{elevencircle}{246A}
\pdfglyphtounicode{elevenparen}{247E}
\pdfglyphtounicode{elevenperiod}{2492}
\pdfglyphtounicode{elevenroman}{217A}
\pdfglyphtounicode{ellipsis}{2026}
\pdfglyphtounicode{ellipsisvertical}{22EE}
\pdfglyphtounicode{emacron}{0113}
\pdfglyphtounicode{emacronacute}{1E17}
\pdfglyphtounicode{emacrongrave}{1E15}
\pdfglyphtounicode{emcyrillic}{043C}
\pdfglyphtounicode{emdash}{2014}
\pdfglyphtounicode{emdashvertical}{FE31}
\pdfglyphtounicode{emonospace}{FF45}
\pdfglyphtounicode{emphasismarkarmenian}{055B}
\pdfglyphtounicode{emptyset}{2205}
\pdfglyphtounicode{enbopomofo}{3123}
\pdfglyphtounicode{encyrillic}{043D}
\pdfglyphtounicode{endash}{2013}
\pdfglyphtounicode{endashvertical}{FE32}
\pdfglyphtounicode{endescendercyrillic}{04A3}
\pdfglyphtounicode{eng}{014B}
\pdfglyphtounicode{engbopomofo}{3125}
\pdfglyphtounicode{enghecyrillic}{04A5}
\pdfglyphtounicode{enhookcyrillic}{04C8}
\pdfglyphtounicode{enspace}{2002}
\pdfglyphtounicode{eogonek}{0119}
\pdfglyphtounicode{eokorean}{3153}
\pdfglyphtounicode{eopen}{025B}
\pdfglyphtounicode{eopenclosed}{029A}
\pdfglyphtounicode{eopenreversed}{025C}
\pdfglyphtounicode{eopenreversedclosed}{025E}
\pdfglyphtounicode{eopenreversedhook}{025D}
\pdfglyphtounicode{eparen}{24A0}
\pdfglyphtounicode{epsilon}{03B5}
\pdfglyphtounicode{epsilontonos}{03AD}
\pdfglyphtounicode{equal}{003D}
\pdfglyphtounicode{equalmonospace}{FF1D}
\pdfglyphtounicode{equalsmall}{FE66}
\pdfglyphtounicode{equalsuperior}{207C}
\pdfglyphtounicode{equivalence}{2261}
\pdfglyphtounicode{erbopomofo}{3126}
\pdfglyphtounicode{ercyrillic}{0440}
\pdfglyphtounicode{ereversed}{0258}
\pdfglyphtounicode{ereversedcyrillic}{044D}
\pdfglyphtounicode{escyrillic}{0441}
\pdfglyphtounicode{esdescendercyrillic}{04AB}
\pdfglyphtounicode{esh}{0283}
\pdfglyphtounicode{eshcurl}{0286}
\pdfglyphtounicode{eshortdeva}{090E}
\pdfglyphtounicode{eshortvowelsigndeva}{0946}
\pdfglyphtounicode{eshreversedloop}{01AA}
\pdfglyphtounicode{eshsquatreversed}{0285}
\pdfglyphtounicode{esmallhiragana}{3047}
\pdfglyphtounicode{esmallkatakana}{30A7}
\pdfglyphtounicode{esmallkatakanahalfwidth}{FF6A}
\pdfglyphtounicode{estimated}{212E}
\pdfglyphtounicode{esuperior}{F6EC}
\pdfglyphtounicode{eta}{03B7}
\pdfglyphtounicode{etarmenian}{0568}
\pdfglyphtounicode{etatonos}{03AE}
\pdfglyphtounicode{eth}{00F0}
\pdfglyphtounicode{etilde}{1EBD}
\pdfglyphtounicode{etildebelow}{1E1B}
\pdfglyphtounicode{etnahtafoukhhebrew}{0591}
\pdfglyphtounicode{etnahtafoukhlefthebrew}{0591}
\pdfglyphtounicode{etnahtahebrew}{0591}
\pdfglyphtounicode{etnahtalefthebrew}{0591}
\pdfglyphtounicode{eturned}{01DD}
\pdfglyphtounicode{eukorean}{3161}
\pdfglyphtounicode{euro}{20AC}
\pdfglyphtounicode{evowelsignbengali}{09C7}
\pdfglyphtounicode{evowelsigndeva}{0947}
\pdfglyphtounicode{evowelsigngujarati}{0AC7}
\pdfglyphtounicode{exclam}{0021}
\pdfglyphtounicode{exclamarmenian}{055C}
\pdfglyphtounicode{exclamdbl}{203C}
\pdfglyphtounicode{exclamdown}{00A1}
\pdfglyphtounicode{exclamdownsmall}{F7A1}
\pdfglyphtounicode{exclammonospace}{FF01}
\pdfglyphtounicode{exclamsmall}{F721}
\pdfglyphtounicode{existential}{2203}
\pdfglyphtounicode{ezh}{0292}
\pdfglyphtounicode{ezhcaron}{01EF}
\pdfglyphtounicode{ezhcurl}{0293}
\pdfglyphtounicode{ezhreversed}{01B9}
\pdfglyphtounicode{ezhtail}{01BA}
\pdfglyphtounicode{f}{0066}
\pdfglyphtounicode{fadeva}{095E}
\pdfglyphtounicode{fagurmukhi}{0A5E}
\pdfglyphtounicode{fahrenheit}{2109}
\pdfglyphtounicode{fathaarabic}{064E}
\pdfglyphtounicode{fathalowarabic}{064E}
\pdfglyphtounicode{fathatanarabic}{064B}
\pdfglyphtounicode{fbopomofo}{3108}
\pdfglyphtounicode{fcircle}{24D5}
\pdfglyphtounicode{fdotaccent}{1E1F}
\pdfglyphtounicode{feharabic}{0641}
\pdfglyphtounicode{feharmenian}{0586}
\pdfglyphtounicode{fehfinalarabic}{FED2}
\pdfglyphtounicode{fehinitialarabic}{FED3}
\pdfglyphtounicode{fehmedialarabic}{FED4}
\pdfglyphtounicode{feicoptic}{03E5}
\pdfglyphtounicode{female}{2640}
\pdfglyphtounicode{ff}{FB00}
\pdfglyphtounicode{ffi}{FB03}
\pdfglyphtounicode{ffl}{FB04}
\pdfglyphtounicode{fi}{FB01}
\pdfglyphtounicode{fifteencircle}{246E}
\pdfglyphtounicode{fifteenparen}{2482}
\pdfglyphtounicode{fifteenperiod}{2496}
\pdfglyphtounicode{figuredash}{2012}
\pdfglyphtounicode{filledbox}{25A0}
\pdfglyphtounicode{filledrect}{25AC}
\pdfglyphtounicode{finalkaf}{05DA}
\pdfglyphtounicode{finalkafdagesh}{FB3A}
\pdfglyphtounicode{finalkafdageshhebrew}{FB3A}
\pdfglyphtounicode{finalkafhebrew}{05DA}
% finalkafqamats;05DA 05B8
% finalkafqamatshebrew;05DA 05B8
% finalkafsheva;05DA 05B0
% finalkafshevahebrew;05DA 05B0
\pdfglyphtounicode{finalmem}{05DD}
\pdfglyphtounicode{finalmemhebrew}{05DD}
\pdfglyphtounicode{finalnun}{05DF}
\pdfglyphtounicode{finalnunhebrew}{05DF}
\pdfglyphtounicode{finalpe}{05E3}
\pdfglyphtounicode{finalpehebrew}{05E3}
\pdfglyphtounicode{finaltsadi}{05E5}
\pdfglyphtounicode{finaltsadihebrew}{05E5}
\pdfglyphtounicode{firsttonechinese}{02C9}
\pdfglyphtounicode{fisheye}{25C9}
\pdfglyphtounicode{fitacyrillic}{0473}
\pdfglyphtounicode{five}{0035}
\pdfglyphtounicode{fivearabic}{0665}
\pdfglyphtounicode{fivebengali}{09EB}
\pdfglyphtounicode{fivecircle}{2464}
\pdfglyphtounicode{fivecircleinversesansserif}{278E}
\pdfglyphtounicode{fivedeva}{096B}
\pdfglyphtounicode{fiveeighths}{215D}
\pdfglyphtounicode{fivegujarati}{0AEB}
\pdfglyphtounicode{fivegurmukhi}{0A6B}
\pdfglyphtounicode{fivehackarabic}{0665}
\pdfglyphtounicode{fivehangzhou}{3025}
\pdfglyphtounicode{fiveideographicparen}{3224}
\pdfglyphtounicode{fiveinferior}{2085}
\pdfglyphtounicode{fivemonospace}{FF15}
\pdfglyphtounicode{fiveoldstyle}{F735}
\pdfglyphtounicode{fiveparen}{2478}
\pdfglyphtounicode{fiveperiod}{248C}
\pdfglyphtounicode{fivepersian}{06F5}
\pdfglyphtounicode{fiveroman}{2174}
\pdfglyphtounicode{fivesuperior}{2075}
\pdfglyphtounicode{fivethai}{0E55}
\pdfglyphtounicode{fl}{FB02}
\pdfglyphtounicode{florin}{0192}
\pdfglyphtounicode{fmonospace}{FF46}
\pdfglyphtounicode{fmsquare}{3399}
\pdfglyphtounicode{fofanthai}{0E1F}
\pdfglyphtounicode{fofathai}{0E1D}
\pdfglyphtounicode{fongmanthai}{0E4F}
\pdfglyphtounicode{forall}{2200}
\pdfglyphtounicode{four}{0034}
\pdfglyphtounicode{fourarabic}{0664}
\pdfglyphtounicode{fourbengali}{09EA}
\pdfglyphtounicode{fourcircle}{2463}
\pdfglyphtounicode{fourcircleinversesansserif}{278D}
\pdfglyphtounicode{fourdeva}{096A}
\pdfglyphtounicode{fourgujarati}{0AEA}
\pdfglyphtounicode{fourgurmukhi}{0A6A}
\pdfglyphtounicode{fourhackarabic}{0664}
\pdfglyphtounicode{fourhangzhou}{3024}
\pdfglyphtounicode{fourideographicparen}{3223}
\pdfglyphtounicode{fourinferior}{2084}
\pdfglyphtounicode{fourmonospace}{FF14}
\pdfglyphtounicode{fournumeratorbengali}{09F7}
\pdfglyphtounicode{fouroldstyle}{F734}
\pdfglyphtounicode{fourparen}{2477}
\pdfglyphtounicode{fourperiod}{248B}
\pdfglyphtounicode{fourpersian}{06F4}
\pdfglyphtounicode{fourroman}{2173}
\pdfglyphtounicode{foursuperior}{2074}
\pdfglyphtounicode{fourteencircle}{246D}
\pdfglyphtounicode{fourteenparen}{2481}
\pdfglyphtounicode{fourteenperiod}{2495}
\pdfglyphtounicode{fourthai}{0E54}
\pdfglyphtounicode{fourthtonechinese}{02CB}
\pdfglyphtounicode{fparen}{24A1}
\pdfglyphtounicode{fraction}{2044}
\pdfglyphtounicode{franc}{20A3}
\pdfglyphtounicode{g}{0067}
\pdfglyphtounicode{gabengali}{0997}
\pdfglyphtounicode{gacute}{01F5}
\pdfglyphtounicode{gadeva}{0917}
\pdfglyphtounicode{gafarabic}{06AF}
\pdfglyphtounicode{gaffinalarabic}{FB93}
\pdfglyphtounicode{gafinitialarabic}{FB94}
\pdfglyphtounicode{gafmedialarabic}{FB95}
\pdfglyphtounicode{gagujarati}{0A97}
\pdfglyphtounicode{gagurmukhi}{0A17}
\pdfglyphtounicode{gahiragana}{304C}
\pdfglyphtounicode{gakatakana}{30AC}
\pdfglyphtounicode{gamma}{03B3}
\pdfglyphtounicode{gammalatinsmall}{0263}
\pdfglyphtounicode{gammasuperior}{02E0}
\pdfglyphtounicode{gangiacoptic}{03EB}
\pdfglyphtounicode{gbopomofo}{310D}
\pdfglyphtounicode{gbreve}{011F}
\pdfglyphtounicode{gcaron}{01E7}
\pdfglyphtounicode{gcedilla}{0123}
\pdfglyphtounicode{gcircle}{24D6}
\pdfglyphtounicode{gcircumflex}{011D}
\pdfglyphtounicode{gcommaaccent}{0123}
\pdfglyphtounicode{gdot}{0121}
\pdfglyphtounicode{gdotaccent}{0121}
\pdfglyphtounicode{gecyrillic}{0433}
\pdfglyphtounicode{gehiragana}{3052}
\pdfglyphtounicode{gekatakana}{30B2}
\pdfglyphtounicode{geometricallyequal}{2251}
\pdfglyphtounicode{gereshaccenthebrew}{059C}
\pdfglyphtounicode{gereshhebrew}{05F3}
\pdfglyphtounicode{gereshmuqdamhebrew}{059D}
\pdfglyphtounicode{germandbls}{00DF}
\pdfglyphtounicode{gershayimaccenthebrew}{059E}
\pdfglyphtounicode{gershayimhebrew}{05F4}
\pdfglyphtounicode{getamark}{3013}
\pdfglyphtounicode{ghabengali}{0998}
\pdfglyphtounicode{ghadarmenian}{0572}
\pdfglyphtounicode{ghadeva}{0918}
\pdfglyphtounicode{ghagujarati}{0A98}
\pdfglyphtounicode{ghagurmukhi}{0A18}
\pdfglyphtounicode{ghainarabic}{063A}
\pdfglyphtounicode{ghainfinalarabic}{FECE}
\pdfglyphtounicode{ghaininitialarabic}{FECF}
\pdfglyphtounicode{ghainmedialarabic}{FED0}
\pdfglyphtounicode{ghemiddlehookcyrillic}{0495}
\pdfglyphtounicode{ghestrokecyrillic}{0493}
\pdfglyphtounicode{gheupturncyrillic}{0491}
\pdfglyphtounicode{ghhadeva}{095A}
\pdfglyphtounicode{ghhagurmukhi}{0A5A}
\pdfglyphtounicode{ghook}{0260}
\pdfglyphtounicode{ghzsquare}{3393}
\pdfglyphtounicode{gihiragana}{304E}
\pdfglyphtounicode{gikatakana}{30AE}
\pdfglyphtounicode{gimarmenian}{0563}
\pdfglyphtounicode{gimel}{05D2}
\pdfglyphtounicode{gimeldagesh}{FB32}
\pdfglyphtounicode{gimeldageshhebrew}{FB32}
\pdfglyphtounicode{gimelhebrew}{05D2}
\pdfglyphtounicode{gjecyrillic}{0453}
\pdfglyphtounicode{glottalinvertedstroke}{01BE}
\pdfglyphtounicode{glottalstop}{0294}
\pdfglyphtounicode{glottalstopinverted}{0296}
\pdfglyphtounicode{glottalstopmod}{02C0}
\pdfglyphtounicode{glottalstopreversed}{0295}
\pdfglyphtounicode{glottalstopreversedmod}{02C1}
\pdfglyphtounicode{glottalstopreversedsuperior}{02E4}
\pdfglyphtounicode{glottalstopstroke}{02A1}
\pdfglyphtounicode{glottalstopstrokereversed}{02A2}
\pdfglyphtounicode{gmacron}{1E21}
\pdfglyphtounicode{gmonospace}{FF47}
\pdfglyphtounicode{gohiragana}{3054}
\pdfglyphtounicode{gokatakana}{30B4}
\pdfglyphtounicode{gparen}{24A2}
\pdfglyphtounicode{gpasquare}{33AC}
\pdfglyphtounicode{gradient}{2207}
\pdfglyphtounicode{grave}{0060}
\pdfglyphtounicode{gravebelowcmb}{0316}
\pdfglyphtounicode{gravecmb}{0300}
\pdfglyphtounicode{gravecomb}{0300}
\pdfglyphtounicode{gravedeva}{0953}
\pdfglyphtounicode{gravelowmod}{02CE}
\pdfglyphtounicode{gravemonospace}{FF40}
\pdfglyphtounicode{gravetonecmb}{0340}
\pdfglyphtounicode{greater}{003E}
\pdfglyphtounicode{greaterequal}{2265}
\pdfglyphtounicode{greaterequalorless}{22DB}
\pdfglyphtounicode{greatermonospace}{FF1E}
\pdfglyphtounicode{greaterorequivalent}{2273}
\pdfglyphtounicode{greaterorless}{2277}
\pdfglyphtounicode{greateroverequal}{2267}
\pdfglyphtounicode{greatersmall}{FE65}
\pdfglyphtounicode{gscript}{0261}
\pdfglyphtounicode{gstroke}{01E5}
\pdfglyphtounicode{guhiragana}{3050}
\pdfglyphtounicode{guillemotleft}{00AB}
\pdfglyphtounicode{guillemotright}{00BB}
\pdfglyphtounicode{guilsinglleft}{2039}
\pdfglyphtounicode{guilsinglright}{203A}
\pdfglyphtounicode{gukatakana}{30B0}
\pdfglyphtounicode{guramusquare}{3318}
\pdfglyphtounicode{gysquare}{33C9}
\pdfglyphtounicode{h}{0068}
\pdfglyphtounicode{haabkhasiancyrillic}{04A9}
\pdfglyphtounicode{haaltonearabic}{06C1}
\pdfglyphtounicode{habengali}{09B9}
\pdfglyphtounicode{hadescendercyrillic}{04B3}
\pdfglyphtounicode{hadeva}{0939}
\pdfglyphtounicode{hagujarati}{0AB9}
\pdfglyphtounicode{hagurmukhi}{0A39}
\pdfglyphtounicode{haharabic}{062D}
\pdfglyphtounicode{hahfinalarabic}{FEA2}
\pdfglyphtounicode{hahinitialarabic}{FEA3}
\pdfglyphtounicode{hahiragana}{306F}
\pdfglyphtounicode{hahmedialarabic}{FEA4}
\pdfglyphtounicode{haitusquare}{332A}
\pdfglyphtounicode{hakatakana}{30CF}
\pdfglyphtounicode{hakatakanahalfwidth}{FF8A}
\pdfglyphtounicode{halantgurmukhi}{0A4D}
\pdfglyphtounicode{hamzaarabic}{0621}
% hamzadammaarabic;0621 064F
% hamzadammatanarabic;0621 064C
% hamzafathaarabic;0621 064E
% hamzafathatanarabic;0621 064B
\pdfglyphtounicode{hamzalowarabic}{0621}
% hamzalowkasraarabic;0621 0650
% hamzalowkasratanarabic;0621 064D
% hamzasukunarabic;0621 0652
\pdfglyphtounicode{hangulfiller}{3164}
\pdfglyphtounicode{hardsigncyrillic}{044A}
\pdfglyphtounicode{harpoonleftbarbup}{21BC}
\pdfglyphtounicode{harpoonrightbarbup}{21C0}
\pdfglyphtounicode{hasquare}{33CA}
\pdfglyphtounicode{hatafpatah}{05B2}
\pdfglyphtounicode{hatafpatah16}{05B2}
\pdfglyphtounicode{hatafpatah23}{05B2}
\pdfglyphtounicode{hatafpatah2f}{05B2}
\pdfglyphtounicode{hatafpatahhebrew}{05B2}
\pdfglyphtounicode{hatafpatahnarrowhebrew}{05B2}
\pdfglyphtounicode{hatafpatahquarterhebrew}{05B2}
\pdfglyphtounicode{hatafpatahwidehebrew}{05B2}
\pdfglyphtounicode{hatafqamats}{05B3}
\pdfglyphtounicode{hatafqamats1b}{05B3}
\pdfglyphtounicode{hatafqamats28}{05B3}
\pdfglyphtounicode{hatafqamats34}{05B3}
\pdfglyphtounicode{hatafqamatshebrew}{05B3}
\pdfglyphtounicode{hatafqamatsnarrowhebrew}{05B3}
\pdfglyphtounicode{hatafqamatsquarterhebrew}{05B3}
\pdfglyphtounicode{hatafqamatswidehebrew}{05B3}
\pdfglyphtounicode{hatafsegol}{05B1}
\pdfglyphtounicode{hatafsegol17}{05B1}
\pdfglyphtounicode{hatafsegol24}{05B1}
\pdfglyphtounicode{hatafsegol30}{05B1}
\pdfglyphtounicode{hatafsegolhebrew}{05B1}
\pdfglyphtounicode{hatafsegolnarrowhebrew}{05B1}
\pdfglyphtounicode{hatafsegolquarterhebrew}{05B1}
\pdfglyphtounicode{hatafsegolwidehebrew}{05B1}
\pdfglyphtounicode{hbar}{0127}
\pdfglyphtounicode{hbopomofo}{310F}
\pdfglyphtounicode{hbrevebelow}{1E2B}
\pdfglyphtounicode{hcedilla}{1E29}
\pdfglyphtounicode{hcircle}{24D7}
\pdfglyphtounicode{hcircumflex}{0125}
\pdfglyphtounicode{hdieresis}{1E27}
\pdfglyphtounicode{hdotaccent}{1E23}
\pdfglyphtounicode{hdotbelow}{1E25}
\pdfglyphtounicode{he}{05D4}
\pdfglyphtounicode{heart}{2665}
\pdfglyphtounicode{heartsuitblack}{2665}
\pdfglyphtounicode{heartsuitwhite}{2661}
\pdfglyphtounicode{hedagesh}{FB34}
\pdfglyphtounicode{hedageshhebrew}{FB34}
\pdfglyphtounicode{hehaltonearabic}{06C1}
\pdfglyphtounicode{heharabic}{0647}
\pdfglyphtounicode{hehebrew}{05D4}
\pdfglyphtounicode{hehfinalaltonearabic}{FBA7}
\pdfglyphtounicode{hehfinalalttwoarabic}{FEEA}
\pdfglyphtounicode{hehfinalarabic}{FEEA}
\pdfglyphtounicode{hehhamzaabovefinalarabic}{FBA5}
\pdfglyphtounicode{hehhamzaaboveisolatedarabic}{FBA4}
\pdfglyphtounicode{hehinitialaltonearabic}{FBA8}
\pdfglyphtounicode{hehinitialarabic}{FEEB}
\pdfglyphtounicode{hehiragana}{3078}
\pdfglyphtounicode{hehmedialaltonearabic}{FBA9}
\pdfglyphtounicode{hehmedialarabic}{FEEC}
\pdfglyphtounicode{heiseierasquare}{337B}
\pdfglyphtounicode{hekatakana}{30D8}
\pdfglyphtounicode{hekatakanahalfwidth}{FF8D}
\pdfglyphtounicode{hekutaarusquare}{3336}
\pdfglyphtounicode{henghook}{0267}
\pdfglyphtounicode{herutusquare}{3339}
\pdfglyphtounicode{het}{05D7}
\pdfglyphtounicode{hethebrew}{05D7}
\pdfglyphtounicode{hhook}{0266}
\pdfglyphtounicode{hhooksuperior}{02B1}
\pdfglyphtounicode{hieuhacirclekorean}{327B}
\pdfglyphtounicode{hieuhaparenkorean}{321B}
\pdfglyphtounicode{hieuhcirclekorean}{326D}
\pdfglyphtounicode{hieuhkorean}{314E}
\pdfglyphtounicode{hieuhparenkorean}{320D}
\pdfglyphtounicode{hihiragana}{3072}
\pdfglyphtounicode{hikatakana}{30D2}
\pdfglyphtounicode{hikatakanahalfwidth}{FF8B}
\pdfglyphtounicode{hiriq}{05B4}
\pdfglyphtounicode{hiriq14}{05B4}
\pdfglyphtounicode{hiriq21}{05B4}
\pdfglyphtounicode{hiriq2d}{05B4}
\pdfglyphtounicode{hiriqhebrew}{05B4}
\pdfglyphtounicode{hiriqnarrowhebrew}{05B4}
\pdfglyphtounicode{hiriqquarterhebrew}{05B4}
\pdfglyphtounicode{hiriqwidehebrew}{05B4}
\pdfglyphtounicode{hlinebelow}{1E96}
\pdfglyphtounicode{hmonospace}{FF48}
\pdfglyphtounicode{hoarmenian}{0570}
\pdfglyphtounicode{hohipthai}{0E2B}
\pdfglyphtounicode{hohiragana}{307B}
\pdfglyphtounicode{hokatakana}{30DB}
\pdfglyphtounicode{hokatakanahalfwidth}{FF8E}
\pdfglyphtounicode{holam}{05B9}
\pdfglyphtounicode{holam19}{05B9}
\pdfglyphtounicode{holam26}{05B9}
\pdfglyphtounicode{holam32}{05B9}
\pdfglyphtounicode{holamhebrew}{05B9}
\pdfglyphtounicode{holamnarrowhebrew}{05B9}
\pdfglyphtounicode{holamquarterhebrew}{05B9}
\pdfglyphtounicode{holamwidehebrew}{05B9}
\pdfglyphtounicode{honokhukthai}{0E2E}
\pdfglyphtounicode{hookabovecomb}{0309}
\pdfglyphtounicode{hookcmb}{0309}
\pdfglyphtounicode{hookpalatalizedbelowcmb}{0321}
\pdfglyphtounicode{hookretroflexbelowcmb}{0322}
\pdfglyphtounicode{hoonsquare}{3342}
\pdfglyphtounicode{horicoptic}{03E9}
\pdfglyphtounicode{horizontalbar}{2015}
\pdfglyphtounicode{horncmb}{031B}
\pdfglyphtounicode{hotsprings}{2668}
\pdfglyphtounicode{house}{2302}
\pdfglyphtounicode{hparen}{24A3}
\pdfglyphtounicode{hsuperior}{02B0}
\pdfglyphtounicode{hturned}{0265}
\pdfglyphtounicode{huhiragana}{3075}
\pdfglyphtounicode{huiitosquare}{3333}
\pdfglyphtounicode{hukatakana}{30D5}
\pdfglyphtounicode{hukatakanahalfwidth}{FF8C}
\pdfglyphtounicode{hungarumlaut}{02DD}
\pdfglyphtounicode{hungarumlautcmb}{030B}
\pdfglyphtounicode{hv}{0195}
\pdfglyphtounicode{hyphen}{002D}
\pdfglyphtounicode{hypheninferior}{F6E5}
\pdfglyphtounicode{hyphenmonospace}{FF0D}
\pdfglyphtounicode{hyphensmall}{FE63}
\pdfglyphtounicode{hyphensuperior}{F6E6}
\pdfglyphtounicode{hyphentwo}{2010}
\pdfglyphtounicode{i}{0069}
\pdfglyphtounicode{iacute}{00ED}
\pdfglyphtounicode{iacyrillic}{044F}
\pdfglyphtounicode{ibengali}{0987}
\pdfglyphtounicode{ibopomofo}{3127}
\pdfglyphtounicode{ibreve}{012D}
\pdfglyphtounicode{icaron}{01D0}
\pdfglyphtounicode{icircle}{24D8}
\pdfglyphtounicode{icircumflex}{00EE}
\pdfglyphtounicode{icyrillic}{0456}
\pdfglyphtounicode{idblgrave}{0209}
\pdfglyphtounicode{ideographearthcircle}{328F}
\pdfglyphtounicode{ideographfirecircle}{328B}
\pdfglyphtounicode{ideographicallianceparen}{323F}
\pdfglyphtounicode{ideographiccallparen}{323A}
\pdfglyphtounicode{ideographiccentrecircle}{32A5}
\pdfglyphtounicode{ideographicclose}{3006}
\pdfglyphtounicode{ideographiccomma}{3001}
\pdfglyphtounicode{ideographiccommaleft}{FF64}
\pdfglyphtounicode{ideographiccongratulationparen}{3237}
\pdfglyphtounicode{ideographiccorrectcircle}{32A3}
\pdfglyphtounicode{ideographicearthparen}{322F}
\pdfglyphtounicode{ideographicenterpriseparen}{323D}
\pdfglyphtounicode{ideographicexcellentcircle}{329D}
\pdfglyphtounicode{ideographicfestivalparen}{3240}
\pdfglyphtounicode{ideographicfinancialcircle}{3296}
\pdfglyphtounicode{ideographicfinancialparen}{3236}
\pdfglyphtounicode{ideographicfireparen}{322B}
\pdfglyphtounicode{ideographichaveparen}{3232}
\pdfglyphtounicode{ideographichighcircle}{32A4}
\pdfglyphtounicode{ideographiciterationmark}{3005}
\pdfglyphtounicode{ideographiclaborcircle}{3298}
\pdfglyphtounicode{ideographiclaborparen}{3238}
\pdfglyphtounicode{ideographicleftcircle}{32A7}
\pdfglyphtounicode{ideographiclowcircle}{32A6}
\pdfglyphtounicode{ideographicmedicinecircle}{32A9}
\pdfglyphtounicode{ideographicmetalparen}{322E}
\pdfglyphtounicode{ideographicmoonparen}{322A}
\pdfglyphtounicode{ideographicnameparen}{3234}
\pdfglyphtounicode{ideographicperiod}{3002}
\pdfglyphtounicode{ideographicprintcircle}{329E}
\pdfglyphtounicode{ideographicreachparen}{3243}
\pdfglyphtounicode{ideographicrepresentparen}{3239}
\pdfglyphtounicode{ideographicresourceparen}{323E}
\pdfglyphtounicode{ideographicrightcircle}{32A8}
\pdfglyphtounicode{ideographicsecretcircle}{3299}
\pdfglyphtounicode{ideographicselfparen}{3242}
\pdfglyphtounicode{ideographicsocietyparen}{3233}
\pdfglyphtounicode{ideographicspace}{3000}
\pdfglyphtounicode{ideographicspecialparen}{3235}
\pdfglyphtounicode{ideographicstockparen}{3231}
\pdfglyphtounicode{ideographicstudyparen}{323B}
\pdfglyphtounicode{ideographicsunparen}{3230}
\pdfglyphtounicode{ideographicsuperviseparen}{323C}
\pdfglyphtounicode{ideographicwaterparen}{322C}
\pdfglyphtounicode{ideographicwoodparen}{322D}
\pdfglyphtounicode{ideographiczero}{3007}
\pdfglyphtounicode{ideographmetalcircle}{328E}
\pdfglyphtounicode{ideographmooncircle}{328A}
\pdfglyphtounicode{ideographnamecircle}{3294}
\pdfglyphtounicode{ideographsuncircle}{3290}
\pdfglyphtounicode{ideographwatercircle}{328C}
\pdfglyphtounicode{ideographwoodcircle}{328D}
\pdfglyphtounicode{ideva}{0907}
\pdfglyphtounicode{idieresis}{00EF}
\pdfglyphtounicode{idieresisacute}{1E2F}
\pdfglyphtounicode{idieresiscyrillic}{04E5}
\pdfglyphtounicode{idotbelow}{1ECB}
\pdfglyphtounicode{iebrevecyrillic}{04D7}
\pdfglyphtounicode{iecyrillic}{0435}
\pdfglyphtounicode{ieungacirclekorean}{3275}
\pdfglyphtounicode{ieungaparenkorean}{3215}
\pdfglyphtounicode{ieungcirclekorean}{3267}
\pdfglyphtounicode{ieungkorean}{3147}
\pdfglyphtounicode{ieungparenkorean}{3207}
\pdfglyphtounicode{igrave}{00EC}
\pdfglyphtounicode{igujarati}{0A87}
\pdfglyphtounicode{igurmukhi}{0A07}
\pdfglyphtounicode{ihiragana}{3044}
\pdfglyphtounicode{ihookabove}{1EC9}
\pdfglyphtounicode{iibengali}{0988}
\pdfglyphtounicode{iicyrillic}{0438}
\pdfglyphtounicode{iideva}{0908}
\pdfglyphtounicode{iigujarati}{0A88}
\pdfglyphtounicode{iigurmukhi}{0A08}
\pdfglyphtounicode{iimatragurmukhi}{0A40}
\pdfglyphtounicode{iinvertedbreve}{020B}
\pdfglyphtounicode{iishortcyrillic}{0439}
\pdfglyphtounicode{iivowelsignbengali}{09C0}
\pdfglyphtounicode{iivowelsigndeva}{0940}
\pdfglyphtounicode{iivowelsigngujarati}{0AC0}
\pdfglyphtounicode{ij}{0133}
\pdfglyphtounicode{ikatakana}{30A4}
\pdfglyphtounicode{ikatakanahalfwidth}{FF72}
\pdfglyphtounicode{ikorean}{3163}
\pdfglyphtounicode{ilde}{02DC}
\pdfglyphtounicode{iluyhebrew}{05AC}
\pdfglyphtounicode{imacron}{012B}
\pdfglyphtounicode{imacroncyrillic}{04E3}
\pdfglyphtounicode{imageorapproximatelyequal}{2253}
\pdfglyphtounicode{imatragurmukhi}{0A3F}
\pdfglyphtounicode{imonospace}{FF49}
\pdfglyphtounicode{increment}{2206}
\pdfglyphtounicode{infinity}{221E}
\pdfglyphtounicode{iniarmenian}{056B}
\pdfglyphtounicode{integral}{222B}
\pdfglyphtounicode{integralbottom}{2321}
\pdfglyphtounicode{integralbt}{2321}
\pdfglyphtounicode{integralex}{F8F5}
\pdfglyphtounicode{integraltop}{2320}
\pdfglyphtounicode{integraltp}{2320}
\pdfglyphtounicode{intersection}{2229}
\pdfglyphtounicode{intisquare}{3305}
\pdfglyphtounicode{invbullet}{25D8}
\pdfglyphtounicode{invcircle}{25D9}
\pdfglyphtounicode{invsmileface}{263B}
\pdfglyphtounicode{iocyrillic}{0451}
\pdfglyphtounicode{iogonek}{012F}
\pdfglyphtounicode{iota}{03B9}
\pdfglyphtounicode{iotadieresis}{03CA}
\pdfglyphtounicode{iotadieresistonos}{0390}
\pdfglyphtounicode{iotalatin}{0269}
\pdfglyphtounicode{iotatonos}{03AF}
\pdfglyphtounicode{iparen}{24A4}
\pdfglyphtounicode{irigurmukhi}{0A72}
\pdfglyphtounicode{ismallhiragana}{3043}
\pdfglyphtounicode{ismallkatakana}{30A3}
\pdfglyphtounicode{ismallkatakanahalfwidth}{FF68}
\pdfglyphtounicode{issharbengali}{09FA}
\pdfglyphtounicode{istroke}{0268}
\pdfglyphtounicode{isuperior}{F6ED}
\pdfglyphtounicode{iterationhiragana}{309D}
\pdfglyphtounicode{iterationkatakana}{30FD}
\pdfglyphtounicode{itilde}{0129}
\pdfglyphtounicode{itildebelow}{1E2D}
\pdfglyphtounicode{iubopomofo}{3129}
\pdfglyphtounicode{iucyrillic}{044E}
\pdfglyphtounicode{ivowelsignbengali}{09BF}
\pdfglyphtounicode{ivowelsigndeva}{093F}
\pdfglyphtounicode{ivowelsigngujarati}{0ABF}
\pdfglyphtounicode{izhitsacyrillic}{0475}
\pdfglyphtounicode{izhitsadblgravecyrillic}{0477}
\pdfglyphtounicode{j}{006A}
\pdfglyphtounicode{jaarmenian}{0571}
\pdfglyphtounicode{jabengali}{099C}
\pdfglyphtounicode{jadeva}{091C}
\pdfglyphtounicode{jagujarati}{0A9C}
\pdfglyphtounicode{jagurmukhi}{0A1C}
\pdfglyphtounicode{jbopomofo}{3110}
\pdfglyphtounicode{jcaron}{01F0}
\pdfglyphtounicode{jcircle}{24D9}
\pdfglyphtounicode{jcircumflex}{0135}
\pdfglyphtounicode{jcrossedtail}{029D}
\pdfglyphtounicode{jdotlessstroke}{025F}
\pdfglyphtounicode{jecyrillic}{0458}
\pdfglyphtounicode{jeemarabic}{062C}
\pdfglyphtounicode{jeemfinalarabic}{FE9E}
\pdfglyphtounicode{jeeminitialarabic}{FE9F}
\pdfglyphtounicode{jeemmedialarabic}{FEA0}
\pdfglyphtounicode{jeharabic}{0698}
\pdfglyphtounicode{jehfinalarabic}{FB8B}
\pdfglyphtounicode{jhabengali}{099D}
\pdfglyphtounicode{jhadeva}{091D}
\pdfglyphtounicode{jhagujarati}{0A9D}
\pdfglyphtounicode{jhagurmukhi}{0A1D}
\pdfglyphtounicode{jheharmenian}{057B}
\pdfglyphtounicode{jis}{3004}
\pdfglyphtounicode{jmonospace}{FF4A}
\pdfglyphtounicode{jparen}{24A5}
\pdfglyphtounicode{jsuperior}{02B2}
\pdfglyphtounicode{k}{006B}
\pdfglyphtounicode{kabashkircyrillic}{04A1}
\pdfglyphtounicode{kabengali}{0995}
\pdfglyphtounicode{kacute}{1E31}
\pdfglyphtounicode{kacyrillic}{043A}
\pdfglyphtounicode{kadescendercyrillic}{049B}
\pdfglyphtounicode{kadeva}{0915}
\pdfglyphtounicode{kaf}{05DB}
\pdfglyphtounicode{kafarabic}{0643}
\pdfglyphtounicode{kafdagesh}{FB3B}
\pdfglyphtounicode{kafdageshhebrew}{FB3B}
\pdfglyphtounicode{kaffinalarabic}{FEDA}
\pdfglyphtounicode{kafhebrew}{05DB}
\pdfglyphtounicode{kafinitialarabic}{FEDB}
\pdfglyphtounicode{kafmedialarabic}{FEDC}
\pdfglyphtounicode{kafrafehebrew}{FB4D}
\pdfglyphtounicode{kagujarati}{0A95}
\pdfglyphtounicode{kagurmukhi}{0A15}
\pdfglyphtounicode{kahiragana}{304B}
\pdfglyphtounicode{kahookcyrillic}{04C4}
\pdfglyphtounicode{kakatakana}{30AB}
\pdfglyphtounicode{kakatakanahalfwidth}{FF76}
\pdfglyphtounicode{kappa}{03BA}
\pdfglyphtounicode{kappasymbolgreek}{03F0}
\pdfglyphtounicode{kapyeounmieumkorean}{3171}
\pdfglyphtounicode{kapyeounphieuphkorean}{3184}
\pdfglyphtounicode{kapyeounpieupkorean}{3178}
\pdfglyphtounicode{kapyeounssangpieupkorean}{3179}
\pdfglyphtounicode{karoriisquare}{330D}
\pdfglyphtounicode{kashidaautoarabic}{0640}
\pdfglyphtounicode{kashidaautonosidebearingarabic}{0640}
\pdfglyphtounicode{kasmallkatakana}{30F5}
\pdfglyphtounicode{kasquare}{3384}
\pdfglyphtounicode{kasraarabic}{0650}
\pdfglyphtounicode{kasratanarabic}{064D}
\pdfglyphtounicode{kastrokecyrillic}{049F}
\pdfglyphtounicode{katahiraprolongmarkhalfwidth}{FF70}
\pdfglyphtounicode{kaverticalstrokecyrillic}{049D}
\pdfglyphtounicode{kbopomofo}{310E}
\pdfglyphtounicode{kcalsquare}{3389}
\pdfglyphtounicode{kcaron}{01E9}
\pdfglyphtounicode{kcedilla}{0137}
\pdfglyphtounicode{kcircle}{24DA}
\pdfglyphtounicode{kcommaaccent}{0137}
\pdfglyphtounicode{kdotbelow}{1E33}
\pdfglyphtounicode{keharmenian}{0584}
\pdfglyphtounicode{kehiragana}{3051}
\pdfglyphtounicode{kekatakana}{30B1}
\pdfglyphtounicode{kekatakanahalfwidth}{FF79}
\pdfglyphtounicode{kenarmenian}{056F}
\pdfglyphtounicode{kesmallkatakana}{30F6}
\pdfglyphtounicode{kgreenlandic}{0138}
\pdfglyphtounicode{khabengali}{0996}
\pdfglyphtounicode{khacyrillic}{0445}
\pdfglyphtounicode{khadeva}{0916}
\pdfglyphtounicode{khagujarati}{0A96}
\pdfglyphtounicode{khagurmukhi}{0A16}
\pdfglyphtounicode{khaharabic}{062E}
\pdfglyphtounicode{khahfinalarabic}{FEA6}
\pdfglyphtounicode{khahinitialarabic}{FEA7}
\pdfglyphtounicode{khahmedialarabic}{FEA8}
\pdfglyphtounicode{kheicoptic}{03E7}
\pdfglyphtounicode{khhadeva}{0959}
\pdfglyphtounicode{khhagurmukhi}{0A59}
\pdfglyphtounicode{khieukhacirclekorean}{3278}
\pdfglyphtounicode{khieukhaparenkorean}{3218}
\pdfglyphtounicode{khieukhcirclekorean}{326A}
\pdfglyphtounicode{khieukhkorean}{314B}
\pdfglyphtounicode{khieukhparenkorean}{320A}
\pdfglyphtounicode{khokhaithai}{0E02}
\pdfglyphtounicode{khokhonthai}{0E05}
\pdfglyphtounicode{khokhuatthai}{0E03}
\pdfglyphtounicode{khokhwaithai}{0E04}
\pdfglyphtounicode{khomutthai}{0E5B}
\pdfglyphtounicode{khook}{0199}
\pdfglyphtounicode{khorakhangthai}{0E06}
\pdfglyphtounicode{khzsquare}{3391}
\pdfglyphtounicode{kihiragana}{304D}
\pdfglyphtounicode{kikatakana}{30AD}
\pdfglyphtounicode{kikatakanahalfwidth}{FF77}
\pdfglyphtounicode{kiroguramusquare}{3315}
\pdfglyphtounicode{kiromeetorusquare}{3316}
\pdfglyphtounicode{kirosquare}{3314}
\pdfglyphtounicode{kiyeokacirclekorean}{326E}
\pdfglyphtounicode{kiyeokaparenkorean}{320E}
\pdfglyphtounicode{kiyeokcirclekorean}{3260}
\pdfglyphtounicode{kiyeokkorean}{3131}
\pdfglyphtounicode{kiyeokparenkorean}{3200}
\pdfglyphtounicode{kiyeoksioskorean}{3133}
\pdfglyphtounicode{kjecyrillic}{045C}
\pdfglyphtounicode{klinebelow}{1E35}
\pdfglyphtounicode{klsquare}{3398}
\pdfglyphtounicode{kmcubedsquare}{33A6}
\pdfglyphtounicode{kmonospace}{FF4B}
\pdfglyphtounicode{kmsquaredsquare}{33A2}
\pdfglyphtounicode{kohiragana}{3053}
\pdfglyphtounicode{kohmsquare}{33C0}
\pdfglyphtounicode{kokaithai}{0E01}
\pdfglyphtounicode{kokatakana}{30B3}
\pdfglyphtounicode{kokatakanahalfwidth}{FF7A}
\pdfglyphtounicode{kooposquare}{331E}
\pdfglyphtounicode{koppacyrillic}{0481}
\pdfglyphtounicode{koreanstandardsymbol}{327F}
\pdfglyphtounicode{koroniscmb}{0343}
\pdfglyphtounicode{kparen}{24A6}
\pdfglyphtounicode{kpasquare}{33AA}
\pdfglyphtounicode{ksicyrillic}{046F}
\pdfglyphtounicode{ktsquare}{33CF}
\pdfglyphtounicode{kturned}{029E}
\pdfglyphtounicode{kuhiragana}{304F}
\pdfglyphtounicode{kukatakana}{30AF}
\pdfglyphtounicode{kukatakanahalfwidth}{FF78}
\pdfglyphtounicode{kvsquare}{33B8}
\pdfglyphtounicode{kwsquare}{33BE}
\pdfglyphtounicode{l}{006C}
\pdfglyphtounicode{labengali}{09B2}
\pdfglyphtounicode{lacute}{013A}
\pdfglyphtounicode{ladeva}{0932}
\pdfglyphtounicode{lagujarati}{0AB2}
\pdfglyphtounicode{lagurmukhi}{0A32}
\pdfglyphtounicode{lakkhangyaothai}{0E45}
\pdfglyphtounicode{lamaleffinalarabic}{FEFC}
\pdfglyphtounicode{lamalefhamzaabovefinalarabic}{FEF8}
\pdfglyphtounicode{lamalefhamzaaboveisolatedarabic}{FEF7}
\pdfglyphtounicode{lamalefhamzabelowfinalarabic}{FEFA}
\pdfglyphtounicode{lamalefhamzabelowisolatedarabic}{FEF9}
\pdfglyphtounicode{lamalefisolatedarabic}{FEFB}
\pdfglyphtounicode{lamalefmaddaabovefinalarabic}{FEF6}
\pdfglyphtounicode{lamalefmaddaaboveisolatedarabic}{FEF5}
\pdfglyphtounicode{lamarabic}{0644}
\pdfglyphtounicode{lambda}{03BB}
\pdfglyphtounicode{lambdastroke}{019B}
\pdfglyphtounicode{lamed}{05DC}
\pdfglyphtounicode{lameddagesh}{FB3C}
\pdfglyphtounicode{lameddageshhebrew}{FB3C}
\pdfglyphtounicode{lamedhebrew}{05DC}
% lamedholam;05DC 05B9
% lamedholamdagesh;05DC 05B9 05BC
% lamedholamdageshhebrew;05DC 05B9 05BC
% lamedholamhebrew;05DC 05B9
\pdfglyphtounicode{lamfinalarabic}{FEDE}
\pdfglyphtounicode{lamhahinitialarabic}{FCCA}
\pdfglyphtounicode{laminitialarabic}{FEDF}
\pdfglyphtounicode{lamjeeminitialarabic}{FCC9}
\pdfglyphtounicode{lamkhahinitialarabic}{FCCB}
\pdfglyphtounicode{lamlamhehisolatedarabic}{FDF2}
\pdfglyphtounicode{lammedialarabic}{FEE0}
\pdfglyphtounicode{lammeemhahinitialarabic}{FD88}
\pdfglyphtounicode{lammeeminitialarabic}{FCCC}
% lammeemjeeminitialarabic;FEDF FEE4 FEA0
% lammeemkhahinitialarabic;FEDF FEE4 FEA8
\pdfglyphtounicode{largecircle}{25EF}
\pdfglyphtounicode{lbar}{019A}
\pdfglyphtounicode{lbelt}{026C}
\pdfglyphtounicode{lbopomofo}{310C}
\pdfglyphtounicode{lcaron}{013E}
\pdfglyphtounicode{lcedilla}{013C}
\pdfglyphtounicode{lcircle}{24DB}
\pdfglyphtounicode{lcircumflexbelow}{1E3D}
\pdfglyphtounicode{lcommaaccent}{013C}
\pdfglyphtounicode{ldot}{0140}
\pdfglyphtounicode{ldotaccent}{0140}
\pdfglyphtounicode{ldotbelow}{1E37}
\pdfglyphtounicode{ldotbelowmacron}{1E39}
\pdfglyphtounicode{leftangleabovecmb}{031A}
\pdfglyphtounicode{lefttackbelowcmb}{0318}
\pdfglyphtounicode{less}{003C}
\pdfglyphtounicode{lessequal}{2264}
\pdfglyphtounicode{lessequalorgreater}{22DA}
\pdfglyphtounicode{lessmonospace}{FF1C}
\pdfglyphtounicode{lessorequivalent}{2272}
\pdfglyphtounicode{lessorgreater}{2276}
\pdfglyphtounicode{lessoverequal}{2266}
\pdfglyphtounicode{lesssmall}{FE64}
\pdfglyphtounicode{lezh}{026E}
\pdfglyphtounicode{lfblock}{258C}
\pdfglyphtounicode{lhookretroflex}{026D}
\pdfglyphtounicode{lira}{20A4}
\pdfglyphtounicode{liwnarmenian}{056C}
\pdfglyphtounicode{lj}{01C9}
\pdfglyphtounicode{ljecyrillic}{0459}
\pdfglyphtounicode{ll}{F6C0}
\pdfglyphtounicode{lladeva}{0933}
\pdfglyphtounicode{llagujarati}{0AB3}
\pdfglyphtounicode{llinebelow}{1E3B}
\pdfglyphtounicode{llladeva}{0934}
\pdfglyphtounicode{llvocalicbengali}{09E1}
\pdfglyphtounicode{llvocalicdeva}{0961}
\pdfglyphtounicode{llvocalicvowelsignbengali}{09E3}
\pdfglyphtounicode{llvocalicvowelsigndeva}{0963}
\pdfglyphtounicode{lmiddletilde}{026B}
\pdfglyphtounicode{lmonospace}{FF4C}
\pdfglyphtounicode{lmsquare}{33D0}
\pdfglyphtounicode{lochulathai}{0E2C}
\pdfglyphtounicode{logicaland}{2227}
\pdfglyphtounicode{logicalnot}{00AC}
\pdfglyphtounicode{logicalnotreversed}{2310}
\pdfglyphtounicode{logicalor}{2228}
\pdfglyphtounicode{lolingthai}{0E25}
\pdfglyphtounicode{longs}{017F}
\pdfglyphtounicode{lowlinecenterline}{FE4E}
\pdfglyphtounicode{lowlinecmb}{0332}
\pdfglyphtounicode{lowlinedashed}{FE4D}
\pdfglyphtounicode{lozenge}{25CA}
\pdfglyphtounicode{lparen}{24A7}
\pdfglyphtounicode{lslash}{0142}
\pdfglyphtounicode{lsquare}{2113}
\pdfglyphtounicode{lsuperior}{F6EE}
\pdfglyphtounicode{ltshade}{2591}
\pdfglyphtounicode{luthai}{0E26}
\pdfglyphtounicode{lvocalicbengali}{098C}
\pdfglyphtounicode{lvocalicdeva}{090C}
\pdfglyphtounicode{lvocalicvowelsignbengali}{09E2}
\pdfglyphtounicode{lvocalicvowelsigndeva}{0962}
\pdfglyphtounicode{lxsquare}{33D3}
\pdfglyphtounicode{m}{006D}
\pdfglyphtounicode{mabengali}{09AE}
\pdfglyphtounicode{macron}{00AF}
\pdfglyphtounicode{macronbelowcmb}{0331}
\pdfglyphtounicode{macroncmb}{0304}
\pdfglyphtounicode{macronlowmod}{02CD}
\pdfglyphtounicode{macronmonospace}{FFE3}
\pdfglyphtounicode{macute}{1E3F}
\pdfglyphtounicode{madeva}{092E}
\pdfglyphtounicode{magujarati}{0AAE}
\pdfglyphtounicode{magurmukhi}{0A2E}
\pdfglyphtounicode{mahapakhhebrew}{05A4}
\pdfglyphtounicode{mahapakhlefthebrew}{05A4}
\pdfglyphtounicode{mahiragana}{307E}
\pdfglyphtounicode{maichattawalowleftthai}{F895}
\pdfglyphtounicode{maichattawalowrightthai}{F894}
\pdfglyphtounicode{maichattawathai}{0E4B}
\pdfglyphtounicode{maichattawaupperleftthai}{F893}
\pdfglyphtounicode{maieklowleftthai}{F88C}
\pdfglyphtounicode{maieklowrightthai}{F88B}
\pdfglyphtounicode{maiekthai}{0E48}
\pdfglyphtounicode{maiekupperleftthai}{F88A}
\pdfglyphtounicode{maihanakatleftthai}{F884}
\pdfglyphtounicode{maihanakatthai}{0E31}
\pdfglyphtounicode{maitaikhuleftthai}{F889}
\pdfglyphtounicode{maitaikhuthai}{0E47}
\pdfglyphtounicode{maitholowleftthai}{F88F}
\pdfglyphtounicode{maitholowrightthai}{F88E}
\pdfglyphtounicode{maithothai}{0E49}
\pdfglyphtounicode{maithoupperleftthai}{F88D}
\pdfglyphtounicode{maitrilowleftthai}{F892}
\pdfglyphtounicode{maitrilowrightthai}{F891}
\pdfglyphtounicode{maitrithai}{0E4A}
\pdfglyphtounicode{maitriupperleftthai}{F890}
\pdfglyphtounicode{maiyamokthai}{0E46}
\pdfglyphtounicode{makatakana}{30DE}
\pdfglyphtounicode{makatakanahalfwidth}{FF8F}
\pdfglyphtounicode{male}{2642}
\pdfglyphtounicode{mansyonsquare}{3347}
\pdfglyphtounicode{maqafhebrew}{05BE}
\pdfglyphtounicode{mars}{2642}
\pdfglyphtounicode{masoracirclehebrew}{05AF}
\pdfglyphtounicode{masquare}{3383}
\pdfglyphtounicode{mbopomofo}{3107}
\pdfglyphtounicode{mbsquare}{33D4}
\pdfglyphtounicode{mcircle}{24DC}
\pdfglyphtounicode{mcubedsquare}{33A5}
\pdfglyphtounicode{mdotaccent}{1E41}
\pdfglyphtounicode{mdotbelow}{1E43}
\pdfglyphtounicode{meemarabic}{0645}
\pdfglyphtounicode{meemfinalarabic}{FEE2}
\pdfglyphtounicode{meeminitialarabic}{FEE3}
\pdfglyphtounicode{meemmedialarabic}{FEE4}
\pdfglyphtounicode{meemmeeminitialarabic}{FCD1}
\pdfglyphtounicode{meemmeemisolatedarabic}{FC48}
\pdfglyphtounicode{meetorusquare}{334D}
\pdfglyphtounicode{mehiragana}{3081}
\pdfglyphtounicode{meizierasquare}{337E}
\pdfglyphtounicode{mekatakana}{30E1}
\pdfglyphtounicode{mekatakanahalfwidth}{FF92}
\pdfglyphtounicode{mem}{05DE}
\pdfglyphtounicode{memdagesh}{FB3E}
\pdfglyphtounicode{memdageshhebrew}{FB3E}
\pdfglyphtounicode{memhebrew}{05DE}
\pdfglyphtounicode{menarmenian}{0574}
\pdfglyphtounicode{merkhahebrew}{05A5}
\pdfglyphtounicode{merkhakefulahebrew}{05A6}
\pdfglyphtounicode{merkhakefulalefthebrew}{05A6}
\pdfglyphtounicode{merkhalefthebrew}{05A5}
\pdfglyphtounicode{mhook}{0271}
\pdfglyphtounicode{mhzsquare}{3392}
\pdfglyphtounicode{middledotkatakanahalfwidth}{FF65}
\pdfglyphtounicode{middot}{00B7}
\pdfglyphtounicode{mieumacirclekorean}{3272}
\pdfglyphtounicode{mieumaparenkorean}{3212}
\pdfglyphtounicode{mieumcirclekorean}{3264}
\pdfglyphtounicode{mieumkorean}{3141}
\pdfglyphtounicode{mieumpansioskorean}{3170}
\pdfglyphtounicode{mieumparenkorean}{3204}
\pdfglyphtounicode{mieumpieupkorean}{316E}
\pdfglyphtounicode{mieumsioskorean}{316F}
\pdfglyphtounicode{mihiragana}{307F}
\pdfglyphtounicode{mikatakana}{30DF}
\pdfglyphtounicode{mikatakanahalfwidth}{FF90}
\pdfglyphtounicode{minus}{2212}
\pdfglyphtounicode{minusbelowcmb}{0320}
\pdfglyphtounicode{minuscircle}{2296}
\pdfglyphtounicode{minusmod}{02D7}
\pdfglyphtounicode{minusplus}{2213}
\pdfglyphtounicode{minute}{2032}
\pdfglyphtounicode{miribaarusquare}{334A}
\pdfglyphtounicode{mirisquare}{3349}
\pdfglyphtounicode{mlonglegturned}{0270}
\pdfglyphtounicode{mlsquare}{3396}
\pdfglyphtounicode{mmcubedsquare}{33A3}
\pdfglyphtounicode{mmonospace}{FF4D}
\pdfglyphtounicode{mmsquaredsquare}{339F}
\pdfglyphtounicode{mohiragana}{3082}
\pdfglyphtounicode{mohmsquare}{33C1}
\pdfglyphtounicode{mokatakana}{30E2}
\pdfglyphtounicode{mokatakanahalfwidth}{FF93}
\pdfglyphtounicode{molsquare}{33D6}
\pdfglyphtounicode{momathai}{0E21}
\pdfglyphtounicode{moverssquare}{33A7}
\pdfglyphtounicode{moverssquaredsquare}{33A8}
\pdfglyphtounicode{mparen}{24A8}
\pdfglyphtounicode{mpasquare}{33AB}
\pdfglyphtounicode{mssquare}{33B3}
\pdfglyphtounicode{msuperior}{F6EF}
\pdfglyphtounicode{mturned}{026F}
\pdfglyphtounicode{mu}{00B5}
\pdfglyphtounicode{mu1}{00B5}
\pdfglyphtounicode{muasquare}{3382}
\pdfglyphtounicode{muchgreater}{226B}
\pdfglyphtounicode{muchless}{226A}
\pdfglyphtounicode{mufsquare}{338C}
\pdfglyphtounicode{mugreek}{03BC}
\pdfglyphtounicode{mugsquare}{338D}
\pdfglyphtounicode{muhiragana}{3080}
\pdfglyphtounicode{mukatakana}{30E0}
\pdfglyphtounicode{mukatakanahalfwidth}{FF91}
\pdfglyphtounicode{mulsquare}{3395}
\pdfglyphtounicode{multiply}{00D7}
\pdfglyphtounicode{mumsquare}{339B}
\pdfglyphtounicode{munahhebrew}{05A3}
\pdfglyphtounicode{munahlefthebrew}{05A3}
\pdfglyphtounicode{musicalnote}{266A}
\pdfglyphtounicode{musicalnotedbl}{266B}
\pdfglyphtounicode{musicflatsign}{266D}
\pdfglyphtounicode{musicsharpsign}{266F}
\pdfglyphtounicode{mussquare}{33B2}
\pdfglyphtounicode{muvsquare}{33B6}
\pdfglyphtounicode{muwsquare}{33BC}
\pdfglyphtounicode{mvmegasquare}{33B9}
\pdfglyphtounicode{mvsquare}{33B7}
\pdfglyphtounicode{mwmegasquare}{33BF}
\pdfglyphtounicode{mwsquare}{33BD}
\pdfglyphtounicode{n}{006E}
\pdfglyphtounicode{nabengali}{09A8}
\pdfglyphtounicode{nabla}{2207}
\pdfglyphtounicode{nacute}{0144}
\pdfglyphtounicode{nadeva}{0928}
\pdfglyphtounicode{nagujarati}{0AA8}
\pdfglyphtounicode{nagurmukhi}{0A28}
\pdfglyphtounicode{nahiragana}{306A}
\pdfglyphtounicode{nakatakana}{30CA}
\pdfglyphtounicode{nakatakanahalfwidth}{FF85}
\pdfglyphtounicode{napostrophe}{0149}
\pdfglyphtounicode{nasquare}{3381}
\pdfglyphtounicode{nbopomofo}{310B}
\pdfglyphtounicode{nbspace}{00A0}
\pdfglyphtounicode{ncaron}{0148}
\pdfglyphtounicode{ncedilla}{0146}
\pdfglyphtounicode{ncircle}{24DD}
\pdfglyphtounicode{ncircumflexbelow}{1E4B}
\pdfglyphtounicode{ncommaaccent}{0146}
\pdfglyphtounicode{ndotaccent}{1E45}
\pdfglyphtounicode{ndotbelow}{1E47}
\pdfglyphtounicode{nehiragana}{306D}
\pdfglyphtounicode{nekatakana}{30CD}
\pdfglyphtounicode{nekatakanahalfwidth}{FF88}
\pdfglyphtounicode{newsheqelsign}{20AA}
\pdfglyphtounicode{nfsquare}{338B}
\pdfglyphtounicode{ngabengali}{0999}
\pdfglyphtounicode{ngadeva}{0919}
\pdfglyphtounicode{ngagujarati}{0A99}
\pdfglyphtounicode{ngagurmukhi}{0A19}
\pdfglyphtounicode{ngonguthai}{0E07}
\pdfglyphtounicode{nhiragana}{3093}
\pdfglyphtounicode{nhookleft}{0272}
\pdfglyphtounicode{nhookretroflex}{0273}
\pdfglyphtounicode{nieunacirclekorean}{326F}
\pdfglyphtounicode{nieunaparenkorean}{320F}
\pdfglyphtounicode{nieuncieuckorean}{3135}
\pdfglyphtounicode{nieuncirclekorean}{3261}
\pdfglyphtounicode{nieunhieuhkorean}{3136}
\pdfglyphtounicode{nieunkorean}{3134}
\pdfglyphtounicode{nieunpansioskorean}{3168}
\pdfglyphtounicode{nieunparenkorean}{3201}
\pdfglyphtounicode{nieunsioskorean}{3167}
\pdfglyphtounicode{nieuntikeutkorean}{3166}
\pdfglyphtounicode{nihiragana}{306B}
\pdfglyphtounicode{nikatakana}{30CB}
\pdfglyphtounicode{nikatakanahalfwidth}{FF86}
\pdfglyphtounicode{nikhahitleftthai}{F899}
\pdfglyphtounicode{nikhahitthai}{0E4D}
\pdfglyphtounicode{nine}{0039}
\pdfglyphtounicode{ninearabic}{0669}
\pdfglyphtounicode{ninebengali}{09EF}
\pdfglyphtounicode{ninecircle}{2468}
\pdfglyphtounicode{ninecircleinversesansserif}{2792}
\pdfglyphtounicode{ninedeva}{096F}
\pdfglyphtounicode{ninegujarati}{0AEF}
\pdfglyphtounicode{ninegurmukhi}{0A6F}
\pdfglyphtounicode{ninehackarabic}{0669}
\pdfglyphtounicode{ninehangzhou}{3029}
\pdfglyphtounicode{nineideographicparen}{3228}
\pdfglyphtounicode{nineinferior}{2089}
\pdfglyphtounicode{ninemonospace}{FF19}
\pdfglyphtounicode{nineoldstyle}{F739}
\pdfglyphtounicode{nineparen}{247C}
\pdfglyphtounicode{nineperiod}{2490}
\pdfglyphtounicode{ninepersian}{06F9}
\pdfglyphtounicode{nineroman}{2178}
\pdfglyphtounicode{ninesuperior}{2079}
\pdfglyphtounicode{nineteencircle}{2472}
\pdfglyphtounicode{nineteenparen}{2486}
\pdfglyphtounicode{nineteenperiod}{249A}
\pdfglyphtounicode{ninethai}{0E59}
\pdfglyphtounicode{nj}{01CC}
\pdfglyphtounicode{njecyrillic}{045A}
\pdfglyphtounicode{nkatakana}{30F3}
\pdfglyphtounicode{nkatakanahalfwidth}{FF9D}
\pdfglyphtounicode{nlegrightlong}{019E}
\pdfglyphtounicode{nlinebelow}{1E49}
\pdfglyphtounicode{nmonospace}{FF4E}
\pdfglyphtounicode{nmsquare}{339A}
\pdfglyphtounicode{nnabengali}{09A3}
\pdfglyphtounicode{nnadeva}{0923}
\pdfglyphtounicode{nnagujarati}{0AA3}
\pdfglyphtounicode{nnagurmukhi}{0A23}
\pdfglyphtounicode{nnnadeva}{0929}
\pdfglyphtounicode{nohiragana}{306E}
\pdfglyphtounicode{nokatakana}{30CE}
\pdfglyphtounicode{nokatakanahalfwidth}{FF89}
\pdfglyphtounicode{nonbreakingspace}{00A0}
\pdfglyphtounicode{nonenthai}{0E13}
\pdfglyphtounicode{nonuthai}{0E19}
\pdfglyphtounicode{noonarabic}{0646}
\pdfglyphtounicode{noonfinalarabic}{FEE6}
\pdfglyphtounicode{noonghunnaarabic}{06BA}
\pdfglyphtounicode{noonghunnafinalarabic}{FB9F}
% noonhehinitialarabic;FEE7 FEEC
\pdfglyphtounicode{nooninitialarabic}{FEE7}
\pdfglyphtounicode{noonjeeminitialarabic}{FCD2}
\pdfglyphtounicode{noonjeemisolatedarabic}{FC4B}
\pdfglyphtounicode{noonmedialarabic}{FEE8}
\pdfglyphtounicode{noonmeeminitialarabic}{FCD5}
\pdfglyphtounicode{noonmeemisolatedarabic}{FC4E}
\pdfglyphtounicode{noonnoonfinalarabic}{FC8D}
\pdfglyphtounicode{notcontains}{220C}
\pdfglyphtounicode{notelement}{2209}
\pdfglyphtounicode{notelementof}{2209}
\pdfglyphtounicode{notequal}{2260}
\pdfglyphtounicode{notgreater}{226F}
\pdfglyphtounicode{notgreaternorequal}{2271}
\pdfglyphtounicode{notgreaternorless}{2279}
\pdfglyphtounicode{notidentical}{2262}
\pdfglyphtounicode{notless}{226E}
\pdfglyphtounicode{notlessnorequal}{2270}
\pdfglyphtounicode{notparallel}{2226}
\pdfglyphtounicode{notprecedes}{2280}
\pdfglyphtounicode{notsubset}{2284}
\pdfglyphtounicode{notsucceeds}{2281}
\pdfglyphtounicode{notsuperset}{2285}
\pdfglyphtounicode{nowarmenian}{0576}
\pdfglyphtounicode{nparen}{24A9}
\pdfglyphtounicode{nssquare}{33B1}
\pdfglyphtounicode{nsuperior}{207F}
\pdfglyphtounicode{ntilde}{00F1}
\pdfglyphtounicode{nu}{03BD}
\pdfglyphtounicode{nuhiragana}{306C}
\pdfglyphtounicode{nukatakana}{30CC}
\pdfglyphtounicode{nukatakanahalfwidth}{FF87}
\pdfglyphtounicode{nuktabengali}{09BC}
\pdfglyphtounicode{nuktadeva}{093C}
\pdfglyphtounicode{nuktagujarati}{0ABC}
\pdfglyphtounicode{nuktagurmukhi}{0A3C}
\pdfglyphtounicode{numbersign}{0023}
\pdfglyphtounicode{numbersignmonospace}{FF03}
\pdfglyphtounicode{numbersignsmall}{FE5F}
\pdfglyphtounicode{numeralsigngreek}{0374}
\pdfglyphtounicode{numeralsignlowergreek}{0375}
\pdfglyphtounicode{numero}{2116}
\pdfglyphtounicode{nun}{05E0}
\pdfglyphtounicode{nundagesh}{FB40}
\pdfglyphtounicode{nundageshhebrew}{FB40}
\pdfglyphtounicode{nunhebrew}{05E0}
\pdfglyphtounicode{nvsquare}{33B5}
\pdfglyphtounicode{nwsquare}{33BB}
\pdfglyphtounicode{nyabengali}{099E}
\pdfglyphtounicode{nyadeva}{091E}
\pdfglyphtounicode{nyagujarati}{0A9E}
\pdfglyphtounicode{nyagurmukhi}{0A1E}
\pdfglyphtounicode{o}{006F}
\pdfglyphtounicode{oacute}{00F3}
\pdfglyphtounicode{oangthai}{0E2D}
\pdfglyphtounicode{obarred}{0275}
\pdfglyphtounicode{obarredcyrillic}{04E9}
\pdfglyphtounicode{obarreddieresiscyrillic}{04EB}
\pdfglyphtounicode{obengali}{0993}
\pdfglyphtounicode{obopomofo}{311B}
\pdfglyphtounicode{obreve}{014F}
\pdfglyphtounicode{ocandradeva}{0911}
\pdfglyphtounicode{ocandragujarati}{0A91}
\pdfglyphtounicode{ocandravowelsigndeva}{0949}
\pdfglyphtounicode{ocandravowelsigngujarati}{0AC9}
\pdfglyphtounicode{ocaron}{01D2}
\pdfglyphtounicode{ocircle}{24DE}
\pdfglyphtounicode{ocircumflex}{00F4}
\pdfglyphtounicode{ocircumflexacute}{1ED1}
\pdfglyphtounicode{ocircumflexdotbelow}{1ED9}
\pdfglyphtounicode{ocircumflexgrave}{1ED3}
\pdfglyphtounicode{ocircumflexhookabove}{1ED5}
\pdfglyphtounicode{ocircumflextilde}{1ED7}
\pdfglyphtounicode{ocyrillic}{043E}
\pdfglyphtounicode{odblacute}{0151}
\pdfglyphtounicode{odblgrave}{020D}
\pdfglyphtounicode{odeva}{0913}
\pdfglyphtounicode{odieresis}{00F6}
\pdfglyphtounicode{odieresiscyrillic}{04E7}
\pdfglyphtounicode{odotbelow}{1ECD}
\pdfglyphtounicode{oe}{0153}
\pdfglyphtounicode{oekorean}{315A}
\pdfglyphtounicode{ogonek}{02DB}
\pdfglyphtounicode{ogonekcmb}{0328}
\pdfglyphtounicode{ograve}{00F2}
\pdfglyphtounicode{ogujarati}{0A93}
\pdfglyphtounicode{oharmenian}{0585}
\pdfglyphtounicode{ohiragana}{304A}
\pdfglyphtounicode{ohookabove}{1ECF}
\pdfglyphtounicode{ohorn}{01A1}
\pdfglyphtounicode{ohornacute}{1EDB}
\pdfglyphtounicode{ohorndotbelow}{1EE3}
\pdfglyphtounicode{ohorngrave}{1EDD}
\pdfglyphtounicode{ohornhookabove}{1EDF}
\pdfglyphtounicode{ohorntilde}{1EE1}
\pdfglyphtounicode{ohungarumlaut}{0151}
\pdfglyphtounicode{oi}{01A3}
\pdfglyphtounicode{oinvertedbreve}{020F}
\pdfglyphtounicode{okatakana}{30AA}
\pdfglyphtounicode{okatakanahalfwidth}{FF75}
\pdfglyphtounicode{okorean}{3157}
\pdfglyphtounicode{olehebrew}{05AB}
\pdfglyphtounicode{omacron}{014D}
\pdfglyphtounicode{omacronacute}{1E53}
\pdfglyphtounicode{omacrongrave}{1E51}
\pdfglyphtounicode{omdeva}{0950}
\pdfglyphtounicode{omega}{03C9}
\pdfglyphtounicode{omega1}{03D6}
\pdfglyphtounicode{omegacyrillic}{0461}
\pdfglyphtounicode{omegalatinclosed}{0277}
\pdfglyphtounicode{omegaroundcyrillic}{047B}
\pdfglyphtounicode{omegatitlocyrillic}{047D}
\pdfglyphtounicode{omegatonos}{03CE}
\pdfglyphtounicode{omgujarati}{0AD0}
\pdfglyphtounicode{omicron}{03BF}
\pdfglyphtounicode{omicrontonos}{03CC}
\pdfglyphtounicode{omonospace}{FF4F}
\pdfglyphtounicode{one}{0031}
\pdfglyphtounicode{onearabic}{0661}
\pdfglyphtounicode{onebengali}{09E7}
\pdfglyphtounicode{onecircle}{2460}
\pdfglyphtounicode{onecircleinversesansserif}{278A}
\pdfglyphtounicode{onedeva}{0967}
\pdfglyphtounicode{onedotenleader}{2024}
\pdfglyphtounicode{oneeighth}{215B}
\pdfglyphtounicode{onefitted}{F6DC}
\pdfglyphtounicode{onegujarati}{0AE7}
\pdfglyphtounicode{onegurmukhi}{0A67}
\pdfglyphtounicode{onehackarabic}{0661}
\pdfglyphtounicode{onehalf}{00BD}
\pdfglyphtounicode{onehangzhou}{3021}
\pdfglyphtounicode{oneideographicparen}{3220}
\pdfglyphtounicode{oneinferior}{2081}
\pdfglyphtounicode{onemonospace}{FF11}
\pdfglyphtounicode{onenumeratorbengali}{09F4}
\pdfglyphtounicode{oneoldstyle}{F731}
\pdfglyphtounicode{oneparen}{2474}
\pdfglyphtounicode{oneperiod}{2488}
\pdfglyphtounicode{onepersian}{06F1}
\pdfglyphtounicode{onequarter}{00BC}
\pdfglyphtounicode{oneroman}{2170}
\pdfglyphtounicode{onesuperior}{00B9}
\pdfglyphtounicode{onethai}{0E51}
\pdfglyphtounicode{onethird}{2153}
\pdfglyphtounicode{oogonek}{01EB}
\pdfglyphtounicode{oogonekmacron}{01ED}
\pdfglyphtounicode{oogurmukhi}{0A13}
\pdfglyphtounicode{oomatragurmukhi}{0A4B}
\pdfglyphtounicode{oopen}{0254}
\pdfglyphtounicode{oparen}{24AA}
\pdfglyphtounicode{openbullet}{25E6}
\pdfglyphtounicode{option}{2325}
\pdfglyphtounicode{ordfeminine}{00AA}
\pdfglyphtounicode{ordmasculine}{00BA}
\pdfglyphtounicode{orthogonal}{221F}
\pdfglyphtounicode{oshortdeva}{0912}
\pdfglyphtounicode{oshortvowelsigndeva}{094A}
\pdfglyphtounicode{oslash}{00F8}
\pdfglyphtounicode{oslashacute}{01FF}
\pdfglyphtounicode{osmallhiragana}{3049}
\pdfglyphtounicode{osmallkatakana}{30A9}
\pdfglyphtounicode{osmallkatakanahalfwidth}{FF6B}
\pdfglyphtounicode{ostrokeacute}{01FF}
\pdfglyphtounicode{osuperior}{F6F0}
\pdfglyphtounicode{otcyrillic}{047F}
\pdfglyphtounicode{otilde}{00F5}
\pdfglyphtounicode{otildeacute}{1E4D}
\pdfglyphtounicode{otildedieresis}{1E4F}
\pdfglyphtounicode{oubopomofo}{3121}
\pdfglyphtounicode{overline}{203E}
\pdfglyphtounicode{overlinecenterline}{FE4A}
\pdfglyphtounicode{overlinecmb}{0305}
\pdfglyphtounicode{overlinedashed}{FE49}
\pdfglyphtounicode{overlinedblwavy}{FE4C}
\pdfglyphtounicode{overlinewavy}{FE4B}
\pdfglyphtounicode{overscore}{00AF}
\pdfglyphtounicode{ovowelsignbengali}{09CB}
\pdfglyphtounicode{ovowelsigndeva}{094B}
\pdfglyphtounicode{ovowelsigngujarati}{0ACB}
\pdfglyphtounicode{p}{0070}
\pdfglyphtounicode{paampssquare}{3380}
\pdfglyphtounicode{paasentosquare}{332B}
\pdfglyphtounicode{pabengali}{09AA}
\pdfglyphtounicode{pacute}{1E55}
\pdfglyphtounicode{padeva}{092A}
\pdfglyphtounicode{pagedown}{21DF}
\pdfglyphtounicode{pageup}{21DE}
\pdfglyphtounicode{pagujarati}{0AAA}
\pdfglyphtounicode{pagurmukhi}{0A2A}
\pdfglyphtounicode{pahiragana}{3071}
\pdfglyphtounicode{paiyannoithai}{0E2F}
\pdfglyphtounicode{pakatakana}{30D1}
\pdfglyphtounicode{palatalizationcyrilliccmb}{0484}
\pdfglyphtounicode{palochkacyrillic}{04C0}
\pdfglyphtounicode{pansioskorean}{317F}
\pdfglyphtounicode{paragraph}{00B6}
\pdfglyphtounicode{parallel}{2225}
\pdfglyphtounicode{parenleft}{0028}
\pdfglyphtounicode{parenleftaltonearabic}{FD3E}
\pdfglyphtounicode{parenleftbt}{F8ED}
\pdfglyphtounicode{parenleftex}{F8EC}
\pdfglyphtounicode{parenleftinferior}{208D}
\pdfglyphtounicode{parenleftmonospace}{FF08}
\pdfglyphtounicode{parenleftsmall}{FE59}
\pdfglyphtounicode{parenleftsuperior}{207D}
\pdfglyphtounicode{parenlefttp}{F8EB}
\pdfglyphtounicode{parenleftvertical}{FE35}
\pdfglyphtounicode{parenright}{0029}
\pdfglyphtounicode{parenrightaltonearabic}{FD3F}
\pdfglyphtounicode{parenrightbt}{F8F8}
\pdfglyphtounicode{parenrightex}{F8F7}
\pdfglyphtounicode{parenrightinferior}{208E}
\pdfglyphtounicode{parenrightmonospace}{FF09}
\pdfglyphtounicode{parenrightsmall}{FE5A}
\pdfglyphtounicode{parenrightsuperior}{207E}
\pdfglyphtounicode{parenrighttp}{F8F6}
\pdfglyphtounicode{parenrightvertical}{FE36}
\pdfglyphtounicode{partialdiff}{2202}
\pdfglyphtounicode{paseqhebrew}{05C0}
\pdfglyphtounicode{pashtahebrew}{0599}
\pdfglyphtounicode{pasquare}{33A9}
\pdfglyphtounicode{patah}{05B7}
\pdfglyphtounicode{patah11}{05B7}
\pdfglyphtounicode{patah1d}{05B7}
\pdfglyphtounicode{patah2a}{05B7}
\pdfglyphtounicode{patahhebrew}{05B7}
\pdfglyphtounicode{patahnarrowhebrew}{05B7}
\pdfglyphtounicode{patahquarterhebrew}{05B7}
\pdfglyphtounicode{patahwidehebrew}{05B7}
\pdfglyphtounicode{pazerhebrew}{05A1}
\pdfglyphtounicode{pbopomofo}{3106}
\pdfglyphtounicode{pcircle}{24DF}
\pdfglyphtounicode{pdotaccent}{1E57}
\pdfglyphtounicode{pe}{05E4}
\pdfglyphtounicode{pecyrillic}{043F}
\pdfglyphtounicode{pedagesh}{FB44}
\pdfglyphtounicode{pedageshhebrew}{FB44}
\pdfglyphtounicode{peezisquare}{333B}
\pdfglyphtounicode{pefinaldageshhebrew}{FB43}
\pdfglyphtounicode{peharabic}{067E}
\pdfglyphtounicode{peharmenian}{057A}
\pdfglyphtounicode{pehebrew}{05E4}
\pdfglyphtounicode{pehfinalarabic}{FB57}
\pdfglyphtounicode{pehinitialarabic}{FB58}
\pdfglyphtounicode{pehiragana}{307A}
\pdfglyphtounicode{pehmedialarabic}{FB59}
\pdfglyphtounicode{pekatakana}{30DA}
\pdfglyphtounicode{pemiddlehookcyrillic}{04A7}
\pdfglyphtounicode{perafehebrew}{FB4E}
\pdfglyphtounicode{percent}{0025}
\pdfglyphtounicode{percentarabic}{066A}
\pdfglyphtounicode{percentmonospace}{FF05}
\pdfglyphtounicode{percentsmall}{FE6A}
\pdfglyphtounicode{period}{002E}
\pdfglyphtounicode{periodarmenian}{0589}
\pdfglyphtounicode{periodcentered}{00B7}
\pdfglyphtounicode{periodhalfwidth}{FF61}
\pdfglyphtounicode{periodinferior}{F6E7}
\pdfglyphtounicode{periodmonospace}{FF0E}
\pdfglyphtounicode{periodsmall}{FE52}
\pdfglyphtounicode{periodsuperior}{F6E8}
\pdfglyphtounicode{perispomenigreekcmb}{0342}
\pdfglyphtounicode{perpendicular}{22A5}
\pdfglyphtounicode{perthousand}{2030}
\pdfglyphtounicode{peseta}{20A7}
\pdfglyphtounicode{pfsquare}{338A}
\pdfglyphtounicode{phabengali}{09AB}
\pdfglyphtounicode{phadeva}{092B}
\pdfglyphtounicode{phagujarati}{0AAB}
\pdfglyphtounicode{phagurmukhi}{0A2B}
\pdfglyphtounicode{phi}{03C6}
\pdfglyphtounicode{phi1}{03D5}
\pdfglyphtounicode{phieuphacirclekorean}{327A}
\pdfglyphtounicode{phieuphaparenkorean}{321A}
\pdfglyphtounicode{phieuphcirclekorean}{326C}
\pdfglyphtounicode{phieuphkorean}{314D}
\pdfglyphtounicode{phieuphparenkorean}{320C}
\pdfglyphtounicode{philatin}{0278}
\pdfglyphtounicode{phinthuthai}{0E3A}
\pdfglyphtounicode{phisymbolgreek}{03D5}
\pdfglyphtounicode{phook}{01A5}
\pdfglyphtounicode{phophanthai}{0E1E}
\pdfglyphtounicode{phophungthai}{0E1C}
\pdfglyphtounicode{phosamphaothai}{0E20}
\pdfglyphtounicode{pi}{03C0}
\pdfglyphtounicode{pieupacirclekorean}{3273}
\pdfglyphtounicode{pieupaparenkorean}{3213}
\pdfglyphtounicode{pieupcieuckorean}{3176}
\pdfglyphtounicode{pieupcirclekorean}{3265}
\pdfglyphtounicode{pieupkiyeokkorean}{3172}
\pdfglyphtounicode{pieupkorean}{3142}
\pdfglyphtounicode{pieupparenkorean}{3205}
\pdfglyphtounicode{pieupsioskiyeokkorean}{3174}
\pdfglyphtounicode{pieupsioskorean}{3144}
\pdfglyphtounicode{pieupsiostikeutkorean}{3175}
\pdfglyphtounicode{pieupthieuthkorean}{3177}
\pdfglyphtounicode{pieuptikeutkorean}{3173}
\pdfglyphtounicode{pihiragana}{3074}
\pdfglyphtounicode{pikatakana}{30D4}
\pdfglyphtounicode{pisymbolgreek}{03D6}
\pdfglyphtounicode{piwrarmenian}{0583}
\pdfglyphtounicode{plus}{002B}
\pdfglyphtounicode{plusbelowcmb}{031F}
\pdfglyphtounicode{pluscircle}{2295}
\pdfglyphtounicode{plusminus}{00B1}
\pdfglyphtounicode{plusmod}{02D6}
\pdfglyphtounicode{plusmonospace}{FF0B}
\pdfglyphtounicode{plussmall}{FE62}
\pdfglyphtounicode{plussuperior}{207A}
\pdfglyphtounicode{pmonospace}{FF50}
\pdfglyphtounicode{pmsquare}{33D8}
\pdfglyphtounicode{pohiragana}{307D}
\pdfglyphtounicode{pointingindexdownwhite}{261F}
\pdfglyphtounicode{pointingindexleftwhite}{261C}
\pdfglyphtounicode{pointingindexrightwhite}{261E}
\pdfglyphtounicode{pointingindexupwhite}{261D}
\pdfglyphtounicode{pokatakana}{30DD}
\pdfglyphtounicode{poplathai}{0E1B}
\pdfglyphtounicode{postalmark}{3012}
\pdfglyphtounicode{postalmarkface}{3020}
\pdfglyphtounicode{pparen}{24AB}
\pdfglyphtounicode{precedes}{227A}
\pdfglyphtounicode{prescription}{211E}
\pdfglyphtounicode{primemod}{02B9}
\pdfglyphtounicode{primereversed}{2035}
\pdfglyphtounicode{product}{220F}
\pdfglyphtounicode{projective}{2305}
\pdfglyphtounicode{prolongedkana}{30FC}
\pdfglyphtounicode{propellor}{2318}
\pdfglyphtounicode{propersubset}{2282}
\pdfglyphtounicode{propersuperset}{2283}
\pdfglyphtounicode{proportion}{2237}
\pdfglyphtounicode{proportional}{221D}
\pdfglyphtounicode{psi}{03C8}
\pdfglyphtounicode{psicyrillic}{0471}
\pdfglyphtounicode{psilipneumatacyrilliccmb}{0486}
\pdfglyphtounicode{pssquare}{33B0}
\pdfglyphtounicode{puhiragana}{3077}
\pdfglyphtounicode{pukatakana}{30D7}
\pdfglyphtounicode{pvsquare}{33B4}
\pdfglyphtounicode{pwsquare}{33BA}
\pdfglyphtounicode{q}{0071}
\pdfglyphtounicode{qadeva}{0958}
\pdfglyphtounicode{qadmahebrew}{05A8}
\pdfglyphtounicode{qafarabic}{0642}
\pdfglyphtounicode{qaffinalarabic}{FED6}
\pdfglyphtounicode{qafinitialarabic}{FED7}
\pdfglyphtounicode{qafmedialarabic}{FED8}
\pdfglyphtounicode{qamats}{05B8}
\pdfglyphtounicode{qamats10}{05B8}
\pdfglyphtounicode{qamats1a}{05B8}
\pdfglyphtounicode{qamats1c}{05B8}
\pdfglyphtounicode{qamats27}{05B8}
\pdfglyphtounicode{qamats29}{05B8}
\pdfglyphtounicode{qamats33}{05B8}
\pdfglyphtounicode{qamatsde}{05B8}
\pdfglyphtounicode{qamatshebrew}{05B8}
\pdfglyphtounicode{qamatsnarrowhebrew}{05B8}
\pdfglyphtounicode{qamatsqatanhebrew}{05B8}
\pdfglyphtounicode{qamatsqatannarrowhebrew}{05B8}
\pdfglyphtounicode{qamatsqatanquarterhebrew}{05B8}
\pdfglyphtounicode{qamatsqatanwidehebrew}{05B8}
\pdfglyphtounicode{qamatsquarterhebrew}{05B8}
\pdfglyphtounicode{qamatswidehebrew}{05B8}
\pdfglyphtounicode{qarneyparahebrew}{059F}
\pdfglyphtounicode{qbopomofo}{3111}
\pdfglyphtounicode{qcircle}{24E0}
\pdfglyphtounicode{qhook}{02A0}
\pdfglyphtounicode{qmonospace}{FF51}
\pdfglyphtounicode{qof}{05E7}
\pdfglyphtounicode{qofdagesh}{FB47}
\pdfglyphtounicode{qofdageshhebrew}{FB47}
% qofhatafpatah;05E7 05B2
% qofhatafpatahhebrew;05E7 05B2
% qofhatafsegol;05E7 05B1
% qofhatafsegolhebrew;05E7 05B1
\pdfglyphtounicode{qofhebrew}{05E7}
% qofhiriq;05E7 05B4
% qofhiriqhebrew;05E7 05B4
% qofholam;05E7 05B9
% qofholamhebrew;05E7 05B9
% qofpatah;05E7 05B7
% qofpatahhebrew;05E7 05B7
% qofqamats;05E7 05B8
% qofqamatshebrew;05E7 05B8
% qofqubuts;05E7 05BB
% qofqubutshebrew;05E7 05BB
% qofsegol;05E7 05B6
% qofsegolhebrew;05E7 05B6
% qofsheva;05E7 05B0
% qofshevahebrew;05E7 05B0
% qoftsere;05E7 05B5
% qoftserehebrew;05E7 05B5
\pdfglyphtounicode{qparen}{24AC}
\pdfglyphtounicode{quarternote}{2669}
\pdfglyphtounicode{qubuts}{05BB}
\pdfglyphtounicode{qubuts18}{05BB}
\pdfglyphtounicode{qubuts25}{05BB}
\pdfglyphtounicode{qubuts31}{05BB}
\pdfglyphtounicode{qubutshebrew}{05BB}
\pdfglyphtounicode{qubutsnarrowhebrew}{05BB}
\pdfglyphtounicode{qubutsquarterhebrew}{05BB}
\pdfglyphtounicode{qubutswidehebrew}{05BB}
\pdfglyphtounicode{question}{003F}
\pdfglyphtounicode{questionarabic}{061F}
\pdfglyphtounicode{questionarmenian}{055E}
\pdfglyphtounicode{questiondown}{00BF}
\pdfglyphtounicode{questiondownsmall}{F7BF}
\pdfglyphtounicode{questiongreek}{037E}
\pdfglyphtounicode{questionmonospace}{FF1F}
\pdfglyphtounicode{questionsmall}{F73F}
\pdfglyphtounicode{quotedbl}{0022}
\pdfglyphtounicode{quotedblbase}{201E}
\pdfglyphtounicode{quotedblleft}{201C}
\pdfglyphtounicode{quotedblmonospace}{FF02}
\pdfglyphtounicode{quotedblprime}{301E}
\pdfglyphtounicode{quotedblprimereversed}{301D}
\pdfglyphtounicode{quotedblright}{201D}
\pdfglyphtounicode{quoteleft}{2018}
\pdfglyphtounicode{quoteleftreversed}{201B}
\pdfglyphtounicode{quotereversed}{201B}
\pdfglyphtounicode{quoteright}{2019}
\pdfglyphtounicode{quoterightn}{0149}
\pdfglyphtounicode{quotesinglbase}{201A}
\pdfglyphtounicode{quotesingle}{0027}
\pdfglyphtounicode{quotesinglemonospace}{FF07}
\pdfglyphtounicode{r}{0072}
\pdfglyphtounicode{raarmenian}{057C}
\pdfglyphtounicode{rabengali}{09B0}
\pdfglyphtounicode{racute}{0155}
\pdfglyphtounicode{radeva}{0930}
\pdfglyphtounicode{radical}{221A}
\pdfglyphtounicode{radicalex}{F8E5}
\pdfglyphtounicode{radoverssquare}{33AE}
\pdfglyphtounicode{radoverssquaredsquare}{33AF}
\pdfglyphtounicode{radsquare}{33AD}
\pdfglyphtounicode{rafe}{05BF}
\pdfglyphtounicode{rafehebrew}{05BF}
\pdfglyphtounicode{ragujarati}{0AB0}
\pdfglyphtounicode{ragurmukhi}{0A30}
\pdfglyphtounicode{rahiragana}{3089}
\pdfglyphtounicode{rakatakana}{30E9}
\pdfglyphtounicode{rakatakanahalfwidth}{FF97}
\pdfglyphtounicode{ralowerdiagonalbengali}{09F1}
\pdfglyphtounicode{ramiddlediagonalbengali}{09F0}
\pdfglyphtounicode{ramshorn}{0264}
\pdfglyphtounicode{ratio}{2236}
\pdfglyphtounicode{rbopomofo}{3116}
\pdfglyphtounicode{rcaron}{0159}
\pdfglyphtounicode{rcedilla}{0157}
\pdfglyphtounicode{rcircle}{24E1}
\pdfglyphtounicode{rcommaaccent}{0157}
\pdfglyphtounicode{rdblgrave}{0211}
\pdfglyphtounicode{rdotaccent}{1E59}
\pdfglyphtounicode{rdotbelow}{1E5B}
\pdfglyphtounicode{rdotbelowmacron}{1E5D}
\pdfglyphtounicode{referencemark}{203B}
\pdfglyphtounicode{reflexsubset}{2286}
\pdfglyphtounicode{reflexsuperset}{2287}
\pdfglyphtounicode{registered}{00AE}
\pdfglyphtounicode{registersans}{F8E8}
\pdfglyphtounicode{registerserif}{F6DA}
\pdfglyphtounicode{reharabic}{0631}
\pdfglyphtounicode{reharmenian}{0580}
\pdfglyphtounicode{rehfinalarabic}{FEAE}
\pdfglyphtounicode{rehiragana}{308C}
% rehyehaleflamarabic;0631 FEF3 FE8E 0644
\pdfglyphtounicode{rekatakana}{30EC}
\pdfglyphtounicode{rekatakanahalfwidth}{FF9A}
\pdfglyphtounicode{resh}{05E8}
\pdfglyphtounicode{reshdageshhebrew}{FB48}
% reshhatafpatah;05E8 05B2
% reshhatafpatahhebrew;05E8 05B2
% reshhatafsegol;05E8 05B1
% reshhatafsegolhebrew;05E8 05B1
\pdfglyphtounicode{reshhebrew}{05E8}
% reshhiriq;05E8 05B4
% reshhiriqhebrew;05E8 05B4
% reshholam;05E8 05B9
% reshholamhebrew;05E8 05B9
% reshpatah;05E8 05B7
% reshpatahhebrew;05E8 05B7
% reshqamats;05E8 05B8
% reshqamatshebrew;05E8 05B8
% reshqubuts;05E8 05BB
% reshqubutshebrew;05E8 05BB
% reshsegol;05E8 05B6
% reshsegolhebrew;05E8 05B6
% reshsheva;05E8 05B0
% reshshevahebrew;05E8 05B0
% reshtsere;05E8 05B5
% reshtserehebrew;05E8 05B5
\pdfglyphtounicode{reversedtilde}{223D}
\pdfglyphtounicode{reviahebrew}{0597}
\pdfglyphtounicode{reviamugrashhebrew}{0597}
\pdfglyphtounicode{revlogicalnot}{2310}
\pdfglyphtounicode{rfishhook}{027E}
\pdfglyphtounicode{rfishhookreversed}{027F}
\pdfglyphtounicode{rhabengali}{09DD}
\pdfglyphtounicode{rhadeva}{095D}
\pdfglyphtounicode{rho}{03C1}
\pdfglyphtounicode{rhook}{027D}
\pdfglyphtounicode{rhookturned}{027B}
\pdfglyphtounicode{rhookturnedsuperior}{02B5}
\pdfglyphtounicode{rhosymbolgreek}{03F1}
\pdfglyphtounicode{rhotichookmod}{02DE}
\pdfglyphtounicode{rieulacirclekorean}{3271}
\pdfglyphtounicode{rieulaparenkorean}{3211}
\pdfglyphtounicode{rieulcirclekorean}{3263}
\pdfglyphtounicode{rieulhieuhkorean}{3140}
\pdfglyphtounicode{rieulkiyeokkorean}{313A}
\pdfglyphtounicode{rieulkiyeoksioskorean}{3169}
\pdfglyphtounicode{rieulkorean}{3139}
\pdfglyphtounicode{rieulmieumkorean}{313B}
\pdfglyphtounicode{rieulpansioskorean}{316C}
\pdfglyphtounicode{rieulparenkorean}{3203}
\pdfglyphtounicode{rieulphieuphkorean}{313F}
\pdfglyphtounicode{rieulpieupkorean}{313C}
\pdfglyphtounicode{rieulpieupsioskorean}{316B}
\pdfglyphtounicode{rieulsioskorean}{313D}
\pdfglyphtounicode{rieulthieuthkorean}{313E}
\pdfglyphtounicode{rieultikeutkorean}{316A}
\pdfglyphtounicode{rieulyeorinhieuhkorean}{316D}
\pdfglyphtounicode{rightangle}{221F}
\pdfglyphtounicode{righttackbelowcmb}{0319}
\pdfglyphtounicode{righttriangle}{22BF}
\pdfglyphtounicode{rihiragana}{308A}
\pdfglyphtounicode{rikatakana}{30EA}
\pdfglyphtounicode{rikatakanahalfwidth}{FF98}
\pdfglyphtounicode{ring}{02DA}
\pdfglyphtounicode{ringbelowcmb}{0325}
\pdfglyphtounicode{ringcmb}{030A}
\pdfglyphtounicode{ringhalfleft}{02BF}
\pdfglyphtounicode{ringhalfleftarmenian}{0559}
\pdfglyphtounicode{ringhalfleftbelowcmb}{031C}
\pdfglyphtounicode{ringhalfleftcentered}{02D3}
\pdfglyphtounicode{ringhalfright}{02BE}
\pdfglyphtounicode{ringhalfrightbelowcmb}{0339}
\pdfglyphtounicode{ringhalfrightcentered}{02D2}
\pdfglyphtounicode{rinvertedbreve}{0213}
\pdfglyphtounicode{rittorusquare}{3351}
\pdfglyphtounicode{rlinebelow}{1E5F}
\pdfglyphtounicode{rlongleg}{027C}
\pdfglyphtounicode{rlonglegturned}{027A}
\pdfglyphtounicode{rmonospace}{FF52}
\pdfglyphtounicode{rohiragana}{308D}
\pdfglyphtounicode{rokatakana}{30ED}
\pdfglyphtounicode{rokatakanahalfwidth}{FF9B}
\pdfglyphtounicode{roruathai}{0E23}
\pdfglyphtounicode{rparen}{24AD}
\pdfglyphtounicode{rrabengali}{09DC}
\pdfglyphtounicode{rradeva}{0931}
\pdfglyphtounicode{rragurmukhi}{0A5C}
\pdfglyphtounicode{rreharabic}{0691}
\pdfglyphtounicode{rrehfinalarabic}{FB8D}
\pdfglyphtounicode{rrvocalicbengali}{09E0}
\pdfglyphtounicode{rrvocalicdeva}{0960}
\pdfglyphtounicode{rrvocalicgujarati}{0AE0}
\pdfglyphtounicode{rrvocalicvowelsignbengali}{09C4}
\pdfglyphtounicode{rrvocalicvowelsigndeva}{0944}
\pdfglyphtounicode{rrvocalicvowelsigngujarati}{0AC4}
\pdfglyphtounicode{rsuperior}{F6F1}
\pdfglyphtounicode{rtblock}{2590}
\pdfglyphtounicode{rturned}{0279}
\pdfglyphtounicode{rturnedsuperior}{02B4}
\pdfglyphtounicode{ruhiragana}{308B}
\pdfglyphtounicode{rukatakana}{30EB}
\pdfglyphtounicode{rukatakanahalfwidth}{FF99}
\pdfglyphtounicode{rupeemarkbengali}{09F2}
\pdfglyphtounicode{rupeesignbengali}{09F3}
\pdfglyphtounicode{rupiah}{F6DD}
\pdfglyphtounicode{ruthai}{0E24}
\pdfglyphtounicode{rvocalicbengali}{098B}
\pdfglyphtounicode{rvocalicdeva}{090B}
\pdfglyphtounicode{rvocalicgujarati}{0A8B}
\pdfglyphtounicode{rvocalicvowelsignbengali}{09C3}
\pdfglyphtounicode{rvocalicvowelsigndeva}{0943}
\pdfglyphtounicode{rvocalicvowelsigngujarati}{0AC3}
\pdfglyphtounicode{s}{0073}
\pdfglyphtounicode{sabengali}{09B8}
\pdfglyphtounicode{sacute}{015B}
\pdfglyphtounicode{sacutedotaccent}{1E65}
\pdfglyphtounicode{sadarabic}{0635}
\pdfglyphtounicode{sadeva}{0938}
\pdfglyphtounicode{sadfinalarabic}{FEBA}
\pdfglyphtounicode{sadinitialarabic}{FEBB}
\pdfglyphtounicode{sadmedialarabic}{FEBC}
\pdfglyphtounicode{sagujarati}{0AB8}
\pdfglyphtounicode{sagurmukhi}{0A38}
\pdfglyphtounicode{sahiragana}{3055}
\pdfglyphtounicode{sakatakana}{30B5}
\pdfglyphtounicode{sakatakanahalfwidth}{FF7B}
\pdfglyphtounicode{sallallahoualayhewasallamarabic}{FDFA}
\pdfglyphtounicode{samekh}{05E1}
\pdfglyphtounicode{samekhdagesh}{FB41}
\pdfglyphtounicode{samekhdageshhebrew}{FB41}
\pdfglyphtounicode{samekhhebrew}{05E1}
\pdfglyphtounicode{saraaathai}{0E32}
\pdfglyphtounicode{saraaethai}{0E41}
\pdfglyphtounicode{saraaimaimalaithai}{0E44}
\pdfglyphtounicode{saraaimaimuanthai}{0E43}
\pdfglyphtounicode{saraamthai}{0E33}
\pdfglyphtounicode{saraathai}{0E30}
\pdfglyphtounicode{saraethai}{0E40}
\pdfglyphtounicode{saraiileftthai}{F886}
\pdfglyphtounicode{saraiithai}{0E35}
\pdfglyphtounicode{saraileftthai}{F885}
\pdfglyphtounicode{saraithai}{0E34}
\pdfglyphtounicode{saraothai}{0E42}
\pdfglyphtounicode{saraueeleftthai}{F888}
\pdfglyphtounicode{saraueethai}{0E37}
\pdfglyphtounicode{saraueleftthai}{F887}
\pdfglyphtounicode{sarauethai}{0E36}
\pdfglyphtounicode{sarauthai}{0E38}
\pdfglyphtounicode{sarauuthai}{0E39}
\pdfglyphtounicode{sbopomofo}{3119}
\pdfglyphtounicode{scaron}{0161}
\pdfglyphtounicode{scarondotaccent}{1E67}
\pdfglyphtounicode{scedilla}{015F}
\pdfglyphtounicode{schwa}{0259}
\pdfglyphtounicode{schwacyrillic}{04D9}
\pdfglyphtounicode{schwadieresiscyrillic}{04DB}
\pdfglyphtounicode{schwahook}{025A}
\pdfglyphtounicode{scircle}{24E2}
\pdfglyphtounicode{scircumflex}{015D}
\pdfglyphtounicode{scommaaccent}{0219}
\pdfglyphtounicode{sdotaccent}{1E61}
\pdfglyphtounicode{sdotbelow}{1E63}
\pdfglyphtounicode{sdotbelowdotaccent}{1E69}
\pdfglyphtounicode{seagullbelowcmb}{033C}
\pdfglyphtounicode{second}{2033}
\pdfglyphtounicode{secondtonechinese}{02CA}
\pdfglyphtounicode{section}{00A7}
\pdfglyphtounicode{seenarabic}{0633}
\pdfglyphtounicode{seenfinalarabic}{FEB2}
\pdfglyphtounicode{seeninitialarabic}{FEB3}
\pdfglyphtounicode{seenmedialarabic}{FEB4}
\pdfglyphtounicode{segol}{05B6}
\pdfglyphtounicode{segol13}{05B6}
\pdfglyphtounicode{segol1f}{05B6}
\pdfglyphtounicode{segol2c}{05B6}
\pdfglyphtounicode{segolhebrew}{05B6}
\pdfglyphtounicode{segolnarrowhebrew}{05B6}
\pdfglyphtounicode{segolquarterhebrew}{05B6}
\pdfglyphtounicode{segoltahebrew}{0592}
\pdfglyphtounicode{segolwidehebrew}{05B6}
\pdfglyphtounicode{seharmenian}{057D}
\pdfglyphtounicode{sehiragana}{305B}
\pdfglyphtounicode{sekatakana}{30BB}
\pdfglyphtounicode{sekatakanahalfwidth}{FF7E}
\pdfglyphtounicode{semicolon}{003B}
\pdfglyphtounicode{semicolonarabic}{061B}
\pdfglyphtounicode{semicolonmonospace}{FF1B}
\pdfglyphtounicode{semicolonsmall}{FE54}
\pdfglyphtounicode{semivoicedmarkkana}{309C}
\pdfglyphtounicode{semivoicedmarkkanahalfwidth}{FF9F}
\pdfglyphtounicode{sentisquare}{3322}
\pdfglyphtounicode{sentosquare}{3323}
\pdfglyphtounicode{seven}{0037}
\pdfglyphtounicode{sevenarabic}{0667}
\pdfglyphtounicode{sevenbengali}{09ED}
\pdfglyphtounicode{sevencircle}{2466}
\pdfglyphtounicode{sevencircleinversesansserif}{2790}
\pdfglyphtounicode{sevendeva}{096D}
\pdfglyphtounicode{seveneighths}{215E}
\pdfglyphtounicode{sevengujarati}{0AED}
\pdfglyphtounicode{sevengurmukhi}{0A6D}
\pdfglyphtounicode{sevenhackarabic}{0667}
\pdfglyphtounicode{sevenhangzhou}{3027}
\pdfglyphtounicode{sevenideographicparen}{3226}
\pdfglyphtounicode{seveninferior}{2087}
\pdfglyphtounicode{sevenmonospace}{FF17}
\pdfglyphtounicode{sevenoldstyle}{F737}
\pdfglyphtounicode{sevenparen}{247A}
\pdfglyphtounicode{sevenperiod}{248E}
\pdfglyphtounicode{sevenpersian}{06F7}
\pdfglyphtounicode{sevenroman}{2176}
\pdfglyphtounicode{sevensuperior}{2077}
\pdfglyphtounicode{seventeencircle}{2470}
\pdfglyphtounicode{seventeenparen}{2484}
\pdfglyphtounicode{seventeenperiod}{2498}
\pdfglyphtounicode{seventhai}{0E57}
\pdfglyphtounicode{sfthyphen}{00AD}
\pdfglyphtounicode{shaarmenian}{0577}
\pdfglyphtounicode{shabengali}{09B6}
\pdfglyphtounicode{shacyrillic}{0448}
\pdfglyphtounicode{shaddaarabic}{0651}
\pdfglyphtounicode{shaddadammaarabic}{FC61}
\pdfglyphtounicode{shaddadammatanarabic}{FC5E}
\pdfglyphtounicode{shaddafathaarabic}{FC60}
% shaddafathatanarabic;0651 064B
\pdfglyphtounicode{shaddakasraarabic}{FC62}
\pdfglyphtounicode{shaddakasratanarabic}{FC5F}
\pdfglyphtounicode{shade}{2592}
\pdfglyphtounicode{shadedark}{2593}
\pdfglyphtounicode{shadelight}{2591}
\pdfglyphtounicode{shademedium}{2592}
\pdfglyphtounicode{shadeva}{0936}
\pdfglyphtounicode{shagujarati}{0AB6}
\pdfglyphtounicode{shagurmukhi}{0A36}
\pdfglyphtounicode{shalshelethebrew}{0593}
\pdfglyphtounicode{shbopomofo}{3115}
\pdfglyphtounicode{shchacyrillic}{0449}
\pdfglyphtounicode{sheenarabic}{0634}
\pdfglyphtounicode{sheenfinalarabic}{FEB6}
\pdfglyphtounicode{sheeninitialarabic}{FEB7}
\pdfglyphtounicode{sheenmedialarabic}{FEB8}
\pdfglyphtounicode{sheicoptic}{03E3}
\pdfglyphtounicode{sheqel}{20AA}
\pdfglyphtounicode{sheqelhebrew}{20AA}
\pdfglyphtounicode{sheva}{05B0}
\pdfglyphtounicode{sheva115}{05B0}
\pdfglyphtounicode{sheva15}{05B0}
\pdfglyphtounicode{sheva22}{05B0}
\pdfglyphtounicode{sheva2e}{05B0}
\pdfglyphtounicode{shevahebrew}{05B0}
\pdfglyphtounicode{shevanarrowhebrew}{05B0}
\pdfglyphtounicode{shevaquarterhebrew}{05B0}
\pdfglyphtounicode{shevawidehebrew}{05B0}
\pdfglyphtounicode{shhacyrillic}{04BB}
\pdfglyphtounicode{shimacoptic}{03ED}
\pdfglyphtounicode{shin}{05E9}
\pdfglyphtounicode{shindagesh}{FB49}
\pdfglyphtounicode{shindageshhebrew}{FB49}
\pdfglyphtounicode{shindageshshindot}{FB2C}
\pdfglyphtounicode{shindageshshindothebrew}{FB2C}
\pdfglyphtounicode{shindageshsindot}{FB2D}
\pdfglyphtounicode{shindageshsindothebrew}{FB2D}
\pdfglyphtounicode{shindothebrew}{05C1}
\pdfglyphtounicode{shinhebrew}{05E9}
\pdfglyphtounicode{shinshindot}{FB2A}
\pdfglyphtounicode{shinshindothebrew}{FB2A}
\pdfglyphtounicode{shinsindot}{FB2B}
\pdfglyphtounicode{shinsindothebrew}{FB2B}
\pdfglyphtounicode{shook}{0282}
\pdfglyphtounicode{sigma}{03C3}
\pdfglyphtounicode{sigma1}{03C2}
\pdfglyphtounicode{sigmafinal}{03C2}
\pdfglyphtounicode{sigmalunatesymbolgreek}{03F2}
\pdfglyphtounicode{sihiragana}{3057}
\pdfglyphtounicode{sikatakana}{30B7}
\pdfglyphtounicode{sikatakanahalfwidth}{FF7C}
\pdfglyphtounicode{siluqhebrew}{05BD}
\pdfglyphtounicode{siluqlefthebrew}{05BD}
\pdfglyphtounicode{similar}{223C}
\pdfglyphtounicode{sindothebrew}{05C2}
\pdfglyphtounicode{siosacirclekorean}{3274}
\pdfglyphtounicode{siosaparenkorean}{3214}
\pdfglyphtounicode{sioscieuckorean}{317E}
\pdfglyphtounicode{sioscirclekorean}{3266}
\pdfglyphtounicode{sioskiyeokkorean}{317A}
\pdfglyphtounicode{sioskorean}{3145}
\pdfglyphtounicode{siosnieunkorean}{317B}
\pdfglyphtounicode{siosparenkorean}{3206}
\pdfglyphtounicode{siospieupkorean}{317D}
\pdfglyphtounicode{siostikeutkorean}{317C}
\pdfglyphtounicode{six}{0036}
\pdfglyphtounicode{sixarabic}{0666}
\pdfglyphtounicode{sixbengali}{09EC}
\pdfglyphtounicode{sixcircle}{2465}
\pdfglyphtounicode{sixcircleinversesansserif}{278F}
\pdfglyphtounicode{sixdeva}{096C}
\pdfglyphtounicode{sixgujarati}{0AEC}
\pdfglyphtounicode{sixgurmukhi}{0A6C}
\pdfglyphtounicode{sixhackarabic}{0666}
\pdfglyphtounicode{sixhangzhou}{3026}
\pdfglyphtounicode{sixideographicparen}{3225}
\pdfglyphtounicode{sixinferior}{2086}
\pdfglyphtounicode{sixmonospace}{FF16}
\pdfglyphtounicode{sixoldstyle}{F736}
\pdfglyphtounicode{sixparen}{2479}
\pdfglyphtounicode{sixperiod}{248D}
\pdfglyphtounicode{sixpersian}{06F6}
\pdfglyphtounicode{sixroman}{2175}
\pdfglyphtounicode{sixsuperior}{2076}
\pdfglyphtounicode{sixteencircle}{246F}
\pdfglyphtounicode{sixteencurrencydenominatorbengali}{09F9}
\pdfglyphtounicode{sixteenparen}{2483}
\pdfglyphtounicode{sixteenperiod}{2497}
\pdfglyphtounicode{sixthai}{0E56}
\pdfglyphtounicode{slash}{002F}
\pdfglyphtounicode{slashmonospace}{FF0F}
\pdfglyphtounicode{slong}{017F}
\pdfglyphtounicode{slongdotaccent}{1E9B}
\pdfglyphtounicode{smileface}{263A}
\pdfglyphtounicode{smonospace}{FF53}
\pdfglyphtounicode{sofpasuqhebrew}{05C3}
\pdfglyphtounicode{softhyphen}{00AD}
\pdfglyphtounicode{softsigncyrillic}{044C}
\pdfglyphtounicode{sohiragana}{305D}
\pdfglyphtounicode{sokatakana}{30BD}
\pdfglyphtounicode{sokatakanahalfwidth}{FF7F}
\pdfglyphtounicode{soliduslongoverlaycmb}{0338}
\pdfglyphtounicode{solidusshortoverlaycmb}{0337}
\pdfglyphtounicode{sorusithai}{0E29}
\pdfglyphtounicode{sosalathai}{0E28}
\pdfglyphtounicode{sosothai}{0E0B}
\pdfglyphtounicode{sosuathai}{0E2A}
\pdfglyphtounicode{space}{0020}
\pdfglyphtounicode{spacehackarabic}{0020}
\pdfglyphtounicode{spade}{2660}
\pdfglyphtounicode{spadesuitblack}{2660}
\pdfglyphtounicode{spadesuitwhite}{2664}
\pdfglyphtounicode{sparen}{24AE}
\pdfglyphtounicode{squarebelowcmb}{033B}
\pdfglyphtounicode{squarecc}{33C4}
\pdfglyphtounicode{squarecm}{339D}
\pdfglyphtounicode{squarediagonalcrosshatchfill}{25A9}
\pdfglyphtounicode{squarehorizontalfill}{25A4}
\pdfglyphtounicode{squarekg}{338F}
\pdfglyphtounicode{squarekm}{339E}
\pdfglyphtounicode{squarekmcapital}{33CE}
\pdfglyphtounicode{squareln}{33D1}
\pdfglyphtounicode{squarelog}{33D2}
\pdfglyphtounicode{squaremg}{338E}
\pdfglyphtounicode{squaremil}{33D5}
\pdfglyphtounicode{squaremm}{339C}
\pdfglyphtounicode{squaremsquared}{33A1}
\pdfglyphtounicode{squareorthogonalcrosshatchfill}{25A6}
\pdfglyphtounicode{squareupperlefttolowerrightfill}{25A7}
\pdfglyphtounicode{squareupperrighttolowerleftfill}{25A8}
\pdfglyphtounicode{squareverticalfill}{25A5}
\pdfglyphtounicode{squarewhitewithsmallblack}{25A3}
\pdfglyphtounicode{srsquare}{33DB}
\pdfglyphtounicode{ssabengali}{09B7}
\pdfglyphtounicode{ssadeva}{0937}
\pdfglyphtounicode{ssagujarati}{0AB7}
\pdfglyphtounicode{ssangcieuckorean}{3149}
\pdfglyphtounicode{ssanghieuhkorean}{3185}
\pdfglyphtounicode{ssangieungkorean}{3180}
\pdfglyphtounicode{ssangkiyeokkorean}{3132}
\pdfglyphtounicode{ssangnieunkorean}{3165}
\pdfglyphtounicode{ssangpieupkorean}{3143}
\pdfglyphtounicode{ssangsioskorean}{3146}
\pdfglyphtounicode{ssangtikeutkorean}{3138}
\pdfglyphtounicode{ssuperior}{F6F2}
\pdfglyphtounicode{sterling}{00A3}
\pdfglyphtounicode{sterlingmonospace}{FFE1}
\pdfglyphtounicode{strokelongoverlaycmb}{0336}
\pdfglyphtounicode{strokeshortoverlaycmb}{0335}
\pdfglyphtounicode{subset}{2282}
\pdfglyphtounicode{subsetnotequal}{228A}
\pdfglyphtounicode{subsetorequal}{2286}
\pdfglyphtounicode{succeeds}{227B}
\pdfglyphtounicode{suchthat}{220B}
\pdfglyphtounicode{suhiragana}{3059}
\pdfglyphtounicode{sukatakana}{30B9}
\pdfglyphtounicode{sukatakanahalfwidth}{FF7D}
\pdfglyphtounicode{sukunarabic}{0652}
\pdfglyphtounicode{summation}{2211}
\pdfglyphtounicode{sun}{263C}
\pdfglyphtounicode{superset}{2283}
\pdfglyphtounicode{supersetnotequal}{228B}
\pdfglyphtounicode{supersetorequal}{2287}
\pdfglyphtounicode{svsquare}{33DC}
\pdfglyphtounicode{syouwaerasquare}{337C}
\pdfglyphtounicode{t}{0074}
\pdfglyphtounicode{tabengali}{09A4}
\pdfglyphtounicode{tackdown}{22A4}
\pdfglyphtounicode{tackleft}{22A3}
\pdfglyphtounicode{tadeva}{0924}
\pdfglyphtounicode{tagujarati}{0AA4}
\pdfglyphtounicode{tagurmukhi}{0A24}
\pdfglyphtounicode{taharabic}{0637}
\pdfglyphtounicode{tahfinalarabic}{FEC2}
\pdfglyphtounicode{tahinitialarabic}{FEC3}
\pdfglyphtounicode{tahiragana}{305F}
\pdfglyphtounicode{tahmedialarabic}{FEC4}
\pdfglyphtounicode{taisyouerasquare}{337D}
\pdfglyphtounicode{takatakana}{30BF}
\pdfglyphtounicode{takatakanahalfwidth}{FF80}
\pdfglyphtounicode{tatweelarabic}{0640}
\pdfglyphtounicode{tau}{03C4}
\pdfglyphtounicode{tav}{05EA}
\pdfglyphtounicode{tavdages}{FB4A}
\pdfglyphtounicode{tavdagesh}{FB4A}
\pdfglyphtounicode{tavdageshhebrew}{FB4A}
\pdfglyphtounicode{tavhebrew}{05EA}
\pdfglyphtounicode{tbar}{0167}
\pdfglyphtounicode{tbopomofo}{310A}
\pdfglyphtounicode{tcaron}{0165}
\pdfglyphtounicode{tccurl}{02A8}
\pdfglyphtounicode{tcedilla}{0163}
\pdfglyphtounicode{tcheharabic}{0686}
\pdfglyphtounicode{tchehfinalarabic}{FB7B}
\pdfglyphtounicode{tchehinitialarabic}{FB7C}
\pdfglyphtounicode{tchehmedialarabic}{FB7D}
% tchehmeeminitialarabic;FB7C FEE4
\pdfglyphtounicode{tcircle}{24E3}
\pdfglyphtounicode{tcircumflexbelow}{1E71}
\pdfglyphtounicode{tcommaaccent}{0163}
\pdfglyphtounicode{tdieresis}{1E97}
\pdfglyphtounicode{tdotaccent}{1E6B}
\pdfglyphtounicode{tdotbelow}{1E6D}
\pdfglyphtounicode{tecyrillic}{0442}
\pdfglyphtounicode{tedescendercyrillic}{04AD}
\pdfglyphtounicode{teharabic}{062A}
\pdfglyphtounicode{tehfinalarabic}{FE96}
\pdfglyphtounicode{tehhahinitialarabic}{FCA2}
\pdfglyphtounicode{tehhahisolatedarabic}{FC0C}
\pdfglyphtounicode{tehinitialarabic}{FE97}
\pdfglyphtounicode{tehiragana}{3066}
\pdfglyphtounicode{tehjeeminitialarabic}{FCA1}
\pdfglyphtounicode{tehjeemisolatedarabic}{FC0B}
\pdfglyphtounicode{tehmarbutaarabic}{0629}
\pdfglyphtounicode{tehmarbutafinalarabic}{FE94}
\pdfglyphtounicode{tehmedialarabic}{FE98}
\pdfglyphtounicode{tehmeeminitialarabic}{FCA4}
\pdfglyphtounicode{tehmeemisolatedarabic}{FC0E}
\pdfglyphtounicode{tehnoonfinalarabic}{FC73}
\pdfglyphtounicode{tekatakana}{30C6}
\pdfglyphtounicode{tekatakanahalfwidth}{FF83}
\pdfglyphtounicode{telephone}{2121}
\pdfglyphtounicode{telephoneblack}{260E}
\pdfglyphtounicode{telishagedolahebrew}{05A0}
\pdfglyphtounicode{telishaqetanahebrew}{05A9}
\pdfglyphtounicode{tencircle}{2469}
\pdfglyphtounicode{tenideographicparen}{3229}
\pdfglyphtounicode{tenparen}{247D}
\pdfglyphtounicode{tenperiod}{2491}
\pdfglyphtounicode{tenroman}{2179}
\pdfglyphtounicode{tesh}{02A7}
\pdfglyphtounicode{tet}{05D8}
\pdfglyphtounicode{tetdagesh}{FB38}
\pdfglyphtounicode{tetdageshhebrew}{FB38}
\pdfglyphtounicode{tethebrew}{05D8}
\pdfglyphtounicode{tetsecyrillic}{04B5}
\pdfglyphtounicode{tevirhebrew}{059B}
\pdfglyphtounicode{tevirlefthebrew}{059B}
\pdfglyphtounicode{thabengali}{09A5}
\pdfglyphtounicode{thadeva}{0925}
\pdfglyphtounicode{thagujarati}{0AA5}
\pdfglyphtounicode{thagurmukhi}{0A25}
\pdfglyphtounicode{thalarabic}{0630}
\pdfglyphtounicode{thalfinalarabic}{FEAC}
\pdfglyphtounicode{thanthakhatlowleftthai}{F898}
\pdfglyphtounicode{thanthakhatlowrightthai}{F897}
\pdfglyphtounicode{thanthakhatthai}{0E4C}
\pdfglyphtounicode{thanthakhatupperleftthai}{F896}
\pdfglyphtounicode{theharabic}{062B}
\pdfglyphtounicode{thehfinalarabic}{FE9A}
\pdfglyphtounicode{thehinitialarabic}{FE9B}
\pdfglyphtounicode{thehmedialarabic}{FE9C}
\pdfglyphtounicode{thereexists}{2203}
\pdfglyphtounicode{therefore}{2234}
\pdfglyphtounicode{theta}{03B8}
\pdfglyphtounicode{theta1}{03D1}
\pdfglyphtounicode{thetasymbolgreek}{03D1}
\pdfglyphtounicode{thieuthacirclekorean}{3279}
\pdfglyphtounicode{thieuthaparenkorean}{3219}
\pdfglyphtounicode{thieuthcirclekorean}{326B}
\pdfglyphtounicode{thieuthkorean}{314C}
\pdfglyphtounicode{thieuthparenkorean}{320B}
\pdfglyphtounicode{thirteencircle}{246C}
\pdfglyphtounicode{thirteenparen}{2480}
\pdfglyphtounicode{thirteenperiod}{2494}
\pdfglyphtounicode{thonangmonthothai}{0E11}
\pdfglyphtounicode{thook}{01AD}
\pdfglyphtounicode{thophuthaothai}{0E12}
\pdfglyphtounicode{thorn}{00FE}
\pdfglyphtounicode{thothahanthai}{0E17}
\pdfglyphtounicode{thothanthai}{0E10}
\pdfglyphtounicode{thothongthai}{0E18}
\pdfglyphtounicode{thothungthai}{0E16}
\pdfglyphtounicode{thousandcyrillic}{0482}
\pdfglyphtounicode{thousandsseparatorarabic}{066C}
\pdfglyphtounicode{thousandsseparatorpersian}{066C}
\pdfglyphtounicode{three}{0033}
\pdfglyphtounicode{threearabic}{0663}
\pdfglyphtounicode{threebengali}{09E9}
\pdfglyphtounicode{threecircle}{2462}
\pdfglyphtounicode{threecircleinversesansserif}{278C}
\pdfglyphtounicode{threedeva}{0969}
\pdfglyphtounicode{threeeighths}{215C}
\pdfglyphtounicode{threegujarati}{0AE9}
\pdfglyphtounicode{threegurmukhi}{0A69}
\pdfglyphtounicode{threehackarabic}{0663}
\pdfglyphtounicode{threehangzhou}{3023}
\pdfglyphtounicode{threeideographicparen}{3222}
\pdfglyphtounicode{threeinferior}{2083}
\pdfglyphtounicode{threemonospace}{FF13}
\pdfglyphtounicode{threenumeratorbengali}{09F6}
\pdfglyphtounicode{threeoldstyle}{F733}
\pdfglyphtounicode{threeparen}{2476}
\pdfglyphtounicode{threeperiod}{248A}
\pdfglyphtounicode{threepersian}{06F3}
\pdfglyphtounicode{threequarters}{00BE}
\pdfglyphtounicode{threequartersemdash}{F6DE}
\pdfglyphtounicode{threeroman}{2172}
\pdfglyphtounicode{threesuperior}{00B3}
\pdfglyphtounicode{threethai}{0E53}
\pdfglyphtounicode{thzsquare}{3394}
\pdfglyphtounicode{tihiragana}{3061}
\pdfglyphtounicode{tikatakana}{30C1}
\pdfglyphtounicode{tikatakanahalfwidth}{FF81}
\pdfglyphtounicode{tikeutacirclekorean}{3270}
\pdfglyphtounicode{tikeutaparenkorean}{3210}
\pdfglyphtounicode{tikeutcirclekorean}{3262}
\pdfglyphtounicode{tikeutkorean}{3137}
\pdfglyphtounicode{tikeutparenkorean}{3202}
\pdfglyphtounicode{tilde}{02DC}
\pdfglyphtounicode{tildebelowcmb}{0330}
\pdfglyphtounicode{tildecmb}{0303}
\pdfglyphtounicode{tildecomb}{0303}
\pdfglyphtounicode{tildedoublecmb}{0360}
\pdfglyphtounicode{tildeoperator}{223C}
\pdfglyphtounicode{tildeoverlaycmb}{0334}
\pdfglyphtounicode{tildeverticalcmb}{033E}
\pdfglyphtounicode{timescircle}{2297}
\pdfglyphtounicode{tipehahebrew}{0596}
\pdfglyphtounicode{tipehalefthebrew}{0596}
\pdfglyphtounicode{tippigurmukhi}{0A70}
\pdfglyphtounicode{titlocyrilliccmb}{0483}
\pdfglyphtounicode{tiwnarmenian}{057F}
\pdfglyphtounicode{tlinebelow}{1E6F}
\pdfglyphtounicode{tmonospace}{FF54}
\pdfglyphtounicode{toarmenian}{0569}
\pdfglyphtounicode{tohiragana}{3068}
\pdfglyphtounicode{tokatakana}{30C8}
\pdfglyphtounicode{tokatakanahalfwidth}{FF84}
\pdfglyphtounicode{tonebarextrahighmod}{02E5}
\pdfglyphtounicode{tonebarextralowmod}{02E9}
\pdfglyphtounicode{tonebarhighmod}{02E6}
\pdfglyphtounicode{tonebarlowmod}{02E8}
\pdfglyphtounicode{tonebarmidmod}{02E7}
\pdfglyphtounicode{tonefive}{01BD}
\pdfglyphtounicode{tonesix}{0185}
\pdfglyphtounicode{tonetwo}{01A8}
\pdfglyphtounicode{tonos}{0384}
\pdfglyphtounicode{tonsquare}{3327}
\pdfglyphtounicode{topatakthai}{0E0F}
\pdfglyphtounicode{tortoiseshellbracketleft}{3014}
\pdfglyphtounicode{tortoiseshellbracketleftsmall}{FE5D}
\pdfglyphtounicode{tortoiseshellbracketleftvertical}{FE39}
\pdfglyphtounicode{tortoiseshellbracketright}{3015}
\pdfglyphtounicode{tortoiseshellbracketrightsmall}{FE5E}
\pdfglyphtounicode{tortoiseshellbracketrightvertical}{FE3A}
\pdfglyphtounicode{totaothai}{0E15}
\pdfglyphtounicode{tpalatalhook}{01AB}
\pdfglyphtounicode{tparen}{24AF}
\pdfglyphtounicode{trademark}{2122}
\pdfglyphtounicode{trademarksans}{F8EA}
\pdfglyphtounicode{trademarkserif}{F6DB}
\pdfglyphtounicode{tretroflexhook}{0288}
\pdfglyphtounicode{triagdn}{25BC}
\pdfglyphtounicode{triaglf}{25C4}
\pdfglyphtounicode{triagrt}{25BA}
\pdfglyphtounicode{triagup}{25B2}
\pdfglyphtounicode{ts}{02A6}
\pdfglyphtounicode{tsadi}{05E6}
\pdfglyphtounicode{tsadidagesh}{FB46}
\pdfglyphtounicode{tsadidageshhebrew}{FB46}
\pdfglyphtounicode{tsadihebrew}{05E6}
\pdfglyphtounicode{tsecyrillic}{0446}
\pdfglyphtounicode{tsere}{05B5}
\pdfglyphtounicode{tsere12}{05B5}
\pdfglyphtounicode{tsere1e}{05B5}
\pdfglyphtounicode{tsere2b}{05B5}
\pdfglyphtounicode{tserehebrew}{05B5}
\pdfglyphtounicode{tserenarrowhebrew}{05B5}
\pdfglyphtounicode{tserequarterhebrew}{05B5}
\pdfglyphtounicode{tserewidehebrew}{05B5}
\pdfglyphtounicode{tshecyrillic}{045B}
\pdfglyphtounicode{tsuperior}{F6F3}
\pdfglyphtounicode{ttabengali}{099F}
\pdfglyphtounicode{ttadeva}{091F}
\pdfglyphtounicode{ttagujarati}{0A9F}
\pdfglyphtounicode{ttagurmukhi}{0A1F}
\pdfglyphtounicode{tteharabic}{0679}
\pdfglyphtounicode{ttehfinalarabic}{FB67}
\pdfglyphtounicode{ttehinitialarabic}{FB68}
\pdfglyphtounicode{ttehmedialarabic}{FB69}
\pdfglyphtounicode{tthabengali}{09A0}
\pdfglyphtounicode{tthadeva}{0920}
\pdfglyphtounicode{tthagujarati}{0AA0}
\pdfglyphtounicode{tthagurmukhi}{0A20}
\pdfglyphtounicode{tturned}{0287}
\pdfglyphtounicode{tuhiragana}{3064}
\pdfglyphtounicode{tukatakana}{30C4}
\pdfglyphtounicode{tukatakanahalfwidth}{FF82}
\pdfglyphtounicode{tusmallhiragana}{3063}
\pdfglyphtounicode{tusmallkatakana}{30C3}
\pdfglyphtounicode{tusmallkatakanahalfwidth}{FF6F}
\pdfglyphtounicode{twelvecircle}{246B}
\pdfglyphtounicode{twelveparen}{247F}
\pdfglyphtounicode{twelveperiod}{2493}
\pdfglyphtounicode{twelveroman}{217B}
\pdfglyphtounicode{twentycircle}{2473}
\pdfglyphtounicode{twentyhangzhou}{5344}
\pdfglyphtounicode{twentyparen}{2487}
\pdfglyphtounicode{twentyperiod}{249B}
\pdfglyphtounicode{two}{0032}
\pdfglyphtounicode{twoarabic}{0662}
\pdfglyphtounicode{twobengali}{09E8}
\pdfglyphtounicode{twocircle}{2461}
\pdfglyphtounicode{twocircleinversesansserif}{278B}
\pdfglyphtounicode{twodeva}{0968}
\pdfglyphtounicode{twodotenleader}{2025}
\pdfglyphtounicode{twodotleader}{2025}
\pdfglyphtounicode{twodotleadervertical}{FE30}
\pdfglyphtounicode{twogujarati}{0AE8}
\pdfglyphtounicode{twogurmukhi}{0A68}
\pdfglyphtounicode{twohackarabic}{0662}
\pdfglyphtounicode{twohangzhou}{3022}
\pdfglyphtounicode{twoideographicparen}{3221}
\pdfglyphtounicode{twoinferior}{2082}
\pdfglyphtounicode{twomonospace}{FF12}
\pdfglyphtounicode{twonumeratorbengali}{09F5}
\pdfglyphtounicode{twooldstyle}{F732}
\pdfglyphtounicode{twoparen}{2475}
\pdfglyphtounicode{twoperiod}{2489}
\pdfglyphtounicode{twopersian}{06F2}
\pdfglyphtounicode{tworoman}{2171}
\pdfglyphtounicode{twostroke}{01BB}
\pdfglyphtounicode{twosuperior}{00B2}
\pdfglyphtounicode{twothai}{0E52}
\pdfglyphtounicode{twothirds}{2154}
\pdfglyphtounicode{u}{0075}
\pdfglyphtounicode{uacute}{00FA}
\pdfglyphtounicode{ubar}{0289}
\pdfglyphtounicode{ubengali}{0989}
\pdfglyphtounicode{ubopomofo}{3128}
\pdfglyphtounicode{ubreve}{016D}
\pdfglyphtounicode{ucaron}{01D4}
\pdfglyphtounicode{ucircle}{24E4}
\pdfglyphtounicode{ucircumflex}{00FB}
\pdfglyphtounicode{ucircumflexbelow}{1E77}
\pdfglyphtounicode{ucyrillic}{0443}
\pdfglyphtounicode{udattadeva}{0951}
\pdfglyphtounicode{udblacute}{0171}
\pdfglyphtounicode{udblgrave}{0215}
\pdfglyphtounicode{udeva}{0909}
\pdfglyphtounicode{udieresis}{00FC}
\pdfglyphtounicode{udieresisacute}{01D8}
\pdfglyphtounicode{udieresisbelow}{1E73}
\pdfglyphtounicode{udieresiscaron}{01DA}
\pdfglyphtounicode{udieresiscyrillic}{04F1}
\pdfglyphtounicode{udieresisgrave}{01DC}
\pdfglyphtounicode{udieresismacron}{01D6}
\pdfglyphtounicode{udotbelow}{1EE5}
\pdfglyphtounicode{ugrave}{00F9}
\pdfglyphtounicode{ugujarati}{0A89}
\pdfglyphtounicode{ugurmukhi}{0A09}
\pdfglyphtounicode{uhiragana}{3046}
\pdfglyphtounicode{uhookabove}{1EE7}
\pdfglyphtounicode{uhorn}{01B0}
\pdfglyphtounicode{uhornacute}{1EE9}
\pdfglyphtounicode{uhorndotbelow}{1EF1}
\pdfglyphtounicode{uhorngrave}{1EEB}
\pdfglyphtounicode{uhornhookabove}{1EED}
\pdfglyphtounicode{uhorntilde}{1EEF}
\pdfglyphtounicode{uhungarumlaut}{0171}
\pdfglyphtounicode{uhungarumlautcyrillic}{04F3}
\pdfglyphtounicode{uinvertedbreve}{0217}
\pdfglyphtounicode{ukatakana}{30A6}
\pdfglyphtounicode{ukatakanahalfwidth}{FF73}
\pdfglyphtounicode{ukcyrillic}{0479}
\pdfglyphtounicode{ukorean}{315C}
\pdfglyphtounicode{umacron}{016B}
\pdfglyphtounicode{umacroncyrillic}{04EF}
\pdfglyphtounicode{umacrondieresis}{1E7B}
\pdfglyphtounicode{umatragurmukhi}{0A41}
\pdfglyphtounicode{umonospace}{FF55}
\pdfglyphtounicode{underscore}{005F}
\pdfglyphtounicode{underscoredbl}{2017}
\pdfglyphtounicode{underscoremonospace}{FF3F}
\pdfglyphtounicode{underscorevertical}{FE33}
\pdfglyphtounicode{underscorewavy}{FE4F}
\pdfglyphtounicode{union}{222A}
\pdfglyphtounicode{universal}{2200}
\pdfglyphtounicode{uogonek}{0173}
\pdfglyphtounicode{uparen}{24B0}
\pdfglyphtounicode{upblock}{2580}
\pdfglyphtounicode{upperdothebrew}{05C4}
\pdfglyphtounicode{upsilon}{03C5}
\pdfglyphtounicode{upsilondieresis}{03CB}
\pdfglyphtounicode{upsilondieresistonos}{03B0}
\pdfglyphtounicode{upsilonlatin}{028A}
\pdfglyphtounicode{upsilontonos}{03CD}
\pdfglyphtounicode{uptackbelowcmb}{031D}
\pdfglyphtounicode{uptackmod}{02D4}
\pdfglyphtounicode{uragurmukhi}{0A73}
\pdfglyphtounicode{uring}{016F}
\pdfglyphtounicode{ushortcyrillic}{045E}
\pdfglyphtounicode{usmallhiragana}{3045}
\pdfglyphtounicode{usmallkatakana}{30A5}
\pdfglyphtounicode{usmallkatakanahalfwidth}{FF69}
\pdfglyphtounicode{ustraightcyrillic}{04AF}
\pdfglyphtounicode{ustraightstrokecyrillic}{04B1}
\pdfglyphtounicode{utilde}{0169}
\pdfglyphtounicode{utildeacute}{1E79}
\pdfglyphtounicode{utildebelow}{1E75}
\pdfglyphtounicode{uubengali}{098A}
\pdfglyphtounicode{uudeva}{090A}
\pdfglyphtounicode{uugujarati}{0A8A}
\pdfglyphtounicode{uugurmukhi}{0A0A}
\pdfglyphtounicode{uumatragurmukhi}{0A42}
\pdfglyphtounicode{uuvowelsignbengali}{09C2}
\pdfglyphtounicode{uuvowelsigndeva}{0942}
\pdfglyphtounicode{uuvowelsigngujarati}{0AC2}
\pdfglyphtounicode{uvowelsignbengali}{09C1}
\pdfglyphtounicode{uvowelsigndeva}{0941}
\pdfglyphtounicode{uvowelsigngujarati}{0AC1}
\pdfglyphtounicode{v}{0076}
\pdfglyphtounicode{vadeva}{0935}
\pdfglyphtounicode{vagujarati}{0AB5}
\pdfglyphtounicode{vagurmukhi}{0A35}
\pdfglyphtounicode{vakatakana}{30F7}
\pdfglyphtounicode{vav}{05D5}
\pdfglyphtounicode{vavdagesh}{FB35}
\pdfglyphtounicode{vavdagesh65}{FB35}
\pdfglyphtounicode{vavdageshhebrew}{FB35}
\pdfglyphtounicode{vavhebrew}{05D5}
\pdfglyphtounicode{vavholam}{FB4B}
\pdfglyphtounicode{vavholamhebrew}{FB4B}
\pdfglyphtounicode{vavvavhebrew}{05F0}
\pdfglyphtounicode{vavyodhebrew}{05F1}
\pdfglyphtounicode{vcircle}{24E5}
\pdfglyphtounicode{vdotbelow}{1E7F}
\pdfglyphtounicode{vecyrillic}{0432}
\pdfglyphtounicode{veharabic}{06A4}
\pdfglyphtounicode{vehfinalarabic}{FB6B}
\pdfglyphtounicode{vehinitialarabic}{FB6C}
\pdfglyphtounicode{vehmedialarabic}{FB6D}
\pdfglyphtounicode{vekatakana}{30F9}
\pdfglyphtounicode{venus}{2640}
\pdfglyphtounicode{verticalbar}{007C}
\pdfglyphtounicode{verticallineabovecmb}{030D}
\pdfglyphtounicode{verticallinebelowcmb}{0329}
\pdfglyphtounicode{verticallinelowmod}{02CC}
\pdfglyphtounicode{verticallinemod}{02C8}
\pdfglyphtounicode{vewarmenian}{057E}
\pdfglyphtounicode{vhook}{028B}
\pdfglyphtounicode{vikatakana}{30F8}
\pdfglyphtounicode{viramabengali}{09CD}
\pdfglyphtounicode{viramadeva}{094D}
\pdfglyphtounicode{viramagujarati}{0ACD}
\pdfglyphtounicode{visargabengali}{0983}
\pdfglyphtounicode{visargadeva}{0903}
\pdfglyphtounicode{visargagujarati}{0A83}
\pdfglyphtounicode{vmonospace}{FF56}
\pdfglyphtounicode{voarmenian}{0578}
\pdfglyphtounicode{voicediterationhiragana}{309E}
\pdfglyphtounicode{voicediterationkatakana}{30FE}
\pdfglyphtounicode{voicedmarkkana}{309B}
\pdfglyphtounicode{voicedmarkkanahalfwidth}{FF9E}
\pdfglyphtounicode{vokatakana}{30FA}
\pdfglyphtounicode{vparen}{24B1}
\pdfglyphtounicode{vtilde}{1E7D}
\pdfglyphtounicode{vturned}{028C}
\pdfglyphtounicode{vuhiragana}{3094}
\pdfglyphtounicode{vukatakana}{30F4}
\pdfglyphtounicode{w}{0077}
\pdfglyphtounicode{wacute}{1E83}
\pdfglyphtounicode{waekorean}{3159}
\pdfglyphtounicode{wahiragana}{308F}
\pdfglyphtounicode{wakatakana}{30EF}
\pdfglyphtounicode{wakatakanahalfwidth}{FF9C}
\pdfglyphtounicode{wakorean}{3158}
\pdfglyphtounicode{wasmallhiragana}{308E}
\pdfglyphtounicode{wasmallkatakana}{30EE}
\pdfglyphtounicode{wattosquare}{3357}
\pdfglyphtounicode{wavedash}{301C}
\pdfglyphtounicode{wavyunderscorevertical}{FE34}
\pdfglyphtounicode{wawarabic}{0648}
\pdfglyphtounicode{wawfinalarabic}{FEEE}
\pdfglyphtounicode{wawhamzaabovearabic}{0624}
\pdfglyphtounicode{wawhamzaabovefinalarabic}{FE86}
\pdfglyphtounicode{wbsquare}{33DD}
\pdfglyphtounicode{wcircle}{24E6}
\pdfglyphtounicode{wcircumflex}{0175}
\pdfglyphtounicode{wdieresis}{1E85}
\pdfglyphtounicode{wdotaccent}{1E87}
\pdfglyphtounicode{wdotbelow}{1E89}
\pdfglyphtounicode{wehiragana}{3091}
\pdfglyphtounicode{weierstrass}{2118}
\pdfglyphtounicode{wekatakana}{30F1}
\pdfglyphtounicode{wekorean}{315E}
\pdfglyphtounicode{weokorean}{315D}
\pdfglyphtounicode{wgrave}{1E81}
\pdfglyphtounicode{whitebullet}{25E6}
\pdfglyphtounicode{whitecircle}{25CB}
\pdfglyphtounicode{whitecircleinverse}{25D9}
\pdfglyphtounicode{whitecornerbracketleft}{300E}
\pdfglyphtounicode{whitecornerbracketleftvertical}{FE43}
\pdfglyphtounicode{whitecornerbracketright}{300F}
\pdfglyphtounicode{whitecornerbracketrightvertical}{FE44}
\pdfglyphtounicode{whitediamond}{25C7}
\pdfglyphtounicode{whitediamondcontainingblacksmalldiamond}{25C8}
\pdfglyphtounicode{whitedownpointingsmalltriangle}{25BF}
\pdfglyphtounicode{whitedownpointingtriangle}{25BD}
\pdfglyphtounicode{whiteleftpointingsmalltriangle}{25C3}
\pdfglyphtounicode{whiteleftpointingtriangle}{25C1}
\pdfglyphtounicode{whitelenticularbracketleft}{3016}
\pdfglyphtounicode{whitelenticularbracketright}{3017}
\pdfglyphtounicode{whiterightpointingsmalltriangle}{25B9}
\pdfglyphtounicode{whiterightpointingtriangle}{25B7}
\pdfglyphtounicode{whitesmallsquare}{25AB}
\pdfglyphtounicode{whitesmilingface}{263A}
\pdfglyphtounicode{whitesquare}{25A1}
\pdfglyphtounicode{whitestar}{2606}
\pdfglyphtounicode{whitetelephone}{260F}
\pdfglyphtounicode{whitetortoiseshellbracketleft}{3018}
\pdfglyphtounicode{whitetortoiseshellbracketright}{3019}
\pdfglyphtounicode{whiteuppointingsmalltriangle}{25B5}
\pdfglyphtounicode{whiteuppointingtriangle}{25B3}
\pdfglyphtounicode{wihiragana}{3090}
\pdfglyphtounicode{wikatakana}{30F0}
\pdfglyphtounicode{wikorean}{315F}
\pdfglyphtounicode{wmonospace}{FF57}
\pdfglyphtounicode{wohiragana}{3092}
\pdfglyphtounicode{wokatakana}{30F2}
\pdfglyphtounicode{wokatakanahalfwidth}{FF66}
\pdfglyphtounicode{won}{20A9}
\pdfglyphtounicode{wonmonospace}{FFE6}
\pdfglyphtounicode{wowaenthai}{0E27}
\pdfglyphtounicode{wparen}{24B2}
\pdfglyphtounicode{wring}{1E98}
\pdfglyphtounicode{wsuperior}{02B7}
\pdfglyphtounicode{wturned}{028D}
\pdfglyphtounicode{wynn}{01BF}
\pdfglyphtounicode{x}{0078}
\pdfglyphtounicode{xabovecmb}{033D}
\pdfglyphtounicode{xbopomofo}{3112}
\pdfglyphtounicode{xcircle}{24E7}
\pdfglyphtounicode{xdieresis}{1E8D}
\pdfglyphtounicode{xdotaccent}{1E8B}
\pdfglyphtounicode{xeharmenian}{056D}
\pdfglyphtounicode{xi}{03BE}
\pdfglyphtounicode{xmonospace}{FF58}
\pdfglyphtounicode{xparen}{24B3}
\pdfglyphtounicode{xsuperior}{02E3}
\pdfglyphtounicode{y}{0079}
\pdfglyphtounicode{yaadosquare}{334E}
\pdfglyphtounicode{yabengali}{09AF}
\pdfglyphtounicode{yacute}{00FD}
\pdfglyphtounicode{yadeva}{092F}
\pdfglyphtounicode{yaekorean}{3152}
\pdfglyphtounicode{yagujarati}{0AAF}
\pdfglyphtounicode{yagurmukhi}{0A2F}
\pdfglyphtounicode{yahiragana}{3084}
\pdfglyphtounicode{yakatakana}{30E4}
\pdfglyphtounicode{yakatakanahalfwidth}{FF94}
\pdfglyphtounicode{yakorean}{3151}
\pdfglyphtounicode{yamakkanthai}{0E4E}
\pdfglyphtounicode{yasmallhiragana}{3083}
\pdfglyphtounicode{yasmallkatakana}{30E3}
\pdfglyphtounicode{yasmallkatakanahalfwidth}{FF6C}
\pdfglyphtounicode{yatcyrillic}{0463}
\pdfglyphtounicode{ycircle}{24E8}
\pdfglyphtounicode{ycircumflex}{0177}
\pdfglyphtounicode{ydieresis}{00FF}
\pdfglyphtounicode{ydotaccent}{1E8F}
\pdfglyphtounicode{ydotbelow}{1EF5}
\pdfglyphtounicode{yeharabic}{064A}
\pdfglyphtounicode{yehbarreearabic}{06D2}
\pdfglyphtounicode{yehbarreefinalarabic}{FBAF}
\pdfglyphtounicode{yehfinalarabic}{FEF2}
\pdfglyphtounicode{yehhamzaabovearabic}{0626}
\pdfglyphtounicode{yehhamzaabovefinalarabic}{FE8A}
\pdfglyphtounicode{yehhamzaaboveinitialarabic}{FE8B}
\pdfglyphtounicode{yehhamzaabovemedialarabic}{FE8C}
\pdfglyphtounicode{yehinitialarabic}{FEF3}
\pdfglyphtounicode{yehmedialarabic}{FEF4}
\pdfglyphtounicode{yehmeeminitialarabic}{FCDD}
\pdfglyphtounicode{yehmeemisolatedarabic}{FC58}
\pdfglyphtounicode{yehnoonfinalarabic}{FC94}
\pdfglyphtounicode{yehthreedotsbelowarabic}{06D1}
\pdfglyphtounicode{yekorean}{3156}
\pdfglyphtounicode{yen}{00A5}
\pdfglyphtounicode{yenmonospace}{FFE5}
\pdfglyphtounicode{yeokorean}{3155}
\pdfglyphtounicode{yeorinhieuhkorean}{3186}
\pdfglyphtounicode{yerahbenyomohebrew}{05AA}
\pdfglyphtounicode{yerahbenyomolefthebrew}{05AA}
\pdfglyphtounicode{yericyrillic}{044B}
\pdfglyphtounicode{yerudieresiscyrillic}{04F9}
\pdfglyphtounicode{yesieungkorean}{3181}
\pdfglyphtounicode{yesieungpansioskorean}{3183}
\pdfglyphtounicode{yesieungsioskorean}{3182}
\pdfglyphtounicode{yetivhebrew}{059A}
\pdfglyphtounicode{ygrave}{1EF3}
\pdfglyphtounicode{yhook}{01B4}
\pdfglyphtounicode{yhookabove}{1EF7}
\pdfglyphtounicode{yiarmenian}{0575}
\pdfglyphtounicode{yicyrillic}{0457}
\pdfglyphtounicode{yikorean}{3162}
\pdfglyphtounicode{yinyang}{262F}
\pdfglyphtounicode{yiwnarmenian}{0582}
\pdfglyphtounicode{ymonospace}{FF59}
\pdfglyphtounicode{yod}{05D9}
\pdfglyphtounicode{yoddagesh}{FB39}
\pdfglyphtounicode{yoddageshhebrew}{FB39}
\pdfglyphtounicode{yodhebrew}{05D9}
\pdfglyphtounicode{yodyodhebrew}{05F2}
\pdfglyphtounicode{yodyodpatahhebrew}{FB1F}
\pdfglyphtounicode{yohiragana}{3088}
\pdfglyphtounicode{yoikorean}{3189}
\pdfglyphtounicode{yokatakana}{30E8}
\pdfglyphtounicode{yokatakanahalfwidth}{FF96}
\pdfglyphtounicode{yokorean}{315B}
\pdfglyphtounicode{yosmallhiragana}{3087}
\pdfglyphtounicode{yosmallkatakana}{30E7}
\pdfglyphtounicode{yosmallkatakanahalfwidth}{FF6E}
\pdfglyphtounicode{yotgreek}{03F3}
\pdfglyphtounicode{yoyaekorean}{3188}
\pdfglyphtounicode{yoyakorean}{3187}
\pdfglyphtounicode{yoyakthai}{0E22}
\pdfglyphtounicode{yoyingthai}{0E0D}
\pdfglyphtounicode{yparen}{24B4}
\pdfglyphtounicode{ypogegrammeni}{037A}
\pdfglyphtounicode{ypogegrammenigreekcmb}{0345}
\pdfglyphtounicode{yr}{01A6}
\pdfglyphtounicode{yring}{1E99}
\pdfglyphtounicode{ysuperior}{02B8}
\pdfglyphtounicode{ytilde}{1EF9}
\pdfglyphtounicode{yturned}{028E}
\pdfglyphtounicode{yuhiragana}{3086}
\pdfglyphtounicode{yuikorean}{318C}
\pdfglyphtounicode{yukatakana}{30E6}
\pdfglyphtounicode{yukatakanahalfwidth}{FF95}
\pdfglyphtounicode{yukorean}{3160}
\pdfglyphtounicode{yusbigcyrillic}{046B}
\pdfglyphtounicode{yusbigiotifiedcyrillic}{046D}
\pdfglyphtounicode{yuslittlecyrillic}{0467}
\pdfglyphtounicode{yuslittleiotifiedcyrillic}{0469}
\pdfglyphtounicode{yusmallhiragana}{3085}
\pdfglyphtounicode{yusmallkatakana}{30E5}
\pdfglyphtounicode{yusmallkatakanahalfwidth}{FF6D}
\pdfglyphtounicode{yuyekorean}{318B}
\pdfglyphtounicode{yuyeokorean}{318A}
\pdfglyphtounicode{yyabengali}{09DF}
\pdfglyphtounicode{yyadeva}{095F}
\pdfglyphtounicode{z}{007A}
\pdfglyphtounicode{zaarmenian}{0566}
\pdfglyphtounicode{zacute}{017A}
\pdfglyphtounicode{zadeva}{095B}
\pdfglyphtounicode{zagurmukhi}{0A5B}
\pdfglyphtounicode{zaharabic}{0638}
\pdfglyphtounicode{zahfinalarabic}{FEC6}
\pdfglyphtounicode{zahinitialarabic}{FEC7}
\pdfglyphtounicode{zahiragana}{3056}
\pdfglyphtounicode{zahmedialarabic}{FEC8}
\pdfglyphtounicode{zainarabic}{0632}
\pdfglyphtounicode{zainfinalarabic}{FEB0}
\pdfglyphtounicode{zakatakana}{30B6}
\pdfglyphtounicode{zaqefgadolhebrew}{0595}
\pdfglyphtounicode{zaqefqatanhebrew}{0594}
\pdfglyphtounicode{zarqahebrew}{0598}
\pdfglyphtounicode{zayin}{05D6}
\pdfglyphtounicode{zayindagesh}{FB36}
\pdfglyphtounicode{zayindageshhebrew}{FB36}
\pdfglyphtounicode{zayinhebrew}{05D6}
\pdfglyphtounicode{zbopomofo}{3117}
\pdfglyphtounicode{zcaron}{017E}
\pdfglyphtounicode{zcircle}{24E9}
\pdfglyphtounicode{zcircumflex}{1E91}
\pdfglyphtounicode{zcurl}{0291}
\pdfglyphtounicode{zdot}{017C}
\pdfglyphtounicode{zdotaccent}{017C}
\pdfglyphtounicode{zdotbelow}{1E93}
\pdfglyphtounicode{zecyrillic}{0437}
\pdfglyphtounicode{zedescendercyrillic}{0499}
\pdfglyphtounicode{zedieresiscyrillic}{04DF}
\pdfglyphtounicode{zehiragana}{305C}
\pdfglyphtounicode{zekatakana}{30BC}
\pdfglyphtounicode{zero}{0030}
\pdfglyphtounicode{zeroarabic}{0660}
\pdfglyphtounicode{zerobengali}{09E6}
\pdfglyphtounicode{zerodeva}{0966}
\pdfglyphtounicode{zerogujarati}{0AE6}
\pdfglyphtounicode{zerogurmukhi}{0A66}
\pdfglyphtounicode{zerohackarabic}{0660}
\pdfglyphtounicode{zeroinferior}{2080}
\pdfglyphtounicode{zeromonospace}{FF10}
\pdfglyphtounicode{zerooldstyle}{F730}
\pdfglyphtounicode{zeropersian}{06F0}
\pdfglyphtounicode{zerosuperior}{2070}
\pdfglyphtounicode{zerothai}{0E50}
\pdfglyphtounicode{zerowidthjoiner}{FEFF}
\pdfglyphtounicode{zerowidthnonjoiner}{200C}
\pdfglyphtounicode{zerowidthspace}{200B}
\pdfglyphtounicode{zeta}{03B6}
\pdfglyphtounicode{zhbopomofo}{3113}
\pdfglyphtounicode{zhearmenian}{056A}
\pdfglyphtounicode{zhebrevecyrillic}{04C2}
\pdfglyphtounicode{zhecyrillic}{0436}
\pdfglyphtounicode{zhedescendercyrillic}{0497}
\pdfglyphtounicode{zhedieresiscyrillic}{04DD}
\pdfglyphtounicode{zihiragana}{3058}
\pdfglyphtounicode{zikatakana}{30B8}
\pdfglyphtounicode{zinorhebrew}{05AE}
\pdfglyphtounicode{zlinebelow}{1E95}
\pdfglyphtounicode{zmonospace}{FF5A}
\pdfglyphtounicode{zohiragana}{305E}
\pdfglyphtounicode{zokatakana}{30BE}
\pdfglyphtounicode{zparen}{24B5}
\pdfglyphtounicode{zretroflexhook}{0290}
\pdfglyphtounicode{zstroke}{01B6}
\pdfglyphtounicode{zuhiragana}{305A}
\pdfglyphtounicode{zukatakana}{30BA}

% entries from zapfdingbats.txt:
\pdfglyphtounicode{a100}{275E}
\pdfglyphtounicode{a101}{2761}
\pdfglyphtounicode{a102}{2762}
\pdfglyphtounicode{a103}{2763}
\pdfglyphtounicode{a104}{2764}
\pdfglyphtounicode{a105}{2710}
\pdfglyphtounicode{a106}{2765}
\pdfglyphtounicode{a107}{2766}
\pdfglyphtounicode{a108}{2767}
\pdfglyphtounicode{a109}{2660}
\pdfglyphtounicode{a10}{2721}
\pdfglyphtounicode{a110}{2665}
\pdfglyphtounicode{a111}{2666}
\pdfglyphtounicode{a112}{2663}
\pdfglyphtounicode{a117}{2709}
\pdfglyphtounicode{a118}{2708}
\pdfglyphtounicode{a119}{2707}
\pdfglyphtounicode{a11}{261B}
\pdfglyphtounicode{a120}{2460}
\pdfglyphtounicode{a121}{2461}
\pdfglyphtounicode{a122}{2462}
\pdfglyphtounicode{a123}{2463}
\pdfglyphtounicode{a124}{2464}
\pdfglyphtounicode{a125}{2465}
\pdfglyphtounicode{a126}{2466}
\pdfglyphtounicode{a127}{2467}
\pdfglyphtounicode{a128}{2468}
\pdfglyphtounicode{a129}{2469}
\pdfglyphtounicode{a12}{261E}
\pdfglyphtounicode{a130}{2776}
\pdfglyphtounicode{a131}{2777}
\pdfglyphtounicode{a132}{2778}
\pdfglyphtounicode{a133}{2779}
\pdfglyphtounicode{a134}{277A}
\pdfglyphtounicode{a135}{277B}
\pdfglyphtounicode{a136}{277C}
\pdfglyphtounicode{a137}{277D}
\pdfglyphtounicode{a138}{277E}
\pdfglyphtounicode{a139}{277F}
\pdfglyphtounicode{a13}{270C}
\pdfglyphtounicode{a140}{2780}
\pdfglyphtounicode{a141}{2781}
\pdfglyphtounicode{a142}{2782}
\pdfglyphtounicode{a143}{2783}
\pdfglyphtounicode{a144}{2784}
\pdfglyphtounicode{a145}{2785}
\pdfglyphtounicode{a146}{2786}
\pdfglyphtounicode{a147}{2787}
\pdfglyphtounicode{a148}{2788}
\pdfglyphtounicode{a149}{2789}
\pdfglyphtounicode{a14}{270D}
\pdfglyphtounicode{a150}{278A}
\pdfglyphtounicode{a151}{278B}
\pdfglyphtounicode{a152}{278C}
\pdfglyphtounicode{a153}{278D}
\pdfglyphtounicode{a154}{278E}
\pdfglyphtounicode{a155}{278F}
\pdfglyphtounicode{a156}{2790}
\pdfglyphtounicode{a157}{2791}
\pdfglyphtounicode{a158}{2792}
\pdfglyphtounicode{a159}{2793}
\pdfglyphtounicode{a15}{270E}
\pdfglyphtounicode{a160}{2794}
\pdfglyphtounicode{a161}{2192}
\pdfglyphtounicode{a162}{27A3}
\pdfglyphtounicode{a163}{2194}
\pdfglyphtounicode{a164}{2195}
\pdfglyphtounicode{a165}{2799}
\pdfglyphtounicode{a166}{279B}
\pdfglyphtounicode{a167}{279C}
\pdfglyphtounicode{a168}{279D}
\pdfglyphtounicode{a169}{279E}
\pdfglyphtounicode{a16}{270F}
\pdfglyphtounicode{a170}{279F}
\pdfglyphtounicode{a171}{27A0}
\pdfglyphtounicode{a172}{27A1}
\pdfglyphtounicode{a173}{27A2}
\pdfglyphtounicode{a174}{27A4}
\pdfglyphtounicode{a175}{27A5}
\pdfglyphtounicode{a176}{27A6}
\pdfglyphtounicode{a177}{27A7}
\pdfglyphtounicode{a178}{27A8}
\pdfglyphtounicode{a179}{27A9}
\pdfglyphtounicode{a17}{2711}
\pdfglyphtounicode{a180}{27AB}
\pdfglyphtounicode{a181}{27AD}
\pdfglyphtounicode{a182}{27AF}
\pdfglyphtounicode{a183}{27B2}
\pdfglyphtounicode{a184}{27B3}
\pdfglyphtounicode{a185}{27B5}
\pdfglyphtounicode{a186}{27B8}
\pdfglyphtounicode{a187}{27BA}
\pdfglyphtounicode{a188}{27BB}
\pdfglyphtounicode{a189}{27BC}
\pdfglyphtounicode{a18}{2712}
\pdfglyphtounicode{a190}{27BD}
\pdfglyphtounicode{a191}{27BE}
\pdfglyphtounicode{a192}{279A}
\pdfglyphtounicode{a193}{27AA}
\pdfglyphtounicode{a194}{27B6}
\pdfglyphtounicode{a195}{27B9}
\pdfglyphtounicode{a196}{2798}
\pdfglyphtounicode{a197}{27B4}
\pdfglyphtounicode{a198}{27B7}
\pdfglyphtounicode{a199}{27AC}
\pdfglyphtounicode{a19}{2713}
\pdfglyphtounicode{a1}{2701}
\pdfglyphtounicode{a200}{27AE}
\pdfglyphtounicode{a201}{27B1}
\pdfglyphtounicode{a202}{2703}
\pdfglyphtounicode{a203}{2750}
\pdfglyphtounicode{a204}{2752}
\pdfglyphtounicode{a205}{276E}
\pdfglyphtounicode{a206}{2770}
\pdfglyphtounicode{a20}{2714}
\pdfglyphtounicode{a21}{2715}
\pdfglyphtounicode{a22}{2716}
\pdfglyphtounicode{a23}{2717}
\pdfglyphtounicode{a24}{2718}
\pdfglyphtounicode{a25}{2719}
\pdfglyphtounicode{a26}{271A}
\pdfglyphtounicode{a27}{271B}
\pdfglyphtounicode{a28}{271C}
\pdfglyphtounicode{a29}{2722}
\pdfglyphtounicode{a2}{2702}
\pdfglyphtounicode{a30}{2723}
\pdfglyphtounicode{a31}{2724}
\pdfglyphtounicode{a32}{2725}
\pdfglyphtounicode{a33}{2726}
\pdfglyphtounicode{a34}{2727}
\pdfglyphtounicode{a35}{2605}
\pdfglyphtounicode{a36}{2729}
\pdfglyphtounicode{a37}{272A}
\pdfglyphtounicode{a38}{272B}
\pdfglyphtounicode{a39}{272C}
\pdfglyphtounicode{a3}{2704}
\pdfglyphtounicode{a40}{272D}
\pdfglyphtounicode{a41}{272E}
\pdfglyphtounicode{a42}{272F}
\pdfglyphtounicode{a43}{2730}
\pdfglyphtounicode{a44}{2731}
\pdfglyphtounicode{a45}{2732}
\pdfglyphtounicode{a46}{2733}
\pdfglyphtounicode{a47}{2734}
\pdfglyphtounicode{a48}{2735}
\pdfglyphtounicode{a49}{2736}
\pdfglyphtounicode{a4}{260E}
\pdfglyphtounicode{a50}{2737}
\pdfglyphtounicode{a51}{2738}
\pdfglyphtounicode{a52}{2739}
\pdfglyphtounicode{a53}{273A}
\pdfglyphtounicode{a54}{273B}
\pdfglyphtounicode{a55}{273C}
\pdfglyphtounicode{a56}{273D}
\pdfglyphtounicode{a57}{273E}
\pdfglyphtounicode{a58}{273F}
\pdfglyphtounicode{a59}{2740}
\pdfglyphtounicode{a5}{2706}
\pdfglyphtounicode{a60}{2741}
\pdfglyphtounicode{a61}{2742}
\pdfglyphtounicode{a62}{2743}
\pdfglyphtounicode{a63}{2744}
\pdfglyphtounicode{a64}{2745}
\pdfglyphtounicode{a65}{2746}
\pdfglyphtounicode{a66}{2747}
\pdfglyphtounicode{a67}{2748}
\pdfglyphtounicode{a68}{2749}
\pdfglyphtounicode{a69}{274A}
\pdfglyphtounicode{a6}{271D}
\pdfglyphtounicode{a70}{274B}
\pdfglyphtounicode{a71}{25CF}
\pdfglyphtounicode{a72}{274D}
\pdfglyphtounicode{a73}{25A0}
\pdfglyphtounicode{a74}{274F}
\pdfglyphtounicode{a75}{2751}
\pdfglyphtounicode{a76}{25B2}
\pdfglyphtounicode{a77}{25BC}
\pdfglyphtounicode{a78}{25C6}
\pdfglyphtounicode{a79}{2756}
\pdfglyphtounicode{a7}{271E}
\pdfglyphtounicode{a81}{25D7}
\pdfglyphtounicode{a82}{2758}
\pdfglyphtounicode{a83}{2759}
\pdfglyphtounicode{a84}{275A}
\pdfglyphtounicode{a85}{276F}
\pdfglyphtounicode{a86}{2771}
\pdfglyphtounicode{a87}{2772}
\pdfglyphtounicode{a88}{2773}
\pdfglyphtounicode{a89}{2768}
\pdfglyphtounicode{a8}{271F}
\pdfglyphtounicode{a90}{2769}
\pdfglyphtounicode{a91}{276C}
\pdfglyphtounicode{a92}{276D}
\pdfglyphtounicode{a93}{276A}
\pdfglyphtounicode{a94}{276B}
\pdfglyphtounicode{a95}{2774}
\pdfglyphtounicode{a96}{2775}
\pdfglyphtounicode{a97}{275B}
\pdfglyphtounicode{a98}{275C}
\pdfglyphtounicode{a99}{275D}
\pdfglyphtounicode{a9}{2720}

% entries from texglyphlist.txt:
% Delta;2206
\pdfglyphtounicode{Ifractur}{2111}
\pdfglyphtounicode{FFsmall}{D804}
\pdfglyphtounicode{FFIsmall}{D807}
\pdfglyphtounicode{FFLsmall}{D808}
\pdfglyphtounicode{FIsmall}{D805}
\pdfglyphtounicode{FLsmall}{D806}
\pdfglyphtounicode{Germandbls}{D800}
\pdfglyphtounicode{Germandblssmall}{D803}
\pdfglyphtounicode{Ng}{014A}
% Omega;2126
\pdfglyphtounicode{Rfractur}{211C}
\pdfglyphtounicode{SS}{D800}
\pdfglyphtounicode{SSsmall}{D803}
\pdfglyphtounicode{altselector}{D802}
\pdfglyphtounicode{angbracketleft}{27E8}
\pdfglyphtounicode{angbracketright}{27E9}
\pdfglyphtounicode{arrowbothv}{2195}
\pdfglyphtounicode{arrowdblbothv}{21D5}
\pdfglyphtounicode{arrowleftbothalf}{21BD}
\pdfglyphtounicode{arrowlefttophalf}{21BC}
\pdfglyphtounicode{arrownortheast}{2197}
\pdfglyphtounicode{arrownorthwest}{2196}
\pdfglyphtounicode{arrowrightbothalf}{21C1}
\pdfglyphtounicode{arrowrighttophalf}{21C0}
\pdfglyphtounicode{arrowsoutheast}{2198}
\pdfglyphtounicode{arrowsouthwest}{2199}
\pdfglyphtounicode{ascendercompwordmark}{D80A}
\pdfglyphtounicode{asteriskcentered}{2217}
\pdfglyphtounicode{bardbl}{2225}
\pdfglyphtounicode{capitalcompwordmark}{D809}
\pdfglyphtounicode{ceilingleft}{2308}
\pdfglyphtounicode{ceilingright}{2309}
\pdfglyphtounicode{circlecopyrt}{20DD}
\pdfglyphtounicode{circledivide}{2298}
\pdfglyphtounicode{circledot}{2299}
\pdfglyphtounicode{circleminus}{2296}
\pdfglyphtounicode{coproduct}{2A3F}
\pdfglyphtounicode{cwm}{200C}
\pdfglyphtounicode{dblbracketleft}{27E6}
\pdfglyphtounicode{dblbracketright}{27E7}
% diamond;2662
% diamondmath;22C4
% dotlessj;0237
% emptyset;2205
\pdfglyphtounicode{emptyslot}{D801}
\pdfglyphtounicode{epsilon1}{03F5}
\pdfglyphtounicode{equivasymptotic}{224D}
\pdfglyphtounicode{flat}{266D}
\pdfglyphtounicode{floorleft}{230A}
\pdfglyphtounicode{floorright}{230B}
\pdfglyphtounicode{follows}{227B}
\pdfglyphtounicode{followsequal}{227D}
\pdfglyphtounicode{greatermuch}{226B}
% heart;2661
\pdfglyphtounicode{interrobang}{203D}
\pdfglyphtounicode{interrobangdown}{D80B}
\pdfglyphtounicode{intersectionsq}{2293}
\pdfglyphtounicode{latticetop}{22A4}
\pdfglyphtounicode{lessmuch}{226A}
\pdfglyphtounicode{lscript}{2113}
\pdfglyphtounicode{natural}{266E}
\pdfglyphtounicode{negationslash}{0338}
\pdfglyphtounicode{ng}{014B}
\pdfglyphtounicode{owner}{220B}
\pdfglyphtounicode{pertenthousand}{2031}
% phi;03D5
% phi1;03C6
\pdfglyphtounicode{pi1}{03D6}
\pdfglyphtounicode{precedesequal}{227C}
\pdfglyphtounicode{prime}{2032}
\pdfglyphtounicode{rho1}{03F1}
\pdfglyphtounicode{ringfitted}{D80D}
\pdfglyphtounicode{sharp}{266F}
\pdfglyphtounicode{similarequal}{2243}
\pdfglyphtounicode{slurabove}{2322}
\pdfglyphtounicode{slurbelow}{2323}
\pdfglyphtounicode{star}{22C6}
\pdfglyphtounicode{subsetsqequal}{2291}
\pdfglyphtounicode{supersetsqequal}{2292}
\pdfglyphtounicode{triangle}{25B3}
\pdfglyphtounicode{triangleinv}{25BD}
\pdfglyphtounicode{triangleleft}{25B9}
\pdfglyphtounicode{triangleright}{25C3}
\pdfglyphtounicode{turnstileleft}{22A2}
\pdfglyphtounicode{turnstileright}{22A3}
\pdfglyphtounicode{twelveudash}{D80C}
\pdfglyphtounicode{unionmulti}{228E}
\pdfglyphtounicode{unionsq}{2294}
\pdfglyphtounicode{vector}{20D7}
\pdfglyphtounicode{visualspace}{2423}
\pdfglyphtounicode{wreathproduct}{2240}
\pdfglyphtounicode{Dbar}{0110}
\pdfglyphtounicode{compwordmark}{200C}
\pdfglyphtounicode{dbar}{0111}
\pdfglyphtounicode{rangedash}{2013}
\pdfglyphtounicode{hyphenchar}{002D}
\pdfglyphtounicode{punctdash}{2014}
\pdfglyphtounicode{visiblespace}{2423}

% entries from additional.tex:
\pdfglyphtounicode{ff}{0066 0066}
\pdfglyphtounicode{fi}{0066 0069}
\pdfglyphtounicode{fl}{0066 006C}
\pdfglyphtounicode{ffi}{0066 0066 0069}
\pdfglyphtounicode{ffl}{0066 0066 006C}
\pdfglyphtounicode{IJ}{0049 004A}
\pdfglyphtounicode{ij}{0069 006A}
\pdfglyphtounicode{longs}{0073}


==> Declaration/declaration.tex <==
% ******************************* Thesis Declaration ***************************

\begin{declaration}

I hereby declare that except where specific reference is made to the work of 
others, the contents of this dissertation are original and have not been 
submitted in whole or in part for consideration for any other degree or 
qualification in this, or any other university. This dissertation is my own 
work and contains nothing which is the outcome of work done in collaboration 
with others, except as specified in the text and Acknowledgements. This 
dissertation contains fewer than 65,000 words including appendices, 
bibliography, footnotes, tables and equations and has fewer than 150 figures.

% Author and date will be inserted automatically from thesis.tex \author \degreedate

\end{declaration}

==> Preamble/preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% Add spaces between paragraphs
%\setlength{\parskip}{0.5em}
% Ragged bottom avoids extra whitespaces between paragraphs
\raggedbottom
% To remove the excess top spacing for enumeration, list and description
%\usepackage{enumitem}
%\setlist[enumerate,itemize,description]{topsep=0em}

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section

\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  %\RequirePackage{helvet}

  % For use with XeLaTeX
  %  \setmainfont[
  %    Path              = ./libertine/opentype/,
  %    Extension         = .otf,
  %    UprightFont = LinLibertine_R,
  %    BoldFont = LinLibertine_RZ, % Linux Libertine O Regular Semibold
  %    ItalicFont = LinLibertine_RI,
  %    BoldItalicFont = LinLibertine_RZI, % Linux Libertine O Regular Semibold Italic
  %  ]
  %  {libertine}
  %  % load font from system font
  %  \newfontfamily\libertinesystemfont{Linux Libertine O}
\fi

% *****************************************************************************
% **************************** Custom Packages ********************************

% ************************* Algorithms and Pseudocode **************************

%\usepackage{algpseudocode}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}


% *********************************** SI Units *********************************
\usepackage{siunitx} % use this package module for SI units


% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

% Add `custombib' in the document class option to use this section
\ifuseCustomBib
   \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib

% If you would like to use biblatex for your reference management, as opposed to the default `natbibpackage` pass the option `custombib` in the document class. Comment out the previous line to make sure you don't load the natbib package. Uncomment the following lines and specify the location of references.bib file

%\RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty, natbib=true]{biblatex}
%\bibliography{References/references} %Location of references.bib only for biblatex

\fi

% changes the default name `Bibliography` -> `References'
\renewcommand{\bibname}{References}


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% *********************** Configure Draft Mode **********************************

% Uncomment to disable figures in `draft'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


% ******************************** Todo Notes **********************************
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}

==> SupplementaryMaterial.tex <==
% last updated in April 2002 by Antje Endemann
% Based on CVPR 07 and LNCS, with modifications by DAF, AZ and elle, 2008 and AA, 2010, and CC, 2011; TT, 2014

%\documentclass[runningheads]{llncs}
\usepackage{graphicx}
\usepackage{multirow}
%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{subfigure}
\usepackage{tabulary}
\usepackage{setspace}
\usepackage{array}
\usepackage{longtable}
\usepackage{makecell}

\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{ruler}
\usepackage{color}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}
\begin{document}
% \renewcommand\thelinenumber{\color[rgb]{0.2,0.5,0.8}\normalfont\sffamily\scriptsize\arabic{linenumber}\color[rgb]{0,0,0}}
% \renewcommand\makeLineNumber {\hss\thelinenumber\ \hspace{6mm} \rlap{\hskip\textwidth\ \hspace{6.5mm}\thelinenumber}}
% \linenumbers
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\pagestyle{headings}
\mainmatter
\def\ECCV14SubNumber{1941}  % Insert your submission number here

\title{Supplementary Material} % Replace with your title

\titlerunning{CVPR15 submission ID \ECCV14SubNumber}

\authorrunning{CVPR15 submission ID \ECCV14SubNumber}

\author{Anonymous CVPR submission}
\institute{Paper ID \ECCV14SubNumber}

\maketitle


\vspace{10pt}
\noindent This supplementary material includes further results which are not included in the submitted paper listed as follows. Importantly, note that the supplementary materials are not necessary to understand the submitted paper.

\begin{itemize}
\item Original test color images used in Section 4.1 \vspace{5pt}
\item Robustness comparison of GW, HM, LC, RT, and LAT for nonlinear intensity deformations (related to Section 4.1 in the submitted paper) \vspace{5pt}
\item Supplementary results for cross-spectral template matching (related to Section 4.2 in the submitted paper) \vspace{5pt}
\item Supplementary results for robust stereo matching (related to Section 4.3 in the submitted paper) \vspace{5pt}
\end{itemize}


\section{Original test color images used in Section 4 of the Submitted Paper}

Fig. 1 presents the original test color images used in Section 4 of the submitted paper.

\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_Mustang.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_PaintedFace.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_bikes.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_TwoMacaws.png}
\linebreak
\linebreak
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_Airplane.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_Baboon.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_Lena.png}
\includegraphics[width=0.24\linewidth]{Figures_Supplementary/Fig1_Peppers.png}
}
\vspace{-5pt}
\caption{The original test color images used in Section 4 of the submitted paper}
\end{figure}

\section{Robustness comparison for nonlinear intensity deformations}

Figs. 2-4 show the examples of robustness comparison for nonlinear intensity deformations with Mustang, Airplane, and Peppers, respectively. Note that, for all test images and deformations, the tendency of results are similar.

\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\subfigure[(a) ORG]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_Deform.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_Deform0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_Deform1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_Deform2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_Deform3.png}}
\subfigure[(b) GW]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_GW.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_GW0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_GW1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_GW2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_GW3.png}}
\subfigure[(c) HM]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_HM.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_HM0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_HM1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_HM2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_HM3.png}}
\subfigure[(d) LC]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_LC.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_LC0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_LC1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_LC2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_LC3.png}}
\subfigure[(e) RT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_RT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_RT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_RT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_RT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_RT3.png}}
\subfigure[(f) LAT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_AT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_AT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_AT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_AT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig4_AT3.png}}}
\vspace{-5pt}
\caption{The robustness comparison for nonlinear intensity deformations for Mustang. For each sub-figure, from left to right, figures are non-deformed image, deformed images by piecewise-linear mapping, deformed images by piecewise-quadratic mapping, deformed images by random mapping with Gaussian distribution, deformed images by random mapping with uniform distribution. The figures are best viewed in color.}
\end{figure}

\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\subfigure[(a) ORG]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig1_Airplane.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_Deform0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_Deform1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_Deform2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_Deform3.png}}
\subfigure[(b) GW]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_GW.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_GW0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_GW1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_GW2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_GW3.png}}
\subfigure[(c) HM]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_HM.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_HM0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_HM1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_HM2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_HM3.png}}
\subfigure[(d) LC]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_LC.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_LC0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_LC1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_LC2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_LC3.png}}
\subfigure[(e) RT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_RT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_RT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_RT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_RT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_RT3.png}}
\subfigure[(f) LAT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_AT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_AT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_AT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_AT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig2_AT3.png}}}
\vspace{-5pt}
\caption{The robustness comparison for nonlinear intensity deformations for Airplane. For each sub-figure, from left to right, figures are non-deformed image, deformed images by piecewise-linear mapping, deformed images by piecewise-quadratic mapping, deformed images by random mapping with Gaussian distribution, deformed images by random mapping with uniform distribution. The figures are best viewed in color.}
\end{figure}

\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\subfigure[(a) ORG]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_Deform.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_Deform0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_Deform1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_Deform2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_Deform3.png}}
\subfigure[(b) GW]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_GW.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_GW0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_GW1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_GW2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_GW3.png}}
\subfigure[(c) HM]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_HM.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_HM0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_HM1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_HM2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_HM3.png}}
\subfigure[(d) LC]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_LC.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_LC0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_LC1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_LC2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_LC3.png}}
\subfigure[(e) RT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_RT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_RT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_RT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_RT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_RT3.png}}
\subfigure[(f) LAT]{\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_AT.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_AT0.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_AT1.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_AT2.png}
\includegraphics[width=0.18\linewidth]{Figures_Supplementary/Fig3_AT3.png}}}
\vspace{-5pt}
\caption{The robustness comparison for nonlinear intensity deformations for Pepper. For each sub-figure, from left to right, figures are non-deformed image, deformed images by piecewise-linear mapping, deformed images by piecewise-quadratic mapping, deformed images by random mapping with Gaussian distribution, deformed images by random mapping with uniform distribution. The figures are best viewed in color.}
\end{figure}

\clearpage




\clearpage
\section{Supplementary results for robust stereo matching}
\vspace{-10pt}
Figs. 7-9 present supplementary results for robust stereo matching providing better understandable visualization.
\vspace{-10pt}




\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\subfigure[(a) ORG]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_ORG.png}}
\subfigure[(a) GW]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left_GW.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right_GW.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_GW.png}}
\subfigure[(a) HM]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left_HM.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right_HM.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_HM.png}}
\subfigure[(a) LC]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left_LC.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right_LC.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_LC.png}}
\subfigure[(a) RT]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left_RT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right_RT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_RT.png}}
\subfigure[(a) LAT]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Left_AT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_Cloth2_Right_AT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig10_AT.png}}

}
\vspace{-5pt}
\caption{Examples of robust stereo matching for Cloth2. For better understandable visualization (corresponding to Fig. 3(b) in the submitted paper), transformed images and disparity map are given. The figures are best viewed in color.}
\end{figure}

\begin{figure}[!h]
\renewcommand{\thesubfigure}{}
\centering{
\subfigure[(a) ORG]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_ORG.png}}
\subfigure[(a) GW]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left_GW.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right_GW.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_GW.png}}
\subfigure[(a) HM]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left_HM.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right_HM.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_HM.png}}
\subfigure[(a) LC]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left_LC.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right_LC.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_LC.png}}
\subfigure[(a) RT]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left_RT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right_RT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_RT.png}}
\subfigure[(a) LAT]{\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Left_AT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_Aloe_Right_AT.png}
\includegraphics[width=0.20\linewidth]{Figures_Supplementary/Fig8_AT.png}}

}
\vspace{-5pt}
\caption{Examples of robust stereo matching for Aloe. For better understandable visualization (corresponding to Fig. 3(c) in the submitted paper), transformed images and disparity map are given. The figures are best viewed in color.}
\end{figure}

%\setlength{\tabcolsep}{1.4pt}

\end{document}


==> abstract.tex <==
Recent advances in computer vision and artificial intelligence have been remarkable, but
techniques for estimating dense correspondences between stereo image pairs, one of the most fundamental and essential tasks for 3D computer vision, still have provided limited abilities. 
To overcome this limitation, this dissertation explores robust stereo confidence estimation tequniques. 
The main contributions of this dissertation are as follows.

First, a confidence feature augmentation is proposed to impose color spatial coherency on the confidence feature and resulting confidence map, based on the assumption that the confidence feature and resulting confidence map are smoothly varying in the spatial domain. A set of robust confidence features is extracted from each superpixel, and then those features are concatenated with pixel-level
confidence features. The features are then enhanced through
adaptive filtering in the feature domain. In addition, the resulting confidence map,
estimated using the confidence feature with a random regression forest,
is further improved through K-nearest neighbor based
aggregation scheme on both pixel- and superpixel-level. Second, we present a learning framework for
estimating the stereo confidence through deep convolutional neural networks, 
where the optimal confidence features are learned from the matching probability together with the disparity map.
The matching probability volume is first generated by refining and normalizing the matching cost volume, and the confidence is then estimated through deep networks with the matching probability and its corresponding disparity as inputs.
Highly discriminative confidence features are learned by leveraging the multi-scale disparity features.
Moreover, the proposed semi-supervised loss enables us to effectively learn the networks even with sparse ground truth disparity maps by using highly confident pixels of intermediate results for computing the image reconstruction loss. Finally, we present a method for jointly estimating disparity and its corresponding confidence from stereo image pairs through generative adversarial networks. Our networks accomplish this through an minmax optimization to learn generative cost aggregation and adversarial confidence estimation networks in an iterative and boosting fashion. Concretely, generative cost aggregation networks are learned to generate confident and un-confident samples that are indistinguished by adversarial confidence estimation networks, while adversarial confidence estimation networks are learned to distinguish confident and un-confident samples. This process is conducted in an adversarial manner to boost both disparity and confidence estimation performance. In addition, a dynamic fusion module is presented to benefit complementary information of matching cost, disparity, and color conditioned on each input in confidence estimation networks.

We believe robust confidence estimation techniques proposed in this dissertation will provide as an essential tool and can potentially benefit various computer vision and machine learning applications.

\renewcommand\thefootnote{}
\footnote{\noindent \textbf{\textit{Keywords}}: stereo confidence estimation, confidence feature, spatial consistency, superpixel-level confidence feature, feature augmentation, random forest, convolutional neural network, generative adversarial network, depth refinement} 

==> chap1.tex <==
\chapter{Introduction}
\label{chap:intro}

\section{Motivations and Contributions}
For decades, machine learning and more recently deep learning have led revolutionary progress on numerous computer vision and image processing tasks such as image recognition, image segmentation, or object detection. Especially, progress has been actively made on the 3D computer vision applications such as 3D image reconstruction, autonomous driving, or scene understanding thanks to the availablity of a large scale 3D data and machine learning algorithms. 
\begin{figure}[b]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.8\linewidth]{images/Figure_Chap1/fig1.pdf}}\\
	\vspace{-20pt}
	\caption[The limitations of stereo matching]{The limitations of stereo matching: stereo matching  remains an unsolved problem in presence of textureless regions, reflection, occlusion, and illuminated variations.}\label{chap1_img:1}
\end{figure}

For the success of those applications, depth estimation is one of the most fundamental and essential tasks. In order to achieve depth information, active depth sensors (e.g., Time-of-Flight, Microsoft Kinect) can be first used. 
Although they enable obtaining accurate depth information in indoor environments,
they perform poorly in outdoor environments due to limited sensing range and vulnerability to illumination.
On the other hand, stereo matching techniques, reconstrucing depth information by establishing dense correspondences across stereo image pairs, can acquire more reliable depth information efficiently and effectively~\cite{Scharstein2002}. However, the stereo matching remains still an unsolved problem in presence of textureless or repeated pattern regions, or occlusion~\cite{Mei2011,Humenberger2010,Egnal2002}. In the point of view of photometric deformation, radiometric variations and sensor noise degrade the performance of stereo matching accuracy~\cite{Zabih1994,Kim2003,Heo2011}.

In general, most stereo matching methods consist of the following pipelines~\cite{Scharstein2002}: 1) matching cost computation,
2) matching cost aggregation, 3) disparity regularization, and 4) post-processing. 
Concretely, the similarity between patches from left and right images is first measured with various cost measures~\cite{Hirschmuller2008,Zbontar2015}, and the matching cost volume is then constructed with those matching costs across disparity candidates. To robustly
compute the matching cost, several approaches
were proposed by using robust cost measures \cite{Min2008,Heo2011,Kim2014} or learning-based approaches \cite{Zbontar2015,Luo2016}.
Moreover, the matching costs are aggregated to
alleviate matching ambiguities by considering local neighbors \cite{Rhemann2011, Yoon2008,
	Lu2012}. Powerful regularization techniques \cite{Hirschmuller2008,
	Felzenszwalb2006} can also be applied by incorporating prior constraints into
an objective function. Those
steps help to yield reliable matching results to some extent,
but they do not fully address the inherent challenging elements of stereo matching, e.g., textureless regions, occlusion regions, or illumination variations, as exemplified in~\figref{chap1_img:1}.

To further improve the matching accuracy, the post-processing step is involved in most approaches in a manner that they first detect mismatched pixels and then filled those pixels with reliable neighboring information~\cite{Hirschmuller2008,Rhemann2011,Egnal2004,Wang2011,Spyropoulos2014}, as shown in~\figref{chap1_img:2}. Until the last few years, there have been extensive literatures in stereo confidence estimation mainly based on handcrafted confidence measures~\cite{Egnal2002,Egnal2004,Mordohai2009}. However, those handcrafted or non-learning based measures have shown limited performance of confidence estimation. To overcome this limitation, 
machine learning-based approaches~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv} have been widely proposed. Formally, a set of
confidence features extracted from stereo matching results of
the training data is used to train a confidence classifier, e.g., random decision forest~\cite{Hirschmuller2002,Haeusler2013,Spyropoulos2014}. Although those methods have shown distinct performance improvement in comparison to existing non-learning based approaches~\cite{Egnal2002,Egnal2004,Mordohai2009},
they still have relied on handcrafted confidence features for training
the confidence classifier, thus they often fail to detect mismatched
pixels under challenging conditions such as real outdoor environments~\cite{Kim2017tip,KITTIbenchmark}. 
Besides conventional handcrafted or shallow classifier-based approaches~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Hirschmuller2002}, with the recent progress of deep convolutional neural networks (CNNs), several approaches have been proposed to measure the stereo confidence through deep CNNs~\cite{Poggi2016bmvc,Seki2016,Poggi2017cvpr,Kim2017icip,Kim2018tip}, and have shown the state-of-the-art performance.
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.24\linewidth]{images/Figure_Chap1/estimated_disparity.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.24\linewidth]{images/Figure_Chap1/gt_disparity.png}}
	\subfigure[(c)]
	{\includegraphics[width=0.24\linewidth]{images/Figure_Chap1/gt_confidence.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.24\linewidth]{images/Figure_Chap1/refined_disparity.png}}\\
	\caption[Confidence estmation for robust stereo matching]{Confidence estmation for robust stereo matching: (a) estimated disparity map using stereo matching algorithms, (b) ground-truth disparity map, (c) ground-truth confidence map, and (d) refined disparity map using (a) and (c).}\label{chap1_img:2}
\end{figure}

To estimate reliable stereo confidence through machine learning approaches, 
this dissertation explores the design strategy of stereo confidence feature and learning techniques of stereo confidence estimator. 
Specifically, this dissertation aims to solve the following two aspects in stereo confidence estimation.

\begin{itemize}
\item \textbf{The design strategy of stereo confidence feature:}
Conventional confidence estimation methods simply make a decision about the confidence of each pixel independently, and such feature is still insufficient for reliable stereo confidence estimation under challenging envirments. In addition, existing deep CNN-based confidence estimation networks~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Kim2017icip,Kim2018tip} have been formulated using matching cost only~\cite{Shaked2017}, disparity only~\cite{Poggi2016bmvc,Seki2016}, or color and disparity~\cite{Fu2018,Tosi2018} as inputs, and they cannot benefit from the joint usage of tri-modal data consisting of matching cost, disparity, and color. To overcome those limitations, this dissertation first presents a new approach for obtaining confidence features that imposes color spatial context information, and then develop a novel deep architecture that simultaneoulsy uses matching cost and disparity as inputs. This dissertation finally proposes the dynamic feature fusion networks to fully exploit tri-modality data consisting of matching cost, disparity, and color spatial context in stereo confidence estimation.
\item \textbf{The learning technique of stereo confidence estimator:}
Conventional confidence estimation techniques estimate the confidence of a pre-determined initial disparity without considering an explicit module to simultaneoulsy improve the initial disparity accuracy, 
thus they provide limited performance improvement. 
Instead, those methods generally adopt the additional disparity refinement module~\cite{Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip} to refine the initial disparity using the estimated confidence. 
To solve those limitations, this dissertation first presents a method for jointly estimating disparity and its confidence from stereo image pairs through deep networks in an iterative manner to simultaneoulsy improve the qualities of disparity and its confidence. This dissertation then proposes an adversarial learning technique to learn the disparity estimation networks and confidence estimation networks in an iterative and boosting fashion. 

\end{itemize}

\section{Outline of the Dissertation}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=1.0\linewidth]{images/Figure_Chap1/fig3.pdf}}\\
	\vspace{-20pt}
	\caption[Outline of the dissertation]{Outline of the dissertation.}\label{chap1_img:3}
\end{figure}


The outline of the dissertation is illustrated in~\figref{chap1_img:3}.
In Chapter 2, we present a new approach that imposes color spatial
consistency on the confidence estimation. 
Our key observation is that the confidence features and resulting
confidence maps are smoothly varying in the spatial domain, and 
highly correlated within the local regions of an image. 
Specifically, a set of robust confidence features is
extracted from each superpixel decomposed using the Gaussian mixture model
(GMM), and then those features are concatenated with pixel-level
confidence features. The features are then enhanced through
adaptive filtering in the feature domain. In addition, the resulting confidence map
is further improved through K-nearest neighbor (K-NN) based
aggregation scheme on both pixel- and superpixel-level.

In Chapter 3, we present a deep architecture that estimates a stereo confidence. 
In contrast to existing methods based on deep CNNs that rely on only one of the
matching cost or disparity, our network
estimates the stereo confidence by using the two heterogeneous inputs
simultaneously. Specifically, the matching probability is
first computed from the matching cost with residual networks and a
pooling module in a manner that yields greater robustness. The
confidence is then estimated through a unified deep network that
combines confidence features extracted both from the matching
probability and its corresponding disparity. In addition, our
method extracts the confidence features from disparity map
by applying multiple convolutional filters. 
To learn our networks in a semi-supervised manner, we propose a novel loss function that use
confident points to compute the image reconstruction loss. 

In Chapter 4, we present a method for jointly learning generative cost aggregation networks 
and adversarial confidence estimation networks in an iterative and boosting fashion. 
Concretely, generative cost aggregation networks are learned to generate confident 
and un-confident samples that are indistinguished by adversarial confidence estimation networks, 
while adversarial confidence estimation networks are learned to distinguish confident 
and un-confident samples. This process is conducted in an adversarial manner to boost 
both disparity and confidence estimation performance. In addition, a dynamic fusion module 
is presented to benefit complementary information of matching cost, disparity, 
and color conditioned on each input in confidence estimation networks. 
%\so{The contribution and relation of each chapter is shown in~\figref{chap1_img:4}}.

Finally, in Chapter 5, we present the conclusion of the dissertation with a summary and a discussion of some perspective directions for further works.

%\begin{figure}[t!]
%	\centering
%	\renewcommand{\thesubfigure}{}
%	\subfigure[]
%	{\includegraphics[width=1.0\linewidth]{images/Figure_Chap1/fig4.pdf}}\\
%	\vspace{-20pt}
%	\caption[Contribution of each chapter]{Contribution of each chapter.}\label{chap1_img:4}
%\end{figure}

==> chap2.tex <==
\chapter{Confidence Feature Augmentation for Robust Stereo Matching}
\label{chap:chap2}

\section{Introduction}\label{chap2_sec:1}
Stereo matching has long been an important and
fundamental topic in the field of computer vision. However, the estimation of
accurate corresponding pixels between stereo image pairs remains an unsolved problem in particular in the presence of textureless
or repeated pattern regions, and occlusions
\cite{Mei2011,Humenberger2010,Egnal2002}. Furthermore, photometric
deformations, such as radiometric variations and sensor noise, pose considerably
more challenges \cite{Zabih1994,Kim2003,Heo2011}. These issues
hinder the application of stereo matching to practical systems.
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_init_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_conf_pix.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_conf_proposed.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_removing_pixel.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_removing_proposed.png}}\\
	\vspace{-5pt}
	\subfigure[(g)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_prop_2015.png}}
	\subfigure[(h)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure1/135_prop_proposed.png}}\\
	\vspace{-5pt}
	\caption[Importance of a spatial coherency in the confidence
	estimation]{Importance of a spatial coherency in the confidence
		estimation: (a) left color image, (b) an initial disparity map
		estimated using census transform and CVF. Confidence maps were
		estimated using (c) the per-pixel classifier \cite{Park2015} and (d)
		the proposed method, respectively. (e) and (f) represent disparity
		maps consisting of disparity values classified as `reliable' by thresholding using (c) and (d).
		Erroneous pixels, which are not determined as inaccurate disparity estimates using the confidence maps, are marked as `yellow'. (g) and (h) represent
		disparity maps refined using the confidence maps in (c) and (d),
		respectively. By leveraging the spatial coherency, the proposed
		method achieves a significant performance gain on both the confidence estimation and
		the disparity map refinement.}
	\label{chap2_fig1}
\end{figure}

In order to address these issues, numerous approaches
\cite{Zabih1994,Faugeras1993,Heo2011,Kim2003,Min2008,Kim2014,Zbontar2015} have been proposed
that focus primarily on developing robust matching cost measures.
The usage of these robust cost measures, however, does not fully address the
inherent problem of stereo matching. Although the application of certain popular
regularization techniques such as semi-global matching (SGM)
\cite{Hirschmuller2008} and cost volume filtering (CVF)
\cite{Rhemann2011} could facilitate the estimation of a reliable solution, they also faces similar limitations.

%To alleviate this problem, --> ambiguous
As an alternative way to alleviate these inherent problems, almost all stereo matching methods involve a post-processing step, where mismatched pixels are first detected using a confidence measure and then these
regions are filled with their neighbor information \cite{Egnal2003,Hirschmuller2008,Wang2011,Spyropoulos2014,Rhemann2011}.
Several methods
\cite{Egnal2003,Mordohai2009,Wang2011,Kong2011,Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv}
have been proposed for detecting mismatched pixels by leveraging various
confidence features. Among them, learning-based approaches
\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv}, which train a
per-pixel classifier with a set of confidence features, demonstrate
distinct strengths as compared to existing simple non-learning based
approaches (\emph{e.g.}, left-right consistency or peak ratio) \cite{Fusiello1997}.
In these learning-based approaches, the manner in which a set of informative confidence features is combined for maximizing the performance of
the classifier is critical \cite{Hirschmuller2002,Haeusler2013,Spyropoulos2014}.
In particular, Park and
Yoon \cite{Park2015} proposed a confidence measure that first extracts a subset of the most important confidence features
by using the permutation importance accuracy measure
\cite{Ulrike2012}, and then uses these confidence features as
input for training the classifier based on a random
decision forest model \cite{Breiman2001,Liaw2002}. However, their method simply
makes a decision about the confidence of each pixel independently without considering the
spatial coherency that may exist in the confidence map. Thus,
such a classifier is still insufficient for reliably
detecting mismatched pixels under challenging conditions.

In general, most stereo matching algorithms employ a spatial
smoothness assumption to produce a more accurate disparity map \cite{Scharstein2002}.
For instance, global methods \cite{Felzenszwalb2006,Felzenszwalb2011,Hirschmuller2008}
explicitly incorporate the spatial smoothness assumption
in a global manner into an energy-minimization framework.
In local methods \cite{Rhemann2011},
matching costs are locally smoothed by applying
edge-preserving filters, yielding a considerable accuracy gain.
In this regard, it is natural to assume that the
confidence maps estimated from most stereo matching methods also tend to be
spatially smooth, except for object boundary regions. This observation
provides useful cues for designing a robust confidence estimator.

In this paper, we propose a new approach for obtaining confidence measures that
imposes spatial consistency on the confidence estimation.
Our confidence estimator consists of two key ingredients: 1) confidence feature
augmentation and 2) confidence map
aggregation.
Specifically, we impose spatial coherency on the confidence estimation by
combining confidence features from both pixel- and
superpixel-level. 
%Gouveia \emph{et al.} \cite{Gouveia2015} also proposed
%a superpixel-based confidence estimation,
%but their method involves a superpixel-based disparity fitting process
%and thus loses pixel-level precision in the confidence estimation.
%In contrast, 
Our confidence feature is augmented by using the confidence
feature computed at the superpixel-level together with the pixel-level
confidence feature. Moreover, the superpixel is further decomposed by applying a
Gaussian mixture model (GMM) using the pixel-level confidence
feature to effectively deal with superpixel segmentation errors and outliers 
caused by occluded pixels within the superpixel. Furthermore, we alleviate the fluctuation of confidence features
by applying efficient high-dimensional filtering. In the testing phase, the
confidence map is refined using the confidence values of the
K-nearest neighbors (K-NN) for each pixel
(or superpixel) under the assumption that pixels with similar
confidence features are likely to have similar confidence
values. 

\figref{chap2_fig1} shows the effectiveness of the proposed confidence estimator.
\figref{chap2_fig1}(b) shows an example of a spatially smooth initial disparity map.
While the existing per-pixel confidence estimator \cite{Park2015} frequently
produces undesired results, in particular on large-textureless regions
and occlusions, as shown in \figref{chap2_fig1}(c), the proposed confidence estimator reliably estimates
mismatched pixels by leveraging spatial coherency as shown in \figref{chap2_fig1}(d).
The experimental results show that our approach consistently outperforms existing confidence measure methods on various benchmarks.

\section{Related Works}\label{chap2_sec:2}
To estimate reliable confidence maps, numerous approaches have been proposed based on various
confidence features and classifiers
\cite{Mordohai2009,Yoon2008,Hu2012,Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Poggi2016bmvc,Seki2016}.
A comparative study of confidence features was provided in
\cite{Hu2012}, where 17 individual confidence features, \emph{e.g.},
left-right difference (LRD), matching score measure (MS), and peak
ratio (PKR), were analyzed by grouping them into 5 categories and evaluating their capability to
predict the mismatched pixel in an estimated disparity map. 
In \cite{Hu2012}, it was concluded that there is no single confidence feature
that can reliably estimate the confidence map across various scenes.

To alleviate these limitations, methods have been proposed for increasing the accuracy of prediction for mismatched pixels, in which individual confidence features
are combineded.
Pfeiffer \emph{et al.} \cite{Pfeiffer2013} utilized stereo confidence cues
from three confidence metrics, peak-ratio naive (PKRN),
maximum likelihood metric (MLM), and local curve (LC) information,
and improved the accuracy of disparity maps
by propagating all the confidence values together with measured disparities in a Bayesian framework.
However, the combination of above three confidence measures
is not always effective and thus, it is difficult to apply this algorithm
for various databases.

Recently, several approaches
\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv} were proposed that attempt to train a
confidence classifier from the training data and determine the
mismatched pixels using the learned classifier. In general, these approaches
first define the confidence feature vector, which consists of a set of different confidence features,
and then train a simple classifier, \emph{e.g.}, random decision forest \cite{Breiman2001}
using the defined confidence features
and ground truth confidence values.
Haeusler \emph{et al.} \cite{Haeusler2013} combined multiple confidence features
and learned the classifier on the correctness of the output disparities.
Spyropoulos \emph{et al.} \cite{Spyropoulos2014} combined diverse confidence features into a feature vector similar to the method presented in
\cite{Haeusler2013}.
They defined confident pixels as ground control points (GCPs) and formulated an a global optimization in a Markov random field (MRF) framework.
However, the performance of those methods is still limited because of their unreliable confidence features and classifiers.
These issues can be addressed by selecting the best set of confidence features
among multiple confidence features.
Park and Yoon \cite{Park2015} utilized the regression forest framework
to select the most important set of confidence features
and then trained the regression forest classifiers again to predict the confidence of
matching pixels using the selected confidence features.
To reduce the computational complexity, Poggi and Mattoccia \cite{Poggi20163dv} employed the set of comfidence features that can be computed in O(1) computation.   
Although some of above confidence features, such as median disparity deviation
values (MDDs), use neighbor information, all these methods determine the confidence using a classifier at a pixel-level without considering a spatial context, which limits the detecting performance. More related to ours is a method of Gouveia \emph{et al.} \cite{Gouveia2015} that constructs the confidence features by combining pixel-level and superpixel-level
features.
Although it extracts meaningful confidence features from superpixels,
those confidence features are defined on a superpixel fitted disparity map, and thus they miss the precision of pixel-wise disparity map.

More recently, there has been an effort to estimate stereo confidence by leveraging deep convolutional neural networks (CNN)~\cite{Poggi2016bmvc,Seki2016,Poggi2017cvpr}, which have shown the improved ability 
in detecting unreliable pixels. 
Poggi and Mattoccia~\cite{Poggi2016bmvc} proposed a novel confidence estimation method based on a deep network using a left disparity map as an input. Similarly, Seki and Pollefeys \cite{Seki2016} proposed a deep confidence estimator using both left and right disparity maps to boost the confidence estimation performance.
Recently, Poggi and Mattoccia \cite{Poggi2017cvpr} proposed the confidence map refinement network that improves the accuracy of the measured confidence maps (using any confidence measures). Although all of those methods demonstrated improved performance compared to a handcrafted feature based confidence measures, they do not use the cost volume which offers useful information in predicting the confidence, and thus those methods might not learn an optimal confidence feature. Unlike them, the proposed method improves the confidence estimation accuracy even with handcrafted features, extracted from the cost volume, by taking into account the local context with the superpixel. Thanks to an elegant combination of superpixel-based schemes and adaptive filtering, our method outperforms the state-of-the-art approaches including both handcrafted approaches and CNN-based approaches.

\section{Proposed Method}\label{chap2_sec:3}
\subsection{Problem Formulation and Overview}\label{chap2_sec:31}
Let us define stereo image pairs $\mathbf{I}^L_i,\mathbf{I}^R_i:\mathcal{I} \to
{\mathbb R}^3$ for pixel $i = [i_\mathrm{x},i_\mathrm{y}]^T$, where
$\mathcal{I} \subset {{\mathbb N}^2}$ is a discrete image domain.
Using existing stereo matching approaches, we first compute a cost volume $C_{i,d}$ with a disparity $d\in \{1,...,d_{\textrm{max}}\}$, where $d_{\textrm{max}}$
is a maximum allowed disparity, and then estimate its associated disparity map $D_i = \textrm{argmin}_{d}
{C_{i,d}}$.
The objective of this study is to estimate a reliable confidence $Q_i \in [0,1]$, which represents the
confidence of $D_i$. Formally, it can be estimated by learning the
classifier $\mathcal{R}:\mathbf{f}_i \to Q^*_i$ with a confidence
feature $\mathbf{f}_i: \mathcal{I} \to {\mathbb R}^{N_\mathbf{f}}$ and the ground truth confidence map $Q^*_i$, estimatd by thresholding an absolute difference between estimated disparity $D_i$ and ground truth disparity $D^*_i$. The confidence feature $\mathbf{f}_i$ is
typically defined using the cost volume $C_{i,d}$ and/or its corresponding disparity
$D_i$, where ${N_\mathbf{f}}$ is the dimension of the confidence
feature. 

% comparison with guided filter
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/color.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/96_init_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/conf_pixel.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/pixel_level.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/conf_color_guided.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/color_guided.png}}\\
	\vspace{-5pt}
	\subfigure[(g)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/conf_proposed.png}}
	\subfigure[(h)]
	{\includegraphics[width=0.4\linewidth]{Figures/figure2/proposed.png}}\\
	\vspace{-5pt}
	\caption[Visual comparison of confidence maps]{Visual comparison of confidence maps: (a) left color
		image, (b) an initial disparity map. (c) represents a confidence map
		estimated using the per-pixel classifier \cite{Park2015}. (e) shows
		a confidence map refined by simply applying the guided filter
		\cite{He2010}. (g) represents our result. (d), (f), and (h)
		represent disparity maps consisting of disparity values classified as `reliable' by thresholding using (c), (e), and (g)
		respectively. Erroneous pixels, which are not determined as inaccurate disparity estimates using the confidence maps, are marked as `yellow'.
		The area under curve (AUC), which will be defined in Sec. V-A and represents that the lower is better, of (c), (e), and (g) is 0.049, 0.046, and 0.041
		respectively. The optimal AUC with a ground truth confidence map is
		0.025.}
	\label{chap2_fig2}
\end{figure}

Most existing stereo matching methods construct the cost volume by employing the spatial
smoothness constraint either globally or locally \cite{Scharstein2002}.
The global methods \cite{Hirschmuller2008} apply an explicit smoothness assumption
and find an optimal disparity by solving an MRF-based optimization problem.
The local methods \cite{Rhemann2011,Kim2014} compute the disparity within a finite support region
by aggregating the pixel-based matching cost to implicitly impose the smoothness
assumption.
In this context, the confidence map estimated from the
smoothly varying disparity map also tends to exhibit similar
attributes, as exemplified in \figref{chap2_fig1}. However, most of conventional approaches
\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv} estimate the confidence map 
by utilizing a confidence
feature vector defined on each pixel and classifying a confidence on each pixel independently.
A structured learning framework has been used to provide structured (\emph{i.e.}, spatially
smooth) outputs by taking into account input data from adjacent
pixels in the classifier \cite{Dollar2013,Tsochantaridis2004,Taskar2005}.
For instance, in \cite{Dollar2013}, a spatially coherent edge map is estimated by designing the structured
classifier that takes advantage of the structure present in
local image patches.
In our work, confidence features often contain severe, dense outliers because of an occlusion,
which poses challenges for designing a reliable structured classifier. Instead of designing a structured classifier for the confidence
estimation, in this study we aim at improving the performance of the confidence
classification even with a conventional classifier (\emph{e.g.}, random regression forest) by exploiting spatially coherent confidence features.

The design of such confidence features is, however,
a non-trivial task. One simple solution is to apply existing edge-preserving filters
(\emph{e.g.}, guided filter \cite{He2010} or bilateral filter
\cite{Tomasi1998}) for aggregating the pixel-level confidence feature (or confidence map) in a
locally adaptive manner, as in cost aggregation schemes in
stereo matching. However, this simple aggregation is not very effective because of the nonlinearity of confidence features and dense outliers
incurred by an occlusion. \figref{chap2_fig2} shows that such a simple filtering
is not effective. Although we assume that the confidence map is spatially smooth,
a conventional smoothing filter cannot improve the performance of the
confidence measure, as shown in \figref{chap2_fig2}(f). However,
the proposed method effectively removes mismatched pixels
as shown in \figref{chap2_fig2}(h).

In our approach, we first decompose a color image using an off-the-shelf superpixel
decomposition method for generating superpixel-level confidence features.
% under the
%assumption that pixels belonging to the same superpixel are
%likely to have similar confidence features and confidence values. 
To effectively address superpixel segmentation errors (due to hard
decisions on object boundaries) and dense outliers such as
occluded pixels within a superpixel, we generate a set of reliable confidence
features through GMM based clustering within each superpixel.
For training the confidence classifier, we adaptively combine the pixel-level and
superpixel-level confidence features for each pixel. Such adaptive confidence features
considerably increase the robustness of the classifier,
while retaining the pixel-level precision on the estimated confidence
map. %Experiments demonstrate that a simple random regression forest     \cite{Liaw2002} trained using our confidence features     provide a significant performance gain.
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.8\linewidth]{Figures/figure3/framework.pdf}}\\
	\vspace{-10pt}
	\caption[Framework of the proposed confidence estimation method]{Framework of the proposed confidence estimation method,
		consisting of confidence feature augmentation (CFA) and hierarchical confidence map aggregation (HCMA).
	}\label{chap2_fig3}
\end{figure}

These robust confidence features are also beneficial in the testing
phase. The estimated confidence map is further enhanced by
leveraging the correlation between the confidence features and
the confidence map. Namely, pixels with similar confidence
features are highly likely to have similar confidence values.
We thus refine the estimated confidence value through an adaptive
summation weighted by the K-NN confidence features in a hierarchical manner.
The overall framework of our approach is summarized in
\figref{chap2_fig3}.
\subsection{Confidence Feature Augmentation (CFA)}\label{chap2_sec:32}
To design a more distinctive confidence feature, we use the
confidence features computed at both pixel- and superpixel-level.
A confidence classifier is then simply trained using a random
regression forest \cite{Liaw2002}.
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/color_seg1.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/gt_seg1.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/occ_color1.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/occ_gt1.png}}
	\subfigure[(e)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/segErr_color1.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/segErr_gt1.png}}\\
	\vspace{-6pt}
	\subfigure[(g)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/superpixel_seg1.png}}
	\subfigure[(h)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/gmm_seg1.png}}\\
	\vspace{-5pt}
	\subfigure[(i)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/occ_superpixel1.png}}
	\subfigure[(j)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/occ_gmm1.png}}
	\subfigure[(k)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/segErr_superpixel1.png}}
	\subfigure[(l)]
	{\includegraphics[width=0.128\linewidth]{Figures/figure4/segErr_gmm1.png}}\\
	\vspace{-5pt}
	\subfigure[(m)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/occlusion.pdf}}
	\subfigure[(n)]
	{\includegraphics[width=0.26\linewidth]{Figures/figure4/segmentationError.pdf}}\\
	\vspace{-5pt}
	\caption[Effectiveness of the proposed confidence feature
	augmentation scheme]{Effectiveness of the proposed confidence feature
		augmentation scheme: (a) left color image, (b) ground truth
		confidence map. (c), (d), (e), and (f) show enlarged windows for (a)
		and (b) with superpixels overlaid. The superpixels marked with the
		`green' contour in (c) and (e) contain occlusion and inaccurate segmentation
		boundary, respectively.
		(g) and (h) represent confidence maps estimated using simple SLIC superpixel
		confidence features ($L=1$) and confidence features augmented using both
		SLIC superpixel and GMM clustering ($L=2$), respectively.
		(i) and (k) show regions enlarged from (g).
		(j) and (l) show regions enlarged from (h).
		(m) and (n) represent the set of 3-dim feature vectors
		computed in the superpixels with the `green' boundaries in (c) and
		(e), respectively.}\label{chap2_fig4}
\end{figure}
\subsubsection{Pixel-level Confidence Feature}
We start with the pixel-level confidence feature vector $\mathbf{f}_i$ for a pixel $i$.
We select the set of the most important confidence features from
various confidence feature candidates as in \cite{Park2015}.
From an estimated cost volume $C_{i,d}$
derived with a cost function (\emph{e.g.}, census transform \cite{Zabih1994}) and its corresponding disparity map $D_i$,
we construct a confidence feature vector $\mathbf{f}_i$ with
the ensemble of independent confidence features.
We employ confidence feature vectors used in
\cite{Park2015}, which consist of two different feature sets according to
the database. One feature set is
composed of left-right consistency (LRC), the distance to the border,
LRD, MDDs in three different scales, MLM,
and the MS, and the other feature set is
composed of MDDs in four different
scales, LRD, MLM,
PKRN, and the negative entropy measure. 
It should be noted that our framework can be incorporated
with any other confidence features.

\subsubsection{Superpixel-level Confidence Feature}
As mentioned earlier, we consider a spatial smoothness assumption for
confidence features.
To this end, we propose two stage image decomposition strategy. We
first decompose the reference image, \emph{e.g.}, $I^L$, into a
set of non-overlapping superpixels $\mathbf{S} = \{\mathcal{S}_m |
\bigcup_m \mathcal{S}_m = \mathcal{I},\,m = 1,...,M_\mathbf{S} \}$,
where $M_\mathbf{S}$ is the number of superpixels. %The superpixel then serves as a basic unit for generating spatially coherent confidence features.
In this study, we used the SLIC superpixel algorithm \cite{Achanta2012}, but any other
off-the-shelf superpixel segmentation approaches can be used. Within
each superpixel region $\mathcal{S}_m$, we generate a set of
reliable confidence features from the pixel-level confidence feature
$\mathbf{f}_i$. In order to deal with superpixel segmentation errors and
outliers caused by occluded pixels within the superpixel, we further
decompose each superpixel into $L$ sub-clusters using the GMM model
\cite{Biernacki2000}. 
The GMM is built using the expectation-maximization (EM) algorithm
\cite{Moon1996}.
Due to the lack of the class label of each pixel, we leverage an unsupervised clustering method instead of supervised methods such as support vector machine (SVM) or decision boundary estimator.
For the superpixel $\mathcal{S}_m$, input
features for clustering based on the GMM model are formed with the
pixel-level confidence feature and spatial information such that
$\mathbf{x}_i = [\mathbf{f}_i^T,i_\mathrm{x},i_\mathrm{y}]^T$ for $i\in
\mathcal{S}_m$. Note that spatial information
$(i_\mathrm{x},i_\mathrm{y})$ is used together so that spatially
adjacent confidence features are grouped.

Let us define the GMM parameter $\theta_m = \{\phi^l_m, \mu^l_m,
\Sigma^l_m | l=1,2,...,L\}$ of each superpixel ${\mathcal{S}_m}$,
where $\phi^l_m, \mu^l_m, \Sigma^l_m$ are mixture weight, mean, and variance of 
segment $m$ for each component $l$.
We also define the multinomial Gaussian distribution of $\mathbf{x}_i$
as $\mathcal{N}(\mathbf{x}_i|\mu^l_m,\Sigma^l_m)$.
In the maximization step, we define the likelihood function to $\mathbf{x}_i$ with respect to $\theta_m$ as follows:
\begin{equation}
	\mathrm{Pr}(\mathbf{x}_i|\theta_m) = \sum\nolimits_{l}{\phi^l_m \mathcal{N}(\mathbf{x}_i|\mu^l_m,\Sigma^l_m)}.
\end{equation}
Note that we set an initial cluster label using K-means clustering.


Based on the estimated parameters $\theta_m$,
we can decompose each superpixel into $L$ sub-clusters.
In the expectation step, with a sub-cluster label $z_l$,
the sub-cluster probability for each pixel $i$ within superpixel ${\mathcal{S}_m}$ can be estimated:
\begin{equation}
	\mathrm{Pr}(z_l=1|\mathbf{x}_i) = \frac{\phi^l_m \mathcal{N}(\mathbf{x}_i|\mu^l_m,\Sigma^l_m)}
	{\sum\nolimits_{k}{\phi^k_m \mathcal{N}(\mathbf{x}_i|\mu^k_m,\Sigma^k_m)}},
\end{equation}
where ${k \in \{1,2,...,M\}}$.
With $\mathrm{Pr}(z_l=1|\mathbf{x}_i)$, we determine which
sub-cluster the pixel $i\in \mathcal{S}_m $ belongs to by
computing $l_i = \mathrm{argmax}_{l}{\mathrm{Pr}(z_l=1|\mathbf{x}_i)}$.
Then, for the simplicity of notation, we re-define a set of the final superpixels $\mathbf{S}' = \{\mathcal{S}'_n | n = 1,...,N_{\mathbf{S}'} \}$ and a set of its associated
superpixel-level features $\{\mathbf{h}_n | n = 1,...,N_{\mathbf{S}'} \}$ over an entire
image, where the number of the final superpixels
$N_{\mathbf{S}'} = LM_{\mathbf{S}}$. Note that it is assumed that
the number of sub-clusters $L$ is fixed for all superpixels.
By repeating the expectation and maximization steps, we obtain the final class labels of each pixes 
	in an unsupervised manner. In our experiments, EM algorithm converges in 50 iterations.
It should be noted that in \cite{Yamaguchi2014} a further refinement scheme of the segmentation
is also proposed, where an image is decomposed into superpixels using color and current disparity map in the slanted-plane smoothing procedure. 
Unlike this, we utilize the confidence features and spatial information
to decompose each superpixel, enabling us to handle superpixels straddling visible and half-occluded regions more effectively.

When the pixel $i$ belongs to $\mathcal{S}'_n$, \emph{i.e.}, $i \in \mathcal{S}'_n$,
the augmented confidence feature $\mathbf{g}_i$ is built by concatenating
the pixel-level confidence feature $\mathbf{f}_i$ and the superpixel-level feature
$\mathbf{h}_n$ as follows:
\begin{equation}\label{chap2_equ:feature_concat}
	\mathbf{g}_i = [\mathbf{f}_i,\mathbf{h}_n]^T.
\end{equation}

Note that pixels belonging to the same superpixel have
the same superpixel-level confidence feature $\mathbf{h}_n$.
As described above, the augmented confidence feature $\mathbf{h}_n$ is more robust to outliers compared to $\mathbf{f}_i$,
but it might lose a pixel-level precision on confidence
estimation. By simultaneously leveraging the pixel-level confidence feature
and superpixel-level confidence feature,
we are capable of encoding the distinctive confidence feature with both pixel- and superpixel-level
constraints. %Even though we use same confidence feature $\mu_n$ within superpixel region, the pixel-varying confidence features used together still
The proposed confidence feature preserves the pixel-level precision on the confidence estimation while maintaining the robustness to
outliers. 
%Interestingly, a superpixel-based approach has been developed in the stereo matching \cite{Yang2009}
%such that disparity fitting results within color segments are
%additionally used for defining an objective function for global optimization, demonstrating highly accurate disparity
%estimation performance.

To further alleviate the fluctuation of the augmented confidence feature $\mathbf{g}_i$,
we filter it out, where the filter kernel is based on
weights defined from confidence feature itself.
Here, we apply an adaptive manifold filter
to efficiently perform high-dimensional filtering
\cite{Gastal2012} such that
\begin{equation}
	\widetilde{\mathbf{g}}_i = \sum\nolimits_{j \in \mathcal{N}_i} w_{i,j}(\mathbf{g}) \mathbf{g}_j,
\end{equation}
where $w_{i,j}(\mathbf{g})$ is the weight function representing the confidence feature similarity,
defined such that
\begin{equation}
	w_{i,j}(\mathbf{g}) = \frac{\mathrm{exp}(-{{\|\mathbf{g}_i-\mathbf{g}_j\|^2}/{\sigma_g}})}{\sum\nolimits_{{k \in \mathcal{N}_i}}
		{\mathrm{exp}(-{{\|\mathbf{g}_i-\mathbf{g}_k\|^2}/{\sigma_g}})}},
\end{equation}
where $\sigma_g$ is the standard deviation of the Gaussian function in feature domain, and the size of local window $\mathcal{N}_i$ is adaptively defined by $\sigma_s$, which is the standard deviation of the Gaussian function in spatial domain, as in \cite{Gastal2012}.
Note that we define the weight $w_{i,j}(\mathbf{g})$ using only confidence feature
without considering spatial distances, since we use the confidence features
within the local window.

In \figref{chap2_fig4}, we demonstrate the effectiveness of the proposed confidence feature augmentation scheme. Two cases that may frequently occur in the superpixels are considered: occlusion, as shown in \figref{chap2_fig4}(c), and segmentation errors, as shown in \figref{chap2_fig4}(e). 
Simply generating superpixel
confidence features within these superpixels, \emph{i.e.}, $L=1$, may lead
to undesired artifacts in the confidence estimation as shown in \figref{chap2_fig4}(g).
Such artifacts were successfully removed in the confidence
map of \figref{chap2_fig4}(h), estimated using augmented confidence features by using both
the SLIC superpixel and GMM clustering ($L=2$). We analyzed this in more depth using
pixel-level confidence features within SLIC superpixels. For the
purpose of visualization, we first apply the principal component
analysis (PCA) \cite{Jolliffe2002} to $\mathbf{x}_i = [\mathbf{f}_i^T,i_\mathrm{x},i_\mathrm{y}]^T$ for
$i\in \mathcal{S}_m$, which is a 10-dimensional feature vector, and then visualize them with three dominant PCA coefficients only. We can clearly see that the pixel-level
confidence features are separated into two distinct classes through
the GMM clustering. This validates the effectiveness of our approach that
re-decomposes the SLIC superpixels through the GMM clustering using the
set of pixel-level confidence features. We found setting
$L=2$ yields the best performance in the confidence estimation.
More detailed analysis will be given in experiments. %Interestingly, when $L=2$, the set of pixel-level confidence features within each SLIC superpixel were classified into two cases of reliable and unreliable confidence features.

\subsubsection{Confidence Classifier Learning}
Finally, using the robust augmented confidence feature $\widetilde{\mathbf{g}}_i$ and
ground truth confidence map $Q^*_i$, we train the random regression forest $\mathcal{R}$
satisfying
\begin{equation}
	\mathcal{R} : \widetilde{\mathbf{g}}_i \to Q^*_i.
\end{equation}

In experiments, we will show that the proposed confidence feature
outperforms existing approaches.
%This provides more robust regression performance compared to existing approaches \cite{Park2015} defined between $f_i$ and $Q^*_i$.

\subsection{Hierarchical Confidence Map Aggregation (HCMA)}\label{chap2_sec:33}
In order to further improve the quality of the confidence
map, we utilize the proposed confidence feature once again in the testing phase by exploiting a hierarchical confidence map aggregation scheme at both pixel- and
superpixel-level. As in confidence feature generation described in
\secref{chap2_sec:32}, we leverage the correlation between the
confidence features and confidence values.

In a symmetric viewpoint of the confidence feature augmentation,
we propose an aggregation scheme on an estimated confidence map $Q_i$ that reuses the
weight of $\widetilde{\mathbf{g}}_i$ at both the pixel- and
superpixel-level. We first define the
superpixel-level confidence feature $\widetilde{\mathbf{g}}_n$ and confidence value $Q_n$
by averaging within each superpixel $\mathcal{S}'_n$ such that $\widetilde{\mathbf{g}}_n = \sum\nolimits_{i \in \mathcal{S}'_n} \widetilde{\mathbf{g}}_i/|\mathcal{S}'_n|$ and $Q_n = \sum\nolimits_{i \in \mathcal{S}'_n} Q_i/|\mathcal{S}'_n|$,
where $|\mathcal{S}'_n|$ is the number of pixels within $\mathcal{S}'_n$.
In order to apply hierarchical aggregation,
we first define augmented confidence feature set $\mathbf{g}^\mathrm{A}$ and augmented confidence value set $Q^\mathrm{A}$ as follows:
\begin{equation}
	\mathbf{g}^\mathrm{A}=\{\widetilde{\mathbf{g}}_i \cup \widetilde{\mathbf{g}}_n|i\in \mathcal{I},n\in 1,...,N_{\mathbf{S}'}\},
\end{equation}
\begin{equation}
	Q^\mathrm{A}=\{Q_i \cup Q_n|i\in \mathcal{I},n\in 1,...,N_{\mathbf{S}'}\}.
\end{equation}

The confidence value is filtered by averaging the confidence values of K-nearest neighbor (K-NN) in 16-dimensional feature space for all pixels and superpixels estimated using the K-nearest neighbor search \cite{Wald2006} with the Euclidean distance:
\begin{equation}
	\widetilde{Q}^\mathrm{A}_u = \sum\nolimits_{v \in \mathcal{N}_u} Q^\mathrm{A}_v/K,
\end{equation}
where $u$ represents an index for all pixels and superpixels within an image, and
$\mathcal{N}_u$ represents K-NN for $u$.
%After the filtering procedure, aggregated confidence values for pixel- and superpixel-level are obtained
%by de-augmenting $\widetilde{Q}^\mathrm{A}_u$ as $\{\widetilde{Q}_i,\widetilde{Q}_n\}$.


Our final confidence value $\widehat{Q}_i$ for each pixel $i$ is then
the weighted sum of $\widetilde{Q}_i$ and $\widetilde{Q}_n$ as follows:
\begin{equation}
	\widehat{Q}_i = \alpha \widetilde{Q}_i + (1-\alpha) \widetilde{Q}_n, \quad i \in \mathcal{S}'_n,
\end{equation}
where $\alpha$ is the weight parameter between the pixel-level confidence value and superpixel-level
confidence value. Algorithm 1 summarizes the proposed confidence measure,
consisting of confidence feature augmentation (CFA) and hierarchical confidence map aggregation (HCMA).

% algorithm pseudo code
\begin{table}[t!]
	\begin{center}
		\begin{tabularx}{1\linewidth}{p{1mm} p{0.5mm}| p{80mm}}
			\hlinewd{0.8pt}
			\multicolumn{3}{ p{165mm} }{{\bf Algorithm 1}:
				Feature Augmentation for Learning Confidence Measure}\\
			\hline
			\multicolumn{3}{ p{165mm} }{{\bf Input}: training set $\mathcal{C}_{\mathrm{train}} = \{\mathbf{I}^L_i,\mathbf{I}^R_i,D^*_i\}$, testing pairs $\{\mathbf{I}^L_i,\mathbf{I}^R_i\}$} \\
			\multicolumn{3}{ p{165mm} }{{\bf Output}: confidence map $\widehat{Q}_i$, disparity map $\widehat{D}_i$}\\
			\\
			~&\multicolumn{2}{ p{165mm} }{{\bf $/*$ Training Procedure $*/$}}\\
			$\mathbf{1:}$&\multicolumn{2}{ p{165mm} }{Construct cost volume $C_{i,d}$ and disparity map $D_{i}$ for $\mathcal{C}_{\mathrm{train}}$.}\\
			$\mathbf{2:}$&\multicolumn{2}{ p{165mm} }{Calculate ground truth confidence map $Q^*_i$ by thresholding \par the absolute difference between $D_i$ and $D^*_i$.}\\
			$\mathbf{3:}$&\multicolumn{2}{ p{165mm} }{Construct the augmented confidence feature $\mathbf{g}_i$ by pixel-level confidence feature $\mathbf{f}_i$ and \par superpixel-level confidence feature $\mathbf{h}_n$.}\\
			$\mathbf{4:}$&\multicolumn{2}{ p{165mm} }{Filter out the confidence feature $\mathbf{g}_i$ to generate $\widetilde{\mathbf{g}}_i$ in Eq. (4).}\\
			$\mathbf{5:}$&\multicolumn{2}{ p{165mm} }{Train the random regression forest $\mathcal{R}$ using $\widetilde{\mathbf{g}}_i$ and $Q^*_i$ in Eq. (6).}\\
			\\
			~&\multicolumn{2}{ p{165mm} }{{\bf $/*$ Testing Procedure $*/$}}\\
			$\mathbf{6:}$&\multicolumn{2}{ p{165mm} }{Estimate $Q_i$ using confidence features $\widetilde{\mathbf{g}}_i$ and $Q^*_i$ for testing stereo pairs $\{\mathbf{I}^L_i,\mathbf{I}^R_i\}$ through \par step $\mathbf{1}$-$\mathbf{5}$.}\\
			$\mathbf{7:}$&\multicolumn{2}{ p{165mm} }{Compute $\widetilde{Q}_i$ and $\widetilde{Q}_n$
				using hierarchical confidence map aggregation on $Q_i$ and $Q_n$ in Eq. (9).}\\
			$\mathbf{8:}$&\multicolumn{2}{ p{165mm} }{Compute $\widehat{Q}_i$ with the weighted sum of $\widetilde{Q}_i$ and $\widetilde{Q}_n$ in Eq. (10).}\\
			$\mathbf{9:}$&\multicolumn{2}{ p{165mm} }{Compute refined disparity map $\widehat{D}_i$ using cost modulation based \par optimization or GCPs-based optimization.}\\
			\hlinewd{0.8pt}
		\end{tabularx}
	\end{center}
\end{table}

\section{Validation}\label{chap2_sec:4}
So far, we have explained the method for obtaining a reliable confidence measure from the estimated initial disparity map. In this section, we describe the validation of 
the effectiveness of our confidence measure, for which we incorporate
the estimated confidence values into optimization schemes, by
using 1) cost modulation based optimization as in \cite{Park2015} and 2) GCPs-based
global optimization as in \cite{Pfeiffer2013,Spyropoulos2014}.

\subsection{Cost Modulation Based Optimization}\label{chap2_sec:41}
Borrowed from \cite{Park2015}, we incorporate the predicted confidence
value into stereo matching by modulating the initial matching costs.
When $C_{i,d}$ denotes the matching cost of pixel $i$ for a
disparity $d$, it is first modulated using $\widehat{Q}_i$ such that
\begin{equation}
	\widehat{C}_{i,d} = \widehat{Q}_i C_{i,d} + (1-\widehat{Q}_i)\sum\nolimits_{d}{C_{i,d}/d_{\textrm{max}}}.
\end{equation}

After modulating the initial cost volumes, the matching costs of confident
pixels remain unchanged and unreliable pixels are flattened.
Therefore, unreliable pixels can be easily dominated by more
confident neighboring pixels in the optimization step.
To produce a final disparity map $\widehat{D}_i$, the modulated cost function $\widehat{C}_{i,d}$ is then
optimized using a global approaches such as SGM \cite{Hirschmuller2008} or belief propagation \cite{Sun2003}.

\begin{table}[t!]
	\caption{Experimental configuration.}
	\begin{center}
		\begin{tabular}{>{\raggedright}m{0.25\linewidth}|
				>{\centering}m{0.14\linewidth} >{\centering}m{0.14\linewidth}|
				>{\centering}m{0.16\linewidth} >{\centering}m{0.14\linewidth}}
			\hlinewd{0.8pt}
			Dataset & MID \cite{Middlebury} & MPI \cite{MPI}  & KITTI \cite{KITTIbenchmark} & ZED  \tabularnewline
			\hline
			\hline
			Confidence Feature & \multicolumn{2}{c|}{Feature Selection 1} & \multicolumn{2}{c}{Feature Selection 2}    \tabularnewline
			\hline
			Training Set & \multicolumn{2}{c|}{MID 2005} & \multicolumn{2}{c}{KITTI 2012 (8 frame)} \tabularnewline
			\hline
			\multirow{2}{*}{Testing  Set} & MID 2006& MPI & KITTI 2015 & \multirow{2}{*}{ZED stereo}  \tabularnewline
			& 21 images & 22 frames & 200 frames &  \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap2_tab1}
\end{table}

% M table
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure5/var_superpixel2.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure5/var_M.pdf}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure5/var_K.pdf}}
	\subfigure[(d)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure5/var_alpha.pdf}}\\
	\vspace{-5pt}
	\caption[Average AUC of proposed confidence measure for MID, MPI, and KITTI dataset]{Average AUC of proposed confidence measure on MID \cite{Middlebury}, MPI \cite{MPI}, and KITTI \cite{KITTIdataset} benchmark,
		as varying (a) the number of superpixels, (b) the number of sub-clusters $M$, (c) the number of K-NN nearest neighborhoods $K$, (d) the pixel-level weight $\alpha$. Note that ZED benchmark \cite{ZED} is not analyzed since it does not have ground truth disparity map.}\label{chap2_fig5}
\end{figure}
% training frame
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure6/MID.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.3\linewidth]{Figures/figure6/KITTI.pdf}}\\
	\vspace{-5pt}
	\caption[AUC values of census-based SGM for MID, MPI, and KITTI dataset]{AUC values of census-based SGM for (a) MID \cite{Middlebury} and MPI \cite{MPI} dataset and (b) KITTI dataset \cite{KITTIdataset} according to the number of training stereo image pairs. `8*' represents the selected frames as described in Sec. V-A.}
	\label{chap2_fig6}
\end{figure}

\subsection{GCPs-Based Optimization}
Our confidence measure can also be incorporated in GCPs-based
optimization. We first set pixels that have a higher value than a threshold $\delta$
as the GCPs and then globally optimize the initial
GCPs through an MRF-based propagation.
As mentioned in \cite{Spyropoulos2014},
there is a trade-off between density and accuracy. Namely, with a low threshold,
the density of GCPs becomes high but the true negative (TN) accuracy is degraded and vice versa.
To prevent disparity errors from being propagated in the optimization,
we focus on increasing the TN accuracy by using a relatively high threshold,
although this degrades the true positive (TP) accuracy.
With the set of GCPs, we define the energy function as in \cite{Xu2013}
to obtain the final disparity map as follows:
\begin{equation}\label{chap2_eq7}
	E(\widehat{\mathbf{D}}) = (\widehat{\mathbf{D}}-\mathbf{W}\mathbf{D})^T(\widehat{\mathbf{D}}-\mathbf{WD})+\lambda \widehat{\mathbf{D}}^T\mathbf{L}\widehat{\mathbf{D}},
\end{equation}
where $\mathbf{D}$ and $\widehat{\mathbf{D}}$ is the vector form of the estimated initial disparity map $D_i$ and output disparity map $\widehat{D}_i$, respectively.
The weight matrix $\mathbf{W}$ is composed with the component $\mathbf{W}_{i,j}$ between pixel $i$ and $j$ is defined as
\begin{equation}\label{chap2_eq7}
	\mathbf{W}_{i,j} = \frac{m_i k_{i,j} \mathrm{exp}(-\|D_i-D_j\|^2/\sigma_D)}
	{\sum\nolimits_{j \in \mathcal{N}^4_i} m_i k_{i,j} \mathrm{exp}(-\|D_i-D_j\|^2/\sigma_D)},
\end{equation}
where $m_i$ is a binary mask to mark the position of GCPs, \emph{i.e.}, it is set to 1 for GCPs and 0 otherwise,
and $k_{i,j}$ is the affinity between the pixel $i$ and $j$ in the feature space of
color intensity and spatial location such that $k_{i,j} = \mathrm{exp}(-\|\mathbf{p}_i-\mathbf{p}_j\|^2/\sigma_p)$. $\mathbf{p}_i = [\mathbf{I}^T_i,i_\mathrm{x},i_\mathrm{y}]^T$ is a feature composed of
color intensity and spatial location with the standard deviation $\sigma_p$. $\sigma_D$ is the standard deviation of the Gaussian function, and
$\mathcal{N}^4_i$ represents a local 4-neighborhood. $\mathbf{L}$ is the sparse Laplacian for regularization
where each element $\mathbf{L}_{i,j} = -k_{i,j}$ for $i \neq j$ and
$\mathbf{L}_{i,i} = \sum\nolimits_{j \in \mathcal{N}^4_i}k_{i,j}$.
With this simple quadratic optimization scheme, we obtain a highly reliable disparity map.

% AUC table
\begin{sidewaystable}[t!]
	\caption[The average AUC values for MID, MPI, and KITTI dataset]{The average AUC values for MID \cite{Middlebury}, MPI \cite{MPI}, and KITTI \cite{KITTIdataset} dataset. The AUC value of ground truth confidence is measured as `optimal'. The result with the lowest AUC value in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.25\linewidth} | 
				>{\centering}m{0.08\linewidth}  >{\centering}m{0.08\linewidth} |
				>{\centering}m{0.08\linewidth}  >{\centering}m{0.08\linewidth} |
				>{\centering}m{0.08\linewidth}  >{\centering}m{0.08\linewidth} |
				>{\centering}m{0.1\linewidth}  }
			\hlinewd{0.8pt}
			\multirow{2}{*}{Methods}
			& \multicolumn{2}{ c |}{MID \cite{Middlebury}} & \multicolumn{2}{ c | }{MPI \cite{MPI}}
			& \multicolumn{3}{ c }{KITTI \cite{KITTIdataset}} \tabularnewline
			\cline{2-8}
			& \multicolumn{2}{ c |}{Census}
			& \multicolumn{2}{ c | }{Census}
			& \multicolumn{2}{ c |}{Census} & MC-CNN \tabularnewline
			&w/SGM &w/CVF &w/SGM &w/CVF &w/SGM &w/CVF &w/CBCA \tabularnewline
			\hline
			\hline
			$\;$Haeusler \emph{et al.} \cite{Haeusler2013}           &0.0530 &0.0512 &0.0532 &0.0499 &0.0556 &0.0460 &0.0124 \tabularnewline
			$\;$Spyropoulos \emph{et al.} \cite{Spyropoulos2014}     &0.0485 &0.0468 &0.0482 &0.0454 &0.0503 &0.0421 &0.0124 \tabularnewline
			$\;$Park \emph{et al.} \cite{Park2015}  (FS1)           &0.0456 &0.0439 &0.0450 &0.0424 &0.0471 &0.0356 &0.0112 \tabularnewline
			$\;$Park \emph{et al.} \cite{Park2015} (FS2)             &0.0461 &0.0445 &0.0455 &0.0431 &0.0469 &0.0348 &0.0115 \tabularnewline
			$\;$Poggi \emph{et al.} (O(1)) \cite{Poggi20163dv}            					 &0.0442 &0.0429 &0.0441 &0.0420 &0.0453 &0.0301 &0.0116 \tabularnewline
			$\;$Gouveia \emph{et al.} \cite{Gouveia2015}             &0.0706 &0.0684 &0.0700 &0.0672 &0.0748 &0.0451 &- \tabularnewline
			$\;$Poggi \emph{et al.} \cite{Poggi2016bmvc}               &0.0435 &0.0403 &0.0423 &0.0411 &0.0437 &0.0288 &0.0113 \tabularnewline
			$\;$Seki \emph{et al.} \cite{Seki2016}                &0.0431 &0.0398 &0.0418 &0.0386 &0.0428 &0.0288 &0.0111 \tabularnewline
			\hline
			$\;$CFA (Ours) (FS1)                            	   &0.0416 &0.0399 &0.0409 &0.0387 &0.0451 &0.0293 &0.0100 \tabularnewline
			$\;$HCMA (Ours)    (FS1)                               &0.0433 &0.0416 &0.0427 &0.0402 &0.0463 &0.0311 &0.0104 \tabularnewline
			$\;$CFA+HCMA (Ours)    (FS1)                           &\textbf{0.0403} &\textbf{0.0386} &\textbf{0.0396} &\textbf{0.0374} &0.0435 &0.0274 &0.0098 \tabularnewline
			\hline  
			$\;$CFA (Ours)     (FS2)                               &0.0423 &0.0406 &0.0420 &0.0396 &0.0429 &0.0288 &0.0097 \tabularnewline
			$\;$HCMA (Ours)       (FS2)                            &0.0447 &0.0417 &0.0432 &0.0408 &0.0446 &0.0302 &0.0100 \tabularnewline
			$\;$CFA+HCMA (Ours)   (FS2)                            &0.0412 &0.0395 &0.0411 &0.0384 &\textbf{0.0414} &\textbf{0.0269} &\textbf{0.0096} \tabularnewline
			\hline        
			$\;$Optimal                                       &0.0340 &0.0322 &0.0335 &0.0312 &0.0348 &0.0166 &0.0038 \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap2_tab2}
\end{sidewaystable}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/MID6.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/MID11.pdf}}
	\subfigure[(c)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/MID12.pdf}}\\
	\vspace{-5pt}
	\subfigure[(d)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/KITTI24.pdf}}
	\subfigure[(e)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/KITTI96.pdf}}
	\subfigure[(f)]
	{\includegraphics[width=0.32\linewidth]{Figures/figure7/KITTI154.pdf}}\\
	\vspace{-5pt}
	\caption[Sparsification curve for MID and KITTI dataset]{Sparsification curve for (a) Bowling2, (b) Flowerpots, and (c) Lampshade1 are selected images from MID \cite{Middlebury}, (d) frame 24, (e) frame 96, and (f) frame 154 are selected images from KITTI  dataset \cite{KITTIdataset}. The sparsification curve for a ground truth confidence map is described as `optimal'.}\label{chap2_fig7}
\end{figure}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.45\linewidth]{Figures/figure8/KITTI_SGM.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.45\linewidth]{Figures/figure8/KITTI_CVF.pdf}}\\	
	\vspace{-5pt}
	\caption[AUC values for KITTI dataset]{AUC values of (a) census-based SGM and (b) census-based CVF for KITTI dataset \cite{KITTIdataset}. We sort the AUC values in the ascending order according to proposed AUC values. The `optimal' AUC values are calculated using ground truth confidence map.}
	\label{chap2_fig8}
\end{figure}

\section{Experimental Results}\label{chap2_sec:5}
\subsection{Experimental Settings}\label{chap2_sec:50}
In this section, we evaluated the proposed method compared to conventional learning-based approaches such as Haeusler \emph{et al.} \cite{Haeusler2013}, Spyropoulos \emph{et al.} \cite{Spyropoulos2014}, Park \emph{et al.} \cite{Park2015}, Poggi \emph{et al.} (O(1)) \cite{Poggi20163dv}, and Gouveia \emph{et al.} \cite{Gouveia2015}, and CNN-based approaches such as Poggi \emph{et al.} \cite{Poggi2016bmvc} and Seki \emph{et al.} \cite{Seki2016} on
various datasets: Middlebury 2006 (MID) \cite{Middlebury}, MPI-Sintel (MPI) \cite{MPI}, KITTI 2015 (KITTI) \cite{KITTIdataset}, and ZED. 
We obtained the results of \cite{Park2015} and \cite{Gouveia2015} by using the author-provided MATLAB code,
while the results of \cite{Haeusler2013}, \cite{Spyropoulos2014}, and \cite{Seki2016}
were obtained using our own MATLAB implementation. For \cite{Poggi20163dv} and \cite{Poggi2016bmvc}, we re-impelemented the algorithms based on author's lua code. 
Note that for \cite{Poggi2016bmvc} we used the same training sets as ours for a fair comparison, unlike the training condition from the original paper \cite{Poggi2016bmvc}.
The proposed method was implemented in MATLAB and was simulated on a PC with Quad-core CPU 4.00GHz.
We also present an anlaysis of the
performance gain resulting from the two key components of our method (CFA and
HCMA). To compute a raw matching cost, we used a census transform with
a $5\times5$ local window and the matching cost
with a convolutional neural network (MC-CNN) method
\cite{Zbontar2015}. For computing the MC-CNN, `KITTI 2015 fast network' was used, provided at the
author's website \cite{MCCNN}. For the census transform,
we applied SGM \cite{Hirschmuller2008} or CVF \cite{Rhemann2011} on
the estimated cost volume. For SGM, we set $P_1 = 0.008$ and $P_2 = 0.126$ as in \cite{Park2015}.
For CVF, we performed the cost volume filtering using the guided
filter \cite{He2010} of a $19 \times 19$-sized local window and regularization
parameter $\epsilon = 0.01^2$ as recommended in \cite{Rhemann2011}.
To produce the MC-CNN results, following
the original MC-CNN paper in \cite{Zbontar2015}, we performed the cost
aggregation using an adaptive cross window (CBCA) \cite{Zhang2009}.
Note that the MC-CNN is one of top-ranked methods in the KITTI benchmark
\cite{KITTIbenchmark}, and we demonstrated that the proposed confidence
measure can be used to improve the quality of such a top-performing
stereo matching algorithm through a post-processing step.
For SLIC superpixels, we decompose the image into a different number of superpixels for each dataset: 500 for MID and 2000 for MPI, KITTI, and ZED.
In CFA, we set $\sigma_g = 1.0$ and $\sigma_s = 51$. In HCMA, we set $K = 20$. For GCPs-based optimization, we set $\sigma_D = 10$ and $\delta=
0.7$ using cross-validation for which we divided the training and testing dataset
into three groups, performed three-fold cross-validations, and then estimated the parameters
that provide the highest performance. Note that $\delta$ is set same as in \cite{Spyropoulos2014}.
Random forest classifiers were trained comprising 50 trees in regression mode, using
the MATLAB TreeBagger package \cite{Matlab},
where `Gini's diversity index (GDI)' \cite{Jost2006} is used as a splitting criteria at each node, and the minimum number of parents and leaf size and the maximum number of split are used as a termination criteria.
% Middlebury dataset (SGM)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_mod_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_mod_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_mod_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_mod_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/10_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_prop_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_prop_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_prop_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_prop_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/8_prop_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_mod_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_mod_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_mod_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_mod_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/15_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_prop_poggi_3dv.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_prop_poggi_bmvc.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_prop_cfa.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_prop_proposed.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figures/figure9/4_prop_gt.png}}\hfill
	\vspace{-6pt}
	\caption[The confidence maps and refined disparity maps of MID dataset]{The confidence maps and refined disparity maps of Middlebury dataset \cite{Middlebury} using (from top to bottom) census-based SGM+mod., SGM+GCPs, CVF+mod., and CVF+GCPs. (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Poggi \emph{et al.} (O(1)) \cite{Poggi20163dv}, (c) Poggi \emph{et al.} \cite{Poggi2016bmvc}, (d) CFA (Ours), (e) CFA+HCMA (Ours), and (f) ground truth confidence map.}\label{chap2_fig9}
\end{figure}

% MPI dataset
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.197\linewidth]{Figures/figure10/14_1_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.197\linewidth]{Figures/figure10/14_1_conf_Seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.197\linewidth]{Figures/figure10/14_1_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.197\linewidth]{Figures/figure10/14_1_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.197\linewidth]{Figures/figure10/14_1_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/14_1_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/14_1_mod_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/14_1_mod_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/14_1_mod_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/14_1_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_conf_Seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_prop_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_prop_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_prop_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/12_1_prop_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_conf_Seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_mod_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_mod_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_mod_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/5_1_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_conf_Seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_conf_cfa.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_conf_proposed.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_prop_seki.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_prop_cfa.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_prop_proposed.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure10/1_1_prop_gt.png}}\hfill
	\vspace{-6pt}
	\caption[The confidence maps and refined disparity maps of MPI dataset]{The confidence maps and refined disparity maps of MPI dataset \cite{MPI} using (from top to bottom) census-based SGM+mod., SGM+GCPs, CVF+mod., and CVF+GCPs. (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Seki \emph{et al.} \cite{Seki2016}, (c) CFA (Ours), (d) CFA+HCMA (Ours), and (e) ground truth confidence map.}\label{chap2_fig10}
\end{figure}

For evaluations, we divided the dataset into the MID \cite{Middlebury} and MPI \cite{MPI} dataset taken
or synthesized under carefully-controlled environments, and
real-world datasets as KITTI \cite{KITTIdataset} and ZED
stereo dataset that we captured. ZED stereo dataset was built with
a ZED stereo camera \cite{ZED}, where the resolution of the stereo image
pairs is full HD (1920$\times$1080). We captured the dataset for
outdoor environment, such as a playground, road, and building, etc. For
MID and MPI, we trained the classifier using 6 images in the Middlebury
2005 dataset \cite{Middlebury} and for KITTI and ZED stereo dataset, we
trained the classifier using 8 stereo pairs of $43^{th}$, $71^{th}$, $82^{th}$, $87^{th}$, $94^{th}$, $120^{th}$, $122^{th}$, and $180^{th}$ frame in KITTI 2012 
dataset \cite{KITTIdataset}, similar to the experimental settings commonly used in other methods \cite{Haeusler2013,Park2015,Poggi20163dv,Seki2016}. 
We further analyzed the effect of the number of training frames in \figref{chap2_fig6}.
Especially, `feature selection 1 (FS1)' was
composed of left-right consistency (LRC), the distance to the border,
LRD, MDDs in three different scales, MLM,
and the MS, and `feature selection 2 (FS2)' was
composed of MDDs in four different
scales, LRD, MLM,
PKRN, and the negative entropy measure. 
The experimental configuration is summarized in \tabref{chap2_tab1}.

To evaluate the performance of the confidence measures quantitatively,
we used the sparsification curve and its area under curve (AUC) as in
\cite{Haeusler2013,Spyropoulos2014,Park2015,Seki2016}. The sparsification
curve draws the bad pixel rates while successively removing the
pixels in descending order of confidence measure values in the
disparity map, thus it is possible to observe the tendency of
prediction errors. AUC quantifies the ability of a confidence
measure to estimate correct matches.
The higher the accuracy of
the confidence measure is, the lower the AUC value is. To evaluate
the quantitative performance, we also measured the average bad matching
percentage (BMP) as in \cite{Middlebury,MPI}. 
Furthermore, we measured the runtime of the proposed method for each dataset. The overall runtime of our method is 4.91, 11.67, 10.34, and 36.58 in seconds for MID (size of 300$\times$400), MPI (size of 1024$\times$436), KITTI (size of 1242$\times$375), and ZED (size of 1920$\times$1080).

\subsection{Parameter Sensitivity Analysis}\label{chap2_sec:51}
We analyzed the performance of the proposed confidence measure as
varying the associated parameters, including the number of superpixels
$M_\mathbf{S}$ and the number of sub-clusters $L$ in CFA, the
number of K-NN nearest neighborhood $K$ and the parameter $\alpha$
weighting between the pixel- and superpixel-level confidence maps in
HCMA, and the number of training images for MID \cite{Middlebury}, MPI \cite{MPI}, 
and KITTI \cite{KITTIdataset}. In these experiments, ZED \cite{ZED} was not analyzed since it does not have
ground truth disparity map.

We evaluated the average AUC for different numbers of segments in
superpixels as shown in \figref{chap2_fig5}(a). If the number of superpixels is too
small, different regions may be mixed in a single superpixel,
producing a high AUC. We segmented an input image into a set of
superpixels that contained about 200 pixels on average. The average
AUC values for varying $L$ are shown in \figref{chap2_fig5}(b). If $L$
is 1, we generated a single superpixel-level confidence feature in
$\mathcal{S}_m$, which may contain inaccurate segmentation errors
and occlusion outliers. We found that setting $L=2$ achieves the best
results. As the value of $L$ increases, the AUC value is degraded 
because of over-fragmented clusters. The average AUC value for varying values of $K$ is
shown in \figref{chap2_fig5}(c). The AUC value decreases as the values of $K$ increases and
converges when $K$ is 20. We set $K$ as 20 in all experiments. The
average AUC value for varying values of $\alpha$ are shown in \figref{chap2_fig5}(d).
As the value of $\alpha$ increases, there is a possibility of missing the spatial
coherency. We set $\alpha$ as 0.4 in all the experiments.

Furthermore, we also evaluated the performance as varying the number of training samples in \figref{chap2_fig6}.
In experiments, the performance variations were marginal as varying the number of training images in KITTI dataset \cite{KITTIdataset}. Thus, we used 8 training images when training our classifier in KITTI dataset \cite{KITTIdataset}. Furthermore, for Middlebury 2005 dataset \cite{Middlebury}, we found that the AUC value decrased until 5 images were used, as increasing the number of training sets, and there was no performance gain when more than 5 images were used. This indicates that it is enough to use 6 images in Middlebury 2005 dataset to learn the classifier \cite{Middlebury}.

% KITTI dataset (MCCNN)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_conf_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_conf_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_prop_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_prop_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/133_prop_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_conf_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_conf_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_prop_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_prop_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/79_prop_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_conf_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_conf_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_prop_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_prop_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/162_prop_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_conf_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_conf_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_prop_2015.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_prop_bmvc.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure11/170_prop_proposed.png}}\hfill
	\vspace{-6pt}
	\caption[The confidence maps and refined disparity maps of KITTI dataset]{The confidence maps and refined disparity maps of KITTI dataset \cite{KITTIdataset} using (from top to bottom) MC-CNN \cite{Zbontar2015} method. (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Park \emph{et al.} \cite{Park2015}, (c) Seki \emph{et al.} \cite{Seki2016}, and (d) CFA+HCMA (Ours).}\label{chap2_fig12}
\end{figure}

% ZED
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/9_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/9_right.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/9_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/9_mod_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/9_mod_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/14_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/14_right.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/14_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/14_prop_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/14_prop_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/12_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/12_right.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/12_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/12_mod_2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/12_mod_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/11_left.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/11_right.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/11_init_depth.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/11_prop_2015.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.196\linewidth]{Figures/figure12/11_prop_proposed.png}}\hfill
	\vspace{-6pt}
	\caption[The resulting disparity map of ZED dataset]{The resulting disparity map of ZED dataset (from top to bottom) census-based SGM + mod., SGM + GCPs., CVF + mod., and CVF + GCPs. This dataset is captured in natural enviornments, thus frequently having illumination variations between stereo pairs. (a) left color image, (b) right color image, (c) initial disparity maps, refined disparity maps using (d) confidence measured by Park \emph{et al.} \cite{Park2015}, and (e) confidence measured by the proposed method.} \label{chap2_fig13}
\end{figure}

% KITTI dataset
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_mod_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_mod_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/86_mod_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_prop_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_prop_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/121_prop_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_mod_poggi_3dv.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_mod_poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/19_mod_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_color.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_conf_Poggi_3DV.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_conf_Poggi_bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_conf_proposed.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_prop_poggi_3dv.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_prop_poggi_bmvc.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figures/figure13/92_prop_proposed.png}}\hfill
	\vspace{-6pt}
	\caption[The confidence maps and refined disparity maps of KITTI dataset]{The confidence maps and refined disparity maps of KITTI dataset \cite{KITTIdataset} using (from top to bottom) census-based SGM+mod., SGM+GCPs, CVF+mod., and CVF+GCPs. (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Poggi \emph{et al.} (O(1)) \cite{Poggi20163dv}, (c) Poggi \emph{et al.} \cite{Poggi2016bmvc}, and (d) CFA+HCMA (Ours).}\label{chap2_fig11}
\end{figure}

\subsection{Confidence Measure Analysis}\label{chap2_sec:52}
We compared the AUC of our method with conventional learning-based approaches 
using handcrafted confidence features \cite{Haeusler2013,Spyropoulos2014,Park2015,Gouveia2015,Poggi20163dv}
and CNN-based methods \cite{Seki2016,Poggi2016bmvc}.
We used census-based SGM
\cite{Zabih1994,Hirschmuller2008}, census-based CVF
\cite{Zabih1994,Rhemann2011}, and MC-CNN \cite{Zbontar2015} to obtain the initial disparity maps.
The optimal AUC can be obtained with a ground truth confidence map.
Sparsification curves for selected frames in the MID and KITTI datasets with census-based SGM
are shown in \figref{chap2_fig7}. The results show that the proposed confidence estimator
exhibits a better performance than conventional
per-pixel classifiers \cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv},
a superpixel-based classifier \cite{Gouveia2015}, and CNN-based approaches \cite{Poggi2016bmvc,Seki2016}. 
\figref{chap2_fig8} describes the AUC values, which are sorted in ascending order, for the
KITTI dataset with sensus-based SGM and census-based CVF respectively.
Park \emph{et al.} \cite{Park2015} showed inferior performances than the proposed method due to the classifier trained with pixel-level confidence features only. CNN-based methods \cite{Poggi2016bmvc,Seki2016} improved confidence estimation performance compared to existing handcrafted methods such as \cite{Park2015}, but they are still inferior to our method as they used only estimated disparity maps to predict unreliable pixels.

The average AUC value with census-based SGM and census-based CVF for MID,
MPI, KITTI and MC-CNN for KITTI is summarized in \tabref{chap2_tab2}. The table shows that
in all cases the confidence maps estimated with proposed method (CFA + HCMA) have the
lowest AUC values, as compared to the per-pixel
classifiers \cite{Haeusler2013,Spyropoulos2014,Park2015}. 
Furthermore, we conducted the experiments to evaluate our method for FS1 and FS2 on all databases in \tabref{chap2_tab2}. 
In experiments, the optimal selected features in our method were varied 
according to databases since there exist the performance gaps according to selected features. 
Based on these observations, we used `FS1' to MID \cite{Middlebury} and MPI \cite{MPI}, 
and `FS2' to KITTI \cite{KITTIdataset} and ZED \cite{ZED} for validation.

Unlike these methods, the proposed approach
outperforms other methods for predicting mismatched pixels.
When either CFA or HCMA are applied, our method outperforms
conventional confidence
measure methods
\cite{Haeusler2013,Spyropoulos2014,Park2015,Gouveia2015}, and
the best performance is achieved when both components are applied, as expected.
This validates the effectiveness of the proposed
aggregation scheme.

\subsection{Stereo Matching Analysis}\label{chap2_sec:53}
To verify the robustness of the confidence measures, we refined the
disparity map using the confidence maps estimated by several
confidence measure approaches including ours. For refining the
disparity maps, we used two different schemes described in Sec. 4,
which are cost modulation (mod.) based optimization \cite{Park2015}
and GCPs-based optimization (GCPs) without additional
post-processing to clearly show the performance gain achieved by the
proposed confidence measure. To evaluate the quantitative
performance, we measured an average bad matching percentage (BMP)
\cite{Middlebury} for the  MID \cite{Middlebury}, MPI \cite{MPI}, and
KITTI \cite{KITTIdataset} datasets. \tabref{chap2_tab3} shows the BMP for
MID \cite{Middlebury}, MPI \cite{MPI}, and KITTI \cite{KITTIdataset}
dataset. For MID, since there are occluded pixels in ground truth
disparity map, which we excluded, and computed the BMP only for visible
pixels. The KITTI benchmark provides a sparse ground truth disparity map
and we evaluated the BMP only for sparse pixels with the ground truth
disparity values. Note that the optimal percentage of BMP was obtained by measuring the ratio of erroneous pixels in which the absolute difference between the refined disparity map using ground truth confidence map and the ground truth disparity map is larger than a pre-defined threshold.
The results of extensive experiments show that the proposed method
achieves the lowest BMP.

% Qualitative
\figref{chap2_fig9}, \figref{chap2_fig10}, and \figref{chap2_fig11} show the disparity
maps refined with the confidence maps estimated from the existing
per-pixel classifiers \cite{Spyropoulos2014}, \cite{Park2015}, \cite{Poggi20163dv},
CNN-based classifiers \cite{Poggi2016bmvc}, \cite{Seki2016}, and
the proposed method. GCPs-based optimization was used to refine the
disparity maps for the MID \cite{Middlebury}, MPI \cite{MPI}, and
KITTI\cite{KITTIdataset} datasets. It is clearly shown that the erroneous matches
are reliably removed using the proposed confidence measure.
For the KITTI benchmark \cite{KITTIdataset}, erroneous disparities usually
occur in textureless regions (sky and road), and conventional
approaches \cite{Spyropoulos2014,Park2015,Poggi20163dv} do not detect uncorrect
pixels and thus they affect the matching quality of the subsequent
disparity estimation pipeline. In contrast, the proposed
method can detect mismatched pixels more reliably.
% bad matching percentage result
\begin{sidewaystable}[t!]
	\caption[The BMP of the resultant disparity map for MID, MPI, and KITTI dataset]{The BMP of the resultant disparity map for MID \cite{Middlebury}, MPI \cite{MPI}, and KITTI \cite{KITTIdataset} dataset. The bad pixel error rate of the refined disparity map using ground truth confidence is measured as `optimal'. The result with the lowest bad pixel error in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.19\linewidth} |
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth}
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth}
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth}
				>{\centering}m{0.05\linewidth}  >{\centering}m{0.05\linewidth} }
			\hlinewd{0.8pt}
			\multirow{3}{*}{Methods} & \multicolumn{4}{ c |}{Middlebury \cite{Middlebury}}
			& \multicolumn{4}{ c | }{MPI-Sintel \cite{MPI}}
			& \multicolumn{4}{ c }{KITTI \cite{KITTIdataset}} \tabularnewline
			\cline{2-13}
			& \multicolumn{4}{ c |}{Census}
			& \multicolumn{4}{ c |}{Census}
			& \multicolumn{4}{ c }{Census} \tabularnewline
			&w/SGM & w/SGM & w/CVF & w/CVF & w/SGM & w/SGM & w/CVF & w/CVF & w/SGM
			& w/SGM & w/CVF & w/CVF \tabularnewline
			\cline{2-13}
			& +mod. & +GCPs & +mod. & +GCPs & +mod. & +GCPs & +mod. & +GCPs
			& +mod. & +GCPs & +mod. & +GCPs \tabularnewline
			\hline
			\hline
			$\;$Initial disparity                                &20.43 &20.43 &17.64 &17.64 &19.54 &19.54 &13.82 &13.82 &23.50 &23.50 &15.21 &15.21 \tabularnewline
			$\;$LRC + WMF                                    &15.61 &15.61 &13.80 &13.80 &16.81 &16.81 &12.37 &12.37 &16.77 &16.77 &11.74 &10.74 \tabularnewline
			$\;$Haeusler \emph{et al.} \cite{Haeusler2013}          &12.35 &14.87 &12.55 &11.23 &12.90 &13.04 &10.96 &10.43 &10.21 &9.36  &10.68 &9.98  \tabularnewline
			$\;$Spyropoulos \emph{et al.} \cite{Spyropoulos2014}    &13.50 &15.37 &12.30 &10.99 &12.77 &11.20 &11.02 &10.50 &9.90  &8.91  &10.21 &9.00  \tabularnewline
			$\;$Park \emph{et al.} \cite{Park2015}                  &12.70 &15.35 &11.25 &10.76 &12.23 &10.69 &10.94 &9.92  &9.82  &7.95  &8.85  &8.81  \tabularnewline
			$\;$Poggi \emph{et al.} (O(1)) \cite{Poggi20163dv}                 		 &14.75 &13.28 &12.22 &10.88 &12.11 &10.23 &10.91 &8.48  &9.77  &7.58  &9.11  &8.76  \tabularnewline
			$\;$Gouveia \emph{et al.} \cite{Gouveia2015}      &14.20 &15.78 &14.32 &13.23 &13.48 &15.15 &12.48 &11.86 &12.49 &11.56 &10.89 &9.10  \tabularnewline
			$\;$Poggi \emph{et al.} \cite{Poggi2016bmvc}       &13.68 &13.19 &11.41 &10.46 &12.07 &10.03 &10.88 &8.12 &9.72  &7.54  &9.04  &8.59    \tabularnewline
			$\;$Seki \emph{et al.} \cite{Seki2016}       	&12.82 &11.87 &11.32 &10.52 &12.01 &9.46 &10.83 &7.63  &9.68  &7.47  &\textbf{8.68}  &8.33  \tabularnewline
			$\;$CFA (Ours)                                   &10.07 &9.68  &9.28  &10.29 &12.01 &11.55 &10.94 &8.00  &9.69  &7.15  &8.91  &7.87  \tabularnewline
			$\;$HCMA (Ours)                                  &11.99 &10.91 &10.52 &11.75 &11.95 &9.21  &10.85 &9.07  &9.79  &7.32  &8.94  &8.81  \tabularnewline
			\hline
			$\;$CFA+HCMA (Ours)                              &\textbf{9.87}  &\textbf{9.19}  &\textbf{9.27}  &\textbf{9.32}  &\textbf{11.78} &\textbf{8.61}
			&\textbf{10.83} &\textbf{7.49}  &\textbf{9.61}  &\textbf{7.12}  &8.83  &\textbf{7.80}  \tabularnewline
			$\;$Optimal                                      &7.46  &4.20  &6.92  &3.64  &7.96  &6.30  &8.96  &5.31  &7.75  &2.39  &7.23  &2.51  \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap2_tab3}
\end{sidewaystable}

Furthermore, when the proposed confidence measure is combined
with a cost computation method, such as MC-CNN \cite{MCCNN}, it
achieves a significantly improved disparity estimation performance.
\figref{chap2_fig12} shows the qualitative results that refined the initial disparity maps
obtained using MC-CNN cost computation for the KITTI benchmark.
\tabref{chap2_tab4} shows the quantitative evaluation for the KITTI
benchmark using the MC-CNN based approach. The refined disparity maps
with GCP-based optimization demonstrate the outstanding performance of
the proposed confidence estimation method as compared to the per-pixel
confidence classifier \cite{Park2015}.

For the ZED dataset, we performed a
subjective evaluation only, since no ground truth disparity map exists.
\figref{chap2_fig13} shows the qualitative results for the ZED dataset.
The refined disparity maps with cost modulation and GCPs-based optimization also support the outstanding performance
of the proposed method when applied to the challenging outdoor database.

% MCCNN result -- BMP (GCP)
\begin{table}[t!]
	\caption[The average BMP of the resultant disparity map for KITTI dataset]{The average BMP of the resultant disparity map for KITTI \cite{KITTIdataset} dataset. Initial disparity is obtained with MC-CNN \cite{Zbontar2015} based approach. The BMP of the refined disparity map using ground truth confidence is measured as `optimal'. The result with the lowest BMP in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.32\linewidth} |
				>{\centering}m{0.4\linewidth}   }
			\hlinewd{0.8pt}
			\multirow{2}{*}{Methods} & {KITTI \cite{KITTIdataset}}\tabularnewline
			\cline{2-2}
			&MC-CNN w/CBCA + GCPs \tabularnewline
			\hline
			\hline
			$\;$Initial disparity                                   &5.6937 \tabularnewline
			$\;$Spyropoulos \emph{et al.} \cite{Spyropoulos2014}    &5.5361 \tabularnewline
			$\;$Park \emph{et al.} \cite{Park2015}                  &5.2239 \tabularnewline
			$\;$Poggi \emph{et al.} \cite{Poggi2016bmvc}            &4.7318 \tabularnewline
			$\;$Seki \emph{et al.} \cite{Seki2016}         		    &4.4661 \tabularnewline
			$\;$CFA (Ours)                                   &4.2621 \tabularnewline
			$\;$HCMA (Ours)                                  &4.8347 \tabularnewline
			\hline
			$\;$CFA+HCMA (Ours)                              &\textbf{4.2477}  \tabularnewline
			$\;$Optimal                                      &2.1760  \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap2_tab4}
\end{table}

\label{chap2_sec:6}
\section{Summary}
In this study, a novel approach for learning-based confidence
measure was proposed. It is assumed that the confidence features and
resulting confidence maps are smoothly varying
in the spatial domain. We first demonstrated that a confidence feature augmentation
that imposes spatial coherency on the confidence features and the
resulting confidence maps can increase the
performance of the confidence estimation.
The confidence map was
further improved through hierarchical confidence map aggregations.
The stereo algorithms using the proposed confidence estimation method exhibited
accurate and robust results for public datasets as well as for challenging outdoor environments.
As future work, we will study the confidence feature
that encodes the spatial coherency in a deep
convolutional neural network framework.

==> chap3.tex <==
\chapter{Unified Confidence Estimation Networks for Robust Stereo Matching}
\label{chap:chap3}

\section{Introduction}\label{chap3_sec:1}
For decades, the stereo matching has been one of the fundamental and essential topics in the fields of computer vision. It
aims to estimate accurate corresponding points for each pixel between a pair of two images taken under different viewpoints of the same scene. Though numerous methods
have been proposed for this task, it still remains an unsolved problem due to
several factors including textureless or repeated pattern regions,
and occlusions \cite{Mei2011,Humenberger2010,Egnal2002}. Besides,
photometric deformations incurred by illumination and/or camera
variations pose additional challenges
\cite{Zabih1994,Kim2003,Heo2011}.

In general, most of the stereo matching methods consist of the following pipelines \cite{Scharstein2002}:
1) matching cost computation, 2) matching cost aggregation, 3) disparity
regularization, and 4) post-processing. Concretely, the similarity between patches from left and right images is first measured with various cost measures~\cite{Hirschmuller2008,Zbontar2015} and the matching cost volume is then constructed with these matching costs across disparity candidates.
Various methods have attempted to improve the matching accuracy at each step. 
To robustly
compute the matching cost, several approaches
were proposed by using robust cost measures \cite{Min2008,Heo2011,Kim2014} or learning-based approaches \cite{Zbontar2015,Luo2016}.
Moreover, the matching costs are aggregated to
alleviate matching ambiguities by considering local neighbors \cite{Rhemann2011, Yoon2008,
	Lu2012}. Powerful regularization techniques \cite{Hirschmuller2008,
	Felzenszwalb2006} can also be applied by incorporating prior constraints into
an objective function. These
approaches help to yield reliable matching results to some extent,
but they do not fully address the inherent problems of stereo
matching.

To further improve the matching accuracy, most approaches involve
the post-processing step. A set of unreliable pixels is first
extracted using confidence measures, and then interpolated using
reliable estimates at neighboring pixels
\cite{Egnal2004,Mordohai2009,Hirschmuller2008,Wang2011,Spyropoulos2014,Rhemann2011}.
Conventionally, mismatched pixels were detected using simple confidence measures such as a left-right consistency or peak ratio
\cite{Fusiello1997}, \cite{Hu2010}. Recently, learning-based approaches have been populary
proposed to boost the performance of confidence estimation
\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv}. Formally, a set of
confidence features extracted from stereo matching results of
the training data is used to train the confidence classifier
\cite{Hirschmuller2002,Haeusler2013,Spyropoulos2014}. In a test
phase, the trained classifier is used to estimate the confidence of
each pixel. These methods have shown distinct strengths in
comparison to existing non-learning based approaches
\cite{Fusiello1997}. However,
they still rely on hand-crafted confidence features for training
the confidence classifier, and thus they often fail to detect mismatched
pixels under challenging conditions \cite{Kim2017tip}.

More recently, convolutional neural networks (CNNs)-based approaches
have been proposed to robustly extract confidence features from a disparity map and estimate the confidence \cite{Seki2016,Poggi2016bmvc}. 
Although they have shown improved performance than the existing methods based on handcrafted features \cite{Haeusler2013,Spyropoulos2014,Park2015,Spyropoulos2016},
they rely on rather limited information in learning the
confidence features. According to \cite{Hu2012}, there exist many
informative features within the cost volume. It was also shown in
many literatures \cite{Haeusler2013,Spyropoulos2014,Park2015,Spyropoulos2016} that the hand-crafted features extracted
from the cost volume can boost the performance of the confidence
estimation. In contrast, most of the existing CNN-based approaches leverage only
single or stereo disparity maps for confidence estimation \cite{Seki2016, Poggi2016bmvc}, which may limit the performance in challenging conditions. Although several methods \cite{Shaked2017,Seki2016} have attempted to use the cost volume in the confidence estimation within deep networks, the direct usage of the raw cost volume cannot boost the confidence estimation performance. Unlike disparity information, the raw matching cost volume has scale variation problem that the absolute value of the matching cost volume varies depending on stereo matching approaches used and its distribution is non-discriminative for reliable and unreliable pixels.
	This prohibits the direct usage of the cost volume in the confidence estimation networks.

% Figure: overall framework
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.8\linewidth]{Figure_final/fig1_overall/overall.pdf}}\\
	\vspace{-15pt}
	\caption[Illustration of the proposed network]{Illustration of the proposed network, consisting of two sub-networks including matching probability volume construction network and confidence estimation network.}\label{chap3_fig1_overall}
\end{figure}

In this paper, we propose a novel deep architecture that simultaneously uses a matching cost volume and disparity map as inputs to estimate the confidence as in \figref{chap3_fig1_overall}. Firstly, we propose a matching probability construction network (MPCN) that extracts the matching probabilities from the cost volume to improve a discriminative power and solve the scale variation problem of the cost volume.
Secondly, we propose a confidence estimation network (CEN) to estimate the reliable confidence by simultaneously leveraging the matching probabilities and their corresponding disparity maps, where multiple convolutional filters with varying sizes are used to extract multi-scale disparity features. These two sub-networks are learned in a joint and boosting manner, enabling us to estimate reliable disparity and confidence maps in a unified framework.

To learn our networks in a supervised manner, vast amount of
stereo image pairs and corresponding dense disparity (or depth) maps
are required. However, in outdoor scenes, 3D laser scanners often
fail to capture depth information of very distant objects. For
instance, no depth information is provided at the upper parts (e.g.
sky) of color images in the KITTI benchmark \cite{KITTIdataset},
making supervised learning of CNNs infeasible for this task.
Alternatively, dense ground truth disparity maps would be generated
through synthetic rendering, as in the MPI sintel \cite{MPI} and
DispNet \cite{Mayer2016}, but they cause domain adaptation problem
inherently when directly used to estimate disparity maps for real
outdoor stereo images. To address the problem of limited training
samples for the stereo matching, we propose a semi-supervised
learning scheme in which the pixels classified as confident through
the estimated confidence map are used to measure the image reconstruction loss~\cite{Godard2017}.



To verify the proposed confidence estimation method, we
employ three post-processing methods such as cost modulation
\cite{Park2015}, ground control points (GCPs)-based propagation \cite{Xu2013}, and aggregated GCPs-based
propagation \cite{Min2015}. Experimental results show that the proposed method outperforms conventional handcrafted feature-based methods and CNN-based methods on various benchmarks, including Middlebury 2006 \cite{Scharstein2007}, Middlebury 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset}.

This manuscript extends the conference version of this work \cite{Kim2017icip}.
It newly adds (1) additional convolutional networks to refine the raw matching cost volume to boost confidence estimation performance; (2) a semi-supervised learning scheme to learn the proposed networks only with the limited sparse ground truth disparity maps;
(3) multi-scale disparity feature extraction networks to extract confidence features from different scale of disparities; and (4) an extensive comparative study with the state-of-the-art confidence estimation algorithms using various datasets.\vspace{-5pt}

\section{Related Works}\label{chap3_sec:2}
\subsection{Hand-crafted Approaches}\label{chap3_sec:21}
Numerous approaches have been proposed for stereo
confidence estimation based on various handcrafted confidence measures \cite{Egnal2002,Egnal2004,Mordohai2009}.
%The general procedure can be summarized as follows. %First, when a
%pair of stereo images and associated ground truth disparity maps are
%given as training data, a ground truth confidence map is computed by
%comparing an estimated disparity map (from stereo matching
%algorithms) and the ground truth disparity map. Then, they extract
%confidence features and train a simple shallow classifier,
%\emph{e.g.} random decision forest \cite{Breiman2001}, by using the
%defined confidence features and ground truth confidence map. 
A comprehensive review provided in \cite{Hu2012} concluded that using single confidence feature would not yield
good performance in confidence estimation.
%there is no single confidence feature that always estimates the consistently reliable confidence map across various databases.
In order to overcome such limitations and improve the prediction
accuracy, there have been various attempts to combine confidence
features and train a simple shallow classifier, e.g. random decision forest \cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv}.
They define the confidence feature, which consists of various stereo
confidence cues from the estimated disparity map and (optionally)
cost volume. Haeusler et al. \cite{Haeusler2013} combined
confidence features consisting of left-right consistency, image gradient, and disparity map variance
for training the classifier.
Similar approach was also proposed in \cite{Spyropoulos2014}. Though
they improved the prediction accuracy over single confidence based
approaches \cite{Egnal2002,Egnal2004}, the performance is still limited since the
combination of confidence features is not optimal.
% Figure: MPN
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=1.0\linewidth]{Figure_final/fig2_mpn/MPN.pdf}}\\
	\vspace{-15pt}
	\caption[Illustration of the matching probability construction network]{Illustration of the matching probability construction network.}\label{chap3_fig2_mpn}
\end{figure}

To select the set of (sub-)optimal confidence features among
multiple confidence features, Park and Yoon \cite{Park2015} proposed
to utilize the regression forest that computes the importance of
confidence features and to train the regression forest classifier
using the selected confidence features. Poggi and Mattoccia
\cite{Poggi20163dv} employed the set of confidence features from
only disparity map that can be computed in O(1) complexity without losing
the confidence estimation performance. While
the above methods detect confident pixels at the pixel-level, Kim
et al. \cite{Kim2017tip} leverages a spatial context to
estimate confidence at the superpixel-level by concatenating pixel-
and superpixel-level confidence features. However, all of these
methods use handcrafted confidence features that might not be
optimal to detect unconfident pixels on challenging scenes.\vspace{-10pt}

\subsection{CNN-based Approaches}\label{chap3_sec:22}
More recently, several approaches have attempted to estimate the
stereo confidence using deep CNNs
\cite{Poggi2016bmvc,Seki2016,Poggi2017cvpr}, demonstrating much
improved performance over existing handcrafted approaches. In \cite{Poggi2016bmvc},
they proposed a novel confidence
estimation network that uses a left disparity map only as an input.
Seki and Pollefeys \cite{Seki2016} proposed to uses both left and
right disparity maps in deep networks for improving the
confidence prediction accuracy. The confidence refinement network
\cite{Poggi2017cvpr} was also developed, which can improve the accuracy
of the measured confidence map by leveraging local consistency of confidence map. Shaked and Wolf
\cite{Shaked2017} estimated both disparity and confidence maps from
cost volume simultaneously, but they do not use the estimated
disparity map as an input of the confidence estimation network.

Tosi et al. \cite{Tosi2017} proposed a novel
self-supervised strategy, which generates training labels by
leveraging a pool of appropriately combined conventional confidence
measures. Poggi et al. \cite{Poggi2017iccv} performed a
quantitative evaluation of confidence measures that use machine
learning algorithms.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/1_cost.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/1_pdf.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/1_top5.pdf}}\hfill
	\vspace{-20pt}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/2_cost.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/2_pdf.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/2_top5.pdf}}\hfill
	\vspace{-20pt}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/3_cost.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/3_pdf.pdf}}\hfill
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/3_top5.pdf}}\hfill
	\vspace{-20pt}
	\subfigure[(a)]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/4_cost.pdf}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/4_pdf.pdf}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig3_topK/4_top5.pdf}}\hfill
	\vspace{-5pt}
	\caption[Effectiveness of top-$K$ matching probability volume]{Effectiveness of top-$K$ matching probability volume: (a) raw matching cost of MC-CNN \cite{Zbontar2015} for the KITTI 2015 dataset \cite{KITTIdataset}, (b) matching probability using Eq. (1), and (c) descending order of top-$K$ matching probabilities using Eq. (2) ($K=5$). First and second row represent reliable pixels, and third and fourth row represent unreliable pixels.}
	\label{chap3_fig3_topK}
\end{figure}

Although CNN-based approaches demonstrated the improved performance
compared to handcrafted features-based methods, they
use disparity or cost volume only, and no attempt has been made to
use both disparity and cost volume. It was shown in existing
handcrafted approaches
\cite{Haeusler2013,Spyropoulos2014,Park2015,Kim2017tip} that using
the confidence features extracted from the cost volume as well as
the disparity improves the confidence prediction accuracy. \vspace{-5pt} 


\section{Proposed Method}\label{chap3_sec:3}
\subsection{Problem Formulation and Model}\label{chap3_sec:31}
Let us define a pair of stereo images $\{I^l,I^r\}$. The objective
of stereo matching is to estimate a disparity $D_i$ for each pixel $i = [i_\mathrm{x},i_\mathrm{y}]^T$ between input stereo
images. Since
most of stereo matching methods have an estimation error, our approach aims
at estimating a confidence of $D_i$ within a
learning framework, and refining $D_i$ using the
confidence map.


For this task, we propose a novel approach that estimates a confidence map using the matching cost volume and disparity map simultaneously in deep CNNs. The overall
network consists of two sub-networks, matching probability
construction network (MPCN) and confidence estimation network (CEN). We first estimate a matching cost volume $C_{i,d}$ using existing matching cost functions across a set of disparity
candidates $d\in \{0,1,...,d_\mathrm{max}\}$ defined for a maximum disparity $d_\mathrm{max}$. Since the direct use of cost volume $C_{i,d}$ to detect the
confidence has trouble in solving the scale variation problem and provides a limited discriminative power, we generate the matching probability volume
$P_{i,d}$ by refining the initial cost volume $C_{i,d}$ in the matching probability construction network as in \figref{chap3_fig2_mpn}. In the confidence estimation network as in \figref{chap3_fig4_cen}, our method then learns
the relationship between the matching probability volume ${P}_{i,d}$
with its associated disparity $D_i$ and a ground truth confidence
$Q^*_i$, computed by thresholding an absolute difference between
the estimated disparity $D_i$ and ground truth disparity
$D^*_i$. %the confidence of $D_i$ can be then estimated such that $Q_i \in [0,1]$. With elaborately constructed matching probability volume,
In this network, the confidence features are extracted using both $P_i$ and $D_i$. Additionally, motivated by methods using handcrafted confidence features \cite{Park2015,Poggi20163dv}, we employ a multi-scale CNN
architecture that encodes confidence features from disparity maps at multiple scales.
Furthermore, since sparse and insufficient ground truth disparity maps are available in most stereo databases \cite{KITTIdataset}, a semi-supervised loss is proposed to learn the network, where we use confident points to compute the  image recontruction loss.\vspace{-10pt}

\subsection{Confidence Estimation Using Cost Volume and Disparity}\label{chap3_sec:32}
\subsubsection{Matching Probability Construction Network}\label{chap3_sec:321}
Although the matching cost volume $C_{i,d}$ includes useful
information to find reliably matched pixels, the raw matching cost volume itself
has a limited discriminative power and the scale variation problem, thus direct use of the cost volume provides limited performance for estimating confidences as described in
\cite{Seki2016,Poggi2017iccv}.
To overcome these limitations, we formulate convolutional layers to aggregate and refine the raw matching costs with learned kernels, followed by the normalization layer.
After passing the raw matching cost volume through a series of
convolutional layers to construct the refined cost volume such that $C' = \mathcal{F}(C;W^c)$ with network parameters $W^c$, we
generate the matching probability volume $P$, which
normalizes the refined matching cost volume $C'$ such that
\begin{equation}
	P_{i,d} = \frac{\textrm{exp}({-C'_{i,d}/\sigma})}{\sum_{u}\textrm{exp}({-C'_{i,u}/\sigma})},
\end{equation}
where $u\in \{1,...,d_\mathrm{max}\}$ and $\sigma$ is a parameter to adjust a
flatness of the matching cost volume. Compared to a softmax module,
this normalization scheme can adjust the flatness of matching probability volume according to $\sigma$, improving the discriminative power as exemplified in \figref{chap3_fig3_topK}. Note that $\sigma$ is defined according to the relative scale of the matching cost. As exemplified in \figref{chap3_fig3_topK}(a), the absolute scale of
raw matching cost $C_{i,d}$ varies for each pixel, and thus they provide a low discriminative power to be used for estimating reliable pixels. This problem
can be alleviated in the matching probability volume $P_{i,d}$ as shown in
\figref{chap3_fig3_topK}(b).
%Thus, the matching cost volume $P_{i,d}$ is used to extract the refined disparity map and reliable confidence features simultaneously.

Furthermore, we can also find that
the majority of matching probabilities $P_{i,d}$ has a value close to 0,
which does not convey useful cues as shown in \figref{chap3_fig3_topK}(b). Such
redundant parts rather distract the performance of confidence
estimation, which will be described in the following section. Thus we also propose a top-$K$ pooling layer, where the
matching probability $P_{i}$ of Eq. (1) is projected into a fixed
length input as follows:
\begin{equation}
	P_{i,k} = \textrm{max}^{k}_{d}{P_{i,d}},
\end{equation}
where $\textrm{max}^{k}(\cdot)$ is the $k$-th maximal value for $k =
\{1, ..., K\}$. As shown in \figref{chap3_fig3_topK}(c), top-$K$ matching probabilities have a consistent shape by descending ordering according to reliable or unreliable pixels. Matching outliers in the unreliable pixels lead to rather scattered (or even uniform) distribution of matching probability, while reliable pixels yield concentrated distribution of probability, thus providing a highly discriminative power for confidence estimation.
Note that this layer has no trainable parameters,
but is differentiable, and thus it can be inserted to any networks as an intermediate layer.
In \figref{chap3_fig3_topK}(c), the top-$K$ matching probabilities demonstrate a high discriminative power to classify reliable pixels.

Moreover, since our confidence estimator predicts the confidence using the cost volume and disparity map simultaneously, we additionally compute its associated disparity map. It can be realized through a winner-take-all (WTA) strategy, but it is not differentiable. To overcome this, we use the soft argmin layer as in \cite{Kendall2017} as follows:
\begin{equation}
	{D}_{i} = \sum\nolimits_{d}{d\times P_{i,d}}.
\end{equation}
This operation is fully differentiable and allows us to regress the
disparity during training. Note that since the matching probability construction network is learned
with the estimated confidence simultaneously, which will be described in the following section, the quality of the disparity map $D$ is gradually improved during training. It is used to learn the confidence estimation networks, which enables us to estimate reliable disparity and confidence maps, different from conventional methods that use fixed disparity maps to learn the confidence estimation networks \cite{Seki2016,Poggi20163dv,Poggi2016bmvc,Shaked2017}. %can be more accurate compared to initial disparity map $D_{i}$.



\subsubsection{Confidence Estimation Network}\label{chap3_sec:322}
At the heart of our strategy to boost the performance of confidence
estimation is the fusion scheme of two inputs, consisting of
the top-$K$ matching probability volume $P$ and its corresponding disparity map $D$. Due to
heterogeneous attributes of them, a direct concatenation of two raw inputs
does not provide an optimal performance. Alternatively, we can
simply fuse intermediate outputs obtained from
sub-networks for two raw inputs, but the prediction output cannot be
fused optimally since the contribution of each input might vary for
each pixel.

To overcome these limitations, we build the deep
architecture inspired by \cite{Li2016}, including a fusion network to estimate the confidence as well as two
sub-networks to extract confidence features. 
Moreover, we extract multi-scale disparity features to improve the
discriminative power of confidence features
by taking different size of convolutional filters as in \cite{Park2015,Poggi20163dv}.
In order to
extract disparity features from different scales, we set different size of convolutional filters for each scale level
$l\in\left\{1,2,...,L\right\}$, where $L$ is the number of scales.
Each disparity feature extractor network is defined such that $A_l^d = \mathcal{F}(D;W_l^d)$ while matching probability feature extractor network is defined such that $A^c = \mathcal{F}(P;W^c)$, 
where $W_l^d$ and $W^c$ are network parameters.
After all intermediate activations, $A^c$ and $A_l^d$, are
concatenated, the confidence map is finally regressed as the output of
fusion network $Q = \mathcal{F}(A^c,A_1^d,...,A_L^d;W^f)$,
where $W^f$ is a fusion network parameter and the sigmoid function is used for the last activation to train
the binary classifier. \figref{chap3_fig5_joint} represents the effectiveness of the proposed fusion strategy.\vspace{-10pt}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.6\linewidth]{Figure_final/fig4_cen/CEN.pdf}}\\
	\vspace{-20pt}
	\caption[Illustration of the confidence estimation network]{Illustration of the confidence estimation network.}
	\label{chap3_fig4_cen}
\end{figure}

\subsection{Network Configuration}\label{chap3_sec:33}
The deep network for the matching probability construction is illustrated in \figref{chap3_fig2_mpn}, and
the configuration of this network is summarized in \tabref{chap3_tab2_1}.
The matching probability construction network consists of a cost volume refinement network, normalization layer, and top-$K$ pooling layer.
To refine the raw matching cost volume, we design the encoder-decoder network with skip layers, consisting of sequential convolutional layers followed by batch normalization (BN) and rectified linear units (ReLU).
We apply $2 \times 2 $ max-pooling operators sequentially, resulting in a total down-sampling factor of 4.
In the decoding procedure, we upsample the intermediate features using bilinear deconvolutional filters, and concatenate the upsampled features using a skip layer. Instead of directly predicting the refined cost volume, we predict a residual cost volume by adding a skip connection from the raw cost volume to the output. As the residual learning alleviates the need for restoring specific cost volume contents, our cost volume refinement network provides significant improvement in refining the raw cost volume.

The deep networks for the confidence estimation are shown in \figref{chap3_fig4_cen}, and the configuration of this network is summarized in \tabref{chap3_tab2_2}. For the confidence estimation network, we leverage $3 \times 3$
convolutional filters sequentially, followed by BN and ReLU. In this network, the pooling operator
is not used to preserve the spatial resolution. To extract multi-scale disparity features with different sizes of receptive fields,
we vary the convolutional filter size relative to scale level
$l\in\left\{1,2,...,L\right\}$ as explained in \tabref{chap3_tab2_2}. Here, we set $L$ as 4. We also apply
Sigmoid operator on the output of the last activation since the
output confidence value is within $[0,1]$.\vspace{-10pt}
\begin{table}[t!]
	\caption[Our network architecture of matching probability construction network]{Our network architecture of matching probability construction network, where `D.F. I/O' denotes downscaling factor of input and output for each layer relative to the input image.}\vspace{10pt}
	\centering
	\begin{tabular}{>{\centering}m{0.20\linewidth} >{\centering}m{0.06\linewidth} 
			>{\centering}m{0.14\linewidth} >{\centering}m{0.11\linewidth} 
			>{\centering}m{0.22\linewidth}}
		\hlinewd{0.8pt}
		Layer & Kernel & Ch I/O&  D.F. I/O & Input \tabularnewline
		\hline
		\hline
		conv1  &$3\times3$  & $d_\mathrm{max}$/64   & 1/1 & raw c.v.  \tabularnewline
		conv1b &$3\times3$  & 64/64   & 1/1 & conv1 \tabularnewline
		pool1  &$2\times2$  & 64/64   & 1/2 & conv1b \tabularnewline
		conv2  &$3\times3$  & 64/128  & 2/2 & pool1 \tabularnewline
		conv2b &$3\times3$  & 128/128 & 2/2 & conv2 \tabularnewline
		pool2  &$2\times2$  & 128/128 & 2/4 & conv2b \tabularnewline
		conv3  &$3\times3$  & 128/128 & 4/4 & pool2 \tabularnewline
		conv3b &$3\times3$  & 128/128 & 4/4 & conv3 \tabularnewline
		upconv2 &$4\times4$ & 128/128 & 4/2 & conv3b \tabularnewline
		conv4 &$3\times3$   & 128/64 & 2/2 & upconv2+conv2b \tabularnewline
		conv4b &$3\times3$ & 64/64 & 2/2 & conv4 \tabularnewline
		upconv1 &$4\times4$ & 64/64 & 2/1 & conv4b \tabularnewline
		conv5 &$3\times3$ & 64/$d_\mathrm{max}$ & 1/1 & upconv1+conv1b \tabularnewline
		Sum &  $1\times1$ & $d_\mathrm{max}$/$d_\mathrm{max}$ & 1/1 
		& raw c.v.+conv5  \tabularnewline
		Norm. &- & $d_\mathrm{max}$/$d_\mathrm{max}$   & 1/1 & Sum \tabularnewline
		Top-$K$ Pooling  &- & $d_\mathrm{max}$/$K$ & 1/1 & Norm. \tabularnewline
		Soft Argmax &- & $d_\mathrm{max}$/1   & 1/1 & Norm. \tabularnewline
		\hlinewd{0.8pt}
	\end{tabular}\label{chap3_tab2_1}
\end{table}

\subsection{Loss Function}\label{chap3_sec:34}
\subsubsection{Matching Probability Construction Network Loss}
A major challenge of CNN-based stereo matching methods is the lack of dense ground truth disparity maps especially in outdoor settings \cite{Tonioni2017}. %Recently, some methods have tried to learn their network
%with a synthesized ground-truth disparity map, and applied it to
%a real image \cite{Mayer2016}, but they face the domain adaptation
%problem inherently.
To overcome this limitation, we propose a semi-supervised learning scheme in a manner that highly confident pixels in the disparity map are used together with sparse ground truth disparities to learn the matching probability construction network. Specifically, with the sparse ground truth disparity $D^*$ and the estimated disparity $D$, we define a novel loss function for the MPCN, consisting of a supervised term
$\mathcal{L}_{sup}$ and an unsupervised term
$\mathcal{L}_{unsup}$ with hyper-parameter $\lambda$ that weighs the
contribution of the latter:
\begin{equation}\label{chap3_equ3}
	\mathcal{L}_{MPCN} = \mathcal{L}_{sup} + \lambda\mathcal{L}_{unsup}.
\end{equation}
The supervised term $\mathcal{L}_{sup}$ is formulated to directly regress the
disparity $D$ with respect to ground truth disparity $D^*$
with $L_1$ norm objective function such that
\begin{equation}
	\mathcal{L}_{sup} = \sum\nolimits_{i} {m_i} {\left|{D_i}-D^*_i\right|},
\end{equation}
where ${m_i}$ is a mask that represents the existence of ground truth disparity map.
It should be noted that this supervised loss $\mathcal{L}_{sup}$ can
provide reliable performance when the network is learned with a
sufficient amounts of training data. To overcome this, we
additionally propose an unsupervised term $\mathcal{L}_{unsup}$ that
leverages the estimated confidence %to boost the performance of matching probability construction network
as follows:
\begin{equation}
	\mathcal{L}_{unsup} = \sum\nolimits_{i}{\mathcal{G}(Q_i;\rho)\left|I^l_{i-D_i}-I^r_i\right|},
\end{equation}
where $\mathcal{G}(Q_i;\rho)$ is a truncation function which has the value 1
when the estimated confidence $Q_i$ is higher than a threshold parameter
$\rho$, and 0 otherwise. As $\rho$ decreases, the density of regions used to compute the loss $\left|I^l_{i-D_i}-I^r_i\right|$ increases,
	but it is more likely that the convergence of networks is disturbed due to unreliable regions used in the loss function.
	Contrarily, as $\rho$ increases, the density of regions used to compute the loss decreases, slowing down the convergence.
	Here, we set $\rho$ in which the density of confident regions used in the loss computation becomes 75\% on average.
This loss function is similar to the image recostruction loss as in \cite{Godard2017} that minimizes the difference between right color image $I^r_i$ and warped left color $I^l_{i-D_i}$. One difference is that our loss function only considers highly confident regions to learn the disparity. To achieve a convergent optimization and avoid the bias problem, we first learn the confidence map with only the supervised loss $\mathcal{L}_{sup}$ until the pre-defined number of epoch,
	and then fine-tuned them with the semi-supervised loss (i.e., $\mathcal{L}_{sup}$ and $\mathcal{L}_{unsup}$). After learning the network, we put the semi-supervised loss in Eq. (6) together with Eq. (5) with reliable confidence. With these loss functions, our method reliably learns the
matching probability construction network with the datasets having only sparse
ground truth disparity map.
\figref{chap3_fig6_loss} shows the importance of a semi-supervised loss function for learning matching probability construction network.

%(DB: Hard to understand. If only (6) is used in the loss, the lack
%of data can be addressed. But, the method uses both (5) and (6),
%meaning that data without GT disparity map is not used when using
%(4). In short, explain how (4) resolves the lack of data.)





\begin{table}[t!]
	\caption[Our network architecture of confidence estimation network]{Our network architecture of confidence estimation network.}\label{chap3_tab2_2}\vspace{10pt}
	\centering
	\begin{tabular}{c c c c c}
		\hlinewd{0.8pt}
		\multicolumn{5}{c}{Matching Probability Feature Extractor}\tabularnewline
		\hlinewd{0.8pt}
		Scale & Layer & Kernel & Ch I/O & Input \tabularnewline
		\hline
		\hline
		\multirow{5}{*}{-}          & conv1$_m$ & $3\times3$ & $K$/256   & top-$K$ m.p.v. \tabularnewline
		& conv2$_m$ & $3\times3$ & 256/128 & conv1$_m$  \tabularnewline
		& conv3$_m$ & $3\times3$ & 128/64  & conv2$_m$  \tabularnewline
		& conv4$_m$ & $3\times3$ & 64/32   & conv3$_m$  \tabularnewline
		& conv5$_m$ & $3\times3$ & 32/1    & conv4$_m$  \tabularnewline
		\hlinewd{0.8pt}
		\multicolumn{5}{c}{Disparity Feature Extractor}\tabularnewline
		\hlinewd{0.8pt}
		Scale & Layer & Kernel &  Ch I/O & Input \tabularnewline
		\hline
		\hline
		\multirow{3}{*}{Scale1} & conv1$_{s1}$ & $3\times3$ & 1/128    & disparity \tabularnewline
		& conv2$_{s1}$ & $3\times3$ & 128/64   & conv1$_{s1}$ \tabularnewline
		& conv3$_{s1}$ & $1\times1$ & 64/1   & conv2$_{s1}$  \tabularnewline
		\hlinewd{0.1pt}
		\multirow{3}{*}{Scale2} & conv1$_{s2}$ & $5\times5$ & 1/128    & disparity \tabularnewline
		& conv2$_{s2}$ & $3\times3$ & 128/64   & conv1$_{s2}$  \tabularnewline
		& conv3$_{s2}$ & $1\times1$ & 64/1   & conv2$_{s2}$  \tabularnewline
		\hlinewd{0.1pt}
		\multirow{3}{*}{Scale3} & conv1$_{s3}$ & $7\times7$ & 1/128    & disparity \tabularnewline
		& conv2$_{s3}$  & $3\times3$ & 128/64   & conv1$_{s3}$  \tabularnewline
		& conv3$_{s3}$  & $1\times1$ & 64/1     & conv2$_{s3}$   \tabularnewline
		\hlinewd{0.1pt}
		\multirow{3}{*}{Scale4} & conv1$_{s4}$ & $9\times9$ & 1/128    & disparity \tabularnewline
		& conv2$_{s4}$ & $3\times3$ & 128/64   & conv1$_{s4}$ \tabularnewline
		& conv3$_{s4}$ & $1\times1$ & 64/1   & conv2$_{s4}$ \tabularnewline
		\hlinewd{0.8pt}
		\multicolumn{5}{c}{Fusion Network}\tabularnewline
		\hlinewd{0.8pt}
		Scale & Layer & Kernel &  Ch I/O & Input \tabularnewline
		\hline
		\hline
		\multirow{4}{*}{-}      & conv1$_{f}$ & $3\times3$ & 5/64  & conv4$_m$+conv2$_{s1}$+...+conv2$_{s4}$\tabularnewline
		& conv2$_{f}$ & $3\times3$ & 64/32 & conv1$_{f}$  \tabularnewline
		& conv3$_{f}$ & $3\times3$ & 32/1  & conv2$_{f}$  \tabularnewline
		& Sigmoid & $1\times1$ & 1/1   & conv3$_{f}$  \tabularnewline
		\hlinewd{0.8pt}
	\end{tabular}
\end{table}        

\subsubsection{Confidence Estimation Network Loss}\label{chap3_sec:341}
Compared to the matching probability construction network, the confidence estimation network needs relatively lower number of parameters, and such shallower networks can be learned even with limited sparse disparities as in \cite{Poggi2016bmvc,Seki2016}. The loss function of the CEN is designed to predict the confidence $Q$ with respect to the ground truth confidence $Q^*$ defined as follows:
\begin{equation}
	Q^*_i = \mathcal{G}(|D^*_i-D_i|;\delta),
\end{equation}
where $\delta$ is a threshold parameter to compare the
ground truth disparity $D^*$ and the estimated disparity $D$ which is the output of the matching
probability construction network.

The loss function for the confidence estimation network $\mathcal{L}_{CEN}$ is then defined as the cross-entropy loss:
\begin{equation}
	\mathcal{L}_{CEN} = -\sum\nolimits_{i}{\left[Q^*_i \text{log}{Q_i}+(1-Q^*_i)\text{log}{\left(1-Q_i\right)}\right]}.
\end{equation}
Note that the ground truth confidence $Q^*$ varies during training unlike existing confidence estimation approaches \cite{Poggi2016bmvc,Seki2016} in which $Q^*$ is fixed during training. 
	Our key contribution is to refine the cost volume during training to provide highly discriminative confidence features and refined disparity maps.
	Note that $Q^*$ is computed by comparing the resultant disparity map and the ground truth disparity map.
	Namely, the cost volume refinement (CVR) network evolves and improves the matching cost and its associated disparity map during training, leading to varying ground truth confidence $Q^*$.\vspace{-5pt}

\section{Validation}\label{chap3_sec:4}
So far we have explained the CNN-based approach to improve the accuracy of the confidence and disparity maps in a boosting manner.
	By evolving the training, the quality of intermediate disparity maps is improved implicitly in \figref{chap3_fig7_evolving}(d) when compared to an initial disparity map in \figref{chap3_fig7_evolving}(c). 
	However, the performance gain is still limited as no confidence map is involved in the cost volume refinement step~\cite{Shaked2017}. 
	In this section, we introduce three validatation methods to prove the effectiveness of our confidence measure in the post-processing step of the stereo matching pipeline.
	With the post-processing steps, the erroneous disparities are corrected using the estimated confidence map as shown in \figref{chap3_fig7_evolving}(f).
\vspace{-5pt}
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_init_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_depthOnly_conf.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_prop_depthOnly.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_matchOnly_conf.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_prop_matchOnly.png}}\\
	\vspace{-5pt}
	\subfigure[(g)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_ours_conf.png}}
	\subfigure[(h)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig5_joint/001_prop_ours.png}}\\
	\vspace{-5pt}
	\caption[Importance of a joint use of matching probability volume and disparity map in the confidence
	estimation]{Importance of a joint use of matching probability volume and disparity map in the confidence
		estimation: (a) left color image, (b) an initial disparity map
		estimated using MC-CNN \cite{Zbontar2015}. Confidence maps were
		estimated using the matching probability volume only in (c), disparity map only in (e),
		and both matching probability volume and disparity map in (g), respectively.
		(d), (f), and (h) represent disparity map refined using the confidence maps in (c), (e), and (g), respectively. By jointly using the matching probability volume and disparity map, our method provide reliable confidence estimation performance.}
	\label{chap3_fig5_joint}
\end{figure}    

\subsection{Cost Modulation Based Optimization}\label{chap3_sec:41}
Following \cite{Park2015}, we first incorporate the predicted confidence
map into stereo matching algorithms by modulating the refined cost volume
such that
\begin{equation}
	\widehat{C}_{i,d} = Q_i C'_{i,d} + (1-Q_i)\sum\nolimits_{d}{C'_{i,d}/d_\mathrm{max}}.
\end{equation}
After modulating the refined cost volume, the refined cost
of confident pixels remain unchanged while those of unconfident
pixels are flattened. Thus unconfident pixels can be easily
dominated by confident neighboring pixels in the optimization step.
To produce a final disparity map $\widehat{D}$, the modulated cost
function $\widehat{C}$ is then optimized using global
approaches such as SGM \cite{Hirschmuller2008} or belief propagation
\cite{Sun2003}.\vspace{-10pt}

\subsection{GCPs-Based Optimization}\label{chap3_sec:42}
The predicted confidence can also be incorporated in GCPs-based optimization as in \cite{Min2015}.
We first set reliable pixels that have a higher value than a threshold $\tau$
as the GCPs, and then globally propagate the initial
GCPs through an MRF-based optimization by minimizing the following energy function:
\begin{equation}\label{chap3_eq7}
	E_{GCP} = {\sum\limits_{i}\left(h_i(\widehat{D}_i-D_i)^2+\lambda_1{\sum\limits_{j \in \mathcal{N}^4_i}} w^{I}_{i,j}(\widehat{D}_i-\widehat{D}_j)^2\right)},
\end{equation}
where $h_i$ is the binary mask to indicate the GCPs, and
$\widehat{D}_i$ is output disparity map. $w^I_{i,j}$ is the affinity
between $i$ and $j$ in the feature space consisting of color $I$
and spatial location, and
$\mathcal{N}^4_i$ represents a local 4-neighborhood. This
simple quadratic optimization can be efficiently solved using \cite{Min2015}.\vspace{-10pt}
% Component Analysis
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_right.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_init_depth.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_gt_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_res_depth_supOnly.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig6_loss/001_res_depth_ours.png}}\\
	\vspace{-5pt}
	\caption[Importance of a semi-supervised loss for learning the matching probability construction network]{Importance of a semi-supervised loss for learning the matching probability construction network: (a) left and (b) right color images, (c) an initial disparity map
		estimated using MC-CNN \cite{Zbontar2015}, (d) sparse ground truth disparity map. Disparity maps estimated from matching probability construction network
		learned (e) with only supervised loss ($\mathcal{L}_{sup}$) and (f) with semi-supervised loss ($\mathcal{L}_{sup}$ and $\mathcal{L}_{unsup}$). The errors within the regions where the ground truth is not defined are efficiently removed with unsupervised loss.}
	\label{chap3_fig6_loss}
\end{figure}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_gt_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_init_depth.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_estimated_depth.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_prop_icip_depth.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_final/fig7_evolving/011_prop_depth.png}}\\
	\vspace{-5pt}
	\caption[The effectiveness of the proposed matching probability volume network]{The effectiveness of the proposed matching probability volume network: (a) left color image, (b) sparse ground truth disparity map, (c) an initial disparity map estimated using MC-CNN \cite{Zbontar2015}, (d) an intermediate disparity map obtained by the proposed matching probability volume network. (e) and (f) represent refined disparity map of (c) and (d), respectively.}
	\label{chap3_fig7_evolving}
\end{figure}

\subsection{Aggregated GCPs-Based Optimization}\label{chap3_sec:43}
We further utilize an aggregated data term to mitigate propagation errors by
inaccurately estimated confidences when interpolating a sparse
disparity map obtained by thresholding the confidence
map. It was shown in \cite{Min2015} that a more robust data
constraint using an aggregated data term leads to a better quality
in the sparse data interpolation. %Similar methodology has also been
%used in \cite{Kim2017tip,Poggi2017cvpr}. They attempted to improve
%the accuracy of the confidence estimation by filtering the estimated
%confidence map. 
In this regard, we define the energy function as
follows:
\begin{equation}\label{chap3_eq7}
	\begin{split}
		& \noindent E_{AGCP} = \\
		& \sum\limits_{i}\left({\sum\limits_{r \in \mathcal{M}_i} h_r c^I_{i,r}(\widehat{D}_i-D_r)^2}
		+\lambda_2{\sum\limits_{j \in \mathcal{N}^4_i}} w^I_{i,j}(\widehat{D}_i-\widehat{D}_j)^2\right),
	\end{split}
\end{equation}
where $\mathcal{M}_i$ represents a set of neighborhoods used to
aggregate the disparity map filtered out with the confidence $Q$. Note that $\mathcal{M}_i$ is not
limited to $\mathcal{N}_4$ neighbors, but usually more neighbors are
used for ensuring a large support according to \cite{Min2015}. We
define $c^I_{i,r}$ using a bilateral kernel between pixel $i$ and $r$
in the feature space consisting of color intensity $I$, spatial location, and
estimated confidence as used in \cite{Kim2017tip}. $w^I_{i,j}$ is defined similar to the above section. This optimization can also be efficiently solved using constant-time edge-aware filtering and sparse matrix solver \cite{Min2015}.\vspace{-5pt}

\begin{table}[t!]
	\caption{Experimental configuration.}\vspace{5pt}
	\begin{center}
		\begin{tabular}{>{\raggedright}m{0.16\linewidth}|
				>{\centering}m{0.14\linewidth} >{\centering}m{0.14\linewidth}|
				>{\centering}m{0.16\linewidth} >{\centering}m{0.14\linewidth}}
			\hlinewd{0.8pt}
			Raw cost & \multicolumn{4}{c}{Census-SGM / MC-CNN}  \tabularnewline
			\hline
			\multirow{2}{*}{Training Set} & \multicolumn{2}{c|}{\multirow{2}{*}{MPI Sintel}} & \multicolumn{2}{c}{KITTI 2012 (w/GT)} \tabularnewline
			& & & \multicolumn{2}{c}{+ KITTI raw data (wo/GT)} \tabularnewline
			\hline
			Testing Set & MID 2006 & MID 2014 & \multicolumn{2}{c}{KITTI 2015} \\
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap3_tab1}
\end{table}

\section{Experimental Results}\label{chap3_sec:5}
\subsection{Experimental Settings}\label{chap3_sec:51}
In the following, we evaluated the proposed method compared to conventional shallow classifier based approaches such as Haeusler et al. \cite{Haeusler2013}, Spyropoulos et al. \cite{Spyropoulos2014}, Park and Yoon \cite{Park2015}, Poggi and Mattoccia (O(1)) \cite{Poggi20163dv}, Kim et al. \cite{Kim2017tip}, and CNN-based approaches such as Poggi and Mattoccia \cite{Poggi2016bmvc}, Seki and Pollefey \cite{Seki2016}, and Shaked et al. \cite{Shaked2017}.
We obtained the results of \cite{Park2015} by using the author-provided MATLAB code,
while the results of \cite{Haeusler2013}, \cite{Spyropoulos2014}, \cite{Seki2016}, and \cite{Shaked2017}
were obtained using our own MATLAB implementation. For \cite{Poggi20163dv} and \cite{Poggi2016bmvc}, we re-impelemented the algorithms based on author's lua code.
For an evaluation, we used the Middlebury (MID) 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and MPI \cite{MPI} dataset taken or synthesized under carefully-controlled environments, and
real-world datasets as KITTI \cite{KITTIdataset}, as described in \tabref{chap3_tab1}. For
MID 2006 and MID 2014, we trained the classifier using 981 images in the MPI dataset
and for KITTI 2015 dataset, we
trained the classifier using 194 stereo pairs in KITTI 2012 dataset \cite{KITTIdataset} for supervised loss $\mathcal{L}_{sup}$, and 40,000 raw stereo image pairs for unsupervised loss $\mathcal{L}_{unsup}$.
To evaluate the performance of the confidence measure quantitatively,
we used the sparsification curve and its area under curve (AUC) as in
\cite{Haeusler2013,Spyropoulos2014,Park2015,Seki2016}. The sparsification
curve draws a bad pixel rate while successively removing
pixels in descending order of confidence values in the
disparity map, thus it enables us to observe the tendency of
prediction errors. AUC quantifies the ability of a confidence
measure to estimate correct matches.
The higher the accuracy of
the confidence measure is, the lower the AUC value is. To evaluate
the disparity refinement performance using the estimated confidence map, we also measured the average bad matching
percentage (BMP) as in \cite{Scharstein2007}.\vspace{-10pt}

\subsection{Implementation Details}\label{chap3_sec:52}
Our networks are trained in an end-to-end manner, given the raw cost volume as an input and the ground truth disparity and ground truth confidence as outputs.
For training and testing networks, we used the {\ttfamily VLFeat MatConvNet toolbox} \cite{Matconvnet}. We make use of the stochastic gradient descent with momentum, and set the learning rate $1e-4$ and the batch size 50. The proposed method was implemented in MATLAB and was simulated on a PC with TitanX GPU.
To compute a raw matching cost, we used a census transform with
a $5\times5$ local window followed by SGM and the matching cost
with a convolutional neural network (MC-CNN) method
\cite{Zbontar2015}. For computing the MC-CNN, `KITTI 2012 fast network' was used, provided at the
author's website \cite{MCCNN}. For the census transform,
we applied SGM \cite{Hirschmuller2008} on
the estimated cost volume by setting $P_1 = 0.008$ and $P_2 = 0.126$ as in \cite{Park2015}. 
We set $\rho$ to 0.9 at which the density of confident regions used in the loss computation becomes 75\% on average. The flatness parameter $\sigma$ for obtaining the matching probability volume is set as 100 and 0.05 for SGM and MC-CNN respectively, according to their relative scales. The pre-defined number of epoch was set empirically to 200 at which the networks is pre-trained and converged with the supervised loss only. The hyper-parameter $\lambda$ is set to 1.\vspace{-10pt}
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/K_mid2006.pdf}}
	\subfigure[(a)]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/K_mid2014.pdf}}	
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/K_kitti2015.pdf}}\\
	\vspace{-5pt}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/L_mid2006_v2.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/L_mid2014_v2.pdf}}
	\subfigure[]
	{\includegraphics[width=0.3\linewidth]{Figure_final/fig8_component/L_kitti2015_v2.pdf}}\\
	\vspace{-5pt}
	\caption[Ablation study]{Ablation study: (a) Average AUC value of different $K$ for top-$K$ pooling layer and (b) different level of multi-scale $L$ for MID 2006, MID 2014, and KITTI 2015 dataset (from left to right). The raw matching cost is MC-CNN \cite{Zbontar2015}.}\label{chap3_fig8_component}
\end{figure}
% Sparsification curve
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/04_mid2006SGM.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/15_mid2006SGM.pdf}}
	\subfigure[(c)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/20_mid2006SGM.pdf}}\\
	\vspace{-5pt}
	\subfigure[(d)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/09_mid2014MCCNN.pdf}}
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/14_mid2014MCCNN.pdf}}
	\subfigure[(f)]
	{\includegraphics[width=0.32\linewidth]{Figure_final/fig9_sparsification/18_mid2014MCCNN.pdf}}\\
	\vspace{-5pt}
	\caption[Sparsification curve for MID 2006 and MI 2014 dataset]{Sparsification curve for (a) `Baby3', (b) `Midd2', and (c) `Wood1' images selected from the MID 2006 dataset \cite{Scharstein2007} using census-SGM, and (d) `Mask', (e) `Playtable', and (f) `Sticks' images selected from the MID 2014 dataset \cite{Scharstein2014} using MC-CNN. The sparsification curve for a ground truth confidence map is described as `optimal'.}\label{chap3_fig9_sparsification}
\end{figure}
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.45\linewidth]{Figure_final/fig10_auc/KITTI2015_SGM.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.45\linewidth]{Figure_final/fig10_auc/KITTI2015_MCCNN.pdf}}\\
	\vspace{-5pt}
	\caption[AUC values for KITTI 2015 dataset]{AUC values of (a) census-based SGM and (b) MC-CNN for the KITTI 2015 dataset \cite{KITTIdataset}. We sort the AUC values in the ascending order according to the proposed AUC values. The `optimal' AUC values are calculated using ground truth confidence map.}
	\label{chap3_fig10_auc}
\end{figure}
% AUC
\begin{sidewaystable}[t!]
	\caption[The average AUC values for MID 2006, MID 2014, and KITTI 2015 dataset]{The average AUC values for MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset. The AUC value of ground truth confidence is measured as `optimal'. The result with the lowest AUC value in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.2\linewidth} |
				>{\centering}m{0.09\linewidth}   >{\centering}m{0.09\linewidth} |
				>{\centering}m{0.09\linewidth}   >{\centering}m{0.09\linewidth} |
				>{\centering}m{0.09\linewidth}   >{\centering}m{0.09\linewidth} }
			\hlinewd{0.8pt}
			Dataset & \multicolumn{2}{ c |}{MID 2006 \cite{Scharstein2007}}
			& \multicolumn{2}{ c | }{MID 2014 \cite{Scharstein2014}}
			& \multicolumn{2}{ c }{KITTI 2015 \cite{KITTIdataset}} \tabularnewline
			\hline
			Raw cost
			& {Census-SGM}
			& {MC-CNN}
			& {Census-SGM}
			& {MC-CNN}
			& {Census-SGM}
			& {MC-CNN}\tabularnewline
			\hline
			\hline
			$\;$Haeusler et al. \cite{Haeusler2013}          &0.0454 &0.0417 &0.0841 &0.0750 &0.0585 &0.0308  \tabularnewline
			$\;$Spyropoulos et al. \cite{Spyropoulos2014}    &0.0447 &0.0420 &0.0839 &0.0752 &0.0536 &0.0323 \tabularnewline
			$\;$Park and Yoon \cite{Park2015}                       &0.0438 &0.0426 &0.0802 &0.0734 &0.0527 &0.0303  \tabularnewline
			$\;$Poggi et al. (O(1)) \cite{Poggi20163dv}      &0.0439 &0.0413 &0.0791 &0.0707 &0.0461 &0.0263  \tabularnewline
			$\;$Kim et al. \cite{Kim2017tip}                 &0.0430 &0.0409 &0.0772 &0.0701 &0.0430 &0.0294   \tabularnewline            
			$\;$Poggi et al. \cite{Poggi2016bmvc}            &0.0454 &0.0402 &0.0769 &0.0716 &0.0419 &0.0258  \tabularnewline
			$\;$Seki et al. \cite{Seki2016}                  &0.0462 &0.0413 &0.0791 &0.0718 &0.0439 &0.0272   \tabularnewline
			$\;$Shaked et al. \cite{Shaked2017}              &0.0464 &0.0495 &0.0806 &0.0736 &0.0531 &0.0292   \tabularnewline
			\hline
			$\;$Proposed wo/CVR  \cite{Kim2017icip}                               &0.0451 &0.0401 &0.0758 &0.0701 &0.0412 &0.0254   \tabularnewline
			$\;$Proposed wo/Top-$K$                             &0.0420 &0.0395 &0.0748 &0.0700 &0.0408 &0.0257   \tabularnewline
			$\;$Proposed wo/MDF                             &0.0423 &0.0392 &0.0741 &0.0697 &0.0411 &0.0252   \tabularnewline
			$\;$Proposed                                            &\textbf{0.0417}  &\textbf{0.0389}  &\textbf{0.0730}  &\textbf{0.0692}  &\textbf{0.0403} &\textbf{0.0247} \tabularnewline
			\hline
			$\;$Optimal                                          &0.0340  &0.0323  &0.0569  &0.0527  &0.0348  &0.0170  \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap3_tab2}
\end{sidewaystable}

% MID 2006 (SGM)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_kim2017_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_mod_cvpr2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_mod_kim2017.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_mod_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/03_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_kim2017_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_gcp_cvpr2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_gcp_kim2017.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_gcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/13_gcp_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_kim2017_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_agcp_cvpr2015.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_agcp_kim2017.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_agcp_ours.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_estimated_depth.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_sgm/01_agcp_gt.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on MID 2006 dataset using census-based SGM]{The confidence and refined disparity maps on MID 2006 dataset \cite{Scharstein2007} using census-based SGM+mod. (1st and 2nd rows), +GCPs (3rd and 4th rows), and +AGCPs (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Park and Yoon \cite{Park2015}, (c) Kim et al. \cite{Kim2017tip}, (d) proposed wo/CVR \cite{Kim2017icip}, (e) proposed, and (f) ground truth confidence map.}\label{chap3_fig11_1}
\end{figure}
\subsection{Component Analysis}\label{chap3_sec:53}
We first analyzed the performance of the proposed confidence
estimation method as varying the number of $K$ in top-$K$ pooling
and the scale $L$ for multi-scale disparity feature extraction in
confidence estimation network. AUC values as varying $K$ are shown
in \figref{chap3_fig8_component}(a). If $K$ is too small, the discriminative power
becomes low. As $K$ increases over 5, the AUC value is degraded
because of the redundancy. We set $K$ as 5 in all experiments. 
\figref{chap3_fig8_component}(b) shows the convergence anlysis for varying numbers of 
	scale $L$ from 1 to 8. 
	The AUC value decreases as $L$ increases, and converges after $L = 4$. Based on these experiments, we set $L = 4$ for considering the trade-off between accuracy and complexity. 

%As qualitative evalution measure, we evaluated the average AUC for estimating confidence
%with cost volume and matching probability volume respectively on (DATABASE?), as shown in \figref{}.
%As expected, the estimated confidence with raw cost volume
%has shown inferior performance compared to the performance of using the matching probability volume, showing the effectiveness of
%proposed matching probability construction network.
%The BMP of the depth estimation network with only supervised loss $\mathcal{L}_{sup}$ and
%with $\mathcal{L}_{unsup}$ are compared in \figref{}. (ADD comments)

%We set $L$ as 4 in all the experiments.
Moreover, for ablation experiments to validate the componets, we evaluated the proposed method without cost volume refinement network (Proposed wo/CVR)~\cite{Kim2017icip} which is the previous version of the proposed method, without top-$K$ pooling layer (Proposed wo/Top-$K$), and without multi-scale disparity feature extraction (Proposed wo/MDF) in quantitative results of average AUC values for various datasets as in \tabref{chap3_tab3}. Quantitative result also shows the effectiveness of multi-scale disparity feature extraction (Proposed wo/MDF) and top-$K$ pooling layer (Proposed wo/Top-$K$).\vspace{-10pt}
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_cvpr2013_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_mod_cvpr2013.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_mod_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_mod_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/02_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_cvpr2013_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gcp_cvpr2013.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gcp_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gcp_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/06_gcp_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_cvpr2013_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_agcp_cvpr2013.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_agcp_poggi.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_agcp_seki.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_agcp_ours.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig11_mid2006_mccnn/15_agcp_gt.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on MID 2006 dataset using MC-CNN]{The confidence and refined disparity maps on MID 2006 dataset \cite{Scharstein2007} using MC-CNN+mod. (1st and 2nd rows), +GCPs (3rd and 4th rows), and +AGCPs (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Haeusler et al.  \cite{Haeusler2013}, (c) Poggi et al. \cite{Poggi2016bmvc}, (d) Seki and Pollefeys \cite{Seki2016}, (e) proposed, and (f) ground truth confidence map.}\label{chap3_fig11_2}
\end{figure}

% MID 2014 (SGM)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_cvpr2014_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_mod_cvpr2014.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_mod_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_mod_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/09_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_cvpr2014_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_gcp_cvpr2014.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_gcp_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_gcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/20_gcp_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_cvpr2014_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_agcp_cvpr2014.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_agcp_poggi.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_agcp_ours.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_estimated_depth.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_sgm/15_agcp_gt.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on MID 2014 dataset using census-based SGM]{The confidence and refined disparity maps on MID 2014 dataset \cite{Scharstein2014} using  census-based SGM+mod. (1st and 2nd rows), +GCPs (3rd and 4th rows), and +AGCPs (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Spyropoulos et al. \cite{Spyropoulos2014}, (c) Poggi et al. \cite{Poggi2016bmvc}, (d) proposed wo/CVR \cite{Kim2017icip}, (e) proposed, and (f) ground truth confidence map.}\label{chap3_fig12_1}
\end{figure}

% MID 2014 (MCCNN)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_mod_cvpr2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_mod_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_mod_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/01_mod_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_gcp_cvpr2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_gcp_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_gcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_estimated_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/14_gcp_gt.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_estimated_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_gt_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_agcp_cvpr2015.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_agcp_poggi.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_agcp_ours.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_estimated_depth.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_final/fig12_mid2014_mccnn/07_agcp_gt.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on MID 2014 dataset using MC-CNN]{The confidence and refined disparity maps on MID 2014 dataset \cite{Scharstein2014} using MC-CNN+mod. (1st and 2nd rows), +GCPs.(3rd and 4th rows), and +AGCPs. (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Park and Yoon \cite{Park2015}, (c) Poggi et al. \cite{Poggi2016bmvc}, (d) proposed wo/CVR \cite{Kim2017icip}, (e) proposed, and (f) ground truth confidence map.}\label{chap3_fig12_2}
\end{figure}


% KITTI 2015 dataset (SGM)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_mod_o1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_mod_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/189_mod_ours.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_gcp_o1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_gcp_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/194_gcp_ours.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_agcp_o1.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_agcp_seki.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_sgm/117_agcp_ours.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on KITTI 2015 dataset using census-based SGM]{The confidence and refined disparity maps on KITTI 2015 dataset \cite{KITTIdataset} using  census-based SGM+mod. (1st and 2nd rows), +GCPs (3rd and 4th rows), and +AGCPs (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Poggi et al. O(1) \cite{Poggi20163dv}, (c) Seki and Pollefeys \cite{Seki2016}, and (d) ours.}\label{chap3_fig13_1}
\end{figure}

% KITTI 2015 dataset (MCCNN)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_mod_o1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_mod_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/085_mod_ours.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_gcp_o1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_gcp_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/006_gcp_ours.png}}\hfill
	\vspace{-8pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_o1_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_ours_conf.png}}\hfill
	\vspace{-8pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_agcp_o1.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_agcp_poggi.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figure_final/fig13_kitti2015_mccnn/155_agcp_ours.png}}\hfill
	\vspace{-8pt}
	\caption[The confidence and refined disparity maps on KITTI 2015 dataset using MC-CNN]{The confidence and refined disparity maps on KITTI 2015 dataset \cite{KITTIdataset} using MC-CNN+mod. (1st and 2nd rows), +GCPs (3rd and 4th rows), and +AGCPs (5th and 6th rows) (a) Color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Poggi et al. O(1) \cite{Poggi20163dv}, (c) Poggi et al. \cite{Poggi2016bmvc}, and (d) ours.}\label{chap3_fig13_2}
\end{figure}





\subsection{Confidence Measure Analysis}\label{chap3_sec:54}
We compared the AUC of our method with conventional learning-based approaches
using handcrafted confidence features \cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip}
and CNN-based methods \cite{Seki2016,Poggi2016bmvc,Shaked2017}.
%We used census-based SGM
%\cite{Zabih1994,Hirschmuller2008} and MC-CNN \cite{Zbontar2015} to obtain the initial disparity maps.
The optimal AUC can be obtained with a ground truth confidence map.
Sparsification curves for selected frames in the MID 2006 \cite{Scharstein2007} and MID
2014 dataset \cite{Scharstein2014} with census-based SGM and MC-CNN are
shown in \figref{chap3_fig9_sparsification}. The results have shown that the proposed
confidence estimator exhibits a better performance than conventional
handcrafted approaches
\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip}
and CNN-based approaches \cite{Poggi2016bmvc,Seki2016,Shaked2017}.
\figref{chap3_fig10_auc} describes the AUC values, which are sorted in
ascending order, for the KITTI 2015 dataset \cite{KITTIdataset} with
census-based SGM and MC-CNN respectively.
The handcrafted approaches showed inferior performance than the
proposed method due to low discriminative power of the handcrafted
confidence features. CNN-based methods
\cite{Poggi2016bmvc,Seki2016,Shaked2017} have improved confidence
estimation performance compared to existing handcrafted methods such
as \cite{Park2015}, but they are still inferior to our method as
they rely on either used only estimated disparity maps or cost
volume to predict unreliable pixels.

Further, to evaluate the robustness of the proposed top-$K$ pooling layer,
we perform experiments for cross-database and
the average AUC values for KITTI, MID, and MPI are summarized in~\tabref{chap3_tab3}.
In this experiment, we trained the network parameters using 8
frames in KITTI 2012 \cite{KITTIbenchmark} as used in
\cite{Seki2016} and 5 images in Middlebury 2006 (MID 2006)
\cite{Scharstein2007} and tested on 21 images in
Middlebury 2006 (MID), 23 images in MPI-Sintel (MPI), and 200 frames
in KITTI 2015 (KITTI). The matching
cost volume was computed with the MC-CNN \cite{Zbontar2015} (KITTI
2015 fast network provided by \cite{MCCNN}). The disparity search
range for KITTI \cite{KITTIdataset} and MID \cite{Middlebury} is 80
and for MPI \cite{MPI}, it varies for each image.
The results show that
the proposed confidence estimator exhibits a
better performance than conventional methods
\cite{Park2015,Seki2016} and the trained network using raw matching
cost volume (wo/Norm.) and matching probability volume (wo/Top-$K$). 
It shows that the method using proposed top-$K$ pooling layer
always achieves the lowest AUC values, demonstrating its outstanding
performance in predicting mismatched pixels of the disparity map.

% AUC table
\begin{sidewaystable}[t!]
	\caption{The average AUC values for KITTI 2015 \cite{KITTIdataset}, MID 2006 \cite{Scharstein2007}, and MPI \cite{MPI} dataset. The AUC value of ground truth confidence is measured as `optimal'. The result with the lowest AUC value in each experiment is highlighted.}\vspace{-5pt}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.25\linewidth}  |
				>{\centering}m{0.1\linewidth}   >{\centering}m{0.1\linewidth}
				>{\centering}m{0.1\linewidth} | >{\centering}m{0.1\linewidth}
				>{\centering}m{0.1\linewidth}   >{\centering}m{0.1\linewidth} }
			\hlinewd{0.8pt}
			{Training} & \multicolumn{3}{ c |}{KITTI 2012}
			& \multicolumn{3}{ c }{MID 2006}\tabularnewline
			\cline{1-7}
			{Testing} & KITTI 2015 & MID 2006 & MPI & KITTI 2015 & MID 2006 & MPI \tabularnewline
			\hline
			\hline
			$\;$Park and Yoon~\cite{Park2015}     &0.0258 &0.0427 &0.0243 &0.0281 &0.0411 &0.0282 \tabularnewline
			$\;$Seki and Pollefeys~\cite{Seki2016}     &0.0272 &0.0418 &0.0226 &0.0293 &0.0413 &0.0256 \tabularnewline
			\hline
			$\;$Proposed (wo/Norm.)                &0.0284 &0.0402 &-    &0.0351 &0.0425 &-
			\tabularnewline
			$\;$Proposed (wo/top-$K$)              &0.0256 &0.0400 &-    &0.0325 &0.0398 &-
			\tabularnewline
			$\;$Proposed                        &\textbf{0.0254} &\textbf{0.0396} &\textbf{0.0209} &\textbf{0.0269} &\textbf{0.0394} &\textbf{0.0209} \tabularnewline
			\hline
			$\;$Optimal                            &0.0170 &0.0330 &0.0155 &0.0170 &0.0330 &0.0155 \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}
	\label{chap3_tab3}\vspace{-18pt}
\end{sidewaystable}


The estimated confidence maps are shown in \figref{chap3_fig11_1} -
\figref{chap3_fig13_2}. The resultant confidence maps of our
method looks different since the confidence maps of ours were
obtained from the matching probability volume while others are
obtained from the raw matching cost volume. Note that the confidence map can also be predicted 
	directly from the matching cost volume without the CVR network, 
	named as `Proposed wo/CVR~\cite{Kim2017icip}' in Fig. 11 - Fig. 14.
	Experimental results demonstrate that the CVR network enables us to estimate more accurate confidence and disparity maps simultaneously in a boosting manner. Moreover, the average AUC
value with census-based SGM and MC-CNN for MID 2006, MID 2014, KITTI
2015 datasets were summarized in \tabref{chap3_tab3}. The proposed method
always yield the lowest AUC values, showing the superiority of the
proposed method compared to the existing CNN-based classifiers
\cite{Poggi2016bmvc,Seki2016,Shaked2017}.\vspace{-10pt}

% MID 2006 (MCCNN)

\subsection{Stereo Matching Analysis}\label{chap3_sec:55}
To verify the robustness of the confidence measures, we refined the
disparity map using the confidence maps estimated by several
confidence measure approaches including ours. For refining the
disparity maps, we used three different schemes described in Sec. 4,
which are cost modulation ( mod.) based optimization \cite{Park2015}
and GCPs-based optimization (GCPs) \cite{Xu2013}, and aggregated GCPs-based optimization (AGCPs) \cite{Min2015} without additional
post-processing to clearly show the performance gain achieved by the confidence measure. Note that there exist several literatures to evaluate the confidence measures, but this experiment is the first attempt to evaluate various confidence measures including both conventional methods and CNN-based methods in refining the disparity map. To evaluate the quantitative
performance, we measured an average BMP
for the  MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and
KITTI 2015 \cite{KITTIdataset} datasets. \tabref{chap3_tab4} and \tabref{chap3_tab5} show the BMP with one/three pixels when using census-based SGM and MC-CNN respectively. For MID 2006 and MID 2014, since there are occluded pixels in ground truth
disparity map, we computed the BMP only for visible
pixels. The KITTI 2015 benchmark provides a sparse ground truth disparity map
thus we evaluated the BMP only for sparse pixels with the ground truth
disparity values.
Note that the optimal percentage of BMP was obtained by measuring the ratio of erroneous pixels in which the absolute difference between the disparity map refined using ground truth confidence map and the ground truth disparity map is larger than one or three pixels, respectively.
The proposed method achieves the lowest BMP in all experiments.

% Qualitative
\figref{chap3_fig11_1} - \figref{chap3_fig13_2} display the disparity
maps refined with the confidence maps estimated from the existing
handcrafted classifiers \cite{Spyropoulos2014}, \cite{Park2015}, \cite{Poggi20163dv}, \cite{Kim2017tip}
CNN-based classifiers \cite{Poggi2016bmvc}, \cite{Seki2016}, \cite{Shaked2017} and
the proposed method. SGM modulation, GCPs-based optimization, and aggregated GCPs-based optimization were used to refine the
disparity maps for the MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and
KITTI 2015 \cite{KITTIdataset} datasets with census-based SGM and MC-CNN respectively. It was clearly shown that the erroneous matches
are reliably removed using the proposed confidence measure.
For the KITTI 2015 dataset \cite{KITTIdataset}, erroneous disparities usually
occur in textureless regions (sky and road) as shown in \figref{chap3_fig13_1} and \figref{chap3_fig13_2}. Conventional
	approaches~\cite{Poggi20163dv,Seki2016,Poggi2016bmvc} show the limited performance for detecting incorrect pixels in textureless regions, and thus they affect the matching quality of the subsequent
disparity estimation pipeline. In contrast, the proposed
method can detect mismatched pixels more reliably.\vspace{-5pt}

\section{Summary}\label{chap3_sec:6}
In this study, we have presented a learning framework for
estimating the stereo confidence through CNNs. We have shown that the
optimal confidence features can be learned from the matching
probability together with the disparity map.
The matching probability volume is first generated by refining and normalizing the matching cost volume, and then the confidence is estimated through deep networks with the matching probability and its corresponding disparity as inputs.
	Highly discriminative confidence features are learned by leveraging the multi-scale disparity features.
	Moreover, the proposed semi-supervised loss enables us to effectively learn the networks even with sparse ground truth disparity maps by using highly confident pixels of intermediate results for computing the image reconstruction loss.
	We validated the effectiveness of the proposed method by obtaining accurate and robust disparity maps on public datasets and challenging outdoor scenes through the depth refinement procedure using the estimated confidence map.

\begin{sidewaystable}[t!]
	\caption{The BMP of the resultant disparity map on MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset with census-based SGM. The bad pixel error rate of the refined disparity map using ground truth confidence is measured as `optimal'. The BMP is measured with one/three pixel errors. The result with the lowest BMP in each experiment is highlighted.}\vspace{-10pt}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.2\linewidth} |
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth} | >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth} |
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth} }
			\hlinewd{0.8pt}
			Dataset & \multicolumn{3}{ c |}{MID 2006 \cite{Scharstein2007}}
			& \multicolumn{3}{ c | }{MID 2014 \cite{Scharstein2014}}
			& \multicolumn{3}{ c }{KITTI 2015 \cite{KITTIdataset}} \tabularnewline
			\hline
			Validations &  +mod. &+GCPS. & +AGCPs. & +mod. &+GCPS. & +AGCPs.  & +mod. &+GCPS. & +AGCPs. \tabularnewline
			\hline
			\hline
			$\;$Initial disparity                            &\scriptsize{20.43/10.18} &\scriptsize{20.43/10.18} &\scriptsize{20.43/10.18} &\scriptsize{43.17/24.46} &\scriptsize{43.17/24.46} &\scriptsize{43.17/24.46}  &\scriptsize{23.50/18.67} &\scriptsize{23.50/18.67} &\scriptsize{23.50/18.67}   \tabularnewline
			$\;$Haeusler et al. \cite{Haeusler2013}          &\scriptsize{16.85/8.36} &\scriptsize{12.66/7.17} &\scriptsize{11.82/7.06} &\scriptsize{38.64/16.55} &\scriptsize{35.45/12.83} &\scriptsize{33.66/10.81}  &\scriptsize{17.51/15.19} &\scriptsize{13.71/11.82} &\scriptsize{11.56/10.18}   \tabularnewline
			$\;$Spyropoulos et al. \cite{Spyropoulos2014}    &\scriptsize{15.73/7.94} &\scriptsize{12.44/6.89} &\scriptsize{11.36/6.51} &\scriptsize{36.19/16.35} &\scriptsize{32.29/12.26} &\scriptsize{31.97/10.62}  &\scriptsize{17.08/14.81} &\scriptsize{13.18/11.36} &\scriptsize{11.46/9.59}   \tabularnewline
			$\;$Park and Yoon \cite{Park2015}                &\scriptsize{14.40/7.12} &\scriptsize{11.22/6.35} &\scriptsize{10.98/6.03} &\scriptsize{35.83/15.75} &\scriptsize{31.08/11.79} &\scriptsize{29.16/10.15}  &\scriptsize{16.92/14.02} &\scriptsize{12.57/9.76} &\scriptsize{10.37/9.18}   \tabularnewline
			$\;$Poggi et al. (O(1)) \cite{Poggi20163dv}      &\scriptsize{14.46/6.85} &\scriptsize{10.80/5.94} &\scriptsize{9.58/5.77}  &\scriptsize{34.17/14.37} &\scriptsize{30.52/10.06} &\scriptsize{27.03/9.90}   &\scriptsize{16.22/13.51} &\scriptsize{10.22/9.08} &\scriptsize{9.69/8.12}    \tabularnewline
			$\;$Kim et al. \cite{Kim2017tip}                 &\scriptsize{13.77/6.13} &\scriptsize{8.77/5.17}  &\scriptsize{7.72/5.08}  &\scriptsize{32.09/14.96} &\scriptsize{28.76/9.75}  &\scriptsize{23.74/8.53}   &\scriptsize{14.97/12.68} &\scriptsize{9.86/8.43}  &\scriptsize{8.50/7.08}    \tabularnewline
			$\;$Poggi et al. \cite{Poggi2016bmvc}            &\scriptsize{13.82/6.14} &\scriptsize{8.62/4.86}  &\scriptsize{7.84/4.63}  &\scriptsize{31.59/13.51} &\scriptsize{28.71/9.39}  &\scriptsize{23.98/8.89}   &\scriptsize{14.22/12.13} &\scriptsize{9.91/8.11}  &\scriptsize{8.68/6.79}    \tabularnewline
			$\;$Seki et al. \cite{Seki2016}                  &\scriptsize{13.39/5.96} &\scriptsize{7.37/4.57}  &\scriptsize{7.62/4.02}  &\scriptsize{31.13/13.34} &\scriptsize{27.13/8.75}  &\scriptsize{23.16/8.88}   &\scriptsize{14.48/11.96} &\scriptsize{8.85/7.03}  &\scriptsize{7.56/6.46}    \tabularnewline
			$\;$Shaked et al. \cite{Shaked2017}              &\scriptsize{16.43/8.06} &\scriptsize{11.77/7.21} &\scriptsize{10.42/7.18} &\scriptsize{37.98/16.52} &\scriptsize{34.11/12.07} &\scriptsize{32.08/11.41}  &\scriptsize{17.88/15.95} &\scriptsize{13.22/10.58} &\scriptsize{12.68/10.41}   \tabularnewline
			\hline
			$\;$Proposed                                       &\scriptsize{\textbf{11.44/5.86}}  &\scriptsize{\textbf{6.82/4.13}}  &\scriptsize{\textbf{6.75/3.69}}  &\scriptsize{\textbf{28.81/13.01}}  &\scriptsize{\textbf{25.63/8.53}} &\scriptsize{\textbf{22.18/8.04}} &\scriptsize{\textbf{13.10/10.68}} &\scriptsize{\textbf{8.03/6.74}} &\scriptsize{\textbf{7.14/6.12}}  \tabularnewline
			\hline
			$\;$Optimal                                      &\scriptsize{7.46/3.67}  &\scriptsize{4.20/2.19}  &\scriptsize{3.45/1.97}  &\scriptsize{23.65/8.00}  &\scriptsize{21.12/6.37}  &\scriptsize{20.53/5.27} &\scriptsize{7.75/6.03} &\scriptsize{5.46/3.86} &\scriptsize{4.57/3.51}   \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap3_tab4}\vspace{-10pt}
\end{sidewaystable}


% bad matching percentage result for MC-CNN
\begin{sidewaystable}
	\caption{The BMP of the resultant disparity map on MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset with MC-CNN. The BMP of the refined disparity map using ground truth confidence is measured as `optimal'. The BMP is measured with one/three pixel errors. The result with the lowest BMP in each experiment is highlighted.}\vspace{-10pt}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.2\linewidth} |
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth} | >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth} |
				>{\centering}m{0.065\linewidth}   >{\centering}m{0.065\linewidth}
				>{\centering}m{0.065\linewidth} }
			\hlinewd{0.8pt}
			Dataset & \multicolumn{3}{ c |}{MID 2006 \cite{Scharstein2007}}
			& \multicolumn{3}{ c | }{MID 2014 \cite{Scharstein2014}}
			& \multicolumn{3}{ c }{KITTI 2015 \cite{KITTIdataset}} \tabularnewline
			\hline
			Validations &  +mod. &+GCPs. & +AGCPs. & +mod. &+GCPs. & +AGCPs.  & +mod. &+GCPs. & +AGCPs. \tabularnewline
			\hline
			\hline
			$\;$Initial disparity                            &\scriptsize{17.04/8.31} &\scriptsize{17.04/8.31} &\scriptsize{17.04/8.31} &\scriptsize{39.56/20.69} &\scriptsize{39.56/20.69} &\scriptsize{39.56/20.69}  &\scriptsize{20.62/15.79} &\scriptsize{20.62/15.79} &\scriptsize{20.62/15.79}   \tabularnewline
			$\;$Haeusler et al. \cite{Haeusler2013}          &\scriptsize{13.76/7.10} &\scriptsize{11.11/6.89} &\scriptsize{9.49/6.13}  &\scriptsize{35.41/15.83} &\scriptsize{32.16/13.58} &\scriptsize{31.18/11.48}  &\scriptsize{16.05/12.16} &\scriptsize{14.06/10.68} &\scriptsize{12.31/10.34}   \tabularnewline
			$\;$Spyropoulos et al. \cite{Spyropoulos2014}    &\scriptsize{13.28/7.02} &\scriptsize{10.83/6.57} &\scriptsize{9.62/5.86}  &\scriptsize{34.12/15.46} &\scriptsize{31.68/12.96} &\scriptsize{30.64/11.02}  &\scriptsize{15.87/11.84} &\scriptsize{12.95/8.84} &\scriptsize{11.31/8.61}   \tabularnewline
			$\;$Park and Yoon \cite{Park2015}                &\scriptsize{13.14/6.86} &\scriptsize{10.63/6.03} &\scriptsize{9.33/5.72}  &\scriptsize{33.68/14.92} &\scriptsize{30.71/11.69} &\scriptsize{28.31/10.71}  &\scriptsize{15.04/11.44} &\scriptsize{12.18/8.36} &\scriptsize{11.28/8.12}   \tabularnewline
			$\;$Poggi et al. (O(1)) \cite{Poggi20163dv}      &\scriptsize{11.90/6.39} &\scriptsize{9.82/5.85}  &\scriptsize{8.28/5.15}  &\scriptsize{32.29/13.75} &\scriptsize{29.65/10.00}  &\scriptsize{27.19/9.44}  &\scriptsize{13.95/10.97} &\scriptsize{11.67/8.12} &\scriptsize{10.46/7.97}   \tabularnewline
			$\;$Kim et al. \cite{Kim2017tip}                 &\scriptsize{12.41/6.18} &\scriptsize{9.94/5.12}  &\scriptsize{8.35/4.93}  &\scriptsize{32.48/13.76} &\scriptsize{28.11/9.92}  &\scriptsize{26.47/9.42}   &\scriptsize{14.16/10.83} &\scriptsize{10.84/7.79} &\scriptsize{9.72/7.54}   \tabularnewline
			$\;$Poggi et al. \cite{Poggi2016bmvc}            &\scriptsize{11.60/6.02} &\scriptsize{9.73/4.63}  &\scriptsize{8.23/4.13}  &\scriptsize{29.81/13.34} &\scriptsize{27.13/9.87}  &\scriptsize{25.71/9.23}   &\scriptsize{14.04/10.08} &\scriptsize{9.65/7.41}  &\scriptsize{8.83/7.11}    \tabularnewline
			$\;$Seki et al. \cite{Seki2016}                  &\scriptsize{11.35/5.78} &\scriptsize{9.64/4.71}  &\scriptsize{7.80/4.02}  &\scriptsize{28.63/12.99} &\scriptsize{26.57/9.34}  &\scriptsize{24.56/8.88}   &\scriptsize{14.37/9.86} &\scriptsize{9.32/6.96}  &\scriptsize{9.02/6.63}   \tabularnewline
			$\;$Shaked et al. \cite{Shaked2017}              &\scriptsize{13.29/6.92} &\scriptsize{12.14/6.92} &\scriptsize{10.46/6.11} &\scriptsize{35.97/16.23} &\scriptsize{31.86/13.92} &\scriptsize{30.76/11.12}  &\scriptsize{16.47/11.18} &\scriptsize{14.04/9.57} &\scriptsize{12.05/10.13}   \tabularnewline
			\hline
			$\;$Proposed                                     &\scriptsize{\textbf{10.65/5.65}}  &\scriptsize{\textbf{8.79/4.03}}  &\scriptsize{\textbf{6.90/3.71}}  &\scriptsize{\textbf{26.71/10.98}} &\scriptsize{\textbf{23.19/8.78}} &\scriptsize{\textbf{22.18/8.15}}  &\scriptsize{\textbf{13.16/9.12}}  &\scriptsize{\textbf{8.03/6.18}}  &\scriptsize{\textbf{7.80/5.98}}  \tabularnewline
			\hline
			$\;$Optimal                                      &\scriptsize{5.92/2.11}  &\scriptsize{4.55/1.84}  &\scriptsize{4.02/1.56}  &\scriptsize{21.87/7.70}  &\scriptsize{18.79/5.87}  &\scriptsize{17.61/4.54}  &\scriptsize{7.29/5.94} &\scriptsize{4.30/3.65}  &\scriptsize{3.59/3.31}   \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap3_tab5}\vspace{-10pt}
\end{sidewaystable}

==> chap4.tex <==
\chapter{Adversarial Confidence Estimation Networks for Robust Stereo Matching}
\label{chap:chap4}

\section{Introduction}\label{chap4_sec:1}
Stereo matching for reconstructing 3-D geometric configuration of a scene is one of the fundamental and essential problems in computer vision and image processing~\cite{Hirschmuller2008,Min2008,Kim2014}. 
For decades, numerous methods have been proposed for this task by leveraging handcrafted~\cite{Yoon2008,Hirschmuller2008} and/or machine learning-based~\cite{Zbontar2015,Shaked2017} techniques. However, because of challenging elements such as reflective surfaces and textureless regions, repeated pattern regions, occlusions~\cite{Mei2011,Humenberger2010,Egnal2002}, or photometric deformations incurred by illumination or camera specification variations~\cite{Zabih1994,Heo2011}, the stereo matching still remains an unsolved problem.

To overcome these challenges, most approaches have involved the post-processing step in a manner that a set of unreliable disparities is first determined using confidence measures, and then refined using neighboring reliable disparities~\cite{Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip,Kim2017icip,Kim2018tip}. Conventionally, hand-designed confidence measures~\cite{Haeusler2013,Spyropoulos2014,Park2015,Kim2017tip} followed by shallow classifiers, such as random decision forest~\cite{Breiman2001,Liaw2002}, have been mainly used, but they have shown limited ability to predict the confidence accurately. 
Recent approaches have attempted to estimate the confidence by leveraging deep convolutional neural networks (CNNs) thanks to their high robustness~\cite{Poggi2016bmvc,Seki2016,Kim2017icip,Kim2018tip}, and have shown highly improved performance in comparison to handcrafted methods~\cite{Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip}. However, those aforementioned techniques estimate the confidence of a pre-determined initial disparity without considering an explicit module to improve the initial disparity accuracy simultaneoulsy, 
thus they provide limited performance improvement. 
Instead, these methods generally adopt the additional disparity refinement scheme~\cite{Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip} to refine the initial disparity using the estimated confidence.

To overcome this limitation, some methods~\cite{Shaked2017,Kim2018tip} have tried to simultaneously improve the qualities of disparity and its corresponding confidence through deep networks. Formally, they formulate two sub-networks that consist of cost aggregation and confidence estimation networks, and simultaneously learn two sub-networks during training. Although an intial disparity and confidence can be evolvingly improved in these frameworks, there does not exists a boosting mechanism that confidence estimation networks can help to improve the cost aggregation networks explicitly. 

More recently, generative adversarial networks (GANs)~\cite{Goodfellow2014} have achieved impressive results in numerous computer vision tasks~\cite{Zhang2016eccv,Zhang2017tog,Ledig2017,Pathak2016,	Radford2016}, by generating perceptually realistic solutions. 
Formally, by leveraging an adversarial learning technique, a generator is learned to generate fake images indistinguishable from real images by a discriminator~\cite{Goodfellow2014}. Some stereo matching approaches~\cite{Pu2018,Huang2017} also exploited the adversarial learning to estimate perceptually realistic disparity maps. However, there exists a limitation that they require dense ground-truth disparity maps to learn discriminator networks, which limits their applicability. In addition, there are no study to investigate how the discriminator networks can be used as the confidence estimator. 

In this paper, we introduce a novel network architecture and learning framework for overcoming the aforementioned limitations of conventional deep CNN-based confidence estimation techniques~\cite{Shaked2017,Kim2018tip}. Inspired by GANs~\cite{Goodfellow2014}, the key idea of our method is to design the cost aggregation and confidence estimation networks to be learned by the minmax optimization so that each network can be improved in an iterative and boosting fashion. Concretely, our networks consist of two sub-networks as shown in~\figref{chap4_fig1}, including generative cost aggregation and adversarial confidence estimation networks. 
Generative cost aggregation networks are learned to generate confident and un-confident samples, indistinguishable by adversarial confidence estimation networks. At the same time, adversarial confidence estimation networks are learned to distinguish confident and un-confident samples. By learning our networks in the minmax optimization fashion, the qualities of disparity and confidence maps, outputs of our networks, can be simultaneoulsy boosted.

Additionally, in order to fully exploit matching cost, disparity, and color image in confidence estimation, we use a dynamic fusion module in adversarial confidence estimation networks in a way that the optimal fusion weight is dynamically determined conditioned on each input. 
%Moreover, to provide more reliable performance, the active balancing of confidence and un-confidence samples is also considered.

We verify the proposed confidence estimation method using aggregated ground control points (AGCPs)-based
propagation as in~\cite{Kim2018tip}. The proposed approach is examined in an ablation study, and evaluated in comparison to conventional handcrafted and deep CNNs-based methods on various benchmarks, including Middlebury 2006 \cite{Scharstein2007}, Middlebury 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset}.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.8\linewidth]{Figure_GAN/fig1/Framework.pdf}}\\
	\vspace{-20pt}
	\caption[Our overall network configuration]{Our overall network configuration that consists of two sub-networks, including generative cost aggregation networks and adversarial confidence estimation networks. Given a left color image and a raw cost as inputs, our networks output disparity and its confidence maps.}\label{chap4_fig1}
\end{figure}

\section{Related Works}\label{chap4_sec:2}
\subsection{Handcrafted Confidence Measures}\label{chap4_sec:21}
Until the last few years, there have been extensive literatures in stereo confidence estimation, mainly based on handcrafted confidence measures~\cite{Egnal2002,Egnal2004,Mordohai2009}.
A comprehensive review by Hu and Mordohai~\cite{Hu2012} concluded that there is no single confidence feature
that yields stably optimal performance.
To solve this limitation, there have been various approaches to benefit from the feature combination among a different set of single confidence measures, and train a shallow classifier such as random decision forest~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv}. Haeusler et al. \cite{Haeusler2013} combined
confidence features consisting of left-right consistency, image gradient, and disparity variance.
Similar approach was also proposed in \cite{Spyropoulos2014}. 
However, the performance of the aforementioned methods is still limited since the selected confidence features are not optimal.
To select the set of (sub-)optimal confidence features among
multiple confidence features, Park and Yoon~\cite{Park2015} proposed to utilize the regression forest that computes the importance of confidence features and train the regression forest classifier using selected confidence features. Poggi and Mattoccia~\cite{Poggi20163dv} employed the set of confidence features from only disparity map that can be computed in O(1) complexity without losing the confidence estimation performance. While the aforementioned methods detect unconfident pixels in a pixel-level, Kim et al.~\cite{Kim2017tip} leveraged a spatial context to
estimate confidence in a superpixel-level by concatenating pixel- and superpixel-level confidence features. However, all of those methods used handcrafted confidence features, and they may not be optimal to detect unconfident pixels on challenging scenes. 

\subsection{Deep CNN-based Confidence Measures}\label{chap4_sec:22}
With the recent progress of deep CNNs, several approaches have been proposed to measure the stereo confidence through deep CNNs~\cite{Poggi2016bmvc,Seki2016,Poggi2017cvpr,Kim2017icip,Kim2018tip}.
A quantitative evaluation of confidence measures that use machine learning approaches has been performed in~\cite{Poggi2017iccv}. Formally, these CNN-based methods first extract the confidence features from only disparity~\cite{Poggi2016bmvc,Seki2016}, estimated confidence~\cite{Poggi2017cvpr}, or both disparity and cost volume~\cite{Kim2017icip,Kim2018tip}, and then predict the confidence. Specifically, in~\cite{Poggi2016bmvc}, a novel confidence estimation network was proposed that only uses a left disparity map as an input. Seki and Pollefeys~\cite{Seki2016} proposed to use both left and right disparity maps in deep networks for improving the confidence prediction accuracy. The confidence refinement networks~\cite{Poggi2017cvpr} were also developed, which can improve the accuracy of the measured confidence map by leveraging a local consistency within confidence map. 
Tosi et al.~\cite{Tosi2017} proposed a novel self-supervised strategy, which generates training labels by leveraging a pool of appropriately combined conventional confidence measures.
There have been attempts to benefit from the color image~\cite{Fu2018,Tosi2018}. They encode the local information to detect high frequency patterns, showing the improvement of confidence estimation. 
Although these aforementioned methods have shown competitive performance, they only estimate the confidence of initial disparity map without considering an explicit module to improve the initial disparity accuracy, thus they provide limited performance improvement.

Recently, some methods~\cite{Shaked2017,Kim2018tip} have tried to improve the qualities of disparity and its corresponding confidence simultaneoulsy. Formally, they formulate two sub-networks that consist of cost aggregation networks and confidence estimation networks, and simultaneously learn two sub-networks during training iterations. Shaked and Wolf~\cite{Shaked2017} jointly estimated both disparity and confidence maps. Kim et al.~\cite{Kim2018tip} also tried to estimate improved disparity and confidence maps through unified deep networks, but there exists the lack of the explicit mechanism to boost each network. 
Unlike these methods, we design an adversarial learning framework to boost cost aggregation and confidence estimation networks.

\subsection{Generative Adversarial Networks}\label{chap4_sec:23}
More recently, GANs~\cite{Goodfellow2014} have achieved impressive results in numerous computer vision and image processing applications, such as image colorization~\cite{Zhang2016eccv,Zhang2017tog}, image super-resolution~\cite{Ledig2017}, image inpainting~\cite{Pathak2016}, or represent learning~\cite{Radford2016}, enabling generating perceptually realistic solutions.
Formally, they take an adversarial loss that forces the generated images to be indistinguishable from real images by adversely learning the generator and discriminator networks. 

In stereo matching literatures, some methods~\cite{Pu2018,Huang2017} also exploited the adversarial learning to estimate perceptually realistic disparity maps. However, although they can boost the disparity estimation networks by using additional discriminator networks, they require dense ground-truth disparity maps to learn the discriminator networks, which limits their applicability on outdoor stereo image pairs such as KITTI benchmark~\cite{KITTIbenchmark}. Moreover, the discriminator networks in these methods cannot operate as confidence estimator, and there are no study to investigate how the discriminator networks can be used as the confidence estimator. Unlike these methods, we adopt an adversarial loss to learn the mapping function that the generated unconfident disparity cannot be distinguished from the generated confident disparity by using the confidence estimator, which can be learned only with sparse ground-truth disparity.

\section{Problem Statement}\label{chap4_sec:3}
\subsection{Confidence Estimation of Pre-determined Initial Depth}\label{chap4_sec:31}
Let us define a pair of stereo images $\{I^l,I^r\}$. The objective of stereo matching is to estimate a disparity $D_i$ between stereo images that is defined for each pixel $i = [i_\mathrm{x},i_\mathrm{y}]^T$ in $I^l$. To this end, the matching costs $C_{i,d}$ between $I^l_i$ and $I^r_{i'}$, where $i'=i-[d,0]^T$, among disparity candidates $d=\{1,...,d_\mathrm{max}\}$ are first measured, and then aggregated and/or optimized for computing a disparity $D_i$. 
Since most existing methods, including recent deep CNN-based methods~\cite{Zbontar2015,Kendall2017}, cannot provide fully reliable solutions due to inherent challenges of stereo matching, several approaches~\cite{Spyropoulos2014,Park2015,Seki2016,Kim2017tip,Kim2017icip} have employed an additional module to estimate a confidence $Q_i$ of an estimated disparity $D_i$. 

Formally, confidence estimation pipeline involves first extracting handcrafted~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip} or matchine learned~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Kim2017icip} features from color images, matching cost volumes, and/or disparity maps within local receptive fields, and then predicting the confidence of initial disparity map using shallow classifiers~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip} or deep convolutional neural networks~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Kim2017icip}. Especially, conventional methods estimate only the confidence $Q_i$ of pre-determined initial disparity map $D_i$. These methods generally adopt the disparity refinement scheme to refine the initial disparity $D_i$ using the estimated confidence $Q_i$. \vspace{-10pt}
%, such as matching cost modulation~\cite{Park2015} or ground control points (GCPs)-based propagation~\cite{Xu2013,Min2015}.

\subsection{Unified Depth and Confidence Estimation}\label{sec:32}
More recently, some methods~\cite{Shaked2017,Kim2018tip} have designed deep networks to simultaneoulsy improve the qualities of disparity $D_i$ and its confidence $Q_i$ at each training iteration. Concretely, these approaches formulate two modules as shown in~\figref{chap4_fig2}(a), including cost aggregation networks that provide the improved matching cost $C^t$ and disparity $D^t$ at $t$-th iteration from an initial cost $C$, i.e., $\{C^t,D^t\}=G(C|W_G)$ or $C^t=G^C(C|W_G)$ and $D^t=G^D(C|W_G)$\footnote{It should be noted that since $D^t$ is derived from $C^t$ with a soft-argmax~\cite{Shaked2017,Kim2018tip}, network parameters of $G^C$ and $G^D$ are shared as $W_G$.}, and confidence estimation networks that estimate the confidence $Q^t$, i.e., $Q^t=F(C^t,D^t|W_F)$, where $W_G$ and $W_F$ represent network parameters, respectively. For the sake of simplicity, let us represent $G(\cdot|W_G)$ and $F(\cdot|W_F)$ as $G(\cdot)$ and $F(\cdot)$, respectively.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.8\linewidth]{Figure_GAN/fig2/woGAN.pdf}}\\
	\subfigure[(b)]
	{\includegraphics[width=0.8\linewidth]{Figure_GAN/fig2/wGAN.pdf}}\\
	\vspace{-5pt}
	\caption[Intuition of our networks]{Intuition of our networks: (a) conventional unified depth and confidence estimation methods~\cite{Shaked2017,Kim2018tip} and (b) ours. Unlike existing methods~\cite{Shaked2017,Kim2018tip}, our networks, consisting of generative cost aggregation and adversarial confidence estimation networks, are designed to be learned in the minmax optimization fashion. Adversarial confidence estimation networks are learned to distinguish generated positive samples (i.e., $\hat{C}^{t}$ and $\hat{D}^{t}$) and generated negative samples using $\mathcal{L}_\mathrm{conf}(G,F)$. The derivative of $\mathcal{L}_\mathrm{conf}(G,F)$ with respect to generative cost aggregation networks is only backpropagated, which enables generative cost aggregation networks generate indistinguishable positive and negative samples that become more reliable samples.}\label{chap4_fig2}
\end{figure}

To learn these networks $\{G,F\}$ in an end-to-end manner, two loss functions can be used. First, to learn cost aggregation networks, the disparity regression loss can be generally used to directly regress the disparity $D^t = G^D(C)$ with respect to a ground-truth dispariy $D^*$ with $L_1$ norm~\cite{Kim2018tip} such that
\begin{equation}\label{loss_disp}
\mathcal{L}_\mathrm{disp}(G) = \mathbb{E}_{C\sim p_{data}(C)}{[\|G^D(C) - D^*\|_1]},
\end{equation}
where it is defined for all $C$ following the data distribution $p_{data}(C)$. Alternatively, $\mathcal{L}_\mathrm{disp}$ can also be defined as the cross-entropy loss~\cite{Shaked2017} with $C^t = G^C(C)$ and $D^*$. %It should be noted that network parameters of $G^C$ and $G^D$ are shared as $W_G$, thus learning $G$ only with $\mathcal{L}_\mathrm{disp}$ enables learning all cost aggregation network parameters $W_G$.

Second, to learn confidence estimation networks, the cross-entropy loss~\cite{Shaked2017,Kim2018tip} according to the ground-truth confidence $Q^*$ is generally used to estimate the confidence $Q$ that distinguishes confident and un-confident samples by maximizing the following energy function:
\begin{equation}\label{loss_conf}
\begin{split}
\mathcal{L}_\mathrm{conf}(G,F)  
&=\mathbb{E}_{C \sim p_{pos}(C)}[\log{F(G(C))}]\\
&\quad+\mathbb{E}_{C \sim p_{neg}(C)}[\log{(1-F(G(C)))}],
\end{split}
\end{equation}
where the first and second terms are defined for positive (or confident) and negative (or un-confident) samples, i.e., $C \sim p_{pos}(C)$ and $C \sim p_{neg}(C)$, respectively. In addition, to build positive and negative samples, the ground-truth confidence is defined such that $Q^* = T(|D^t-D^*|_1;\rho)$ with a truncation function $T$~\cite{Kim2018tip}, where $Q^*_i=1$ if $|D^t_i-D^*_i|_1<\rho$, $Q^*_i=0$ otherwise. 
Note that the ground-truth confidence $Q^*$ is actively varying according to the estimated disparity $D^t$ as evolving training iterations. 

The total loss function can be defined as $\mathcal{L}_\mathrm{disp}(G) + \lambda\mathcal{L}_\mathrm{conf}(G,F)$, where $\lambda$ controls the relative importance of the two objectives, and the networks can be learned by solving each corresponding loss function:
\begin{equation}\label{optimization_prev}
\{G^*,F^*\} =\arg\!\min_{G} \mathcal{L}_\mathrm{disp}(G)+ \lambda\arg\!\max_{G,F} \mathcal{L}_\mathrm{conf}(G,F).
\end{equation}
Since in these frameworks two networks $\{G,F\}$ are learned in an iterative manner, an initial disparity map $D$ and confidence map $Q$ can be evolvingly improved as $D^t$ and $Q^t$. Although these methods~\cite{Shaked2017,Kim2018tip} have shown the state-of-the-art performance compared to existing confidence estimation methods~\cite{Poggi2016bmvc,Seki2016} that use fixed ground-truth confidence $Q^*$ (i.e., $D^t=D$) during training, they have no explicit module such that confidence estimation networks $F$ improve the cost aggregation networks $G$ explicitly. 
By maximizing $\mathcal{L}_\mathrm{conf}(G,F)$, cost aggregation networks $G$ generates positive and negative samples that are well \emph{distinguished} by confidence estimation networks $F$, and cannot boost the ability of $G$ to generate reliable matching cost and disparity maps. 



\begin{figure*}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=1.0\linewidth]{Figure_GAN/fig3/CostAggregationNetwork.pdf}}\\
	\vspace{-15pt}
	\caption[Illustration of generative cost aggregation networks]{Illustration of generative cost aggregation networks $G$, consisting of a residual cost aggregation module, a normalization layer, a top-$K$ pooling layer, and a soft-argmax layer.}\label{chap4_fig3}
\end{figure*}

Moreover, existing deep confidence estimation networks~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Kim2017icip,Kim2018tip} have been formulated using matching cost only~\cite{Shaked2017}, disparity map only~\cite{Poggi2016bmvc,Seki2016}, unified matching cost and disparity map~\cite{Kim2017icip,Kim2018tip}, or color and disparity map~\cite{Fu2018,Tosi2018} as inputs, and they cannot benefit from the joint usage of tri-modal data, including matching cost, disparity, and color.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[]
	{\includegraphics[width=0.6\linewidth]{Figure_GAN/fig4/ConfidenceEstimationNetwork.pdf}}\\
	\vspace{-20pt}
	\caption[Illustration of adversarial confidence estimation networks]{Illustration of adversarial confidence estimation networks $F$, consisting of tri-modal feature extractors for color, disparity, and matching costs, an adaptive fusion module, and a confidence estimator.}\label{chap4_fig4}
\end{figure}

\section{Proposed Method}\label{chap4_sec:4}
\subsection{Motivation and Overview}\label{chap4_sec:41}
To alleviate aforementioned limitations of existing methods~\cite{Shaked2017,Kim2018tip}, we present a novel network architecture and learning technique, inspired by GANs~\cite{Goodfellow2014}. The proposed networks consist of two sub-networks, including \emph{generative cost aggregation networks} and \emph{adversarial confidence estimation networks}. The objective of our approach is to design the networks so that each network can be improved in an iterative and boosting manner. Toward this end, we design two networks to be learned in the minmax optimization fashion. Concretely, generative cost aggregation networks are designed to learn the mapping function from an initial cost $C$ to refind costs $C^t$ and disparity maps $D^t$ at $t$-th iterations such that $\{C^t,D^t\}=G(C|W_G)$. This mapping function is trained to generate positive (or confident) and negative (or un-confident) samples, \emph{indistinguishable} by adversarial confidence estimation networks. At the same time, adversarial confidence estimation networks are trained to distinguish positive and negative samples of refind costs $C^t$, disparity maps $D^t$, and color images $I^l$ with confidence $Q^t$ as following mapping: $Q^t=F(C^t,D^t,I^l|W_F)$. We formulate two networks $G$ and $F$ to play the two-player minimax game, thus they can be learned in a boosting fashion during training iterations, as illustrated in~\figref{chap4_fig2}(b). 

Moreover, by using an additional color image $I^l$, adversarial confidence estimation networks also provide edge-preserved confidence maps. 
To fully exploit tri-modality data consisting of matching cost $C^t$, and disparity $D^t$, and color image $I^l$, adversarial confidence estimation networks have the dynamic fusion module where the optimal fusion weight is dymanically determined conditioned on each input.

\subsection{Network Architectures}\label{chap4_sec:42}
\subsubsection{Generative Cost Aggregation Networks}
Similar to~\cite{Kim2018tip}, generative cost aggregation networks consist of a residual cost aggregation module, a normalization layer, and a top-$K$ pooling layer, as shown in~\figref{chap4_fig3}. 
Specifically, the networks first aggregate the raw matching cost $C$ using the encoder-decoder networks with skip layers similar to U-Net~\cite{Ronneberger2015}, consisting of sequential convolutional layers followed by batch normalization (BN) and rectified linear units (ReLU). In networks, we sequentially apply $2\times2$ max-pooling operators, resulting in a total down-sampling factor of $4$. In the decoding parts, the intermediate features are upsampled using bilinear deconvolutional filters~\cite{Jaderberg2015,Ronneberger2015}, and concatenated with corresponding encoder features using skip layers. With the residual sum, the refined matching cost $T^t$ at $t$-th iteration is estimated. Note that the network parameters $W_G$ are defined only on the residual cost aggregation module. Namely, there are no trainable parameters at following layers.

We also use the normalization scheme that generates the matching probability volume $P^t$ at $t$-th iteration to deal with the scale variation problems within cost volume~\cite{Kendall2017,Kim2017icip} as follows:
\begin{equation}
P^t_{i,d} = \frac{\exp({-R^t_{i,d}/\sigma})}
{\sum\nolimits_{u}{\exp({-R^t_{i,u}/\sigma})}},
\end{equation}	
where $u=\{1,...,d_\mathrm{max}\}$, and $\sigma$ is a hyper-parameter for adjusting the flatness of the matching cost. 

Furthermore, to deal with redundant parts in $P^t$ that distract the performance of confidence
estimation, we also use a top-$K$ pooling layer~\cite{Kim2018tip}, where $P^t$ is projected into a fixed
length, which is a refined cost $C^t$, as follows:
\begin{equation}
C^t_{i,k} = \textrm{max}^{k}_{d}{P^t_{i,d}},
\end{equation}
where $\textrm{max}^{k}(\cdot)$ is the $k$-th maximal value for $k =
\{1, ..., K\}$.

Finally, to estimate optimal disparity map $D^t$ at $t$-th iteration, we employ the soft-argmax layer~\cite{Kendall2017,Kim2018tip} as follows:
\begin{equation}
D^t_i = \sum\nolimits_{d} d \times P^t_{i,d}.
\end{equation}		

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/001_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/init_depth_MCCNN.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/res_conf_wColor.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/res_depth_wColor.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/res_conf_woColor.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig5/res_depth_woColor.png}}\\
	\vspace{-5pt}
	\caption[The effects of the color feature extractor in confidence estimation networks]{The effects of the color feature extractor in our confidence estimation networks: (a) a left color image, (b) an initial disparity map
		estimated using MC-CNN \cite{Zbontar2015}, (c) an estimated confidence map using cost and disparity as input, (d) a refined disparity map by (c) using AGCPs-based propagation, (e) an estimated confidence map using cost, disparity, and color, and (f) a refined disparity map by (e) using AGCPs-based propagation.
		With color feature extractor, an estimated confidence map effectively leverages a spatial context from a left color image.}
	\label{chap4_fig5}
\end{figure}

\subsubsection{Adversarial Confidence Estimation Networks}
Adversarial confidence estimation networks take tri-modal data consisting of refind matching cost $C^t$, disparity $D^t$, and color image $I^l$ as inputs, and output their corresponding confidence $Q^t$, as shown in~\figref{chap4_fig4}. Especially, unlike~\cite{Kim2018tip}, our confidence estimation networks additionally use the color information, enabling us to leverage a spatial context~\cite{Kim2017tip} and estimate edge-preserved confidence maps. \figref{chap4_fig5} shows the effectiveness of the proposed confidence estimation. Similar to generative cost aggregation networks, adversarial confidence estimation networks also consist of sequential convolutional filters, followed by BN and ReLU. The pooling operation is not used to preserve the spatial resolution.

Concretly, adversarial confidence estimation networks first extract convolutional features $f_{C^t}$, $f_{D^t}$, and $f_{I^l}$ from $C^t$, $D^t$, and $I^l$ through network parameters corresponding each modality feature extractor $W^C_F$, $W^D_F$, and $W^I_F$, respectively, and then fuse them. 
To fuse these tri-modality features, one simple solution is the concatenation of them as in~\cite{Kim2018tip}. However, this simple technique cannot guarantee the optimal fusion weights, since the fusion weights are learned during training and fixed at inference. To alleviate this limitation, inspired by~\cite{Jia2016}, we introduce an adaptive fusion module for a dynamic combination of $f_{C^t}$, $f_{D^t}$, and $f_{I^l}$, where the optimal fusion weight $W^{H,*}_F$ can be learned with respect to each input with an additional convolutional network such that $W^{H,*}_F=H(f_{C^t},f_{D^t},f_{I^l}|W^{H}_F)$ with network parameters $W^{H}_F$. Unlike the fixed fusion weights as in~\cite{Kim2018tip}, the $W^{H,*}_F$ is estimated conditioned on inputs, thus providing more optimal fusion solution, as shown in~\figref{chap4_fig6}. The confidence is finally estimated through remaining networks with parameters $W^{P}_F$. Following those, 
the confidence $Q^t$ can be estimated as
\begin{equation}
\begin{split}
Q^t &= F(C^t,D^t,I^l|W_F)\\
&= F(f_{C^t},f_{D^t},f_{I^l}|W^{H,*}_F,W^{P}_F)\\
&= F(f_{C^t},f_{D^t},f_{I^l}|H(f_{C^t},f_{D^t},f_{I^l}|W^{H}_F),W^{P}_F),
\end{split}
\end{equation}
where $W_F=\{W^{C}_F,W^{D}_F,W^{I}_F,W^{H}_F,W^{P}_F\}$. It should be noted that as in~\cite{Kim2018tip} multi-scale confidence features can also be used in our approach, but such a multi-scale scheme additionally increases the computational complexity, thus we do not consider multi-scale confidence features.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/075_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/init_depth_MCCNN.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/res_conf_concat.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/res_depth_concat.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/res_conf_df.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig6/res_depth_df.png}}\\
	\vspace{-5pt}
	\caption[The effects of the proposed dynamic fusion module in confidence estimation networks]{The effects of the proposed dynamic fusion module in our confidence estimation networks: (a) a left color image, (b) an initial disparity map
		estimated using MC-CNN \cite{Zbontar2015}, (c) an estimated confidence map by concatenation fusion, (d) a refined disparity map by (c) using AGCPs-based propagation, (e) an estimated confidence map by dynamic fusion, and (f) a refined disparity map by (e) using AGCPs-based propagation.
		Confidence map using dynamic fusion can detect unreliable disparities more accurately compared to concatenation fusion.}
	\label{chap4_fig6}
\end{figure}

\subsection{Loss Functions}\label{chap4_sec:43}
\subsubsection{Loss for Generative Cost Aggregation Networks}
To learn generative cost aggregation networks, we employ $L_1$ norm to directly regress the disparity with respect to a ground-truth disparity as a supervised loss function. However, since there exists the lack of dense ground-truth disparities especially under outdoor settings~\cite{KITTIbenchmark}, using the supervised loss function only cannot guarantee reliable performance. To overcome this, similar to~\cite{Kim2018tip}, we further employ an unsupervised loss function using an image reconstruction loss~\cite{Godard2017}. The loss function $\mathcal{L}_\mathrm{disp}(G)$ is defined as follows:
\begin{equation}\label{prop_loss_disp}
\begin{split}
\mathcal{L}_\mathrm{disp}(G)
=&\mathbb{E}_{C\sim p_{data}(C)}{[\|G^D(C) - D^*\|_1]}\\
&+\mathbb{E}_{C\sim p_{data}(C)}{[\|I^r(G^D(C)) - I^l\|_1]},
\end{split}
\end{equation}
where $I^r(G^D(C))$ is a warped right color image using an estimated disparity $G^D(C)$, implemented by a bilinear sampler~\cite{Jaderberg2015} that enables an end-to-end learning. It should be noted that using $\mathcal{L}_\mathrm{disp}$ only cannot guarantee the perceptually plausible disparity maps~\cite{Pu2018,Huang2017}. However, in our method, by learning generative cost aggregation networks $G$ with the loss function $\mathcal{L}_\mathrm{conf}$ for confidence estimation networks, which will be described in the following, as well as $\mathcal{L}_\mathrm{disp}$, more perceptually plausible disparity maps can be estimated. 

\subsubsection{Loss for Adversarial Confidence Estimation Networks}
To learn adversarial confidence estimation networks, we employ the cross-entropy loss function~\cite{Shaked2017,Kim2018tip} with respect to the ground-truth confidence map. However, unlike existing methods~\cite{Shaked2017,Kim2018tip}, we design the loss function $\mathcal{L}_\mathrm{conf}(G,F)$ to adversarially learn two networks $G$ and $F$. More importantly, we design the loss function such that adversarial confidence estimation networks $F$ distinguish positive and negative samples more discriminatively, while generative confidence estimation networks $G$ generate negative samples that have the distribution more similar to that of positive samples as evolving training iterations~\cite{Goodfellow2014}. Following this design strategy, the loss function $\mathcal{L}_\mathrm{conf}(G,F)$ is defined as follows:
\begin{equation}\label{prop_loss_conf_original}
\begin{split}
&\mathcal{L}_\mathrm{conf}(G,F)\\
&=\mathbb{E}_{\hat{C}^{t}\sim p_{pos}(C^t),\hat{D}^{t}\sim p_{pos}(D^t),I^{l}\sim p_{pos}(I^l)}[\log{F(\hat{C}^{t},\hat{D}^{t},I^{l})}]\\
&\quad+\mathbb{E}_{C\sim p_{neg}(C),I^l\sim p_{neg}(I^l)}[\log{(1-F(G(C),I^l))}],
\end{split}
\end{equation}
where $\hat{C}^t$ and $\hat{D}^t$ represent generated positive samples from generative cost aggregation networks $G$ with respect to the ground-truth confidence map $Q^*$. Importantly, although positive samples $\hat{C}^{t}$ and $\hat{D}^{t}$ are estimated from $G$, the derivative of $\mathcal{L}_\mathrm{conf}$ with respect to $G$ for positive samples cannot be backpropagated, while the derivative for negative samples is only backpropagated. 
As exemplified in~\figref{chap4_fig7}, by using the adversarial confidence loss $\mathcal{L}_\mathrm{conf}$, our method provides more plausible intermediate disparity and confidence maps.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/052_left.png}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/init_depth_MCCNN.png}}\\
	\vspace{-5pt}
	\subfigure[(c)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/res_depth_woGan.png}}
	\subfigure[(d)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/res_conf_woGan.png}}\\
	\vspace{-5pt}
	\subfigure[(e)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/res_depth_wGan.png}}
	\subfigure[(f)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig7/res_conf_wGan.png}}\\
	\vspace{-5pt}
	\caption[The effects of the proposed adversarial confidence loss]{The effects of the proposed adversarial learning technique: (a) a left color image, (b) an initial disparity map
		estimated using MC-CNN \cite{Zbontar2015}. (c) and (d) are an intermediate disparity map and an estimated confidence map without adversarial confidence learning, (e) and (f) are obtained with adversarial confidence learning. By learning the disparity map and confidence map in an adversarial manner, our method provides more plausible intermediate disparity and confidence maps.}
	\label{chap4_fig7}
\end{figure}

\subsubsection{Full Objective}
Similar to GANs~\cite{Goodfellow2014}, to learn our full networks consisting of generative cost aggregation networks and adversarial confidence estimation networks, we formulate the minmax optimization to simultaneoulsy boost each network. The total loss fuction $\mathcal{L}_\mathrm{total}$ is defined as follows:
\begin{equation} \mathcal{L}_\mathrm{total}(G,F) = \mathcal{L}_\mathrm{disp}(G) + \lambda\mathcal{L}_\mathrm{conf}(G,F),
\end{equation}
and the networks are then optimized in an adversarial fashion such that
\begin{equation}\label{optimization}
\begin{split}
\{G^*,F^*\} 
&=\arg\!\min_{G} \max_{F} {\mathcal{L}_\mathrm{total}(G,F)}\\
&=\arg\!\min_{G} \mathcal{L}_\mathrm{disp}(G)\\
&\quad+ \lambda\arg\!\min_{G} \max_{F} \mathcal{L}_\mathrm{conf}(G,F).
\end{split}
\end{equation}
Within this optimization, $G$ can be trained to generate the disparity map not only more similar to the ground-truth disparity map but also having indistinguishable positive and negative samples by $F$, thus providing more reliable and error-reduced disparity maps. 
With evolvingly improved hard positive and negative samples, the ability of confidence estimation of $F$ can also be improved at the same time. 

\section{Validation}\label{chap4_sec:4}
So far we have explained our network configurations and loss functions to improve the accuracies of the disparity and confidence map in an iterative and boosting manner. %By evolving training iterations, the quality of intermediate disparity maps is improved implicitly compared to an initial disparity map. 
%However, the performance gain is still limited as no confidence map is involved in the refinement step~\cite{Shaked2017}. 
In this section, we introduce the validatation method to prove the effectiveness of our confidence estimation method in the post-processing step of the stereo matching pipeline.

Concretley, as described in~\cite{Kim2018tip}, the predicted confidence
can be incorporated in AGCPs-based propagation as in~\cite{Min2015}.
First, we set GCPs that are classified as confident pixels in confidence estimation networks.
Then, we globally propagate the GCPs through an Markov random field (MRF)-based optimization.
We utilize an aggregated data term to mitigate propagation errors by
inaccurately estimated confidences. It was shown in \cite{Min2015} that a more robust data
constraint using an aggregated data term leads to a better quality
in the sparse data interpolation. In this regard, we define the energy function for refined disparity map $\bar{D}$ according to final disparity map $D'$ (i.e., $D^t$ after convergence) as follows:
\begin{equation}\label{eq7}
\begin{split}
& \sum\limits_{i}\left({\sum\limits_{v \in \mathcal{M}_i} h_v c^I_{i,v}(\bar{D}_i-D'_v)^2}
+\gamma{\sum\limits_{j \in \mathcal{N}^4_i}} w^I_{i,j}(\bar{D}_i-\bar{D}_j)^2\right),
\end{split}
\end{equation}
where $\mathcal{M}_i$ represents a set of neighborhoods, and is not
limited to a local 4-neighborhood, but more neighbors are used for ensuring a large support. We
define $c^I_{i,v}$ using a bilateral kernel between pixel $i$ and $v$
in the feature space consisting of color intensity $I$ and spatial location. $h_v$ is the binary mask to indicate the GCPs. Similar to $c^I_{i,v}$, $w^I_{i,j}$ is the affinity between $i$ and $j$ in the feature space consisting of color intensity $I$
and spatial location, and
$\mathcal{N}^4_i$ represents a local 4-neighborhood. $\gamma$ constrols the relative importance of data and smoothness terms. This
simple quadratic optimization can be efficiently solved using \cite{Min2015}.

% Convergence analysis : figure
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_woGan_ep1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_woGan_ep1.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_woGan_ep2.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_woGan_ep2.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_woGan_ep3.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_woGan_ep3.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_wGan_ep1.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_wGan_ep1.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_wGan_ep2.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_wGan_ep2.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_depth_wGan_ep3.png}}\hfill
	\subfigure[(g)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig8/010_conf_wGan_ep3.png}}\hfill
	\vspace{-5pt}
	\caption[Visualizations of intermediate disparity and confidence maps as evolving training iterations on MID 2006 dataset]{Visualizations of intermediate disparity and confidence maps as evolving training iterations on MID 2006 dataset~\cite{Scharstein2007}: 
		(a) a color image and an initial disparity, and results by (top) Kim et al.~\cite{Kim2018tip} and (bottom) Ours at each epoch of 50 in (b), (c), 100 in (d), (e), and 150 in (f), (g).}\label{chap4_fig8}
\end{figure}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/002_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/009_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/019_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_left.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_depth_woGan.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_conf_woGan.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_agcp_depth_woGan.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_depth_wGan.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_conf_wGan.png}}\hfill
	\subfigure[(g)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig9/020_agcp_depth_wGan.png}}\hfill
	\vspace{-5pt}
	\caption[Comparisons of unified depth and confidence estimation methods on MID 2006 dataset]{Comparisons of unified depth and confidence estimation methods on MID 2006 dataset~\cite{Scharstein2007}, using census-SGM (first two raws) and MC-CNN (last two rows): (a) color images, and final disparity, confidence, and refined disparity maps with propagation of (b), (c), (d) Kim at el.~\cite{Kim2018tip} and (e), (f), (g) Ours.}\label{chap4_fig9}
\end{figure}

\section{Experimental Results}\label{chap4_sec:4}
\subsection{Training Details}\label{chap4_sec:41}
In practice, when generative cost aggregation networks are poor at early stage during training, adversarial confidence estimation networks can easily distinguish generated samples because generated negative samples are clearly different from generated positive samples. In this case, $\log{(1-F(G(C),I^l))}$ in $\mathcal{L}_\mathrm{conf}$ easily saturates. To solve this, rather than training $G$ by minimizing $\log{(1-F(G(C),I^l))}$, we train $G$ to maximize $\log{F(G(C),I^l)}$ similar to~\cite{Goodfellow2014}, and thus the training optimization can be reformulated as follows:
\begin{equation}
\begin{split}
\{G^*,&F^*\} = \arg\!\min_G \mathcal{L}_\mathrm{disp}(G)
+\lambda\arg\!\max_F \mathcal{L}_\mathrm{conf}(G,F)\\
&+\lambda\arg\!\max_G \mathbb{E}_{C\sim p_{neg}(C),I^l\sim p_{neg}(I^l)}[\log{F(G(C),I^l)}],\\ 
\end{split}
\end{equation} 
This objective function results in the same fixed point of the dynamics of $G$ and $F$ but provides much stronger gradients at early strategy during training.

% MID 2014
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/001_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/013_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_agcp_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/022_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_left.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_agcp_depth_woGan.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.14\linewidth]{Figure_GAN/fig10/023_agcp_depth_wGan.png}}\hfill
	\vspace{-5pt}
	\caption[Comparisons of unified depth and confidence estimation methods on MID 2014 dataset]{Comparisons of unified depth and confidence estimation methods on MID 2014 dataset~\cite{Scharstein2014}, using census-SGM (first two raws) and MC-CNN (last two raws): (a) color images, and final disparity, confidence, and refined disparity maps with propagation of (b), (c), (d) Kim at el.~\cite{Kim2018tip} and (e), (f), (g) Ours.}\label{chap4_fig10}
\end{figure}

The proposed method was implemented in MATLAB with {\ttfamily VLFeat MatConvNet toolbox}~\cite{Matconvnet} and simulated on a PC with TitanX GPU. We make use of the stochastic gradient descent with momentum, and set the learning rate to $1\times 10^{-5}$ and the batch size to 20. To compute a raw matching cost, we used a census transform with
a $5\times5$ local window and MC-CNN~\cite{Zbontar2015}, respectively. 
For the census transform,
we applied SGM~\cite{Hirschmuller2008} on
estimated cost volumes by setting $P_1 = 0.008$ and $P_2 = 0.126$ as in \cite{Park2015}. 
For computing the MC-CNN, `KITTI 2012 fast network' was used, provided at the
author's website~\cite{MCCNN}. We set $\rho$ as 0.9 in all experiments, and $\sigma$ as 100 and 0.05 for census-SGM and MC-CNN, respectively.

\subsection{Experimental Settings}\label{chap4_sec:42}
In the following, we evaluated the proposed method in comparison to conventional shallow classifier-based approaches, such as Haeusler et al.~\cite{Haeusler2013}, Spyropoulos et al.~\cite{Spyropoulos2014}, Park and Yoon~\cite{Park2015}, Poggi and Mattoccia~\cite{Poggi20163dv}, Kim et al.~\cite{Kim2017tip}, and CNNs-based approaches using disparity only as an input, such as Poggi and Mattoccia (CCNN)~\cite{Poggi2016bmvc}, Seki and Pollefey (PBCP)~\cite{Seki2016}, matching cost only as an input, such as Shaked et al.~\cite{Shaked2017}, both disparity and matching cost as inputs, such as Kim et al.~\cite{Kim2018tip}, and both color and disparity as inputs, such as Fu et al. (LFN)~\cite{Fu2018}. We obtained the results of~\cite{Park2015} by using the author-provided code,
while the results of~\cite{Haeusler2013},~\cite{Spyropoulos2014},~\cite{Seki2016}, and~\cite{Shaked2017}
were obtained by our own implementation. For~\cite{Poggi20163dv} and~\cite{Poggi2016bmvc}, we re-impelemented them based on author-provided code.

Following experimental settings of~\cite{Kim2018tip}, we also seperately trained the networks for indoor and outdoor datasets.
For indoor setting, we used MPI dataset~\cite{MPI} and evaluated
the networks using Middlebury 2006 (MID 2006) dataset~\cite{Scharstein2007} and Middlebury 2014 (MID 2014) dataset~\cite{Scharstein2014}. 
We cropped the training database as 256 $\times$ 256-sized patches and used about 100,000 patches. For outdoor database, we used 194 stereo pairs on KITTI 2012 dataset~\cite{KITTIdataset} for the supervised loss and 40,000 raw stereo pairs for the unsupervised loss in $\mathcal{L}_\mathrm{disp}$, and evaluated the networks on KITTI 2015 dataset~\cite{KITTIdataset}. Note that to optimize the loss function  $\mathcal{L}_\mathrm{disp}$, consisting of supervised- and unsupervised losses, we used both supervised- and unsupervised losses after performing 200 epoches with the supervised loss only. 

To evaluate the performance of confidence estimation quantitatively,
we used the sparsification curve and its area under curve (AUC) as used in~\cite{Haeusler2013,Spyropoulos2014,Park2015,Seki2016}. The sparsification
curve draws a bad pixel rate while successively removing
pixels in descending order of confidence values in the
disparity map, thus it enables us to observe the tendency of
prediction errors. AUC quantifies the ability of a confidence
measure to estimate correct matches.
For the higher accuracy of
the confidence measure, its AUC value is lower. Moreover, we measured mean squared errors (MSE) between estimated confidence and ground-truth confidence. To evaluate
the disparity refinement performance, we also measured the bad matching
percentage (BMP) as in~\cite{Scharstein2007}. Note that the BMP was obtained by measuring the ratio of erroneous pixels.\vspace{-10pt}
% KITTI 2015
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_agcp_depth_woGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/003_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_agcp_depth_woGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/013_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_agcp_depth_woGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_depth_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_conf_wGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/106_agcp_depth_wGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_depth_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_conf_woGan.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_agcp_depth_woGan.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_depth_wGan.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_conf_wGan.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig11/113_agcp_depth_wGan.png}}\hfill
	\vspace{-5pt}
	\caption[Comparisons of unified depth and confidence estimation methods on KITTI 2015 dataset]{Comparisons of unified depth and confidence estimation methods on KITTI 2015~\cite{KITTIdataset}, using census-SGM (1-4 rows) and MC-CNN (5-8 rows): (a) color images and disparity, (b) final disparity, (c) confidence, and (d) refined disparity maps with propagation of (top) Kim at el.~\cite{Kim2018tip} and (bottom) Ours.}\label{chap4_fig11}
\end{figure}

\subsection{Unified Depth and Confidence Estimation Analysis}\label{chap4_sec:42}
In order to demonstrate the synergistic effects of proposed framework, which simultaneously generates disparity and confidence maps, we first analyzed the convergence in comparison to existing unified method, Kim et al.~\cite{Kim2018tip}. 
\figref{chap4_fig8} shows the qualitative results by evolving iterations, and \figref{chap4_fig9},~\figref{chap4_fig10}, and~\figref{chap4_fig11} shows qualitative results of ours in comparison to~\cite{Kim2018tip}.
For quantitative evaluations, we measured the average BMP of intermediate disparity maps at every 50 epoches, as shown in~\tabref{chap4_tab4} and ~\figref{chap4_fig12}(a).
Note that the conventional methods~\cite{Poggi2016bmvc,Seki2016,Kim2017icip} estimate confidence map on fixed disparity map,
while the proposed method, as well as~\cite{Shaked2017,Kim2018tip}, generates the intermediate disparity map by refining raw cost volumes and predicts the confidence map accordingly. In~\cite{Shaked2017,Kim2018tip}, the BMP decreasing as evolving the number of iterations, but saturated. The proposed method shows the lowest BMP, demonstrating the superiority of the proposed method in a boosting manner. In addition, we further analyzed the confidence estimation performance as evolving the iterations. For quantitative evaluations, we measured the MSE between estimated confidence and ground-truth confidence. \figref{chap4_fig12}(b) shows the MSE values for MID 2014 dataset~\cite{Scharstein2014} obtained by MC-CNN
for evolving epochesIn these experiments, we did not measure the sparsification curve and AUC since the intial disparities are actively varied as evovling iterations, which demonstrates the performance of our confidence estimation gradually improves.\vspace{-10pt}
% Convergence Analysis : graph
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig12/BMP_disparity.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.4\linewidth]{Figure_GAN/fig12/MSE_confidence.pdf}}\\
	\vspace{-5pt}
	\caption[The effectiveness of unified depth and confidence estimation of ours]{The effectiveness of unified depth and confidence estimation of Ours in comparison to Kim et al. \cite{Kim2018tip}: (a) bad matching percentage (BMP) of intermediate disparity maps, and (b) mean squared error (MSE) of estimated confidence maps as evolving training iterations.}\label{chap4_fig12}
\end{figure}

% Table Ours
\begin{sidewaystable}
	\caption[The BMP of the final disparity map on MID 2006, MID 2014 and KITTI 2015 dataset]{The BMP of the final disparity map on MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset with census-based SGM. The BMP is measured with one and three pixel errors. The result with the lowest BMP in each experiment is highlighted.}\vspace{-10pt}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.16\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} }
			\hlinewd{0.8pt}
			\multirow{3}{*}{Datasets} & \multicolumn{4}{ c |}{MID 2006~\cite{Scharstein2007}}
			& \multicolumn{4}{ c |}{MID 2014~\cite{Scharstein2014}}
			& \multicolumn{4}{ c }{KITTI 2015~\cite{KITTIdataset}} \tabularnewline
			\cline{2-13}
			& \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c}{MC-CNN} \tabularnewline
			\cline{2-13}
			& $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px  \tabularnewline
			\hline
			\hline
			Shaked et al.~\cite{Shaked2017}                 
			& 10.16 & 8.12  & 13.58 & 8.66  & 25.79 & 14.23 & 28.56 & 15.02  & 13.32 & 11.45  & 14.08 & 7.94 \tabularnewline			
			Shaked et al.~\cite{Shaked2017} w/AGCPs                
			& 9.15 & 5.15  & 11.03 & 6.10  & 23.92 & 12.87 & 25.24 & 12.68  & 11.71 & 9.58  & 12.15 & 6.41 \tabularnewline
			Kim et al.~\cite{Kim2018tip}                 
			& 8.32 & 5.86  & 9.12 & 5.49  & 24.65 & 11.08 & 25.69 & 12.01  & 9.27 & 8.67  & 10.51 & 8.24 \tabularnewline			
			Kim et al.~\cite{Kim2018tip} w/AGCPs                
			& 6.75 & 3.69  & 6.90 & 3.71  & 22.18 & 8.04 & 22.18 & 8.15  & 7.14 & 6.12  & 7.80 & 5.98 \tabularnewline	
			\hline
			Ours                                     &\textbf{7.88} & \textbf{5.05}  &\textbf{8.49} & \textbf{4.93}  &\textbf{17.23} & \textbf{9.45}  &\textbf{23.27} & \textbf{11.69}  &\textbf{8.41} & \textbf{7.85} &\textbf{9.12} & \textbf{7.76}   \tabularnewline
			Ours w/AGCPs                                    &\textbf{5.84} & \textbf{2.66}  &\textbf{4.87} & \textbf{2.51}  &\textbf{20.59} & \textbf{7.17}  &\textbf{20.36} & \textbf{7.39}  &\textbf{2.66} & \textbf{6.97} &\textbf{5.46} & \textbf{4.05}   \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap4_tab4}\vspace{-10pt}
\end{sidewaystable}





\subsection{Confidence Estimation Analysis}\label{chap4_sec:43}
\subsubsection{Ablation Study}\label{chap4_sec:431}
We then analyzed our confidence estimation networks with ablation evaluations, i.e., ours without color feature extractor and dynamic fusion module. For quantitative evaluations, we measured the average AUC values for various set of inputs and fusion methods.

First of all, ablation experiments to validate the effects of color feature extractor show that the confidence estimator can be improved by extracting the color feature as shown in~\tabref{chap4_tab1}. Qualitative result also shows the effectiveness of color feature extractor.
\figref{chap4_fig5}(d) and \figref{chap4_fig5}(f) exemplify the refined disparity with the estimated confidence that uses only cost volume and disparity, and tri-modalities such as cost volume, disparity, and color as inputs, respectively, showing the superiority of our method. Secondly, to verify the effectiveness of fusing tri-modalities, i.e., cost volume, disparity, and color, in confidence estimation, we evaluated two
different fusion methods; concatenation and dynamic fusion.
The evaluation of each fusion method in~\tabref{chap4_tab1} shows the effects of
the adaptive weight learned with dynamic fusion module.
\figref{chap4_fig6}(d) is the refined disparity with the estimated confidence which uses concatenate fusion, and \figref{chap4_fig6}(f) is the refined disparity with the confidence estimated with dynamic fusion.
% Ablation study: census-SGM
\begin{table*}[t!]
	%\renewcommand{\arraystretch}{1}
	\caption[Ablation study for each component of our method]{Ablation study for each component or our method on MID 2006~\cite{Scharstein2007}, MID 2014~\cite{Scharstein2014}, and KITTI 2015~\cite{KITTIbenchmark} dataset, when the raw matching cost is obtained using (top) census-SGM~\cite{Hirschmuller2008} and (bottom) MC-CNN~\cite{Zbontar2015}.}
	\label{chap4_tab1}
	\begin{center}
		\begin{tabular}{ 
				>{\raggedright}m{0.13\linewidth} >{\raggedright}m{0.16\linewidth}
				>{\centering}m{0.08\linewidth}  
				>{\centering}m{0.08\linewidth} >{\centering}m{0.08\linewidth} 
				>{\centering}m{0.08\linewidth} >{\centering}m{0.08\linewidth}}
			\hlinewd{0.8pt}	
			\multicolumn{2}{l}{Methods} & \cite{Kim2018tip}& \cite{Fu2018}  & Ours wo/col. &  Ours wo/dyn. & Ours  \tabularnewline
			\hline	
			\hline	
			%\textbf{Modality} & &  & &   \tabularnewline
			\multicolumn{2}{l}{Matching cost} 	  & \checkmark &  &  \checkmark & \checkmark & \checkmark  \tabularnewline
			\multicolumn{2}{l}{Disparity} & \checkmark & \checkmark &   \checkmark & \checkmark & \checkmark \tabularnewline
			\multicolumn{2}{l}{Color} 	  &  & \checkmark &   & \checkmark & \checkmark \tabularnewline
			\hline
			%\textbf{Fusion method} & & &   &  \tabularnewline
			\multicolumn{2}{l}{Concatenation} & \checkmark & \checkmark &   &\checkmark &  \tabularnewline
			\multicolumn{2}{l}{Dynamic fusion} & & & \checkmark  & & \checkmark \tabularnewline
			\hline	
			\multirow{3}{*}{{\shortstack{Census\\-SGM}}}	
			&MID 2006 & 0.0417 & 0.0416 & 0.0416 & 0.0413 & 0.0411   \tabularnewline
			&MID 2014 & 0.0730 & 0.0752 & 0.0725 & 0.0712  & 0.0702   \tabularnewline
			&KITTI 2015 & 0.0403 & 0.0405 & 0.0398 & 0.0399  & 0.0391   \tabularnewline
			\hline	
			\multirow{3}{*}{{\shortstack{MC\\-CNN}}}	
			&MID 2006 & 0.0389 & 0.0393 & 0.0385 & 0.0382 & 0.0376    \tabularnewline
			&MID 2014 & 0.0692 & 0.0692 & 0.0690 & 0.0690  & 0.0688   \tabularnewline
			&KITTI 2015 & 0.0247 & 0.0253 & 0.0242 & 0.0240  & 0.0231   \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}
\end{table*}

% AUC
\begin{sidewaystable}
	\caption[The average AUC and MSE values for MID 2006 and KITTI 2015 dataset]{The average AUC and MSE values for MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset. The AUC value of ground truth confidence is measured as `Lower bound'. The result with the lowest AUC value in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.20\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} |
				>{\centering}m{0.05\linewidth} >{\centering}m{0.05\linewidth} }
			\hlinewd{0.8pt}
			\multirow{3}{*}{Datasets} & \multicolumn{4}{ c |}{MID 2006~\cite{Scharstein2007}}
			& \multicolumn{4}{ c |}{MID 2014~\cite{Scharstein2014}}
			& \multicolumn{4}{ c }{KITTI 2015~\cite{KITTIdataset}} \tabularnewline
			\cline{2-13}
			& \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c}{MC-CNN} \tabularnewline
			\cline{2-13}
			& AUC & MSE & AUC & MSE & AUC & MSE & AUC & MSE & AUC & MSE & AUC & MSE  \tabularnewline
			\hline
			\hline
			Haeusler et al. \cite{Haeusler2013}          &0.0454 & 0.1892 &0.0417 & 0.1777 &0.0841 & 0.1965 &0.0750 &0.1756 &0.0585 & 0.3295 &0.0308 & 0.3218\tabularnewline
			Spyropoulos et al. \cite{Spyropoulos2014}    &0.0447 &0.1451  &0.0420 & 0.1478 &0.0839 & 0.1681 &0.0752 & 0.1377 &0.0536 & 0.2783  &0.0323 & 0.1976 \tabularnewline
			Park and Yoon \cite{Park2015}                       &0.0438 & 0.1112 &0.0426 & 0.1049 &0.0802 & 0.1633 &0.0734 & 0.1078 &0.0527 & 0.2019 &0.0303 & 0.1270 \tabularnewline
			Poggi et al. \cite{Poggi20163dv}      &0.0439 & 0.1148 &0.0413 & 0.1025 &0.0791 & 0.1326 &0.0707 & 0.1046  &0.0461 & 0.1628 &0.0263 & 0.1488 \tabularnewline
			Kim et al. \cite{Kim2017tip}                 &0.0430 & 0.1219 &0.0409 & 0.1354 &0.0772 & 0.1403 &0.0701 & 0.1266 &0.0430 & 0.2356 &0.0294 & 0.2330 \tabularnewline            
			CCNN \cite{Poggi2016bmvc}            &0.0454 & 0.0890 &0.0402 & 0.0953 &0.0769 & 0.1129 &0.0716 & 0.1014 &0.0419 & 0.1088 &0.0258 & 0.1254 \tabularnewline
			PBCP \cite{Seki2016}                  &0.0462 & 0.0983 &0.0413 & 0.0909 &0.0791 &  0.1204 &0.0718 & 0.1090 &0.0439 & 0.1355 &0.0272 &  0.1532 \tabularnewline
			Shaked et al. (Conf)~\cite{Shaked2017}              &0.0464 & 0.1138 &0.0495 & 0.1049 &0.0806 & 0.1063 &0.0736 & 0.1014 &0.0531 & 0.1067 &0.0292 & 0.1358 \tabularnewline			
			LFN \cite{Fu2018}            &0.0416 & 0.0802 &0.0393 & 0.0823 &0.0752 & 0.1071 &0.0692 & 0.0898 &0.0405 & 0.0919 &0.0253 & 0.1077 \tabularnewline	
			Kim et al. (Conf)~\cite{Kim2018tip}               &0.0419 & 0.0855 &0.0394 & 0.0828 &0.0749 & 0.1035 &0.0694 & 0.0912 &0.0407 & 0.0927  &0.0250 & 0.1108  \tabularnewline	
			Ours (Conf)                                            &\textbf{0.0411} & \textbf{0.0781} &\textbf{0.0376} & \textbf{0.0716} &\textbf{0.0702} & \textbf{0.0823} &\textbf{0.0688} & \textbf{0.0754} &\textbf{0.0391} & \textbf{0.0628} &\textbf{0.0231} & \textbf{0.0990} \tabularnewline
			\hline
			Lower bound                                          &0.0340 & -&0.0323 & - &0.0569 & - &0.0527 & - &0.0348 & - &0.0170 & - \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap4_tab2}
\end{sidewaystable}
% Sparsification curve
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/mid2006_sgm_average_sparsification.pdf}}
	\subfigure[(b)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/mid2006_mccnn_average_sparsification.pdf}}	
	\subfigure[(c)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/mid2014_sgm_average_sparsification.pdf}}\\
	\vspace{-5pt}
	\subfigure[(d)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/mid2014_mccnn_average_sparsification.pdf}}
	\subfigure[(e)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/kitti2015_sgm_average_sparsification.pdf}}
	\subfigure[(f)]
	{\includegraphics[width=0.32\linewidth]{Figure_GAN/fig13/kitti2015_mccnn_average_sparsification.pdf}}\\
	\vspace{-5pt}
	\caption[Sparsification curves for MID 2006, MID 2014, and KITTI 2015 dataset]{Sparsification curves for MID 2006~\cite{Scharstein2007} using (a) census-SGM and (b) MC-CNN, MID 2014~\cite{Scharstein2014} using (c) census-SGM and (d) MC-CNN, and KITTI 2015 dataset~\cite{KITTIdataset} using (e) census-SGM and (f) MC-CNN, respectively. The sparsification curve for the ground-truth confidence map is described as `Lower bound'.}\label{chap4_fig13}
\end{figure}

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure[(a)]
	{\includegraphics[width=0.45\linewidth]{Figure_GAN/fig14/KITTI2015_SGM.pdf}}
	\vspace{-5pt}
	\subfigure[(b)]
	{\includegraphics[width=0.45\linewidth]{Figure_GAN/fig14/KITTI2015_MCCNN.pdf}}\\
	\vspace{-5pt}
	\caption[AUC values for KITTI 2015 dataset]{AUC values of (a) census-based SGM and (b) MC-CNN for the KITTI 2015 dataset~\cite{KITTIdataset}. We sort the AUC values in the ascending order according to the proposed AUC values. The `Lower bound' of AUC values are computed using the ground-truth confidence map.}
	\label{chap4_fig14}
\end{figure}


\subsubsection{Comparison to Other Methods}\label{chap4_sec:431}
In order to measure the performance of confidence estimator in comparison to other methods, we compared the average AUC values of our method with conventional learning-based approaches
using handcrafted confidence measures~\cite{Haeusler2013,Spyropoulos2014,Park2015,Poggi20163dv,Kim2017tip}
and CNN-based methods~\cite{Seki2016,Poggi2016bmvc,Shaked2017,Fu2018}. 
In these experiments, we only evaluated our confidence estimator, thus we denote our methods as `Ours (Conf)'. Furthermore, for fair comparison, we also evaluated the confidence estimation performance only for~\cite{Shaked2017,Kim2018tip}, i.e., Shaked et al. (Conf)~\cite{Shaked2017} and Kim et al. (Conf)~\cite{Kim2018tip}. The lower bound of AUC can be obtained with a ground-truth confidence map.
Sparsification curves for MID
2014 dataset~\cite{Scharstein2014} and KITTI 2015 dataset~\cite{KITTIdataset} with census-based SGM and MC-CNN are
shown in~\figref{chap4_fig13}. 
The results have shown that the proposed
confidence estimator exhibits a better performance than both conventional
handcrafted approaches and CNN-based approaches. \figref{chap4_fig14} describes the AUC values, which are sorted in
ascending order, for the KITTI 2015 dataset~\cite{KITTIdataset} with
census-based SGM and MC-CNN, respectively. The average AUC and MSE
values with census-based SGM and MC-CNN for MID 2006, MID 2014, and KITTI
2015 datasets were summarized in~\tabref{chap4_tab2}. The handcrafted approaches showed inferior performance than the
proposed method due to low discriminative power of the handcrafted
confidence features. CNN-based methods~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Fu2018} have improved confidence
estimation performance compared to existing handcrafted methods such
as~\cite{Park2015}, but they are still inferior to our method as
they rely on either used only estimated disparity maps or cost
volume to predict unreliable pixels. Especially, the proposed method
always yields the lowest AUC values, showing the superiority of the
proposed method compared to the existing CNN-based methods~\cite{Poggi2016bmvc,Seki2016,Shaked2017,Fu2018}.

In addition, the estimated confidence maps are qualitatively shown in~\figref{chap4_fig15},~\figref{chap4_fig16}, and~\figref{chap4_fig17}. 
Experimental results demonstrate that the proposed networks enable us to estimate more accurate confidence and disparity maps simultaneously in a boosting manner.

% bad matching percentage result for Census-based SGM
\begin{sidewaystable}
	\caption[The BMP of the resultant disparity map on MID 2006, MID 2014, and KITTI 2015 dataset]{The BMP of the resultant disparity map on MID 2006 \cite{Scharstein2007}, MID 2014 \cite{Scharstein2014}, and KITTI 2015 \cite{KITTIdataset} dataset with census-based SGM. The bad pixel error rate of refined disparity maps using ground-truth confidence is measured as `Lower bound'. The BMP is measured with one and three pixel errors. The result with the lowest BMP in each experiment is highlighted.}
	\begin{center}
		\begin{tabular}{ >{\raggedright}m{0.18\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} |
				>{\centering}m{0.04\linewidth} >{\centering}m{0.04\linewidth} }
			\hlinewd{0.8pt}
			\multirow{3}{*}{Datasets} & \multicolumn{4}{ c |}{MID 2006~\cite{Scharstein2007}}
			& \multicolumn{4}{ c |}{MID 2014~\cite{Scharstein2014}}
			& \multicolumn{4}{ c }{KITTI 2015~\cite{KITTIdataset}} \tabularnewline
			\cline{2-13}
			& \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c|}{MC-CNN} & \multicolumn{2}{c|}{Census-SGM} & \multicolumn{2}{c}{MC-CNN} \tabularnewline
			\cline{2-13}
			& $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px & $>$1px & $>$3px  \tabularnewline
			\hline
			\hline
			Initial disparity                            & 20.43 & 10.18 & 17.04 & 8.31 & 43.17 & 24.46 & 39.56 & 20.69 & 23.50 & 18.67 & 20.62 & 15.79    \tabularnewline
			Haeusler et al. \cite{Haeusler2013}          & 11.82 & 7.06 & 9.49 & 6.13  & 33.66 & 10.81 & 31.18 & 11.48 & 11.56 & 10.18 & 12.31 & 10.34     \tabularnewline
			Spyropoulos et al. \cite{Spyropoulos2014}    & 11.36 & 6.51 & 9.62 & 5.86  & 31.97 & 10.62 & 30.64 & 11.02 & 11.46 & 9.59 & 11.31 & 8.61    \tabularnewline
			Park and Yoon \cite{Park2015}                & 10.98 & 6.03 & 9.33 & 5.72  & 29.16 & 10.15 & 28.31 & 10.71 & 10.37 & 9.18 & 11.28 & 8.12    \tabularnewline
			Poggi et al. \cite{Poggi20163dv}      & 9.58 & 5.77  & 8.28 & 5.15  & 27.03 & 9.90  & 27.19 & 9.44  & 9.69 & 8.12  & 10.46 & 7.97    \tabularnewline
			Kim et al. \cite{Kim2017tip}        & 7.72 & 5.08  & 8.35 & 4.93  & 23.74 & 8.53  & 26.47 & 9.42  & 8.50 & 7.08  & 9.72 & 7.54     \tabularnewline
			CCNN \cite{Poggi2016bmvc}            		 & 7.84 & 4.63  & 8.23 & 4.13  & 23.98 & 8.89  & 25.71 & 9.23  & 8.68 & 6.79  & 8.83 & 7.11    \tabularnewline
			PBCP \cite{Seki2016}                  		 & 7.62 & 4.02  & 7.80 & 4.02  & 23.16 & 8.88  & 24.56 & 8.88  & 7.56 & 6.46  & 9.02 & 6.63    \tabularnewline
			Shaked et al. (Conf)\cite{Shaked2017}              & 10.42 & 7.18 & 10.46 & 6.11 & 32.08 & 11.41 & 30.76 & 11.12 & 12.68 & 10.41 & 12.05 & 10.13  \tabularnewline
			LFN \cite{Fu2018}              			 & 7.27 & 3.86  & 7.18 & 3.82  & 22.65 & 8.62  & 23.17 & 8.38  & 7.28 & 6.21  & 8.52 & 6.49 \tabularnewline
			Kim et al. (Conf)\cite{Kim2018tip}         & 7.16 & 3.85  & 7.27 & 3.76  & 22.58 & 8.40 & 23.09 & 8.55  & 7.24 & 6.18  & 8.20 & 6.18  \tabularnewline			
			Ours (Conf)                                     &\textbf{6.38} & \textbf{3.35}  &\textbf{6.27} & \textbf{3.23}  &\textbf{21.96} & \textbf{7.93}  &\textbf{21.87} & \textbf{7.52}  &\textbf{6.83} & \textbf{5.94} &\textbf{7.69} & \textbf{5.77}   \tabularnewline
			\hline
			Lower bound                                      & 3.45 & 1.97  & 4.02 & 1.56  & 20.53 & 5.27  & 17.61 & 4.54  & 4.57 & 3.51  & 3.59 & 3.31 \tabularnewline
			\hlinewd{0.8pt}
		\end{tabular}
	\end{center}\label{chap4_tab3}
\end{sidewaystable}

\subsection{Depth Refinement Comparison}\label{chap4_sec:43}
To verify the robustness of the confidence measures, we refined the
disparity map using the confidence map estimated by several
confidence measure approaches including ours. For refining the
disparity maps, we used AGCPs-based propogation without additional
post-processing to clearly show the performance gain achieved by the confidence measure. 
To evaluate the quantitative
performance, we measured an average BMP
for the  MID 2006~\cite{Scharstein2007}, MID 2014~\cite{Scharstein2014}, and
KITTI 2015~\cite{KITTIdataset} datasets. \tabref{chap4_tab3} show the BMP with thresholds of one and three pixels for MID 2006~\cite{Scharstein2007}, MID 2014~\cite{Scharstein2014}, and KITTI 2015~\cite{KITTIdataset} dataset when using census-based SGM and MC-CNN, respectively. For MID 2006 and MID 2014, since there are occluded pixels in ground-truth disparity map, we computed the BMP only for visible
pixels. The KITTI 2015 benchmark provides a sparse ground truth disparity map
thus we evaluated the BMP only for sparse pixels with the ground-truth
disparity values. The proposed method achieves the lowest BMP in all experiments.

\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_gt_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_agcp_cvpr2015.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_agcp_poggi.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_agcp_seki.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_agcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_sgm/06_agcp_gt.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_cvpr2015_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_seki2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_gt_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_agcp_cvpr2015.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_agcp_poggi.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_agcp_seki.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_agcp_ours.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig15_mccnn/13_agcp_gt.png}}\hfill
	\vspace{-5pt}
	\caption[The confidence and refined disparity maps on MID 2006 dataset]{The confidence and refined disparity maps on MID 2006 dataset~\cite{Scharstein2007} using census-SGM (first two raws), and MC-CNN (last two raws). (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Park and Yoon~\cite{Park2015}, (c) CCNN~\cite{Poggi2016bmvc}, (d) PBCP~\cite{Seki2016}, (e) Ours (Conf), and (f) ground-truth confidence map.}\label{chap4_fig15}
\end{figure} 
% MID 2014 (MCCNN)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_shaked_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_kim2018tip_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_gt_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_agcp_poggi2016bmvc.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_agcp_shaked.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_agcp_kim2018tip.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_agcp_ours.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_sgm/21_agcp_gt.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_poggi2016bmvc_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_shaked_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_kim2018tip_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_ours_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_gt_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_agcp_poggi2016bmvc.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_agcp_shaked.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_agcp_kim2018tip.png}}\hfill
	\subfigure[(e)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_agcp_ours.png}}\hfill
	\subfigure[(f)]
	{\includegraphics[width=0.163\linewidth]{Figure_GAN/fig16_mccnn/10_agcp_gt.png}}\hfill
	\vspace{-5pt}
	\caption[The confidence and refined disparity maps on MID 2014 dataset]{The confidence and refined disparity maps on MID 2014 dataset \cite{Scharstein2014} using census-SGM (first two raws), and MC-CNN (last two rows). (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Poggi et al. \cite{Poggi2016bmvc}, (c) Shaked et al.~\cite{Shaked2017}, (d) Kim et al. (Conf)~\cite{Kim2018tip}, (e) Ours (Conf), and (f) ground-truth confidence map.}\label{chap4_fig16}
\end{figure}
% KITTI 2015 dataset (MCCNN)
\begin{figure}[t!]
	\centering
	\renewcommand{\thesubfigure}{}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_cvpr2014_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_LFN_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_ours_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_init_depth.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_agcp_cvpr2014.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_agcp_LFN.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_sgm/019_agcp_ours.png}}\hfill
	\vspace{-8.5pt}
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_left.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_cvpr2014_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_LFN_conf.png}}\hfill
	\subfigure
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_ours_conf.png}}\hfill
	\vspace{-8.5pt}
	\subfigure[(a)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_init_depth.png}}\hfill
	\subfigure[(b)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_agcp_cvpr2014.png}}\hfill
	\subfigure[(c)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_agcp_LFN.png}}\hfill
	\subfigure[(d)]
	{\includegraphics[width=0.246\linewidth]{Figure_GAN/fig17_mccnn/007_agcp_ours.png}}\hfill
	\vspace{-5pt}
	\caption[The confidence and refined disparity maps on KITTI 2015 dataset]{The confidence and refined disparity maps on KITTI 2015 dataset~\cite{KITTIdataset} using census-SGM (first two rows), and MC-CNN (last two rows). (a) color images and initial disparity maps, refined disparity maps with confidence maps estimated by (b) Spyropoulos et al.~\cite{Spyropoulos2014}, (c) LFN~\cite{Fu2018}, and (d) Ours (Conf).}\label{chap4_fig17}
\end{figure}

\figref{chap4_fig15}, \figref{chap4_fig16}, and \figref{chap4_fig17} display the disparity
maps refined with the confidence maps estimated from the existing
handcrafted classifiers~\cite{Spyropoulos2014},~\cite{Park2015},~\cite{Poggi20163dv},~\cite{Kim2017tip}, CNN-based classifiers~\cite{Poggi2016bmvc},~\cite{Seki2016},~\cite{Shaked2017},~\cite{Fu2018}, and
the proposed method, respectively. 
It was clearly shown that the erroneous matches
are reliably removed using the proposed confidence measure.
For the KITTI 2015 dataset~\cite{KITTIdataset}, erroneous disparities usually
occur in textureless regions (sky and road), as exemplified in~\figref{chap4_fig17}. Conventional
approaches~\cite{Poggi20163dv,Seki2016,Poggi2016bmvc,Fu2018} show the limited performance for detecting incorrect pixels in textureless regions, and thus they affect the matching quality of the subsequent
disparity estimation pipeline. In contrast, the proposed
method can detect mismatched pixels more reliably.

\section{Summary}\label{chap4_sec:5}
We presented a method that jointly estimates disparity and its confidence map through deep networks in an iterative and boosting fashion. The key idea of this method is to design generative cost aggregation and adversarial confidence estimation networks to be learned by the minmax optimization. In addition, the dynamic fusion module is presented to benefit complementary information of matching cost, disparity, and color image in confidence estimation networks conditioned on each input.

==> chap5.tex <==
\chapter{Conclusion}
\label{chap:conclusion}
In this dissertation, we have studied stereo confidence estimation techniques by leveraging machine learning approaches. We conclude this dissertation with a summary and possible directions for future research.

\section{Summary}
First of all, 
a novel approach for learning-based confidence
measure was proposed. It is assumed that the confidence features and
resulting confidence maps are smoothly varying
in the spatial domain. We first demonstrated that a confidence feature augmentation
that imposes spatial coherency on the confidence features and the
resulting confidence maps can increase the
performance of the confidence estimation.
The confidence map was
further improved through hierarchical confidence map aggregations.
The stereo algorithms using the proposed confidence estimation method exhibited
accurate and robust results for public datasets as well as for challenging outdoor environments.

Second, we have presented a learning framework for
estimating the stereo confidence through CNNs. We have shown that the
optimal confidence features can be learned from the matching
probability together with the disparity map.
The matching probability volume is first generated by refining and normalizing the matching cost volume, and then the confidence is estimated through deep networks with the matching probability and its corresponding disparity as inputs.
Highly discriminative confidence features are learned by leveraging the multi-scale disparity features.
Moreover, the proposed semi-supervised disparity loss enables us to effectively learn the networks even with sparse ground-truth disparity maps by using highly confident pixels of intermediate results for computing the image reconstruction loss.
We validated the effectiveness of the proposed method by obtaining accurate and robust disparity maps on public datasets and challenging outdoor scenes through the depth refinement procedure using the estimated confidence map.

Finally, we presented generative disparity and adversarial confidence network.
By boosting each network within adversarial learning,
the performance of both disparity generator and confidence discriminator improved.
Moreover, we use tri-modality, including color, cost volume, and disparity, as inputs to boost the confidence estimation performance.
By finding adaptive weight of each modality 
further improve the confidence prediction gain.


%First of all, the confidence feature augmentation scheme 
%by concatenating pixel- and superpixel-level confidence feature
%for constructing robust confidence feature.
%Unlike exisiting confidence features, we effectively encode the spatial context to confidence feature
%with Gaussian mixture model.
%In addition, we filter the confidence map to obtain smoothly varying confidence map using K-nearest neighbor scheme.
%Secondly, we presented the unified framework of disparity and confidence estimation, which formulates within a convolutional neural network. In contrast to the previous confidence %estimation networks,
%we jointly obtain disparity and confidence simultaneosly.
%Furthermore, we extract the confidence feature from matching cost volume
%using normalization layer and top-K pooling layer.
%Finally, we presented generative disparity and adversarial confidence network.
%By boosting each network within adversarial learning,
%the performance of both disparity generator and confidence discriminator improved.
%Also, we use tri-modality, including color, cost volume, and disparity, as input
%to boost the confidence estimation performance.
%By finding adaptive weight of each modality 
%further improve the confidence prediction gain.

\section{Further Works}
Although this dissertation proposed robust stereo confidence estimation approaches, there are still 
many directions for further research. 
First of all, the adaptive weight in Chapter 4 is globally determined and
does not consider the local variations effectively.
However, since each local patches have different characteristics, optimal informative confidence feature might be different in a pixel-level. 
To solve this limitation, the locally-varying adaptive weight can be used, and this enables the confidence of each patch can be effectively estimated. In addition, there is no consideration of temporal relationship for stereo confidence.
We extract the confidence feature from only spatial information, however,
temprol information might be a useful cue.
3D convolutional neural network or Long-Short term memory (LSTM) module can be used to capture
temporal information.




==> contents.tex <==
\addcontentsline{toc}{chapter}{Contents}
\tableofcontents
\newpage
\addcontentsline{toc}{chapter}{List of Figures}
\listoffigures
\newpage
\addcontentsline{toc}{chapter}{List of Tables}
\listoftables
\newpage
%\printglossaries
%\printglossary[type=\acronymtype,title=Abbreviations]


==> cover.tex <==

\title{Local Area Transform for Cross-Modality Correspondence Matching and Deep Scene Recognition}

\author{Seungchul Ryu}

\department{Department of Electrical and Electronic Engineering}
\degree{Doctor of Philosophy}
\degreemonth{Feb}
\degreeyear{2019}
\thesisdate{Feb 1, 2019}

%\chairman{Arthur C. Smith}{Chairman, Department Committee on Graduate Theses}

\makecovertitle
\maketitle

\newpage
% You can generate signature format by un-commenting the followings - q1.kim
\begin{titlepage}
\begin{center}
{\hskip 3cm
 {\def\baselinestretch{1.5}\large\bf
 \hfill This certifies that the dissertation\\
 \hfill of Seungchul Ryu is approved.
     \par}}
    \vskip 2cm%
\vfill
{\hfill\large \underline{\hskip 9cm}}\vspace*{0.2cm}\\
\hfill \large Thesis Supervisor: {\bf Kwanghoon Sohn}\\
\vskip 1.5cm
%%
{\hfill\large \underline{\hskip 9cm}}\vspace*{0.2cm}\\
\hfill \large Committee Member: {\bf Jaihie Kim}\\
\vskip 1.5cm
%%
{\hfill\large \underline{\hskip 9cm}}\vspace*{0.2cm}\\
\hfill \large Committee Member: {\bf Sangyoun Lee}\\
\vskip 1.5cm
%%
{\hfill\large \underline{\hskip 9cm}}\vspace*{0.2cm}\\
\hfill \large Committee Member: {\bf Bumsub Ham}\\
\vskip 1.5cm
%%
{\hfill\large \underline{\hskip 9cm}}\vspace*{0.2cm}\\
\hfill \large Committee Member: {\bf Dongbo Min}\\
\vskip 1cm
%%
%%
\vfill
	\def\baselinestretch{1.5}\large
	{Graduate School \\
	YONSEI UNIVERSITY \\
	February 2019}
\vskip -2cm
  \end{center}
\end{titlepage}

%\includepdf[pagecommand={\thispagestyle{empty}},pages={1}]{signatures.pdf}

% TODO
\begin{titlepage}
\begin{center}
\vfill
\emph{I would like to dedicate this dissertation to my loving family...}
\vfill
\end{center}
\end{titlepage}

% \addcontentsline{toc}{chapter}{\bfseries Acknowledgments \vspace{-7pt}}
%\includepdf[pagecommand={\thispagestyle{empty}},pages={1-2}]{acknowledgments_kor.pdf}

\setcounter{savepage}{\thepage}
\begin{abstractpage}
\pagenumbering{roman}
\input{abstract}
\end{abstractpage}

%\section*{Acknowledgments}
%This is the acknowledgements section.  You should replace this with your own acknowledgements.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -*-latex-*-

